Kodaira vanishing theorems for Kahler Lie algebroids

A Lie algebroid is a generalization of Lie algebra that provides a general framework to describe the symmetries of a manifold. In this paper, we generalize the Kodaira vanishing theorem, which is a basic result in complex geometry, to Kahler Lie algebroids. The generalization of the Kodaira vanishing theorem states that the kernel of the Lie algebroid Laplace operator on Lie algebroid positive line bundle-valued (p,q)-forms vanishes when p+q is sufficiently large. The most difficult part of the proof of the generalized Kodaira vanishing theorem is the generalization of the Kahler identities to Lie algebroids. In this paper, we provide an approach by using local coordinate calculation.

==> 2/define_symbols.tex <==
\begin{align*}
    *:  f (\basexi{\indexI} \wedge \basedualxi{\indexJp})       &\mapsto
    f (\basedualxi{\indexIpc} \wedge \basexi{\indexJpc})   
\end{align*}

%%%%这里有要修正的东西

\begin{align*}
    \partial \xi_i
    &
        =
        \sum_{j<k}^n
        \coefA{i}{jk}
        \basexi{j} \wedge \basexi{k} 
        =
        \sum_{j,k=1}^n
        \frac{1}{2}
        \coefA{i}{j k}
        \basexi{j}\wedge\basexi{k}
        =
        \sum_{j,k=1}^n
        \frac{1}{2}
        \sgn
            {\order{j,k}}
            {j,k}
        \coefA{i}{\order{j,k}}
        \basexi{j}\wedge\basexi{k}
    \\
    \partialbar \xi_i
    &
        =
        \sum_{j,k}^n
        \coefB{i}{jk}
        \basexi{j} \wedge \basedualxi{k}
    \\
    \partialbar \basedualxi{i}
    &   
        =
        \sum_{j<k}^n
        \coefD{i}{jk}
        \basedualxi{j} \wedge \basedualxi{k}
        =
        \sum_{j,k=1}^n
        \frac{1}{2}
        \coefD{i}{jk}
        \basedualxi{j} \wedge \basedualxi{k}
        =
        \sum_{j,k=1}^n
        \frac{1}{2}
        \sgn
            {\order{j,k}}
            {j,k}
        \coefD{i}{\order{j,k}}
        \basedualxi{j}\wedge\basedualxi{k}
    \\
    \partial \basedualxi{i}
        &= \sum_{j,k}^n
            \coefC{\indexi{}}{j k}
            \xi_j \wedge \basedualxi{k} 
\end{align*}

==> 2/pf_for_dual_of_d=star_d_star.tex <==
Suppose  $\psi\in\Apq{p}{q}\subset\Ak{p+q}(M)$ and $\phi\in\Ak{p+q-1}(M)$, then we can use Stoke's theorem on $\phi\wedge\overline{\star\psi}$, which is a $(2n-1)$-Lie algebroid form, and obtain
\begin{align}
    \int_{M}
    \innerprod{\LieagbdDiff (\phi\wedge\overline{\star\psi})}{\Omega}{}
    =0.
    \label{EQ-Part 1-(1)-use stock on phi wedge bar star psi}
\end{align}
Plugging the equality $\LieagbdDiff (\phi\wedge\overline{\star\psi})=
    (\LieagbdDiff \phi)
    \wedge
    \overline{\star\psi}
    +
    (-1)^{p+q-1}
    \phi
    \wedge
    \LieagbdDiff(\overline{\star\psi})
$ into (\ref{EQ-Part 1-(1)-use stock on phi wedge bar star psi}), we obtain
\begin{align*}
    0=&
    \int_{M}
    \innerprod
        {(\LieagbdDiff \phi)\wedge\overline{\star\psi}}
        {\Omega}
        {}
    +
    (-1)^{p+q-1}
    \int_{M}
    \innerprod
        {\phi\wedge\LieagbdDiff(\overline{\star\psi})}
        {\Omega}
        {}
    \\
    =&
    \pinnerprod
        {\LieagbdDiff \phi}
        {\psi}
        {\Ak{p+q}(M)}
    +
    (-1)^{p+q-1}
    \int_{M}
    \innerprod
        {\phi\wedge\LieagbdDiff(\overline{\star\psi})}
        {\Omega}
        {}
    \\
    =&
    \pinnerprod
        {\phi}
        {\LieagbdDiff^{*}\psi}
        {\Ak{p+q}(M)}
    +
    (-1)^{p+q-1}
    \int_{M}
    \innerprod
        {\phi\wedge\LieagbdDiff(\overline{\star\psi})}
        {\Omega}
        {}.
\end{align*}
We plug $(-1)^{n^2}(-1)^{p+q}\star\star=\id$ in front of the second $\LieagbdDiff$ and obtain
\begin{align*}
    0=&
        \pinnerprod
            {\phi}
            {\LieagbdDiff^{*}\psi}
            {\Ak{p+q}(M)}
        +
        (-1)^{p+q-1}
        \int_{M}
        \innerprod
            {
                \phi\wedge
                (-1)^{n^2}(-1)^{p+q}\star\star
                \LieagbdDiff(\overline{\star\psi})
            }
            {\Omega}
            {}
    \\
    =&
        \pinnerprod
            {\phi}
            {\LieagbdDiff^{*}\psi}
            {\Ak{p+q}(M)}
        +
        (-1)^{p+q-1}
        \int_{M}
        \innerprod
            {
                \phi\wedge
                (-1)^{n^2}(-1)^{p+q}\star
                \overline{\star\LieagbdDiff\star\psi}
            }
            {\Omega}
            {}
    \text{potential problem}
    \\
    =&
        \pinnerprod
            {\phi}
            {\LieagbdDiff^{*}\psi}
            {\Ak{p+q}(M)}
        +
        (-1)
        (-1)^{n^2}
        \pinnerprod
            {\phi}
            {\star\LieagbdDiff\star\psi}
            {},
\end{align*}
which implies $\LieagbdDiff^{*}=(-1)^{n^2}\star\LieagbdDiff\star$.


==> 2/pf_for_star_square_is_equal_to__-1_n2_p+q_.tex <==
It is enough to verify the identity on a local chart $U$. The local expression of the Hodge star on $f\,\basexi{\indexI}\wedge\basedualxi{\indexJp}\in\Apq{p}{q}(U)$ is
    \begin{align*}
        \star
        (f\,\basexi{\indexI}\wedge\basedualxi{\indexJp})
        =
        2^{p+q-n}
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\indexI,\indexJp,\indexIc,\indexJpc}
        f\,
        \basedualxi{\indexIc}\wedge\basexi{\indexJpc}.
    %\label{EQ-Part 1-(1)-the first time apply star}
    \end{align*}
    Applying the Hodge star to $\basedualxi{\indexIc}\wedge\basexi{\indexJpc}$, we obtain
    \begin{align}
        \star
        (\basedualxi{\indexIc}\wedge\basexi{\indexJpc})
        &=
            \star
            \bigg(
            \sgn
                {\indexIc,\indexJpc}
                {\indexJpc,\indexIc}
            \basexi{\indexJpc}\wedge\basedualxi{\indexIc}
            \bigg)
        \nonumber
        \\
        &=
            \sgn
                {\indexIc,\indexJpc}
                {\indexJpc,\indexIc}
            2^{n-q+n-p-n}
            \sgn
                {1^{'},\cdots,n^{'},1,\cdots,n,}
                {\indexJpc,\indexIc,\indexJp,\indexI}
            \basedualxi{\indexJp}\wedge\basexi{\indexI}
        \nonumber
        \\
        &=
            \sgn
                {\indexIc,\indexJpc}
                {\indexJpc,\indexIc}
            2^{n-q+n-p-n}
            \sgn
                {1^{'},\cdots,n^{'},1,\cdots,n,}
                {\indexJpc,\indexIc,\indexJp,\indexI}
            \sgn 
                {\indexJp,\indexI}
                {\indexI,\indexJp}
            \basexi{\indexI}\wedge\basedualxi{\indexJp}
        \nonumber
        \\
        &=
            \sgn
                {\indexIc,\indexJpc}
                {\indexJpc,\indexIc}
            2^{n-q+n-p-n}
            \sgn
                {1^{'},\cdots,n^{'},1,\cdots,n,}
                {\indexJpc,\indexIc,\indexJp,\indexI}
            \sgn 
                {\indexJp,\indexI}
                {\indexI,\indexJp}
            \basexi{\indexI}\wedge\basedualxi{\indexJp}
        \nonumber
        \\
        &=
            2^{n-q+n-p-n}
            \sgn
                {1^{'},\cdots,n^{'},1,\cdots,n,}
                {\indexIc,\indexJpc,\indexI,\indexJp}
            \basexi{\indexI}\wedge\basedualxi{\indexJp}.
    \label{EQ-Part 1-(1)-star on Ic Jpc}
    \end{align}
    Observe that $\star^{2}(f\,\basexi{\indexI}\wedge\basedualxi{\indexJp})$ is equal to
    \begin{align}
        2^{p+q-n}
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\indexI,\indexJp,\indexIc,\indexJpc}
        f\,
        \star
        (\basedualxi{\indexIc}\wedge\basexi{\indexJpc}).
    \label{EQ-Part 1-(1)-the second time apply star}
    \end{align}
    We plug (\ref{EQ-Part 1-(1)-star on Ic Jpc}) into (\ref{EQ-Part 1-(1)-the second time apply star}) and obtain
    \begin{align*}
        &
            2^{p+q-n}
            \sgn
                {1,\cdots,n,1^{'},\cdots,n^{'}}
                {\indexI,\indexJp,\indexIc,\indexJpc}
            2^{n-q+n-p-n}
            \sgn
                {1^{'},\cdots,n^{'},1,\cdots,n,}
                {\indexIc,\indexJpc,\indexI,\indexJp}
            f\,
            \basexi{\indexI}\wedge\basedualxi{\indexJp}
        %\\
        %\bigg\downarrow&
        %    \text{Since\,} 2^{p+q-n+n-q+n-p-n}=2^{0}
        \\
        =&
            \sgn
                {1,\cdots,n,1^{'},\cdots,n^{'}}
                {\indexI,\indexJp,\indexIc,\indexJpc}
            \sgn
                {1^{'},\cdots,n^{'},1,\cdots,n,}
                {\indexI,\indexJp,\indexIc,\indexJpc}
            \sgn
                {\indexIc,\indexJpc,\indexI,\indexJp}
                {\indexI,\indexJp,\indexIc,\indexJpc}
            f\,
            \basexi{\indexI}\wedge\basedualxi{\indexJp}
        \\
        =&
            \sgn
                {1,\cdots,n,1^{'},\cdots,n^{'}}
                {1^{'},\cdots,n^{'},1,\cdots,n,}
            (-1)^{(p+q)(n-p+n-q)}
            f\,
            \basexi{\indexI}\wedge\basedualxi{\indexJp}
        \\
        =&
            (-1)^{n^2}
            (-1)^{(p+q)^2}
            f\,
            \basexi{\indexI}\wedge\basedualxi{\indexJp},
    \end{align*}
    where $(-1)^{(p+q)^2}=(-1)^{p+q}$.

==> 3/2_Lie_agbd_Bochner___Kodaira___Nakano_identity.tex <==
%前面得插一段classical kodaira nakano 的引入

In classical differential geometry, a holomorphic vector bundle over a complex manifold is a vector bundle compatible with the complex structure of the base manifold. That is to say, all entries of the transition matrices are holomorphic functions. Furthermore, recall that a holomorphic vector bundle equipped with a Hermitian metric is called a Hermitian vector bundle. We generalize these concepts to the K\"{a}hler Lie algebroid.

\begin{definition}
For a K\"{a}hler Lie algebroid $\g \to M$, we say a complex vector bundle $E \to M$ is a \keyword{Lie algebroid holomorphic vector bundle} if its transition matrices 
\begin{align*}
    \{\phi_{\alpha,\beta}:\C^{\rank_{\C}(E)}\to\C^{\rank_{\C}(E)}\}
\end{align*}
associated with an open covering of $M$ are Lie algebroid holomorphic. That is to say, $\LieagbdPartialbar (\phi_{\alpha,\beta})_{i,j}=0$ for all entries of the transition matrix. We say a complex vector bundle is a \keyword{Lie algebroid Hermitian vector bundle} if it is equipped with a Hermitian metric.
\end{definition}
As the entries of the transition matrix are all Lie algebroid holomorphic, the operator $\LieagbdPartialbar$ can act on $E$-valued differential forms. That is to say,
\begin{align*}
    \LieagbdPartialbar:\Apq{p}{q}(M,E)\to\Apq{p}{q+1}(M,E)
\end{align*}
is well defined when $E$ is a Lie algebroid holomorphic vector bundle.


Next, we generalize the Chern connection. Before giving its formal definition, we define the splitting of a connection.
\begin{definition}
Suppose that 
$
    \LieagbdConn{}{}:
    \secsp{M}{E}
    \to
    \Apq{1}{0}(M,E)\oplus\Apq{0}{1}(M,E)
$, then we define the holomorphic part as
\begin{align*}
    \LieagbdConn{1,0}{}:\secsp{M}{E}\to\Apq{1}{0}(M,E)
\end{align*}
and the anti-holomorphic part as
\begin{align*}
    \LieagbdConn{0,1}{}:\secsp{M}{E}\to\Apq{0}{1}(M,E).
\end{align*}
\end{definition}
Using the splitting $\LieagbdConn{}{}=\LieagbdConn{1,0}{}+\LieagbdConn{0,1}{}$, we define the Lie algebroid Chern connection.
\begin{definition}[Lie algebroid Chern connection]
For a Lie algebroid Hermitian vector bundle $E$, a Lie algebroid Chern connection on $E$ is a Lie algebroid connection 
\begin{align*}
    \LieagbdConn{}{}:
    \secsp{M}{E}
    \to
    \Apq{1}{0}(M,E)\oplus\Apq{0}{1}(M,E),
\end{align*}
which is compatible with the Hermitian metric, i.e.,
\begin{align*}
    \LieagbdDiff 
    \langle \alpha,\beta \rangle
    (\gamma)
    =
    \langle \LieagbdChernConn{}{\gamma}\alpha,\beta \rangle
    +
    \langle \alpha,\LieagbdChernConn{}{\gamma}\beta \rangle
\end{align*}
for any $\alpha,\beta,\gamma\in\secsp{M}{E}$, and its anti-holomorphic part $\LieagbdChernConn{0,1}{}=\LieagbdPartialbar:\secsp{M}{E} \to  \Apq{0}{1}(M,E)$.
\end{definition}


\begin{proposition}
There exists a unique Lie algebroid Chern connection for a Lie algebroid Hermitian vector bundle.
\end{proposition}
\begin{proof}
The proof is similar to the proof of the existence and uniqueness of the classical Chern connection. Suppose $\{e_{i}\}$ is a Lie algebroid holomorphic frame for $E$ and set $h_{ij}=\langle e_i,e_j\rangle$. Using the holomorphic frame, we consider the $\Ak{1}(M)$-valued matrix $(\theta_{ij})$ such that $\LieagbdChernConn{}{}(e_{i})=\sum_{j}\theta_{ij}e_j$. Observing that $\LieagbdChernConn{}{}(e_i)\in\Apq{1}{0}(M,E)$ since $\LieagbdPartialbar(e_i)=0$, then
\begin{align*}
    (\LieagbdPartial+\LieagbdPartialbar)h_{i,j}
    =
    \LieagbdDiff h_{i,j}
    &=
    \LieagbdDiff
    \langle e_i,e_j \rangle
    \\
    &=
    \langle \LieagbdChernConn{}{} e_i,e_j \rangle
    +
    \langle e_i,\LieagbdChernConn{}{} e_j \rangle
    \\
    &=
    \langle \sum_{k}\theta_{ik}e_k,e_j \rangle
    +
    \langle e_i,\sum_{k}\theta_{jk}e_k \rangle
    \\
    &=
    \sum_{k}
    \theta_{ik} h_{kj}
    +
    \sum_{k}
    \overline{\theta_{jk}} h_{ik},
\end{align*}
where $\theta_{ik} h_{kj}\in \Apq{1}{0}(M)$ and $\overline{\theta_{jk}} h_{ik}\in \Apq{0}{1}(M)$. This illustrates the relation between the Hermitian metric matrix $(h_{ij})$ and the structure matrix $(\theta_{ij})$ for $\LieagbdChernConn{}{}$ such that the Chern connection is uniquely determined by the Hermitian metric. Moreover, the type $(1,0)$-part $\LieagbdPartial h_{i,j}=\sum_{k}\theta_{ik} h_{kj}$ in the equation gives $\theta=\LieagbdPartial h \cdot h^{-1}$.
\end{proof}


The curvature tensor $R(\LieagbdChernConn{}{})=\LieagbdChernConn{}{}^2$ for the Lie algebroid Chern connection is $(1,1)$-type since $(\LieagbdChernConn{0,1}{})^2=\LieagbdPartialbar^{2}=0$ and the curvature matrix $\Theta^{2,0}=-(\overline{(\Theta)^{0,2}})^{tr}=0$ by the property that the connection matrix $\theta$ is skew-Hermitian. Thus, the expansion of the curvature tensor in terms of $\LieagbdChernConn{1,0}{}$ and $\LieagbdChernConn{0,1}{}$ is
\begin{align*}
    \LieagbdChernConn{1,0}{}
    \,
    \LieagbdChernConn{0,1}{}
    +
    \LieagbdChernConn{0,1}{}
    \,
    \LieagbdChernConn{1,0}{}
    .
\end{align*}


We can further simplify the notations on the right-hand side using the superbracket $[\LieagbdChernConn{1,0}{},\LieagbdChernConn{0,1}{}]$. This involves the concept called superbundle \cite{BGV}.
\begin{definition}
A \keyword{superspace} $V$ is a $\mathbb{Z}_2$-graded vector space $V=V^{+}\oplus V^{-}$. A \keyword{superbundle} $\mathcal{E}\to M$ is a vector bundle $\mathcal{E}\to M$ admitting a splitting $\mathcal{E}=\mathcal{E}^{+}\oplus\mathcal{E}^{-}$ such that $\mathcal{E}_{x}=\mathcal{E}^{+}_{x}\oplus \mathcal{E}^{-}_{x}$ is a superspace for all $x\in M$. 
\end{definition}
An operator $D$ is called even (degree $(D)=0$) if it preserves the degree of the element in $\mathcal{E}$:
\begin{align*}
    D:\mathcal{E}^{+}\to\mathcal{E}^{+}
    \qquad\text{and}\qquad
    D:\mathcal{E}^{-}\to\mathcal{E}^{-},
\end{align*}
 and is called odd (degree $(D)=1$) if it swamps the degree of the elements in $\mathcal{E}$:
 \begin{align*}
     D:\mathcal{E}^{+}\to\mathcal{E}^{-}
     \qquad\text{and}\qquad
     D:\mathcal{E}^{+}\to\mathcal{E}^{-}.
 \end{align*}
With the degree of superoperators, the \keyword{superbracket} is defined by 
\begin{align*}
    [D_1,D_2]
    =
    D_{1}D_{2}
    -(-1)^{|(D_1)\cdot(D_2)}
    D_{2}D_{1}.
\end{align*}
Looking at the space of $E$-valued Lie algebroid forms $\mathcal{E}=\bigoplus_{p,q}\Apq{p}{q}(M,E)$, we define the $\mathbb{Z}_2$ grading
\begin{align*}
    \mathcal{E}^{+}
    =
    \bigoplus_{\text{p+q are even}}
    \Apq{p}{q}(M,E)
    \qquad\text{and}\qquad
    \mathcal{E}^{-}
    =
    \bigoplus_{\text{p+q are odd}}
    \Apq{p}{q}(M,E).
\end{align*}
Following the definitions, we can see that $\LieagbdChernConn{}{}$, $\LieagbdChernConn{1,0}{}$, and $\LieagbdChernConn{0,1}{}$ are all odd-degree operators. Consequently, the superbracket between $\LieagbdChernConn{1,0}{}$ and $\LieagbdChernConn{0,1}{}$ yields
\begin{align*}
    R(\LieagbdChernConn{}{})
    =
    \LieagbdChernConn{1,0}{}\,\LieagbdChernConn{0,1}{}
    -
    (-1)^{(-1)(-1)}
    \LieagbdChernConn{0,1}{}\,\LieagbdChernConn{1,0}{}
    =
    [\LieagbdChernConn{1,0}{},\LieagbdChernConn{0,1}{}]
    .
\end{align*}


Let us define and generalize some notations and equations that help us achieve the aim: exploring a generalization of the Bochner–Kodaira–Nakano identity on the Lie algebroid. The first one is \keyword{Lie algebroid Laplacians} induced by the Lie algebroid Chern connection:
\begin{align*}
    \LieagbdLpls{1,0}{}&
    :=
        {\LieagbdChernConn{1,0}{}}^{*}
        \,
        \LieagbdChernConn{1,0}{}
    +
        \LieagbdChernConn{1,0}{}
        \,
        {\LieagbdChernConn{1,0}{}}^{*}
    =
    [\LieagbdChernConn{1,0}{},{\LieagbdChernConn{1,0}{}}^*]
    \\
    \LieagbdLpls{0,1}{}&
    :=
    {\LieagbdChernConn{0,1}{}}^{*}\,\LieagbdChernConn{0,1}{} 
    +
    \LieagbdChernConn{0,1}{}\,{\LieagbdChernConn{0,1}{}}^{*}
    =\LieagbdPartialbar^{*}\,\LieagbdPartialbar+\LieagbdPartialbar\,\LieagbdPartialbar^{*}.
\end{align*}
We can use the notation \keyword{$\LieagbdPartialbar$-Laplacian} or $\LieagbdLpls{}{\LieagbdPartialbar}$ for $\LieagbdLpls{0,1}{}$. Then, let us generalize the exterior and interior multiplications of the Lie algebroid K\"{a}hler form. In Section \ref{sec:Lie algebroid Kahler identities}, we have already defined $L$ and $\Lambda$ on the space of Lie algebroid forms in Theorem \ref{thm-Lie algebroid K\"{a}hler identities}. We generalize these to the bundle-valued Lie algebroid forms,
\begin{align*}
    L:=\Apq{p}{q}(M,E)
    &\to\Apq{p+1}{q+1}(M,E)
    \\
    \phi\otimes e
    &\mapsto \omega\wedge\phi\otimes e,
\end{align*}
and the formal adjoint of $L$,
\begin{align*}
    \Lambda:=L^*:\Apq{p}{q}(M,E)\to\Apq{p-1}{q-1}(M,E),
\end{align*}
on the space of $E$-valued Lie algebroid differential forms. Another generalization concerns the Lie algebroid K\"{a}hler identities on bundle-valued $(p,q)$-forms.
\begin{proposition}
For a K\"{a}hler Lie algebroid $\g\to M$ and a Lie algebroid Hermitian vector bundle $E\to M$, the Lie algebroid K\"{a}hler identities on $E$-valued $(p,q)$-forms are:
\begin{align*}
    [\Lambda,\LieagbdChernConn{1,0}{}]&=\sqrt{-1}{\LieagbdChernConn{0,1}{}}^{*},
    \\
    [\Lambda,\LieagbdChernConn{0,1}{}]&=\sqrt{-1}{\LieagbdChernConn{1,0}{}}^{*},
    \\
    [{\LieagbdChernConn{1,0}{}}^*,L]&=\sqrt{-1}\LieagbdChernConn{0,1}{},
    \\
    [{\LieagbdChernConn{0,1}{}}^*,L]&=\sqrt{-1}\LieagbdChernConn{1,0}{}.
\end{align*}
\end{proposition}
\begin{proof}
We can pick a local normal frame on $E$ such that the connection $\LieagbdChernConn{1,0}{}=\LieagbdDiff+\phi$, where $\phi$ vanishes at the origin of the local coordinate. Then, we use $\LieagbdChernConn{1,0}{}$ and $\LieagbdChernConn{0,1}{}$ to replace $\LieagbdPartial$ and $\LieagbdPartialbar$ in the Lie algebroid K\"{a}hler identities in Theorem \ref{thm-Lie algebroid K\"{a}hler identities}.
\end{proof}


Using all the ingredients we have defined and constructed, we can obtain the Lie algebroid version of the Bochner–Kodaira–Nakano identity, which formally agrees with the identity on a complex manifold (e.g., \cite{GH1994}), and the proof is similar as well.
\begin{lemma}
    For a K\"{a}hler Lie algebroid, the equation
    \begin{align}
        \LieagbdLpls{}{\LieagbdPartialbar}
        =
        \LieagbdLpls{1,0}{}
        +
        \sqrt{-1}[\LieagbdChernConn{2}{},\Lambda]
        \label{EQ-Part 1-(3)-lie agbd BK identity}
    \end{align}
    holds and is called the \keyword{Lie algebroid Bochner–Kodaira–Nakano identity}.
\end{lemma}
\begin{proof}
Following the definition of $\LieagbdLpls{}{\LieagbdPartialbar}$,
\begin{align*}
    \LieagbdLpls{}{\LieagbdPartialbar}
    &=
    [\LieagbdPartialbar,\LieagbdPartialbar^{*}]
    \\
    &=
    [\LieagbdChernConn{0,1}{},{\LieagbdChernConn{0,1}{}}^*]
    .
\end{align*}
We use the identity $[\Lambda,\LieagbdChernConn{1,0}{}]=\sqrt{-1}{\LieagbdChernConn{0,1}{}}^{*}$ and plug it into the expansion of the above Laplacian, obtaining the following formula:
\begin{align}
    \LieagbdLpls{}{\LieagbdPartialbar}
    =
    -\sqrt{-1}
    \big[\LieagbdChernConn{0,1}{},[\Lambda,\LieagbdChernConn{1,0}{}]\big].
    \label{EQ-Part 1-(3)-eq 1 in the pf of lie agbd BK identity}
\end{align}
We now look at the Jacobi identity:
\begin{align*}
    \big[ \LieagbdChernConn{0,1}{},[\Lambda,\LieagbdChernConn{1,0}{}]\big]
    +
    \big[ \Lambda,[\LieagbdChernConn{1,0}{},\LieagbdChernConn{0,1}{}]\big]
    +
    \big[ \LieagbdChernConn{1,0}{},[\LieagbdChernConn{0,1}{},\Lambda]\big]
    =0.
\end{align*}
We replace the right-hand side of (\ref{EQ-Part 1-(3)-eq 1 in the pf of lie agbd BK identity}) with the last two terms in the Jacobi identity and deduce
\begin{align}
    \LieagbdLpls{}{\LieagbdPartialbar}
    &=
    \sqrt{-1}
    \big[ \Lambda,[\LieagbdChernConn{1,0}{},\LieagbdChernConn{0,1}{}]\big]
    +
    \sqrt{-1}
    \big[ \LieagbdChernConn{1,0}{},[\LieagbdChernConn{0,1}{},\Lambda]\big]
    \nonumber\\
    &=
    \sqrt{-1}
    \big[ \Lambda,[\LieagbdChernConn{1,0}{},\LieagbdChernConn{0,1}{}]\big]
    +
    \sqrt{-1}
    \big[ \LieagbdChernConn{1,0}{},-\sqrt{-1}{\LieagbdChernConn{1,0}{}}^*\big]
    \nonumber\\
    &=
    \sqrt{-1}
    \big[ \Lambda,[\LieagbdChernConn{1,0}{},\LieagbdChernConn{0,1}{}]\big]
    +
    [\LieagbdChernConn{1,0}{},{\LieagbdChernConn{1,0}{}}^{*}],
\label{EQ-Part 1-(3)-eq 2 in the pf of lie agbd BK identity}
\end{align}
where we use the Lie algebroid K\"{a}hler identity $
[\Lambda,\LieagbdChernConn{0,1}{}]
=
\sqrt{-1}{\LieagbdChernConn{1,0}{}}^*
$ in the second equal sign. 

Recalling that $\LieagbdLpls{1,0}{}=[\LieagbdChernConn{1,0}{},{\LieagbdChernConn{1,0}{}}^{*}]$ and $\LieagbdChernConn{2}{}=[\LieagbdChernConn{1,0}{},\LieagbdChernConn{0,1}{}]$, we conclude the Lie algebroid Bochner–Kodaira–Nakano identity from (\ref{EQ-Part 1-(3)-eq 2 in the pf of lie agbd BK identity}).
\end{proof}


==> 3/3Lie_agbd_Kodaira_vanishing_theorem.tex <==
Applying the Lie algebroid Bochner–Kodaira–Nakano identity, we can establish the Lie algebroid Kodaira vanishing theorem. The original statement of the theorem on the complex manifold is that the cohomology group of a positive line bundle vanishes when its degree is large enough. For a Lie algebroid, however, the Hodge theory between the space of harmonic E-valued Lie algebroid $(p,q)$-forms, i.e., $\kernel(\Delta_{\LieagbdPartialbar}|_{\Apq{p}{q}(M,E)})$, and the sheaf cohomology of $E$ for a Lie algebroid holomorphic vector bundle $E$ over $M$, i.e., $H^p(M,\Omega^q(E))$, is yet to be developed. Our vanishing theorem is slightly weaker than the classical case and gives some sufficient conditions: the type $(p,q)$ such that $p+q$ is large enough, which implies the kernel of $\nabla_{\LieagbdPartialbar}$ is trivial. First, let us define the Lie algebroid positive line bundle.

% \begin{definition}
%     For a K\"{a}hler Lie algebroid $(M,\g,\omega)$, we say a Lie algebroid holomorphic line bundle $E\to M$ is \keyword{positive} if there is a Hermitian metric on $E$ such that the curvature of the corresponding Lie algebroid Chern connection is equal to $\sqrt{-1}\omega$. Meanwhile, we say $E\to M$ is \keyword{negative} if the corresponding Lie algebroid Chern connection is equal to $-\sqrt{-1}\omega$.
% \end{definition}

\begin{definition}
    A Lie algebroid holomorphic line bundle $E\to M$ is \keyword{positive}, if there is a hermitian metric on $E$ such that the curvature $R\in\Apq{1}{1}(M)$ of the Chern connection satisfies that $\sqrt{-1}R$ is positive definite. Meanwhile, we say $E\to M$ is \keyword{negative} if $-\sqrt{-1}R$ is positive definite.
\end{definition}


Recall that the operator $L$ is the exterior multiplication of $\omega$ and $\Lambda$ is its dual. Both operators are even-degree operators. In the classical case, their commutator $[L,\Lambda]=L\Lambda-\Lambda L$ is a scalar multiplication, and this result can be generalized to the K\"{a}hler Lie algebroid.
\begin{lemma}
For a K\"{a}hler Lie algebroid $(M,\g,\omega)$ and the vector bundle $E\to M$, the commutator $[L,\Lambda]$ on $\Apq{p}{q}(M,E)$ is equal to $(p+q-n)\id$, where $\id:\Apq{p}{q}(M,E)\to\Apq{p}{q}(M,E)$ is an identity map.
\end{lemma}
\begin{proof}
    It is enough to verify the identity on a local neighborhood. Recall that locally 
    $\omega=
        \frac{\sqrt{-1}}{2}
        \displaystyle\sum_{k=1}^{n}
        \basexi{k}\wedge\basedualxi{k^{'}}
    $. Using the notations that $e_{\basexi{k}}:=\basexi{k}\wedge$ and $\contract{\basexi{k}}:=(e_{\basexi{k}})^{*}$, we can compute the expressions of $L$ and $\Lambda$:
    \begin{align*}
        L=e_{\omega}=
        \frac{\sqrt{-1}}{2}
        \displaystyle\sum_{k=1}^{n}
        e_{\basexi{k}}
        \,
        e_{\basedualxi{k^{'}}}
        \qquad\text{and}\qquad
        \Lambda=\iotaW=
        -\frac{\sqrt{-1}}{2}
        \displaystyle\sum_{k=1}^{n}
        \contract{\basedualxi{k^{'}}}
        \,
        \contract{\basexi{k}}.
    \end{align*}
    Then, for any $(p,q)$-Lie algebroid form $\basexi{\indexI}\wedge\basedualxi{\indexJp}$, we can expect that the applications of $L$ and $\Lambda$ on $\basexi{\indexI}\wedge\basedualxi{\indexJp}$ will be similar to the classical case. 
    
    \input{3/calculate p+q-n.tex}
    From the calculations above, we cancel the repeated terms and obtain $[L,\Lambda]=e_{\omega}\,\contract{\omega}-\contract{\omega}\, e_{\omega}=(|\indexI\cap\indexJ|-|\indexIc\cap\indexJc|)\mathrm{\id}=(p+q-n)\mathrm{\id}$.
\end{proof}

We are now ready to state and prove the vanishing theorem.
\begin{theorem}[Lie algebroid Kodaira–Nakano vanishing theorem]
    Give a K\"{a}hler Lie algebroid $\g\to M$ and a positive line bundle $E\to M$. The kernel of 
    \begin{align*}
        \LieagbdLpls{}{\LieagbdPartialbar}
        :\Apq{p}{q}(M,E)\to\Apq{p}{q}(M,E)
    \end{align*}
    vanishes when $p+q>n$. The same result holds on a negative line bundle under the change of the condition that $p+q<n$.
\end{theorem}
\begin{proof}
By the definition of positivity, the curvature of the Lie algebroid Chern connection for $E$ is a closed positive $(1,1)$-form. Thus, it determines a Lie algebroid K\"{a}hler form $\omega$. Use this Lie algebroid K\"{a}hler form in the Lie algebroid Bochner–Kodaira–Nakano identity
\begin{align*}
    \LieagbdLpls{}{\LieagbdPartialbar}
    =
    \LieagbdLpls{1,0}{}+\sqrt{-1}[\LieagbdChernConn{2}{},\Lambda]
    .
\end{align*}
The $\LieagbdLpls{1,0}{}$ in the equation is a non-negative operator (i.e., $\innerprod{\LieagbdLpls{1,0}{}\phi}{\phi}{}\geq 0, \forall \phi\in \Apq{p}{q}(M,E)$) and $\LieagbdChernConn{2}{}$ is equal to $\sqrt{-1}L$ from the definition of a positive line bundle. Thus, we obtain
\begin{align*}
    \LieagbdLpls{}{\LieagbdPartialbar}
    =
    \LieagbdLpls{1,0}{}-[L,\Lambda]
    =
    \LieagbdLpls{1,0}{}+(p+q-n)\mathrm{\id},
\end{align*}
which this implies that $\LieagbdLpls{}{\LieagbdPartialbar}$ has a trivial kernel if $p+q>n$.
\end{proof}


% \textcolor{blue}{
% Looking at
% $
%     \kernel
%     (\LieagbdLpls{}{\LieagbdPartialbar})
%     =
%     \kernel(\LieagbdPartialbar)
%     \cap
%     \kernel(\LieagbdPartialbar^{*})
% $. An element $\phi$ in
% \begin{align*}
%     \kernel
%     (
%     \LieagbdLpls{}{\LieagbdPartialbar}
%     :\Apq{p}{q}(M,E)\to\Apq{p}{q}(M,E)
%     )
% \end{align*}
% implies that $\star\phi$ is in
% \begin{align*}
%     \kernel
%     (\LieagbdLpls{}{\LieagbdPartialbar}
%     :\Apq{n-q}{n-p}(M,E)\to\Apq{n-q}{n-p}(M,E))
% \end{align*}
% since
% $
%     \star
%     (\LieagbdPartialbar\star\phi)
%     =
%     -(-1)^{n^2}\,
%     \LieagbdPartialbar^{*}\phi
%     =
%     0
% $ and
% $
%     \star
%     (\LieagbdPartialbar^{*}\star\phi)
%     =
%     -(-1)^{n^2}\,
%     \LieagbdPartialbar\phi
%     =
%     0
% $, where the Hodge star is an injective map. Therefore we can obtain the following corollary.
% \begin{corollary}
% Give a K\"{a}hler Lie algebroid $(M,\g,\omega)$ and a positive line bundle $E\to M$. The kernel of 
% \begin{align*}
%     \LieagbdLpls{}{\LieagbdPartialbar}
%     :\Apq{p}{q}(M,E)\to\Apq{p}{q}(M,E)
% \end{align*}
% vanishes when $p+q\neq n$.
% \end{corollary}
% }




The following corollary will be applied to the kernel of the (Lie algebroid) Dolbeault operator.
\begin{corollary}
\label{cor-vanishign theorem for Dolbeault}
Suppose $M\to\g$ is a K\"{a}hler Lie algebroid and $E\to M$ a positive Lie algebroid holomorphic line bundle. The kernel of 
\begin{align*}
    \LieagbdPartialbar+\LieagbdPartialbar^{*}
    :\Apq{p}{q}(M,E)
    \to
    \Apq{p}{q+1}(M,E)
    \oplus
    \Apq{p}{q-1}(M,E)
\end{align*}
vanishes when $p+q>n$. The same result holds on a negative line bundle under the change of the condition that $p+q<n$.
\end{corollary}
\begin{proof}
The Laplace operator $
\LieagbdLpls{}{\LieagbdPartialbar}
=
\LieagbdPartialbar^{*}\LieagbdPartialbar
+
\LieagbdPartialbar\LieagbdPartialbar^{*}
=
(\LieagbdPartialbar+\LieagbdPartialbar^{*})^{2}
$, so 
\begin{align*}
    \ker(\LieagbdPartialbar+\LieagbdPartialbar^{*})
    \subset
    \ker(\LieagbdLpls{}{\LieagbdPartialbar})
\end{align*}
is clear. On the other side, if $s\in\ker(\LieagbdLpls{}{\LieagbdPartialbar})$, then
\begin{align*}
    0=
    \pinnerprod
        {\LieagbdLpls{}{\LieagbdPartialbar}s}
        {s}
        {\Apq{p}{q}}
    &=
    \pinnerprod
        {(\LieagbdPartialbar+\LieagbdPartialbar^{*})^{2} s}
        {t}
        {\Apq{p}{q}}
    \\
    &=
    \pinnerprod
        {(\LieagbdPartialbar+\LieagbdPartialbar^{*}) s}
        {(\LieagbdPartialbar+\LieagbdPartialbar^{*}) s}
        {\Apq{p}{q+1}(M,E)
        \oplus
        \Apq{p}{q-1}(M,E)}
    \\
    &=
    ||(\LieagbdPartialbar+\LieagbdPartialbar^{*}) s||^{2}
    ,
\end{align*}
which implies that $s\in\ker(\LieagbdPartialbar+\LieagbdPartialbar^{*})$ as well, thereby completing the proof of Corollary \ref{cor-vanishign theorem for Dolbeault}.
\end{proof}


% The corollary \ref{cor-vanishign theorem for Dolbeault} gives the following proposition directly.
% \begin{proposition}
% \label{prop-no harmonic section}
% There is no non-trivial Lie algebroid holomorphic section, i.e. $s\in\secsp{M}{E}$ which $\LieagbdPartialbar s=0$, on a positive Lie algebroid holomorphic line bundle $E\to M$.  
% \end{proposition}
% \begin{proof}
% For any section of type $(0,0)$, it is in the kernel of $\LieagbdPartialbar^{*}$ since $(0,0)$ is the lowest degree. So 
% \begin{align*}
%     \kernel
%     \big(
%     \LieagbdLpls{}{\LieagbdPartialbar}:
%     \Apq{0}{0}(M,E)
%     \to
%     \Apq{0}{0}(M,E)
%     \big)
%     =
%     \kernel
%     \big(
%     \LieagbdPartialbar:
%     \Apq{0}{0}(M,E)
%     \to
%     \Apq{0}{1}(M,E)
%     \big)
%     ,
% \end{align*}
% which is a trivial because of corollary \ref{cor-vanishign theorem for Dolbeault}.
% \end{proof}

==> 3/For__i,j_,_calculation_for_LHS.tex <==
Let us look at the left-hand side for $\basexi{\indexI},\basedualxi{\indexJp}$. The Lie bracket is $\LieagbdPartialbar\,\iotaW-\iotaW\,\LieagbdPartialbar$, where the first term $\LieagbdPartialbar\,\iotaW(\basexi{i}\wedge\basedualxi{j})=0$ since 
\begin{align*}
    \iotaW(\basexi{i}\wedge\basedualxi{j})
    =
    \begin{cases}
        0           & i\neq j
    \\
        2\sqrt{-1}  & i=j
    \end{cases}
\end{align*}
is a constant function vanishing under $\LieagbdPartialbar$. This leads to the remaining part, $-\iotaW\,\LieagbdPartialbar(\basexi{i}\wedge\basedualxi{j})$. The expression of $\LieagbdPartialbar(\basexi{i}\wedge\basedualxi{j})$ is
\begin{align}
    \LieagbdPartialbar
    (\basexi{i}\wedge\basedualxi{j^{'}})
    =&
        \displaystyle\sum_{k=1}^{n}
        \displaystyle\sum_{l^{'}=1}^{n}
        (\LieagbdPartialbar\basexi{i})
        \wedge
        \basedualxi{j^{'}}
        -
        \displaystyle\sum_{l_{1}^{'}=1}^{n}
        \displaystyle\sum_{l_{2}^{'}=1}^{n}
        \basexi{i}
        \wedge
        (\LieagbdPartialbar\basedualxi{j^{'}})
    \notag
    \\
    =&
        \displaystyle\sum_{k=1}^{n}
        \displaystyle\sum_{l^{'}=1}^{n}
        \coefB{i}{k l^{'}}
        \basexi{k}\wedge\basedualxi{l^{'}}
        \wedge
        \basedualxi{j^{'}}
        -
        \displaystyle\sum_{l_{1}^{'}=1}^{n}
        \displaystyle\sum_{l_{2}^{'}=1}^{n}
        \basexi{i}
        \wedge
        \frac{1}{2}
        \sgn
            {\order{l_{1}^{'},l_{2}^{'}}}
            {l_{1}^{'},l_{2}^{'}}
        \coefD{j^{'}}{\order{l_{1}^{'},l_{2}^{'}}}
        \basedualxi{l_{1}^{'}}
        \wedge
        \basedualxi{l_{2}^{'}}.
    \label{EQ-Kahler identity on Lie agbd-calculation for LHS of (i,j)-no1}
\end{align}
We plug $\iotaW$ into the front of (\ref{EQ-Kahler identity on Lie agbd-calculation for LHS of (i,j)-no1}) and obtain
\begin{align}
    %%%the first step-1:3-0
    \iotaW\,\LieagbdPartialbar
    (\basexi{i}\wedge\basedualxi{j^{'}})
    &
        =
        -\frac{\sqrt{-1}}{2}
        \displaystyle\sum_{h=1}^{n}
        \iota_{\basedualxi{h^{'}}}\,\iota_{\basexi{h}}
        \begin{pmatrix*}[l]
            \displaystyle\sum_{k=1}^{n}
            \displaystyle\sum_{l^{'}=1}^{n}
            \coefB{i}{k l^{'}}
            \basexi{k}\wedge\basedualxi{l^{'}}
            \wedge
            \basedualxi{j^{'}}
            \\
            -
            \\
            \displaystyle\sum_{l_{1}^{'}=1}^{n}
            \displaystyle\sum_{l_{2}^{'}=1}^{n}
            \basexi{i}
            \wedge
            \frac{1}{2}
            \sgn
                {\order{l_{1}^{'},l_{2}^{'}}}
                {l_{1}^{'},l_{2}^{'}}
            \coefD{j^{'}}{\order{l_{1}^{'},l_{2}^{'}}}
            \basedualxi{l_{1}^{'}}
            \wedge
            \basedualxi{l_{2}^{'}}
        \end{pmatrix*}.
    \label{EQ-Kahler identity on Lie agbd-calculation for LHS of (i,j)-no2}
\end{align}
Using the contractions $\contract{\basexi{h}}(\basexi{k})=2\delta_{h,k}$ and $\contract{\basedualxi{h}}(\basedualxi{k})=2\delta_{h,k}$, we simplify (\ref{EQ-Kahler identity on Lie agbd-calculation for LHS of (i,j)-no2}) as follows:
\begin{align*}
    \iotaW\,\LieagbdPartialbar
    (\basexi{i}\wedge\basedualxi{j^{'}})
    &
        =
        -\frac{\sqrt{-1}}{2}
        \begin{pmatrix*}[l]
            \displaystyle\sum_{h=1}^{n}
            \displaystyle\sum_{l^{'}=1}^{n}
            \iota_{\basedualxi{h^{'}}}
            (
            2
            \coefB{i}{h l^{'}}
            \basedualxi{l^{'}}
            \wedge
            \basedualxi{j^{'}}
            )
            \\
            -
            \\
            \displaystyle\sum_{l_{1}^{'}=1}^{n}
            \displaystyle\sum_{l_{2}^{'}=1}^{n}
            \frac{1}{2}
            \sgn
                {\order{l_{1}^{'},l_{2}^{'}}}
                {l_{1}^{'},l_{2}^{'}}
            \iota_{\basedualxi{i^{'}}}
            (
            2
            \coefD{j^{'}}{\order{l_{1}^{'},l_{2}^{'}}}
            \basedualxi{l_{1}^{'}}
            \wedge
            \basedualxi{l_{2}^{'}}
            )
        \end{pmatrix*}
    \\
    %%%the first step-1:3-3
    &
        =
        -\sqrt{-1}
        \begin{pmatrix*}[l]
            \displaystyle\sum_{l^{'}=1}^{n}
            2\coefB{i}{l l^{'}}
            \basedualxi{j^{'}}
            \\
            -
            \\
            \displaystyle\sum_{l^{'}=1}^{n}
            2\coefB{i}{j l^{'}}
            \basedualxi{l^{'}}
            \\
            -
            \\
            \displaystyle\sum_{l_{2}^{'}=1}^{n}
            \frac{1}{2}
            \sgn
                {\order{i^{'},l_{2}^{'}}}
                {i^{'},l_{2}^{'}}
            2\coefD{j^{'}}{\order{i^{'},l_{2}^{'}}}
            \basedualxi{l_{2}^{'}}
            \\
            +
            \\
            \displaystyle\sum_{l_{1}^{'}=1}^{n}
            \frac{1}{2}
            \sgn
                {\order{l_{1}^{'},i^{'}}}
                {l_{1}^{'},i^{'}}
            2\coefD{j^{'}}{\order{l_{1}^{'},i^{'}}}
            \basedualxi{l_{1}^{'}}
        \end{pmatrix*}.
\end{align*}
We use the constraint $\coefB{l}{j i} -\coefB{i}{j l}=\sgn{\order{i,l}}{i,l}\coefD{j}{\order{i,l}}$ to simplify the term
\begin{align*}
    \iotaW\,\LieagbdPartialbar
    (\basexi{i}\wedge\basedualxi{j^{'}})
    &=
        -2\sqrt{-1}
        \begin{pmatrix*}[l]
            \displaystyle\sum_{l^{'}=1}^{n}
            \coefB{i}{l l^{'}}
            \basedualxi{j^{'}}
            \\
            -
            \\
            \displaystyle\sum_{l^{'}=1}^{n}
            \coefB{i}{j l^{'}}
            \basedualxi{l^{'}}
            \\
            -
            \\
            \displaystyle\sum_{l^{'}=1}^{n}
            \sgn
                {\order{i^{'},l^{'}}}
                {i^{'},l^{'}}
            \coefD{j^{'}}{\order{i^{'},l^{'}}}
            \basedualxi{l^{'}}
        \end{pmatrix*}
    \\
    &=
        -2\sqrt{-1}
        \begin{pmatrix*}[l]
            \displaystyle\sum_{l^{'}=1}^{n}
            \coefB{i}{l l^{'}}
            \basedualxi{j^{'}}
            \\
            -
            \\
            \displaystyle\sum_{l^{'}=1}^{n}
            (
            \coefB{i}{j l^{'}}
            +
            \sgn
                {\order{i^{'},l^{'}}}
                {i^{'},l^{'}}
            \coefD{j^{'}}{\order{i^{'},l^{'}}}
            )
            \basedualxi{l^{'}}
        \end{pmatrix*}
    \\
    &
        =
        -2\sqrt{-1}
        \begin{pmatrix*}[l]
            \displaystyle\sum_{l^{'}=1}^{n}
            \coefB{i}{l l^{'}}
            \basedualxi{j^{'}}
            -
            \displaystyle\sum_{l^{'}=1}^{n}
            \coefB{l^{'}}{j i}
            \basedualxi{l^{'}}
        \end{pmatrix*}.
\end{align*}
We conclude the left-hand side:
\begin{align}
    [\LieagbdPartialbar,\iotaW]
    (\basexi{i}\wedge\basedualxi{j})
    =
    -2\sqrt{-1}
    \begin{pmatrix*}[l]
        \displaystyle\sum_{l^{'}=1}^{n}
        \coefB{i}{l l^{'}}
        \basedualxi{j^{'}}
        -
        \displaystyle\sum_{l^{'}=1}^{n}
        \coefB{l^{'}}{j i}
        \basedualxi{l^{'}}
    \end{pmatrix*}.
    \label{EQ-Kahler identity on Lie agbd-calculation for LHS of (i,j)-result}
\end{align}

==> 3/For__i,j_,_calculation_for_RHS.tex <==
Next, let us look at the right-hand side. Recall that $\LieagbdPartial^{*}=-(-1)^{n^2}\star\,\LieagbdPartialbar\,\star$, so the right-hand side can be written as
\begin{align}
    \sqrt{-1}\LieagbdPartial^{*}
    (\basexi{i}\wedge\basedualxi{j^{'}})
    =
    -\sqrt{-1}(-1)^{n^2}\star\,\LieagbdPartialbar\,\star
    (\basexi{i}\wedge\basedualxi{j^{'}}).
    \label{EQ-Kahler identity on Lie agbd-calculation for RHS of (i,j)-no1}
\end{align}
Calculating (\ref{EQ-Kahler identity on Lie agbd-calculation for RHS of (i,j)-no1}) step-by-step, we first apply the Hodge star to $(\basexi{i}\wedge\basedualxi{j^{'}})$:
\begin{align}
    \star(\basexi{i}\wedge\basedualxi{j^{'}})
    =
    2^{2-n}
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {i,j^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
        \basedualxi{1}
        \wedge\cdots\wedge
        \widehat{\basedualxi{i}}
        \wedge\cdots\wedge
        \basedualxi{n}
        \wedge
        \basexi{1^{'}}
        \wedge\cdots\wedge
        \widehat{\basexi{j^{'}}}
        \wedge\cdots\wedge
        \basexi{n^{'}}.
    \label{EQ-Kahler identity on Lie agbd-calculation for RHS of (i,j)-no2}
\end{align}
We then apply $\LieagbdPartialbar$ to (\ref{EQ-Kahler identity on Lie agbd-calculation for RHS of (i,j)-no2}) and obtain
\begin{align}
    &
        \LieagbdPartialbar\,\star(\basexi{i}\wedge\basedualxi{j^{'}})
    \notag
    \\
    =&
        2^{2-n}
        \begin{pmatrix*}[l]
            \displaystyle\sum_{k\neq i}
            \begin{matrix*}[l]
                \sgn
                    {1,\cdots,n,1^{'},c\dots,n^{'}}
                    {i,j^{'},1,\dots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
                \sgn
                    {1,\cdots,\widehat{i},\cdots,n}
                    {k,1,\cdots,\widehat{i},\cdots,\widehat{k},\cdots,n}
                \\
                \basedualxi{1}
                \wedge\cdots\wedge
                \widehat{\basedualxi{i}}
                \wedge\cdots\wedge
                (\LieagbdPartialbar\basedualxi{k})
                \wedge\cdots\wedge
                \basedualxi{n}
                \wedge
                \basexi{1^{'}}
                \wedge\cdots\wedge
                \widehat{\basexi{j^{'}}}
                \wedge\cdots\wedge
                \basexi{n^{'}}
            \end{matrix*}
            \\
            +
            \\
            \displaystyle\sum_{l^{'}\neq j^{'}}
            \begin{matrix*}[l]
                \sgn
                    {1,\cdots,n,1^{'},\cdots,n^{'}}
                    {i,j^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
                \sgn
                    {1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
                    {l^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,\widehat{l^{'}},\cdots,n^{'}}
                \\
                \basedualxi{1}
                \wedge\cdots\wedge
                \widehat{\basedualxi{i}}
                \wedge\cdots\wedge
                \basedualxi{n}
                \wedge
                \basexi{1^{'}}
                \wedge\cdots\wedge
                \widehat{\basexi{j^{'}}}
                \wedge\cdots\wedge
                (\LieagbdPartialbar\basexi{l^{'}})
                \wedge\cdots\wedge
                \basexi{n^{'}}
            \end{matrix*}
        \end{pmatrix*}
    \notag
    \\
    =&
        2^{2-n}
        \begin{pmatrix*}[l]
            \displaystyle\sum_{k\neq i}
            \begin{pmatrix*}[l]
                \sgn
                    {1,\cdots,n,1^{'},\cdots,n^{'}}
                    {i,j^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
                \sgn
                    {1,\cdots,\widehat{i},\cdots,n}
                    {k,1,\cdots,\widehat{i},\cdots,\widehat{k},\cdots,n}
                \\
                \basedualxi{1}
                \wedge\cdots\wedge
                \widehat{\basedualxi{i}}
                \wedge\cdots\wedge
                \basedualxi{k-1}
                \wedge
                \begin{pmatrix*}[l]
                    \frac{1}{2}
                    \coefD{k}{i k}
                    \basedualxi{i}\wedge\basedualxi{k}
                    \\
                    +
                    \\
                    \frac{1}{2}
                    \coefD{k}{k i}
                    \basedualxi{k}\wedge\basedualxi{i}
                \end{pmatrix*}
                \wedge
                \basedualxi{k+1}
                \wedge\cdots\wedge
                \basedualxi{n}
                \wedge
                \\
                \basexi{1^{'}}
                \wedge\cdots\wedge
                \widehat{\basexi{j^{'}}}
                \wedge\cdots\wedge
                \basexi{n^{'}}
            \end{pmatrix*}
            \\
            +
            \\
            \displaystyle\sum_{l^{'}\neq j^{'}}
            \begin{pmatrix*}[l]
                \sgn
                    {1,\cdots,n,1^{'},\cdots,n^{'}}
                    {i,j^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
                \sgn
                    {1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
                    {l^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,\widehat{l^{'}},\cdots,n^{'}}
                \\
                \basedualxi{1}
                \wedge\cdots\wedge
                \widehat{\basedualxi{i}}
                \wedge\cdots\wedge
                \basedualxi{n}
                \wedge
                \\
                \basexi{1^{'}}
                \wedge\cdots\wedge
                \widehat{\basexi{j^{'}}}
                \wedge\cdots\wedge
                \basexi{(l-1)^{'}}
                \wedge
                \begin{pmatrix*}[l]
                    \coefB{l^{'}}{l^{'} i}
                    \basexi{l^{'}}\wedge\basedualxi{i}
                    \\
                    +
                    \\
                    \coefB{l^{'}}{j^{'} i}
                    \basexi{j^{'}}\wedge\basedualxi{i}
                \end{pmatrix*}
                \wedge
                \basexi{(l+1)^{'}}
                \wedge\cdots\wedge
                \basexi{n^{'}}
            \end{pmatrix*}
        \end{pmatrix*}.
    \label{EQ-Kahler identity on Lie agbd-calculation for RHS of (i,j)-no3}
\end{align}
Looking at the component with $
    \begin{pmatrix*}[l]
    \frac{1}{2}
    \coefD{k}{i k}
    \basedualxi{i}\wedge\basedualxi{k}
    \\
    +
    \\
    \frac{1}{2}
    \coefD{k}{k i}
    \basedualxi{k}\wedge\basedualxi{i}
    \end{pmatrix*}
$, it can be simplified to 
\begin{align*}
    \sgn{k,i}{\order{k,i}}\coefD{k}{k i}\basedualxi{k}\wedge\basedualxi{i}.
\end{align*}
For the component with coefficient $B$, we break the sum and rearrange the terms in (\ref{EQ-Kahler identity on Lie agbd-calculation for RHS of (i,j)-no3}):
\begin{align}
    &
        \LieagbdPartialbar\,\star(\basexi{i}\wedge\basedualxi{j^{'}})
    \notag
    \\
    =&
        2^{2-n}
        \begin{pmatrix*}[l]
            \displaystyle\sum_{k\neq i}
            \begin{pmatrix*}[l]
                \sgn
                    {1,\cdots,n,1^{'},\cdots,n^{'}}
                    {i,j^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
                \sgn
                    {1,\cdots,\widehat{i},\cdots,n}
                    {k,1,\cdots,\widehat{i},\cdots,\widehat{k},\cdots,n}
                \\
                \basedualxi{1}
                \wedge\cdots\wedge
                \widehat{\basedualxi{i}}
                \wedge\cdots\wedge
                \basedualxi{k-1}
                \wedge
                \sgn
                    {k,i}
                    {\order{k,i}}
                \coefD{k}{k i}
                \basedualxi{k}\wedge\basedualxi{i}
                \wedge
                \basedualxi{k+1}
                \wedge\cdots\wedge
                \basedualxi{n}
                \\
                \wedge\basexi{1^{'}}
                \wedge\cdots\wedge
                \widehat{\basexi{j^{'}}}
                \wedge\cdots\wedge
                \basexi{n^{'}}
            \end{pmatrix*}
            \\
            +
            \\
            \displaystyle\sum_{l^{'}\neq j^{'}}
            \begin{pmatrix*}[l]
                \sgn
                    {1,\cdots,n,1^{'},\cdots,n^{'}}
                    {i,j^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
                \sgn
                    {1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
                    {l^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,\widehat{l^{'}},\cdots,n^{'}}
                \\
                \basedualxi{1}
                \wedge\cdots\wedge
                \widehat{\basedualxi{i}}
                \wedge\cdots\wedge
                \basedualxi{n}
                \\
                \wedge\basexi{1^{'}}
                \wedge\cdots\wedge
                \widehat{\basexi{j^{'}}}
                \wedge\cdots\wedge
                \basexi{(l-1)^{'}}
                \wedge
                \coefB{l^{'}}{l^{'} i}
                \basexi{l^{'}}\wedge\basedualxi{i}
                \wedge
                \basexi{(l+1)^{'}}
                \wedge\cdots\wedge
                \basexi{n^{'}}
            \end{pmatrix*}
            \\
            +
            \\
            \displaystyle\sum_{l^{'}\neq j^{'}}
            \begin{pmatrix*}[l]
                \sgn
                    {1,\cdots,n,1^{'},\cdots,n^{'}}
                    {i,j^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
                \sgn
                    {1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
                    {l^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,\widehat{l^{'}},\cdots,n^{'}}
                \\
                \basedualxi{1}
                \wedge\cdots\wedge
                \widehat{\basedualxi{i}}
                \wedge\cdots\wedge
                \basedualxi{n}
                \\
                \wedge\basexi{1^{'}}
                \wedge\cdots\wedge
                \widehat{\basexi{j^{'}}}
                \wedge\cdots\wedge
                \basexi{(l-1)^{'}}
                \wedge
                \coefB{l^{'}}{j^{'} i}
                \basexi{j^{'}}\wedge\basedualxi{i}
                \wedge
                \basexi{(l+1)^{'}}
                \wedge\cdots\wedge
                \basexi{n^{'}}
            \end{pmatrix*}
        \end{pmatrix*}
    \notag
    \\
    =&
        2^{2-n}
        \begin{pmatrix*}[l]
            \displaystyle\sum_{k\neq i}
            \begin{pmatrix*}[l]
                \sgn
                    {1,\cdots,n,1^{'},\cdots,n^{'}}
                    {i,j^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
                \sgn
                    {1,\cdots,\widehat{i},\cdots,n}
                    {k,1,\cdots,\widehat{i},\cdots,\widehat{k},\cdots,n}
                \sgn
                    {1,\cdots,\widehat{i},\cdots,k-1,k,i,k+1,\cdots,n}
                    {1,\cdots,n}
                \\
                \sgn
                    {k,i}
                    {\order{k,i}}
                \\
                \coefD{k}{\order{k,i}}
                \basedualxi{1}
                \wedge\cdots\wedge
                \basedualxi{n}
                \wedge
                \basexi{1^{'}}
                \wedge\cdots\wedge
                \widehat{\basexi{j^{'}}}
                \wedge\cdots\wedge
                \basexi{n^{'}}
            \end{pmatrix*}
            \\
            +
            \\
            \displaystyle\sum_{l^{'}\neq j^{'}}
            \begin{pmatrix*}[l]
                \sgn
                    {1,\cdots,n,1^{'},\cdots,n^{'}}
                    {i,j^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
                \sgn
                    {1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
                    {l^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,\widehat{l^{'}},\cdots,n^{'}}
                \\
                \sgn
                    {1,\cdots,\widehat{i}\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,(l-1)^{'},l^{'},i,(l+1)^{'},\cdots,n^{'}}
                    {1,\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
                \\
                \coefB{l^{'}}{l^{'} i}
                \basedualxi{1}
                \wedge\cdots\wedge
                \basedualxi{n}
                \wedge
                \basexi{1^{'}}
                \wedge\cdots\wedge
                \widehat{\basexi{j^{'}}}
                \wedge\cdots\wedge
                \basexi{n^{'}}
            \end{pmatrix*}
            \\
            +
            \\
            \displaystyle\sum_{l^{'}\neq j^{'}}
            \begin{pmatrix*}[l]
                \sgn
                    {1,\cdots,n,1^{'},\cdots,n^{'}}
                    {i,j^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
                \sgn
                    {1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
                    {l^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,\widehat{l^{'}},\cdots,n^{'}}
                \\
                \sgn
                    {1,\cdots,\widehat{i}\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,(l-1)^{'},j^{'},i,(l+1)^{'},\cdots,n^{'}}
                    {1,\cdots,n,1^{'},\cdots,\widehat{l^{'}},\cdots,n^{'}}
                \\
                \coefB{l^{'}}{j^{'} i}
                \basedualxi{1}
                \wedge\cdots\wedge
                \basedualxi{n}
                \wedge
                \basexi{1^{'}}
                \wedge\cdots\wedge
                \widehat{\basexi{l^{'}}}
                \wedge\cdots\wedge
                \basexi{n^{'}}
            \end{pmatrix*}
        \end{pmatrix*}.
    \label{EQ-Kahler identity on Lie agbd-calculation for RHS of (i,j)-no4}
\end{align}
The next step is applying $\star$ to (\ref{EQ-Kahler identity on Lie agbd-calculation for RHS of (i,j)-no4}). Observe that the exterior product of the frames in (\ref{EQ-Kahler identity on Lie agbd-calculation for RHS of (i,j)-no4}), like $\basedualxi{1}\wedge\cdots\wedge\basedualxi{n}\wedge\basexi{1^{'}}\wedge\cdots\wedge\widehat{\basexi{j^{'}}}\wedge\cdots\wedge\basexi{n^{'}}$, is not in the standard form where the holomorphic frames are in front of the anti-holomorphic frames. The expression of the Hodge star applying to this type of local frames is
\begin{align*}
    \star
    (\basedualxi{\indexIc}\wedge\basexi{\indexJpc})
    =
    2^{(|\indexIc|+|\indexJpc|-n)}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}{\indexIc,\indexJpc,\indexI,\indexJp}\basexi{\indexI}\wedge\basedualxi{\indexJp},
\end{align*}
where $\indexI$ and $\indexJp$ are the arrays of the index numbers. We use this formula and obtain the following expression: 
\begin{align}
    &
        \star\,\LieagbdPartialbar\,\star(\basexi{i}\wedge\basedualxi{j^{'}})
    \notag
    \\
    =&
        2^{2-n}
        \begin{pmatrix*}[l]
            \displaystyle\sum_{k\neq i}
            \begin{pmatrix*}[l]
                \sgn
                    {1,\cdots,n,1^{'},\cdots,n^{'}}
                    {i,j^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
                \sgn
                    {1,\cdots,\widehat{i},\cdots,n}
                    {k,1,\cdots,\widehat{i},\cdots,\widehat{k},\cdots,n}
                \sgn
                    {1,\cdots,\widehat{i},\cdots,k-1,k,i,k+1,\cdots,n}
                    {1,\cdots,n}
                \\
                \sgn
                    {k,i}
                    {\order{k,i}}
                \\
                \coefD{k}{\order{k,i}}
                \star
                (
                \basedualxi{1}
                \wedge\cdots\wedge
                \basedualxi{n}
                \wedge
                \basexi{1^{'}}
                \wedge\cdots\wedge
                \widehat{\basexi{j^{'}}}
                \wedge\cdots\wedge
                \basexi{n^{'}}
                )
            \end{pmatrix*}
            \\
            +
            \\
            \displaystyle\sum_{l^{'}\neq j^{'}}
            \begin{pmatrix*}[l]
                \sgn
                    {1,\cdots,n,1^{'},\cdots,n^{'}}
                    {i,j^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
                \sgn
                    {1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
                    {l^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,\widehat{l^{'}},\cdots,n^{'}}
                \\
                \sgn
                    {1,\cdots,\widehat{i}\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,(l-1)^{'},l^{'},i,(l+1)^{'},\cdots,n^{'}}
                    {1,\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
                \\
                \coefB{l^{'}}{l^{'} i}
                \star
                (
                \basedualxi{1}
                \wedge\cdots\wedge
                \basedualxi{n}
                \wedge
                \basexi{1^{'}}
                \wedge\cdots\wedge
                \widehat{\basexi{j^{'}}}
                \wedge\cdots\wedge
                \basexi{n^{'}}
                )
            \end{pmatrix*}
            \\
            +
            \\
            \displaystyle\sum_{l^{'}\neq j^{'}}
            \begin{pmatrix*}[l]
                \sgn
                    {1,\cdots,n,1^{'},\cdots,n^{'}}
                    {i,j^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
                \sgn
                    {1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
                    {l^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,\widehat{l^{'}},\cdots,n^{'}}
                \\
                \sgn
                    {1,\cdots,\widehat{i}\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,(l-1)^{'},j^{'},i,(l+1)^{'},\cdots,n^{'}}
                    {1,\cdots,n,1^{'},\cdots,\widehat{l^{'}},\cdots,n^{'}}
                \\
                \coefB{l^{'}}{j^{'} i}
                \star
                (
                \basedualxi{1}
                \wedge\cdots\wedge
                \basedualxi{n}
                \wedge
                \basexi{1^{'}}
                \wedge\cdots\wedge
                \widehat{\basexi{l^{'}}}
                \wedge\cdots\wedge
                \basexi{n^{'}}
                )
            \end{pmatrix*}
        \end{pmatrix*}
    \notag
    \\
    =&
        2^{2-n}
        \begin{pmatrix*}[l]
            \displaystyle\sum_{k\neq i}
            \begin{pmatrix*}[l]
                \sgn
                    {1,\cdots,n,1^{'},\cdots,n^{'}}
                    {i,j^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
                \sgn
                    {1,\cdots,\widehat{i},\cdots,n}
                    {k,1,\cdots,\widehat{i},\cdots,\widehat{k},\cdots,n}
                \sgn
                    {1,\cdots,\widehat{i},\cdots,k-1,k,i,k+1,\cdots,n}
                    {1,\cdots,n}
                \\
                \sgn
                    {k,i}
                    {\order{k,i}}
                \\
                \coefD{k}{\order{k,i}}
                2^{n+n-1-n}
                \sgn
                    {1^{'},\cdots,n^{'},1,\cdots,n}
                    {j^{'},1,\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
                \basexi{j^{'}}
            \end{pmatrix*}
            \\
            +
            \\
            \displaystyle\sum_{l^{'}\neq j^{'}}
            \begin{pmatrix*}[l]
                \sgn
                    {1,\cdots,n,1^{'},\cdots,n^{'}}
                    {i,j^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
                \sgn
                    {1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}                       {l^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,\widehat{l^{'}},\cdots,n^{'}}
                \\
                \sgn
                    {1,\cdots,\widehat{i}\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,(l-1)^{'},l^{'},i,(l+1)^{'},\cdots,n^{'}}
                    {1,\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
                \\
                \coefB{l^{'}}{l^{'} i}
                2^{n+n-1-n}
                \sgn
                    {1^{'},\cdots,n^{'},1,\cdots,n}
                    {j^{'},1,\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
                \basexi{j^{'}}
            \end{pmatrix*}
            \\
            +
            \\
            \displaystyle\sum_{l^{'}\neq j^{'}}
            \begin{pmatrix*}[l]
                \sgn
                    {1,\cdots,n,1^{'},\cdots,n^{'}}
                    {i,j^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
                \sgn
                    {1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
                    {l^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,\widehat{l^{'}},\cdots,n^{'}}
                \\
                \sgn
                    {1,\cdots,\widehat{i}\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,(l-1)^{'},j^{'},i,(l+1)^{'},\cdots,n^{'}}
                    {1,\cdots,n,1^{'},\cdots,\widehat{l^{'}},\cdots,n^{'}}
                \\
                \coefB{l^{'}}{j^{'} i}
                2^{n+n-1-n}
                \sgn
                    {1^{'},\cdots,n^{'},1,\cdots,n}
                    {l^{'},1,\cdots,n,1^{'},\cdots,\widehat{l^{'}},\cdots,n^{'}}
                \basexi{l^{'}}
            \end{pmatrix*}
        \end{pmatrix*}
    \nonumber\\
    =&
        2
        \begin{pmatrix*}[l]
            \displaystyle\sum_{k\neq i}
            \begin{pmatrix*}[l]
                \sgn
                    {1,\cdots,n,1^{'},\cdots,n^{'}}
                    {i,j^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
                \sgn
                    {1,\cdots,\widehat{i},\cdots,n}
                    {k,1,\cdots,\widehat{i},\cdots,\widehat{k},\cdots,n}
                \sgn
                    {1,\cdots,\widehat{i},\cdots,k-1,k,i,k+1,\cdots,n}
                    {1,\cdots,n}
                \\
                \sgn
                    {1^{'},\cdots,n^{'},1,\cdots,n}
                    {j^{'},1,\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
                \\
                \sgn
                    {k,i}
                    {\order{k,i}}
                \\
                \coefD{k}{\order{k,i}}
                \basexi{j^{'}}
            \end{pmatrix*}
            \\
            +
            \\
            \displaystyle\sum_{l^{'}\neq j^{'}}
            \begin{pmatrix*}[l]
                \sgn
                    {1,\cdots,n,1^{'},\cdots,n^{'}}
                    {i,j^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
                \sgn
                    {1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
                    {l^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,\widehat{l^{'}},\cdots,n^{'}}
                \\
                \sgn
                    {1,\cdots,\widehat{i}\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,(l-1)^{'},l^{'},i,(l+1)^{'},\cdots,n^{'}}
                    {1,\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
                \sgn
                    {1^{'},\cdots,n^{'},1,\cdots,n}
                    {j^{'},1,\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
                \\
                \coefB{l^{'}}{l^{'} i}
                \basexi{j^{'}}
            \end{pmatrix*}
            \\
            +
            \\
            \displaystyle\sum_{l^{'}\neq j^{'}}
            \begin{pmatrix*}[l]
                \sgn
                    {1,\cdots,n,1^{'},\cdots,n^{'}}
                    {i,j^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
                \sgn
                    {1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
                    {l^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,\widehat{l^{'}},\cdots,n^{'}}
                \\
                \sgn
                    {1,\cdots,\widehat{i}\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,(l-1)^{'},j^{'},i,(l+1)^{'},\cdots,n^{'}}
                    {1,\cdots,n,1^{'},\cdots,\widehat{l^{'}},\cdots,n^{'}}
                \sgn
                    {1^{'},\cdots,n^{'},1,\cdots,n}
                    {l^{'},1,\cdots,n,1^{'},\cdots,\widehat{l^{'}},\cdots,n^{'}}
                \\
                \coefB{l^{'}}{j^{'} i}
                \basexi{l^{'}}
            \end{pmatrix*}
        \end{pmatrix*}.
    \label{EQ-Kahler identity on Lie agbd-calculation for RHS of (i,j)-no5}
\end{align}
The signs of permutations in (\ref{EQ-Kahler identity on Lie agbd-calculation for RHS of (i,j)-no5}) can be simplified. The simplification can be found in Section \ref{apex-simplification for RHS of (i,j)}. We obtain the simplification of (\ref{EQ-Kahler identity on Lie agbd-calculation for RHS of (i,j)-no5}):
\begin{align}
        \star\,\LieagbdPartialbar\,\star(\basexi{i}\wedge\basedualxi{j^{'}})
    =
        2
        \begin{pmatrix*}[l]
            \displaystyle\sum_{k\neq i}
            (-1)^{n^2}
            \coefD{k}{\order{k,i}}
            \basexi{j^{'}}
            \\
            +
            \\
            \displaystyle\sum_{l^{'}\neq j^{'}}
            (-1)^{n^2}
            \coefB{l^{'}}{l^{'} i}
            \basexi{j^{'}}
            \\
            +
            \\
            \displaystyle\sum_{l^{'}\neq j^{'}}
            -(-1)^{n^2}
            \coefB{l^{'}}{j^{'} i}
            \basexi{l^{'}}
        \end{pmatrix*}
    =
        2(-1)^{n^2}
        \begin{pmatrix*}[l]
            \displaystyle\sum_{k\neq i}
            \coefD{k}{\order{k,i}}
            \basexi{j^{'}}
            \\
            +
            \\
            \displaystyle\sum_{l^{'}\neq j^{'}}
            \coefB{l^{'}}{l^{'} i}
            \basexi{j^{'}}
            \\
            -
            \\
            \displaystyle\sum_{l^{'}\neq j^{'}}
            \coefB{l^{'}}{j^{'} i}
            \basexi{l^{'}}
        \end{pmatrix*}
    .
\label{EQ-Kahler identity on Lie agbd-calculation for RHS of (i,j)-no6}
\end{align}
We rewrite 
$
\displaystyle\sum_{l^{'}\neq j^{'}}
\coefB{l^{'}}{l^{'} i}
\basexi{j^{'}}
=
\begin{pmatrix*}[l]
    \displaystyle\sum_{l^{'}=1}^{n}
    \coefB{l^{'}}{l^{'} i}
    \basexi{j^{'}}
\end{pmatrix*}
-
\coefB{j^{'}}{j^{'} i}
\basexi{j^{'}}
$
and
$
\displaystyle\sum_{l^{'}\neq j^{'}}
\coefB{l^{'}}{j^{'} i}
\basexi{l^{'}}
=
\begin{pmatrix*}[l]
                \displaystyle\sum_{l^{'}=1}^{n}
                \coefB{l^{'}}{j^{'} i}
                \basexi{l^{'}}
            \end{pmatrix*}
            -
                \coefB{j^{'}}{j^{'} i}
                \basexi{j^{'}}
$
. Then, (\ref{EQ-Kahler identity on Lie agbd-calculation for RHS of (i,j)-no6}) can be written into
\begin{align}
        2(-1)^{n^2}
        \begin{pmatrix*}[l]
            \displaystyle\sum_{l=1}^{n}
            \sgn
                {l,i}
                {\order{l,i}}
            \coefD{l}{\order{l,i}}
            \basexi{j^{'}}
            \\
            +
            \\
            \begin{pmatrix*}[l]
                \displaystyle\sum_{l^{'}=1}^{n}
                \coefB{l^{'}}{l^{'} i}
                \basexi{j^{'}}
            \end{pmatrix*}
            -
            \coefB{j^{'}}{j^{'} i}
            \basexi{j^{'}}
            \\
            -
            \\
            (
            \begin{pmatrix*}[l]
                \displaystyle\sum_{l^{'}=1}^{n}
                \coefB{l^{'}}{j^{'} i}
                \basexi{l^{'}}
            \end{pmatrix*}
            -
            \coefB{j^{'}}{j^{'} i}
            \basexi{j^{'}}
            )
        \end{pmatrix*}
    =
        2(-1)^{n^2}
        \begin{pmatrix*}[l]
            \displaystyle\sum_{l=1}^{n}
            \sgn
                {l,i}
                {\order{l,i}}
            \coefD{l}{\order{l,i}}
            \basexi{j^{'}}
            \\
            +
            \\
            \displaystyle\sum_{l^{'}=1}^{n}
            \coefB{l^{'}}{l^{'} i}
            \basexi{j^{'}}
            \\
            -
            \\
            \displaystyle\sum_{l^{'}=1}^{n}
            \coefB{l^{'}}{j^{'} i}
            \basexi{l^{'}}
        \end{pmatrix*}
    .
\label{EQ-Kahler identity on Lie agbd-calculation for RHS of (i,j)-no7}
\end{align}
Using $l$ to replace $l^{'}$ in $\displaystyle\sum_{l^{'}=1}^{n}\coefB{l^{'}}{l^{'} i}\basexi{j^{'}}$, we further simplify (\ref{EQ-Kahler identity on Lie agbd-calculation for RHS of (i,j)-no7}) and obtain
\begin{align}
        2(-1)^{n^2}
        \begin{pmatrix*}[l]
            \displaystyle\sum_{l=1}^{n}
            \sgn
                {l,i}
                {\order{l,i}}
            \coefD{l}{\order{l,i}}
            \basexi{j^{'}}
            \\
            +
            \\
            \displaystyle\sum_{l=1}^{n}
            \coefB{l}{l i}
            \basexi{j^{'}}
            \\
            -
            \\
            \displaystyle\sum_{l^{'}=1}^{n}
            \coefB{l^{'}}{j^{'} i}
            \basexi{l^{'}}
        \end{pmatrix*}
    =
        2(-1)^{n^2}
        \begin{pmatrix*}[l]
            \displaystyle\sum_{l=1}^{n}
            \sgn
                {l,i}
                {\order{l,i}}
            \coefD{l}{\order{l,i}}
            \basexi{j^{'}}
            +
            \coefB{l}{l i}
            \basexi{j^{'}}
            \\
            -
            \\
            \displaystyle\sum_{l^{'}=1}^{n}
            \coefB{l^{'}}{j^{'} i}
            \basexi{l^{'}}
        \end{pmatrix*},
\end{align}
then we use the constraint for coefficients $B$ and $D$ to achieve the final simplification of 
$\star\,\LieagbdPartialbar\,\star(\basexi{i}\wedge\basedualxi{j^{'}})$:
\begin{align*}
        \star\,\LieagbdPartialbar\,\star(\basexi{i}\wedge\basedualxi{j^{'}})
    =
        2(-1)^{n^2}
        \begin{pmatrix*}[l]
            \displaystyle\sum_{l=1}^{n}
            \coefB{i}{l l}
            \basexi{j^{'}}
            \\
            -
            \\
            \displaystyle\sum_{l^{'}=1}^{n}
            \coefB{l^{'}}{j^{'} i}
            \basexi{l^{'}}
        \end{pmatrix*}.
\end{align*}
Recall that $\partial^{*}=-(-1)^{n^2}\star\,\partialbar\,\star$. Thus, we can conclude that the right-hand side
\begin{align*}
    \sqrt{-1}\partial^{*}(\basexi{i}\wedge\basedualxi{j})
    =
    -2\sqrt{-1}
    \begin{pmatrix*}[l]
        \displaystyle\sum_{l=1}^{n}
        \coefB{i}{l l}
        \basexi{j^{'}}
        -
        \displaystyle\sum_{l^{'}=1}^{n}
        \coefB{l^{'}}{j^{'} i}
        \basexi{l^{'}}
     \end{pmatrix*}
\end{align*}
is equal to the left-hand side (\ref{EQ-Kahler identity on Lie agbd-calculation for LHS of (i,j)-result}).




==> 3/For_f__I,J_,_calculation_both_side.tex <==
Our proof comprises the following steps:
\begin{enumerate}
    \item Calculate $
    [\LieagbdPartialbar,\iotaW]
    (f\basexi{\indexI}\wedge\basedualxi{\indexJp})$.

    \item Calculate $
    \sqrt{-1}\LieagbdPartial^{*}
    (f\basexi{\indexI}\wedge\basedualxi{\indexJp})
    $.

    \item Calculate $
    (\LieagbdPartialbar f)
    \wedge
    \iotaW(\basexi{\indexI}\wedge\basedualxi{\indexJp})
    -
    (\iotaW\,\LieagbdPartialbar\,f)
    \basexi{\indexI}\wedge\basedualxi{\indexJp}
    $, which is obtained from Step 1.

    \item Calculate $
    -\sqrt{-1}(-1)^{n^{2}}
    \star
    \bigg(
        (\LieagbdPartialbar f)
        \wedge
        \star(\basexi{\indexI}\wedge\basedualxi{\indexJp})
    \bigg)
    $, which is obtained from Step 2.

    \item Assemble the results from Steps 3 and 4 and obtain the expression of $
    \sqrt{-1}\LieagbdPartial^{*}
    (f\basexi{\indexI}\wedge\basedualxi{\indexJp})
    $, then check this is equal to the expression of $
    [\LieagbdPartialbar,\iotaW]
    (f\basexi{\indexI}\wedge\basedualxi{\indexJp})$.
\end{enumerate}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% start expand the LHS %%%%%%%%%%%%%%
\keyword{Step 1: } Applying $
[\LieagbdPartialbar,\iotaW]
=
\LieagbdPartialbar\,\iotaW
-
\iotaW\,\LieagbdPartialbar
$ to $(f\basexi{\indexI}\wedge\basedualxi{\indexJp})$,
\begin{align*}
    [\LieagbdPartialbar,\iotaW](f\basexi{\indexI}\wedge\basedualxi{\indexJp})
    =&
        \LieagbdPartialbar\,\iotaW
        (f\basexi{\indexI}\wedge\basedualxi{\indexJp})
        -
        \iotaW\,\LieagbdPartialbar
        (f\basexi{\indexI}\wedge\basedualxi{\indexJp})
    \\
    =&
        \LieagbdPartialbar
        \begin{pmatrix*}[l]
            (\iotaW f)
            \wedge
            \basexi{\indexI}\wedge\basedualxi{\indexJp}
            +
            f\,\iotaW(\basexi{\indexI}\wedge\basedualxi{\indexJp})
        \end{pmatrix*}
        -
        \iotaW
        \begin{pmatrix*}[l]
            (\LieagbdPartialbar f)
            \wedge\basexi{\indexI}\wedge\basedualxi{\indexJp}
            +
            f\,
            \LieagbdPartialbar(\basexi{\indexI}\wedge\basedualxi{\indexJp})
        \end{pmatrix*},
\end{align*}
where $\iotaW f=0$. Continuing the calculation,
\begin{align}
    &
        \LieagbdPartialbar
        \begin{pmatrix*}[l]
            f\,\iotaW(\basexi{\indexI}\wedge\basedualxi{\indexJp})
        \end{pmatrix*}
        -
        \iotaW\begin{pmatrix*}[l]
            (\LieagbdPartialbar f)
            \wedge\basexi{\indexI}\wedge\basedualxi{\indexJp}
            +
            f\,
            \LieagbdPartialbar(\basexi{\indexI}\wedge\basedualxi{\indexJp})
        \end{pmatrix*}
\notag
    \\
    =&
        (\LieagbdPartialbar f)
        \wedge
        \iotaW(\basexi{\indexI}\wedge\basedualxi{\indexJp})
        +
        f\,\LieagbdPartialbar\,\iotaW
        (\basexi{\indexI}\wedge\basedualxi{\indexJp})
        -
        \begin{pmatrix*}
            (\iotaW\,\LieagbdPartialbar\,f)
            \basexi{\indexI}\wedge\basedualxi{\indexJp}
            +
            f\cdot\iotaW\,\LieagbdPartialbar
            (\basexi{\indexI}\wedge\basedualxi{\indexJp})
        \end{pmatrix*} 
\notag
    \\
    =&
        f\,(\LieagbdPartialbar\,\iotaW-\iotaW\,\LieagbdPartialbar)
        (\basexi{\indexI}\wedge\basedualxi{\indexJp})
        +
        (\LieagbdPartialbar f)
        \wedge
        \iotaW(\basexi{\indexI}\wedge\basedualxi{\indexJp})
        -
        (\iotaW\,\LieagbdPartialbar\,f)
        \basexi{\indexI}\wedge\basedualxi{\indexJp}
\notag
    \\
    =&
        f\,[\LieagbdPartialbar,\iotaW]
        (\basexi{\indexI}\wedge\basedualxi{\indexJp})
        +
        (\LieagbdPartialbar f)
        \wedge
        \iotaW(\basexi{\indexI}\wedge\basedualxi{\indexJp})
        -
        (\iotaW\,\LieagbdPartialbar\,f)
        \basexi{\indexI}\wedge\basedualxi{\indexJp}
    .
\label{EQ-For f (I,J), calculation both side-expression of LHS}
\end{align}
We can separate (\ref{EQ-For f (I,J), calculation both side-expression of LHS}) into two parts:
\begin{itemize}
    \item The first part is $
    f\,[\LieagbdPartialbar,\iotaW]
    (\basexi{\indexI}\wedge\basedualxi{\indexJp})
    $.

    \item The second part is
    \begin{align}
        (\LieagbdPartialbar f)
        \wedge
        \iotaW(\basexi{\indexI}\wedge\basedualxi{\indexJp})
        -
        (\iotaW\,\LieagbdPartialbar\,f)
        \basexi{\indexI}\wedge\basedualxi{\indexJp}
        ,
    \label{EQ-For f (I,J), calculation both side-expression of LHS, the second part}
    \end{align}
    which is equal to a corresponding term in the expression of $
    \sqrt{-1}\LieagbdPartial^{*}
    (f\basexi{\indexI}\wedge\basedualxi{\indexJp})
    $. We return to this later.
\end{itemize}
%%%%%%%%%%%%%% finish expand the LHS %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% start expand the RHS %%%%%%%%%%%%%%
\keyword{Step 2:} Recall that $
\partial^{*}=-(-1)^{n^2}\star\,\LieagbdPartialbar\,\star
$. Thus, we complete the following calculation:
\begin{align}
    &
        -\sqrt{-1}(-1)^{n^{2}}
        \star\,\LieagbdPartialbar\,\star
        (f\basexi{\indexI}\wedge\basedualxi{\indexJp})
\notag
    \\
    =&
        -\sqrt{-1}(-1)^{n^{2}}
        \star\,\LieagbdPartialbar
        \big(
            f\,\star
            (\basexi{\indexI}\wedge\basedualxi{\indexJp})
        \big)
\notag
    \\
    =&
        -\sqrt{-1}(-1)^{n^{2}}
        \star
        \bigg(
            (\LieagbdPartialbar f)
            \wedge
            \star(\basexi{\indexI}\wedge\basedualxi{\indexJp})
            +
            f\, \LieagbdPartialbar\,\star
            (\basexi{\indexI}\wedge\basedualxi{\indexJp})
        \bigg)
\notag
    \\
    =&
        -\sqrt{-1}(-1)^{n^{2}}
        \star
        \bigg(
            (\LieagbdPartialbar f)
            \wedge
            \star(\basexi{\indexI}\wedge\basedualxi{\indexJp})
        \bigg)
        +
        \sqrt{-1}f\,
        \bigg(
            -(-1)^{n^{2}}
            \star\,\LieagbdPartialbar\,\star
            (\basexi{\indexI}\wedge\basedualxi{\indexJp})
        \bigg)
\notag
    \\
    =&
        -\sqrt{-1}(-1)^{n^{2}}
        \star
        \bigg(
            (\LieagbdPartialbar f)
            \wedge
            \star(\basexi{\indexI}\wedge\basedualxi{\indexJp})
        \bigg)
        +
        f\,\sqrt{-1}\LieagbdPartial^{*}
        (\basexi{\indexI}\wedge\basedualxi{\indexJp})
    .
\label{EQ-For f (I,J), calculation both side-expression of RHS}
\end{align}
Summarizing the above computation, we can separate (\ref{EQ-For f (I,J), calculation both side-expression of LHS}) into two parts:
\begin{itemize}
    \item The first part is $
    f\,\sqrt{-1}\LieagbdPartial^{*}
    (\basexi{\indexI}\wedge\basedualxi{\indexJp})
    $.

    \item The second part is 
    \begin{align}
        -\sqrt{-1}(-1)^{n^{2}}
        \star
        \bigg(
            (\LieagbdPartialbar f)
            \wedge
            \star(\basexi{\indexI}\wedge\basedualxi{\indexJp})
        \bigg)
        ,
    \label{EQ-For f (I,J), calculation both side-expression of RHS, the second part}
    \end{align}
     which we check in the next step and is equal to (\ref{EQ-For f (I,J), calculation both side-expression of LHS, the second part}).
\end{itemize}
%%%%%%%%%%%%%% finish expand the LHS %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% start checking the LHD second part %%%%%%%%%%%%%%
%\label{EQ-For f (I,J), calculation both side-step3, first part in LHS}
\keyword{Step 3:} Using $
    \iotaW
    =
    -\frac{\sqrt{-1}}{2}\displaystyle\sum_{r=1}^{n}\contract{\basedualxi{r^{'}}}\,\contract{\basexi{r}}
$ and the definition of $\LieagbdPartialbar$, we can write
\begin{align}
    &
        (\LieagbdPartialbar f)
        \wedge
        \iotaW(\basexi{\indexI}\wedge\basedualxi{\indexJp})
        -
        (\iotaW\,\LieagbdPartialbar\,f)
        \basexi{\indexI}\wedge\basedualxi{\indexJp}
\notag
    \\
    =&
        (
        \displaystyle\sum_{j^{'}=1}^{n}
        \rho(\basedualv{j^{'}})(f) 
        \basedualxi{j^{'}}
        )
        \wedge
        (-\frac{\sqrt{-1}}{2})
        \displaystyle\sum_{r=1}^{n}
        \contract{\basedualxi{r^{'}}}\,\contract{\basexi{r}}
        (
        \basexi{\indexI}\wedge\basedualxi{\indexJp}
        )
\label{EQ-For f (I,J), calculation both side-step3, first part in LHS}
    \\
    &   
        -
\notag
    \\
    &
        (-\frac{\sqrt{-1}}{2})
        \displaystyle\sum_{r=1}^{n}
        \contract{\basedualxi{r^{'}}}\,\contract{\basexi{r}}
        \big(
        \displaystyle\sum_{j=1}^{n}
        \rho(\basedualv{j^{'}})(f)\,
        \basedualxi{j^{'}}
        \wedge
        \basexi{\indexI}
        \wedge
        \basedualxi{\indexJp}
        \big)
    .
\label{EQ-For f (I,J), calculation both side-step3, second part in LHS}
\end{align}

%%%%


To simplify (\ref{EQ-For f (I,J), calculation both side-step3, first part in LHS}), we write 
\begin{align*}
    \contract{\basedualxi{r^{'}}}\,\contract{\basexi{r}}
    (\basexi{\indexI}\wedge\basedualxi{\indexJp})
    =& 
        \contract{\basedualxi{r^{'}}}
        \big(
            2\,
            \sgn
                {\indexI,\indexJp}
                {r,\indexI\backslash\{r\},\indexJp}
            \basexi{\indexI\backslash\{r\}}\wedge\basedualxi{\indexJp}
        \big)
    \\
    =&
        4\,
        \sgn
            {\indexI,\indexJp}
            {r,\indexI\backslash\{r\},\indexJp}
        \sgn
            {\indexI\backslash\{r\},\indexJp}
            {r^{'},\indexI\backslash\{r\},\indexJp\backslash\{r'\}}
        \basexi{\indexI\backslash\{r\}}\wedge\basedualxi{\indexJp\backslash\{r'\}}
    \\
    =&
        4\,
        \sgn
            {\indexI,\indexJp}
            {r,r^{'},\indexI\backslash\{r\},\indexJp\backslash\{r'\}}
        \basexi{\indexI\backslash\{r\}}\wedge\basedualxi{\indexJp\backslash\{r'\}}
\end{align*}
for $r\in\indexI\cap\indexJ$ and $
\contract{\basedualxi{r^{'}}}\,\contract{\basexi{r}}
(\basexi{\indexI}\wedge\basedualxi{\indexJp})
=0
$ for $r\in(\indexI\cup\indexJ)^{C}$. We then plug this into (\ref{EQ-For f (I,J), calculation both side-step3, first part in LHS}):
\begin{align}
    &
        \displaystyle\sum_{j^{'}=1}^{n}
        \rho(\basedualv{j^{'}})(f)\,
        \basedualxi{j^{'}}
        \wedge
        (-\frac{\sqrt{-1}}{2})
        \displaystyle\sum_{r\in\indexI\cap\indexJ}
        4\, \sgn
            {\indexI,\indexJp}
            {r,r^{'},\indexI\backslash\{r\},\indexJp\backslash\{r^{'}\}}
        \basexi{\indexI\backslash\{r\}}
        \wedge
        \basedualxi{\indexJp\backslash\{r^{'}\}}
    .
\label{EQ-For f (I,J), calculation both side-step3, first part in LHS, simplifying no1}
\end{align}
The terms such that $j^{'}\in\indexJp\backslash\{r^{'}\}$ are zero due to the repeated frames in the wedge product. We separate the sum into two cases, $j^{'}\in\indexJpc$ and $j^{'}=r^{'}$, and rewrite (\ref{EQ-For f (I,J), calculation both side-step3, first part in LHS, simplifying no1}):
\begin{align*}
    &
        \begin{pmatrix*}[l]
            \displaystyle\sum_{j^{'}\in\indexJpc}
            \rho(\basedualv{j^{'}})(f)\,
            \basedualxi{j^{'}}
            \wedge
            (-\frac{\sqrt{-1}}{2})
            \displaystyle\sum_{r\in\indexI\cap\indexJ}
            4\, \sgn
                {\indexI,\indexJp}
                {r,r^{'},\indexI\backslash\{r\},\indexJp\backslash\{r^{'}\}}
            \basexi{\indexI\backslash\{r\}}
            \wedge
            \basedualxi{\indexJp\backslash\{r^{'}\}}
            \\
            +
            \\
            \displaystyle\sum_{j^{'}=r^{'}}
            \rho(\basedualv{j^{'}})(f)\,
            \basedualxi{j^{'}}
            \wedge
            (-\frac{\sqrt{-1}}{2})
            \displaystyle\sum_{r\in\indexI\cap\indexJ}
            4\, \sgn
                {\indexI,\indexJp}
                {r,r^{'},\indexI\backslash\{r\},\indexJp\backslash\{r^{'}\}}
            \basexi{\indexI\backslash\{r\}}
            \wedge
            \basedualxi{\indexJp\backslash\{r^{'}\}}
        \end{pmatrix*}
    \\
    =&
        \begin{pmatrix*}[l]
            -2\sqrt{-1}
            \displaystyle\sum_{j^{'}\in\indexJpc}
            \displaystyle\sum_{r\in\indexI\cap\indexJ}
            \sgn
                {\indexI,\indexJp}
                {r,r^{'},\indexI\backslash\{r\},\indexJp\backslash\{r^{'}\}}
            \rho(\basedualv{j^{'}})(f)\,
            \basedualxi{j^{'}}
            \wedge
            \basexi{\indexI\backslash\{r\}}
            \wedge
            \basedualxi{\indexJp\backslash\{r^{'}\}}
            \\
            +
            \\
            -2\sqrt{-1}
            \displaystyle\sum_{r\in\indexI\cap\indexJ}
            \sgn
                {\indexI,\indexJp}
                {r,r^{'},\indexI\backslash\{r\},\indexJp\backslash\{r^{'}\}}
            \rho(\basedualv{r^{'}})(f)\,
            \basedualxi{r^{'}}
            \wedge
            \basexi{\indexI\backslash\{r\}}
            \wedge
            \basedualxi{\indexJp\backslash\{r^{'}\}}
        \end{pmatrix*}
    .
\end{align*}
Checking that
\begin{itemize}
    \item 
$
        \basedualxi{r^{'}}
        \wedge
        \basexi{\indexI\backslash\{r\}}
        \wedge
        \basedualxi{\indexJp\backslash\{r^{'}\}}
    =
        \sgn
            {r^{'},\indexI\backslash\{r\},\indexJp\backslash\{r^{'}\}}
            {\indexI\backslash\{r\},\indexJp}
        \basexi{\indexI\backslash\{r\}}
        \wedge
        \basedualxi{\indexJp}
$,
    \item 
$
        \sgn
            {\indexI,\indexJp}
            {r,r^{'},\indexI\backslash\{r\},\indexJp\backslash\{r^{'}\}}
        \sgn
            {r^{'},\indexI\backslash\{r\},\indexJp\backslash\{r^{'}\}}
            {\indexI\backslash\{r\},\indexJp}
        =
        \sgn
            {\indexI,\indexJp}
            {r,\indexI\backslash\{r\},\indexJp}
$,
\end{itemize}
we conclude that the expression of $
(\LieagbdPartialbar f)
\wedge
\iotaW(\basexi{\indexI}\wedge\basedualxi{\indexJp})
$ is 
\begin{align}
    \begin{pmatrix*}[l]
        (-2\sqrt{-1})
        \displaystyle\sum_{j^{'}\in{\indexJpc}}
        \displaystyle\sum_{r\in\indexI\cap\indexJ}
        \sgn
            {\indexI,\indexJp}
            {r,r^{'},\indexI\backslash\{r\},\indexJp\backslash\{r^{'}\}}
        \rho(\basedualv{j^{'}})(f)\,
        \basedualxi{j^{'}}
        \wedge
        \basexi{\indexI\backslash\{r\}}
        \wedge
        \basedualxi{\indexJp\backslash\{r^{'}\}}
        \\
        +
        \\(-2\sqrt{-1})
        \displaystyle\sum_{r\in\indexI\cap\indexJ}
        \sgn
            {\indexI}
            {r,\indexI\backslash\{r\}}
        \rho(\basedualv{r^{'}})(f)\,
        \basexi{\indexI\backslash\{r\}}
        \wedge
        \basedualxi{\indexJp}
    \end{pmatrix*}
    .
\label{EQ-For f (I,J), calculation both side-step 3, before final result, the simplified first term}
\end{align}

Next, we simplify (\ref{EQ-For f (I,J), calculation both side-step3, second part in LHS}). Observing that $\basedualxi{j^{'}}
\wedge
\basexi{\indexI}
\wedge
\basedualxi{\indexJp}=0
$ when $j^{'}\in\indexJp$, we first simplify (\ref{EQ-For f (I,J), calculation both side-step3, second part in LHS}) to
\begin{align}
    (-\frac{\sqrt{-1}}{2})
    \displaystyle\sum_{r=1}^{n}
    \contract{\basedualxi{r^{'}}}\,\contract{\basexi{r}}
    \big(
        \displaystyle\sum_{j\in\indexJpc}
        \rho(\basedualv{j^{'}})(f)\,
        \basedualxi{j^{'}}
        \wedge
        \basexi{\indexI}
        \wedge
        \basedualxi{\indexJp}
    \big)
    .
\label{EQ-For f (I,J), calculation both side-step3, second part in LHS,simplying no1}
\end{align}
We then observe that $
\contract{\basedualxi{r^{'}}}\,\contract{\basexi{r}}
(
    \basedualxi{j^{'}}
    \wedge
    \basexi{\indexI}
    \wedge
    \basedualxi{\indexJp}
)
$ is equal to zero except for $r\in\indexI\cap\indexJ$ or $r=j\in\indexI\cap\indexJc$. Thus, (\ref{EQ-For f (I,J), calculation both side-step3, second part in LHS,simplying no1}) can be split into
\begin{align}
    &
        \begin{pmatrix*}[l]
            (-\frac{\sqrt{-1}}{2})
            \displaystyle\sum_{r\in\indexI\cap\indexJ}
            \contract{\basedualxi{r^{'}}}\,\contract{\basexi{r}}
            \big(
                \displaystyle\sum_{j\in\indexJpc}
                \rho(\basedualv{j^{'}})(f)\,
                \basedualxi{j^{'}}
                \wedge
                \basexi{\indexI}
                \wedge
                \basedualxi{\indexJp}
            \big)
        \\
        +
        \\
            (-\frac{\sqrt{-1}}{2})
            \displaystyle\sum_{r\in\indexI\cap\indexJc}
            \contract{\basedualxi{r^{'}}}\,\contract{\basexi{r}}
            \big(
                \rho(\basedualv{r^{'}})(f)\,
                \basedualxi{r^{'}}
                \wedge
                \basexi{\indexI}
                \wedge
                \basedualxi{\indexJp}
            \big)
        \end{pmatrix*}
\notag
    \\
    =&
        \begin{pmatrix*}[l]
            (-\frac{\sqrt{-1}}{2})
            \displaystyle\sum_{r\in\indexI\cap\indexJ}
            \displaystyle\sum_{j\in\indexJpc}
            \rho(\basedualv{j^{'}})(f)\,
            \contract{\basedualxi{r^{'}}}\,\contract{\basexi{r}}
            \big(
                \basedualxi{j^{'}}
                \wedge
                \basexi{\indexI}
                \wedge
                \basedualxi{\indexJp}
            \big)
        \\
        +
        \\
            (-\frac{\sqrt{-1}}{2})
            \displaystyle\sum_{r\in\indexI\cap\indexJc}
            \rho(\basedualv{r^{'}})(f)\,
            \contract{\basedualxi{r^{'}}}\,\contract{\basexi{r}}
            \big(
                \basedualxi{r^{'}}
                \wedge
                \basexi{\indexI}
                \wedge
                \basedualxi{\indexJp}
            \big)
        \end{pmatrix*},
\label{EQ-For f (I,J), calculation both side-step3, second part in LHS,simplying no2}
\end{align}
in which
\begin{align}
    \contract{\basedualxi{r^{'}}}\,\contract{\basexi{r}}
    (
        \basedualxi{j^{'}}
        \wedge
        \basexi{\indexI}
        \wedge
        \basedualxi{\indexJp}
    )
    =&
        \contract{\basedualxi{r^{'}}}
        \big(
            2\,
            \sgn
                {j^{'},\indexI,\indexJp}
                {r,j^{'},\indexI\backslash\{r\},\indexJp}
            \basedualxi{j^{'}}
            \wedge
            \basexi{\indexI\backslash\{r\}}
            \wedge
            \basedualxi{\indexJp}
        \big)
\notag
    \\
    =&
        4\,
        \sgn
            {j^{'},\indexI,\indexJp}
            {r,j^{'},\indexI\backslash\{r\},\indexJp}
        \sgn
            {j^{'},\indexI\backslash\{r\},\indexJp}
            {r^{'},j^{'},\indexI\backslash\{r\},\indexJp\backslash\{r^{'}\}}
        \basedualxi{j^{'}}
        \wedge
        \basexi{\indexI\backslash\{r\}}
        \wedge
        \basedualxi{\indexJp\backslash\{r^{'}\}}
\notag
    \\
    =&
        4\,
        \sgn
            {j^{'},\indexI,\indexJp}
            {r,r^{'},j^{'},\indexI\backslash\{r\},\indexJp\backslash\{r^{'}\}}
        \basedualxi{j^{'}}
        \wedge
        \basexi{\indexI\backslash\{r\}}
        \wedge
        \basedualxi{\indexJp\backslash\{r^{'}\}}
    \\
    =&
        4\,
        \sgn
            {\indexI,\indexJp}
            {r,r^{'},\indexI\backslash\{r\},\indexJp\backslash\{r^{'}\}}
        \basedualxi{j^{'}}
        \wedge
        \basexi{\indexI\backslash\{r\}}
        \wedge
        \basedualxi{\indexJp\backslash\{r^{'}\}},
\label{EQ-For f (I,J), calculation both side-step3, second part in LHS,calculate contraction no1}
\end{align}
where the number $2$ in the first row is obtained from $\contract{\basexi{r}}(\basexi{r})=2$ since $\norm{\basexi{r}}{h}=2$, and
\begin{align}
    \contract{\basedualxi{r^{'}}}\,\contract{\basexi{r}}
    (
        \basedualxi{r^{'}}
        \wedge
        \basexi{\indexI}
        \wedge
        \basedualxi{\indexJp}
    )
    =&
        \contract{\basedualxi{r^{'}}}
        \big(
            2\,
            \sgn
                {r^{'},\indexI,\indexJp}
                {r,r^{'},\indexI\backslash\{r\},\indexJp}
            \basedualxi{r^{'}}
            \wedge
            \basexi{\indexI\backslash\{r\}}
            \wedge
            \basedualxi{\indexJp}
        \big)
\notag
    \\
    =&
        4\,
        \sgn
            {r^{'},\indexI,\indexJp}
            {r,r^{'},\indexI\backslash\{r\},\indexJp}
        \basexi{\indexI\backslash\{r\}}
        \wedge
        \basedualxi{\indexJp}
\notag
    \\
    =&
        -4\,
        \sgn
            {\indexI,\indexJp}
            {r,\indexI\backslash\{r\},\indexJp}
        \basexi{\indexI\backslash\{r\}}
        \wedge
        \basedualxi{\indexJp}
    .
\label{EQ-For f (I,J), calculation both side-step3, second part in LHS,calculate contraction no2}
\end{align}
Plugging (\ref{EQ-For f (I,J), calculation both side-step3, second part in LHS,calculate contraction no1}) and (\ref{EQ-For f (I,J), calculation both side-step3, second part in LHS,calculate contraction no2}) into (\ref{EQ-For f (I,J), calculation both side-step3, second part in LHS,simplying no2}), we conclude that the expression of $
(\iotaW\,\LieagbdPartialbar\,f)
\basexi{\indexI}\wedge\basedualxi{\indexJp}
$ is
\begin{align}
    &
        \begin{pmatrix*}[l]
        (-\frac{\sqrt{-1}}{2})
        \displaystyle\sum_{r\in\indexI\cap\indexJ}
        \displaystyle\sum_{j\in\indexJpc}
        \rho(\basedualv{j^{'}})(f)\,
        4\,
        \sgn
            {\indexI,\indexJp}
            {r,r^{'},\indexI\backslash\{r\},\indexJp\backslash\{r^{'}\}}
        \basedualxi{j^{'}}
        \wedge
        \basexi{\indexI\backslash\{r\}}
        \wedge
        \basedualxi{\indexJp\backslash\{r^{'}\}}
        \\
        +
        \\
        (-\frac{\sqrt{-1}}{2})
        \displaystyle\sum_{r\in\indexI\cap\indexJc}
        \rho(\basedualv{r^{'}})(f)\,
        (-4)\,
        \sgn
            {\indexI}
            {r,\indexI\backslash\{r\}}
        \basexi{\indexI\backslash\{r\}}
        \wedge
        \basedualxi{\indexJp}
    \end{pmatrix*}
\notag
    \\
    =&
        \begin{pmatrix*}[l]
        (-2\sqrt{-1})
        \displaystyle\sum_{r\in\indexI\cap\indexJ}
        \displaystyle\sum_{j\in\indexJpc}
        \sgn
            {\indexI,\indexJp}
            {r,r^{'},\indexI\backslash\{r\},\indexJp\backslash\{r^{'}\}}
        \rho(\basedualv{j^{'}})(f)\,
        \basedualxi{j^{'}}
        \wedge
        \basexi{\indexI\backslash\{r\}}
        \wedge
        \basedualxi{\indexJp\backslash\{r^{'}\}}
        \\
        +
        \\
        (-2\sqrt{-1})
        \displaystyle\sum_{r\in\indexI\cap\indexJc}
        (-1)
        \sgn
            {\indexI}
            {r,\indexI\backslash\{r\}}
        \rho(\basedualv{r^{'}})(f)\,
        \basexi{\indexI\backslash\{r\}}
        \wedge
        \basedualxi{\indexJp}
    \end{pmatrix*}
    .
\label{EQ-For f (I,J), calculation both side-step 3, before final result, the simplified second term}
\end{align}

Finally, we conclude that $
(\LieagbdPartialbar f)
\wedge
\iotaW(\basexi{\indexI}\wedge\basedualxi{\indexJp})
-
(\iotaW\,\LieagbdPartialbar\,f)
\basexi{\indexI}\wedge\basedualxi{\indexJp}
$ is equal to (\ref{EQ-For f (I,J), calculation both side-step 3, before final result, the simplified first term}) \(-\) (\ref{EQ-For f (I,J), calculation both side-step 3, before final result, the simplified second term}), which is
\begin{align*}
    &
    \begin{pmatrix*}[l]
        (-2\sqrt{-1})
        \displaystyle\sum_{j^{'}\in{\indexJpc}}
        \displaystyle\sum_{r\in\indexI\cap\indexJ}
        \sgn
            {\indexI,\indexJp}
            {r,r^{'},\indexI\backslash\{r\},\indexJp\backslash\{r^{'}\}}
        \rho(\basedualv{j^{'}})(f)\,
        \basedualxi{j^{'}}
        \wedge
        \basexi{\indexI\backslash\{r\}}
        \wedge
        \basedualxi{\indexJp\backslash\{r^{'}\}}
        \\
        +
        \\
        (-2\sqrt{-1})
        \displaystyle\sum_{r\in\indexI\cap\indexJ}
        \sgn
            {\indexI}
            {r,\indexI\backslash\{r\}}
        \rho(\basedualv{r^{'}})(f)\,
        \basexi{\indexI\backslash\{r\}}
        \wedge
        \basedualxi{\indexJp}
    \end{pmatrix*}
    \\
    &-
    \\
    &
    \begin{pmatrix*}[l]
        (-2\sqrt{-1})
        \displaystyle\sum_{r\in\indexI\cap\indexJ}
        \displaystyle\sum_{j\in\indexJpc}
        \sgn
            {\indexI,\indexJp}
            {r,r^{'},\indexI\backslash\{r\},\indexJp\backslash\{r^{'}\}}
        \rho(\basedualv{j^{'}})(f)\,
        \basedualxi{j^{'}}
        \wedge
        \basexi{\indexI\backslash\{r\}}
        \wedge
        \basedualxi{\indexJp\backslash\{r^{'}\}}
        \\
        +
        \\
        (-2\sqrt{-1})
        \displaystyle\sum_{r\in\indexI\cap\indexJc}
        (-1)
        \sgn
            {\indexI}
            {r,\indexI\backslash\{r\}}
        \rho(\basedualv{r^{'}})(f)\,
        \basexi{\indexI\backslash\{r\}}
        \wedge
        \basedualxi{\indexJp}
    \end{pmatrix*}
    .
\end{align*}
The cancellation is clear and results in the final simplified expression:
\begin{align}
    &
        \begin{pmatrix*}[l]
            (-2\sqrt{-1})
            \displaystyle\sum_{r\in\indexI\cap\indexJ}
            \sgn
                {\indexI}
                {r,\indexI\backslash\{r\}}
            \rho(\basedualv{r^{'}})(f)\,
            \basexi{\indexI\backslash\{r\}}
            \wedge
            \basedualxi{\indexJp}
            \\
            +
            \\
            (-2\sqrt{-1})
            \displaystyle\sum_{r\in\indexI\cap\indexJc}
            (-1)
            \sgn
                {\indexI}
                {r,\indexI\backslash\{r\}}
            \rho(\basedualv{r^{'}})(f)\,
            \basexi{\indexI\backslash\{r\}}
            \wedge
            \basedualxi{\indexJp}
        \end{pmatrix*}
\notag
    \\
    =&
        (-2\sqrt{-1})
        \displaystyle\sum_{r\in\indexI}
        \sgn
            {\indexI}
            {r,\indexI\backslash\{r\}}
        \rho(\basedualv{r^{'}})(f)\,
        \basexi{\indexI\backslash\{r\}}
        \wedge
        \basedualxi{\indexJp}.
\label{EQ-For f (I,J), calculation both side-step 3, result}
\end{align}

%%%%%%%%%%%%%% finish checking the LHS second part %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% start checking the RHS second part %%%%%%%%%%%%%%
\keyword{Step 4:} Recalling the definitions of $(\LieagbdPartialbar f)$ and $\star$, we obtain
\begin{align}
    (\LieagbdPartialbar f)
    \wedge
    \star(\basexi{\indexI}\wedge\basedualxi{\indexJp})
    =
    \bigg(
        \displaystyle\sum_{i=1}^{n}
        \rho(\basedualv{i^{'}})(f)\,\basedualxi{i}
    \bigg)
    \wedge
    \bigg(
        2^{p+q-n}
        \sgn
            {1,\cdots,n,1^{'},1^{'},\cdots,n^{'}}
            {\indexI,\indexJp,\indexIc,\indexJpc}
        \basedualxi{\indexIc}\wedge\basexi{\indexJpc}
    \bigg)
    .
\label{EQ-For f (I,J), calculation both side-step4,equation no1}
\end{align}
It can be observed that the terms such that $i\in\indexIc$ are zero due to the repeated $\basedualxi{i}$ in the wedge product of frames. Thus, we simplify (\ref{EQ-For f (I,J), calculation both side-step4,equation no1}) to
\begin{align}
    &
    \bigg(
        \displaystyle\sum_{i\in\indexI}
        \rho(\basedualv{i^{'}})(f)\,\basedualxi{i}
    \bigg)
    \wedge
    \bigg(
        2^{p+q-n}
        \sgn
            {1,\cdots,n,1^{'},1^{'},\cdots,n^{'}}
            {\indexI,\indexJp,\indexIc,\indexJpc}
        \basedualxi{\indexIc}\wedge\basexi{\indexJpc}
    \bigg)
\notag
    \\
    =&
        \displaystyle\sum_{i\in\indexI}
        2^{p+q-n}
        \rho(\basedualv{i^{'}})(f)\,
        \sgn
            {1,\cdots,n,1^{'},1^{'},\cdots,n^{'}}
            {\indexI,\indexJp,\indexIc,\indexJpc}
        \basedualxi{i}
        \wedge
        \basedualxi{\indexIc}\wedge\basexi{\indexJpc}
    .
\label{EQ-For f (I,J), calculation both side-step4,equation no2}
\end{align}
We rearrange (\ref{EQ-For f (I,J), calculation both side-step4,equation no2}) by taking 
\begin{align*}
    \basedualxi{i}
    \wedge
    \basedualxi{\indexIc}\wedge\basexi{\indexJpc}
    =
    \sgn
        {i,\indexIc,\indexJpc}
        {\order{\indexIc\cup\{i\}},\indexJpc}
    \basedualxi{\order{\indexIc\cup\{i\}}}
    \wedge
    \basexi{\indexJpc}
,
\end{align*}
then the simplified expression of $
(\LieagbdPartialbar f)
\wedge
\star(\basexi{\indexI}\wedge\basedualxi{\indexJp})
$ is
\begin{align}
    \displaystyle\sum_{i\in\indexI}
    2^{p+q-n}
    \rho(\basedualv{i^{'}})(f)\,
    \sgn
        {1,\cdots,n,1^{'},1^{'},\cdots,n^{'}}
        {\indexI,\indexJp,\indexIc,\indexJpc}
    \sgn
        {i,\indexIc,\indexJpc}
        {\order{\indexIc\cup\{i\}},\indexJpc}
    \basedualxi{\order{\indexIc\cup\{i\}}}
    \wedge
    \basexi{\indexJpc}
    .
\label{EQ-For f (I,J), calculation both side-step4,equation no3}
\end{align}


Finally, we apply $\star$ to (\ref{EQ-For f (I,J), calculation both side-step4,equation no3}):
\begin{align*}
    \displaystyle\sum_{i\in\indexI}
    2^{p+q-n}
    \rho(\basedualv{i^{'}})(f)\,
    \sgn
        {1,\cdots,n,1^{'},1^{'},\cdots,n^{'}}
        {\indexI,\indexJp,\indexIc,\indexJpc}
    \sgn
        {i,\indexIc,\indexJpc}
        {\order{\indexIc\cup\{i\}},\indexJpc}
    \star
    (
        \basedualxi{\order{\indexIc\cup\{i\}}}
        \wedge
        \basexi{\indexJpc}
    )
    ,
\end{align*}
in which
\begin{align*}
    \star
    (
        \basedualxi{\order{\indexIc\cup\{i\}}}
        \wedge
        \basexi{\indexJpc}
    )
    =&
        2^{(n-p+1)+(n-q)-n}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\order{\indexIc\cup\{i\}},\indexJpc,\indexI\backslash\{i\},\indexJp}
        \basexi{\indexI\backslash\{i\}}
        \wedge
        \basedualxi{\indexJp}
    \\
    =&
        2^{n-p-q+1}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\order{\indexIc\cup\{i\}},\indexJpc,\indexI\backslash\{i\},\indexJp}
        \basexi{\indexI\backslash\{i\}}
        \wedge
        \basedualxi{\indexJp}
    ,
\end{align*}
so the expression of $
\star
\bigg(
    (\LieagbdPartialbar f)
    \wedge
    \star(\basexi{\indexI}\wedge\basedualxi{\indexJp})
\bigg)
$ is
\begin{align}
    \displaystyle\sum_{j\in\indexJ}
    2\,
    \rho(\basedualv{i^{'}})(f)\,
    \begin{pmatrix*}[l]
        \sgn
            {1,\cdots,n,1^{'},1^{'},\cdots,n^{'}}
            {\indexI,\indexJp,\indexIc,\indexJpc}
        \\
        \sgn
            {i,\indexIc,\indexJpc}
            {\order{\indexIc\cup\{i\}},\indexJpc}
        \\
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\order{\indexIc\cup\{i\}},\indexJpc,\indexI\backslash\{i\},\indexJp}
    \end{pmatrix*}
    \basexi{\indexI\backslash\{i\}}
    \wedge
    \basedualxi{\indexJp}
    .
\label{EQ-For f (I,J), calculation both side-step4,close to finish, unsimplified}
\end{align}
We simplify the signs of permutations through
\begin{itemize}
    \item 
$
    \sgn
        {i,\indexIc,\indexJpc}
        {\order{\indexIc\cup\{i\}},\indexJpc}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\order{\indexIc\cup\{i\}},\indexJpc,\indexI\backslash\{i\},\indexJp}
    =
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {i,\indexIc,\indexJpc,\indexI\backslash\{i\},\indexJp}
$,
    \item 
$
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {i,\indexIc,\indexJpc,\indexI\backslash\{i\},\indexJp}
    =
    (-1)^{(n-p+n-q)(p-1+q)}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {i,\indexI\backslash\{i\},\indexJp,\indexIc,\indexJpc}
    \\
    =
    (-1)^{(p+q)(p-1+q)}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {i,\indexI\backslash\{i\},\indexJp,\indexIc,\indexJpc}
    =
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {i,\indexI\backslash\{i\},\indexJp,\indexIc,\indexJpc}
    \\
    =
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\indexI,\indexJp,\indexIc,\indexJpc}
    \sgn
        {\indexI}
        {i,\indexI\backslash\{i\}}
$,
    \item 
$
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\indexI,\indexJp,\indexIc,\indexJpc}
    \sgn
        {1,\cdots,n,1^{'},1^{'},\cdots,n^{'}}
        {\indexI,\indexJp,\indexIc,\indexJpc}
    =
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {1,\cdots,n,1^{'},1^{'},\cdots,n^{'}}
    =
    (-1)^{n^2}
$
\end{itemize}
and obtain
\begin{align*}
    \begin{pmatrix*}[l]
        \sgn
            {1,\cdots,n,1^{'},1^{'},\cdots,n^{'}}
            {\indexI,\indexJp,\indexIc,\indexJpc}
        \\
        \sgn
            {i,\indexIc,\indexJpc}
            {\order{\indexIc\cup\{i\}},\indexJpc}
        \\
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\order{\indexIc\cup\{i\}},\indexJpc,\indexI\backslash\{i\},\indexJp}
    \end{pmatrix*}
    =
    (-1)^{n^2}
    \sgn
        {\indexI}
        {i,\indexI\backslash\{i\}}
    .
\end{align*}


We can now conclude that the expression of $
-\sqrt{-1}(-1)^{n^2}
\star
\bigg(
    (\LieagbdPartialbar f)
    \wedge
    \star(\basexi{\indexI}\wedge\basedualxi{\indexJp})
\bigg)
$ is
\begin{align}
    &
        -\sqrt{-1}(-1)^{n^2}
        \displaystyle\sum_{i\in\indexI}
        2\,
        \rho(\basedualv{i^{'}})(f)\,
        (-1)^{n^2}
        \sgn
            {\indexI}
            {i,\indexI\backslash\{i\}}
        \basexi{\indexI\backslash\{i\}}
        \wedge
        \basedualxi{\indexJp}
\notag
    \\
    =&
        -2\sqrt{-1}
        \displaystyle\sum_{i\in\indexI}
        \sgn
            {\indexI}
            {i,\indexI\backslash\{i\}}
        \rho(\basedualv{i^{'}})(f)\,
        \basexi{\indexI\backslash\{i\}}
        \wedge
        \basedualxi{\indexJp}.
\label{EQ-For f (I,J), calculation both side-step4,result}
\end{align}
%%%%%%%%%%%%%% finish checking the RHS second part %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% start ??? %%%%%%%%%%%%%%
\keyword{Step 5:} Recalling Step 1, the left-hand side $[\LieagbdPartialbar,\iotaW]
(f\,\basexi{\indexI}\wedge\basedualxi{\indexJp})$ is equal to 
\begin{align*}
    f\,[\LieagbdPartialbar,\iotaW]
    (\basexi{\indexI}\wedge\basedualxi{\indexJp})
    +
    (\LieagbdPartialbar f)
    \wedge
    \iotaW(\basexi{\indexI}\wedge\basedualxi{\indexJp})
    -
    (\iotaW\,\LieagbdPartialbar\,f)
    \basexi{\indexI}\wedge\basedualxi{\indexJp}
    .
\end{align*}
The second term in the above expression, $
(\LieagbdPartialbar f)
\wedge
\iotaW(\basexi{\indexI}\wedge\basedualxi{\indexJp})
-
(\iotaW\,\LieagbdPartialbar\,f)
\basexi{\indexI}\wedge\basedualxi{\indexJp}
$, is equal to (\ref{EQ-For f (I,J), calculation both side-step 3, result}). Therefore,
\begin{align*}
    [\LieagbdPartialbar,\iotaW]
    (f\,\basexi{\indexI}\wedge\basedualxi{\indexJp})
    =
        \begin{pmatrix*}[l]
            f\,[\LieagbdPartialbar,\iotaW]
            (\basexi{\indexI}\wedge\basedualxi{\indexJp})
            \\
            +
            \\
            (-2\sqrt{-1})
            \displaystyle\sum_{r\in\indexI}
            \sgn
                {\indexI}
                {r,\indexI\backslash\{r\}}
            \rho(\basedualv{r^{'}})(f)\,
            \basexi{\indexI\backslash\{r\}}
            \wedge
            \basedualxi{\indexJp}
        \end{pmatrix*}
    .
\end{align*}


Recalling Step 2, the right-hand side $
\sqrt{-1}\LieagbdPartial^{*}
(f\basexi{\indexI}\wedge\basedualxi{\indexJp})
$ is equal to
\begin{align*}
    f\,\sqrt{-1}\LieagbdPartial^{*}
    (\basexi{\indexI}\wedge\basedualxi{\indexJp})
    +
    (-\sqrt{-1})(-1)^{n^{2}}
    \star
    \bigg(
        (\LieagbdPartialbar f)
        \wedge
        \star(\basexi{\indexI}\wedge\basedualxi{\indexJp})
    \bigg)
    .
\end{align*}
The second term in the above expression, $(-\sqrt{-1})(-1)^{n^{2}}
\star
\bigg(
    (\LieagbdPartialbar f)
    \wedge
    \star(\basexi{\indexI}\wedge\basedualxi{\indexJp})
\bigg)$, is equal to (\ref{EQ-For f (I,J), calculation both side-step4,result}). Therefore,
\begin{align*}
    \sqrt{-1}\LieagbdPartial^{*}
    (f\basexi{\indexI}\wedge\basedualxi{\indexJp})
    =
    \begin{pmatrix*}[l]
        f\,\sqrt{-1}\LieagbdPartial^{*}
        (\basexi{\indexI}\wedge\basedualxi{\indexJp})
        \\
        +
        \\
        (-2\sqrt{-1})
        \displaystyle\sum_{i\in\indexI}
        \sgn
            {\indexI}
            {i,\indexI\backslash\{i\}}
        \rho(\basedualv{i^{'}})(f)\,
        \basexi{\indexI\backslash\{i\}}
        \wedge
        \basedualxi{\indexJp}
    \end{pmatrix*}
    .
\end{align*}
We complete the proof by observing that the left-hand side and the right-hand side are the same.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% start assemble and compare %%%%%%%%%%%%%%



==> 3/result_for_idct-2-LHS.tex <==
\begin{align*}
    \begin{pmatrix*}[l]
            [\LieagbdPartialbar,\iotaW]
            %%%%补
            (\basexi{\alpha})
            \wedge
            \basexi{\indexI}\wedge\basedualxi{\indexJp}
            -
            \basexi{\alpha}
            \wedge
            [\LieagbdPartialbar,\iotaW]
            (\basexi{\indexI}\wedge\basedualxi{\indexJp})
            \\
            +
            \\
            (-2\sqrt{-1})
            \begin{pmatrix*}[l]
                \displaystyle\sum_{\indexi{k}\in\indexI}
                \begin{matrix*}[l]
                    \sgn
                        {\indexi{k},\alpha}
                        {\order{\indexi{k},\alpha}}
                    \coefD{\indexi{k}}{\order{\indexi{k},\alpha}}
                    \basexi{\indexI}
                    \wedge
                    \basedualxi{\indexJp}
                \end{matrix*}
                \\
                +
                \\
                \displaystyle\sum_{\indexj{l}\in\indexJp}
                \begin{matrix*}[l]
                    \coefB{\indexjp{l}}{\indexjp{l} \alpha}
                    \basexi{\indexI}
                    \wedge
                    \basedualxi{\indexJp}
                \end{matrix*}
                \\
                +
                \\
                \displaystyle\sum_{\indexi{k}\in\indexI}
                \begin{matrix*}[l]
                    \sgn
                        {\indexI}
                        {\indexi{k},\indexI\backslash\{\indexi{k}\}}
                    \sgn
                        {\indexi{k},\alpha}
                        {\order{\indexi{k},\alpha}}
                    \coefD{\alpha}{\order{\indexi{k} \alpha}}
                    \basexi{\alpha}
                    \wedge
                    \basexi{(\indexI\backslash\{\indexi{k}\})}
                    \wedge
                    \basedualxi{\indexJp}
                \end{matrix*}
                \\
                +
                \\
                \displaystyle\sum_{\indexi{k}\in\indexI}
                \displaystyle\sum_{s\in\indexIc\backslash\{\alpha\}}
                \begin{matrix*}[l]
                    \sgn
                        {\indexI}
                        {\indexi{k},\indexI\backslash\{\indexi{k}\}}
                    \sgn
                        {s,\indexI\backslash\{\indexi{k}\}}
                        {\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
                    \sgn
                        {\indexi{k},\alpha}
                        {\order{\indexi{k},\alpha}}
                    \\
                    \coefD{s}{\order{\indexi{k},\alpha}}
                    \basexi{\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
                    \wedge
                    \basedualxi{\indexJp}
                \end{matrix*}
                \\
                +
                \\
                \displaystyle\sum_{\indexj{l}\in\indexJp}
                \displaystyle\sum_{t^{'}\in\indexJpc}
                \begin{matrix*}[l]
                    (-1)
                    \sgn
                        {t^{'},\indexI,\indexJp}
                        {\indexjp{l},\indexI,\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
                    \coefB{t^{'}}{\indexjp{l} \alpha}
                    \basexi{\indexI}
                    \wedge
                    \basedualxi{\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
                \end{matrix*}
            \end{pmatrix*}
        \end{pmatrix*}
\end{align*}

==> 3/result_for_idct-2-RHS.tex <==
\begin{align*}
    \begin{pmatrix*}[l]
        (\sqrt{-1}\LieagbdPartial^{*}\basexi{\alpha})
        \wedge
        \basexi{\indexI}\wedge\basedualxi{\indexJp}
        -
        \basexi{\alpha}
        \wedge
        \sqrt{-1}\LieagbdPartial^{*}
        (\basexi{\indexI}\wedge\basedualxi{\indexJp})
        \\
        +
        \\
        (-2\sqrt{-1})
        \begin{pmatrix*}[l]
            \displaystyle\sum_{k\in\indexI}
            \begin{matrix*}[l]
                \sgn
                    {\order{k,\alpha}}
                    {k,\alpha}
                \coefD{k}{\order{k,\alpha}}
                \basexi{\indexI}
                \wedge
                \basedualxi{\indexJp}
            \end{matrix*}
            \\
            +
            \\
            \displaystyle\sum_{l^{'}\in\indexJp}
            \begin{matrix*}[l]
                \coefB{l^{'}}{l^{'} \alpha}
                \basexi{\indexI}
                \wedge
                \basedualxi{\indexJp}
            \end{matrix*}
            \\
            +
            \\
            \displaystyle\sum_{r\in\indexI}
            \begin{matrix*}[l]
                \sgn
                    {r,\alpha}
                    {\order{\alpha,r}}
                \sgn
                    {r,\indexI\backslash\{r\}}
                    {\indexI}
                \coefD{\alpha}{\order{\alpha,r}}
                \basexi{\alpha}
                \wedge
                \basexi{(\indexI\backslash\{r\})}
                \wedge
                \basedualxi{\indexJp}
            \end{matrix*}
            \\
            +
            \\
            \displaystyle\sum_{\indexic{k}\in\indexIc\backslash\{\alpha\}}
            \displaystyle\sum_{r\in\indexI}
            \begin{matrix*}[l]
                \sgn
                    {r,\indexI\backslash\{r\}}
                    {\indexI}
                \sgn
                    {\order{(\indexI\backslash\{r\})\cup\{\indexic{k}\}}}
                    {\indexic{k},\indexI\backslash\{r\}}
                \sgn
                    {\order{r,\alpha}}
                    {r,\alpha}
                \\
                \coefD{\indexic{k}}{\order{\alpha, r}}
                \basexi{\order{(\indexI\backslash\{r\})\cup\{\indexic{k}\}}}
                \wedge 
                \basedualxi{\indexJp}
            \end{matrix*}
            \\
            +
            \\
            \displaystyle\sum_{\indexjpc{l}\in\indexJpc}
            \displaystyle\sum_{u^{'}\in\indexJp}
            \begin{matrix*}[l]
                (-1)
                \sgn
                    {u^{'},\indexI,\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
                    {\indexjpc{l},\indexI,\indexJp}
                \coefB{\indexjpc{l}}{u^{'} \alpha}
                \basexi{\indexI}
                \wedge
                \basedualxi{\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
            \end{matrix*}
        \end{pmatrix*}
    \end{pmatrix*}
\end{align*}



==> 4/For__alpha,_I,_J_,_calculation_for_LHS,_conclude.tex <==
\begin{lemma}
\label{lemma-the final version of the LHS}
\begin{align}
    &
    [\LieagbdPartialbar,\iotaW]
    (\basexi{\alpha}\wedge\basexi{\indexI}\wedge\basedualxi{\indexJp})
\notag
\\
    =&
    \begin{pmatrix*}[l]
        [\partialbar,\iotaW]
        \wedge
        \basexi{\indexI}\wedge\basedualxi{\indexJp}
        -
        \basexi{\alpha}
        \wedge
        [\partialbar,\iotaW]
        (\basexi{\indexI}\wedge\basedualxi{\indexJp})
        \\
        +
        \\
        (-2\sqrt{-1})
        \begin{pmatrix*}[l]
            \displaystyle\sum_{\indexi{k}\in\indexI}
            \begin{matrix*}[l]
                \sgn
                    {\order{\indexi{k},\alpha}}
                    {\indexi{k},\alpha}
                \coefD{\indexi{k}}{\order{\indexi{k},\alpha}}
                \basexi{\indexI}
                \wedge
                \basedualxi{\indexJp}
            \end{matrix*}
            \\
            +
            \\
            \displaystyle\sum_{\indexj{l}\in\indexJp}
            \begin{matrix*}[l]
                \coefB{\indexjp{l}}{\indexjp{l} \alpha}
                \basexi{\indexI}
                \wedge
                \basedualxi{\indexJp}
            \end{matrix*}
            \\
            +
            \\
            \displaystyle\sum_{\indexi{k}\in\indexI}
            \begin{matrix*}[l]
                \sgn
                    {\indexI}
                    {\indexi{k},\indexI\backslash\{\indexi{k}\}}
                \sgn
                    {\order{\indexi{k},\alpha}}
                    {\indexi{k},\alpha}
                \\
                \coefD{\alpha}{\order{\indexi{k},\alpha}}
                \basexi{\alpha}
                \wedge
                \basexi{(\indexI\backslash\{\indexi{k}\})}
                \wedge
                \basedualxi{\indexJp}
            \end{matrix*}
            \\
            +
            \\
            \displaystyle\sum_{\indexi{k}\in\indexI}
            \displaystyle\sum_{s\in\indexIc\backslash\{\alpha\}}
            \begin{matrix*}[l]
                \sgn
                    {s,\indexI}
                    {\indexi{k},\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
                \sgn
                    {\order{\alpha,\indexi{k}}}
                    {\alpha,\indexi{k}}  
                \\
                \coefD{s}{\order{\indexi{k},\alpha}}
                \basexi{\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
                \wedge
                \basedualxi{\indexJp}
            \end{matrix*}
            \\
            +
            \\
            \displaystyle\sum_{\indexj{l}\in\indexJp}
            \displaystyle\sum_{t^{'}\in\indexJpc}
            \begin{matrix*}[l]
                \sgn
                    {t^{'},\indexI,\indexJp}
                    {\indexjp{l},\indexI,\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
                \\
                (-1)
                \coefB{t^{'}}{\indexjp{l} \alpha}
                \basexi{\indexI}
                \wedge
                \basedualxi{\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
            \end{matrix*}
        \end{pmatrix*}
    \end{pmatrix*}.
\label{EQ-For (alpha, I, J), calculation for LHS-total summary}
\end{align}
\end{lemma}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{proof}
Recall that (\ref{EQ-For (alpha, I, J), calculation for LHS-half summary}) is 
\begin{align*}
    \begin{pmatrix*}[l]
        [\LieagbdPartialbar,\iotaW]
        (\basexi{\alpha})
        \wedge
        \basexi{\indexI}\wedge\basedualxi{\indexJp}
        \\
        -
        \\
        \basexi{\alpha}
        \wedge
        [\LieagbdPartialbar,\iotaW]
        (\basexi{\indexI}\wedge\basedualxi{\indexJp})
        \\
        +
        \\
        (-\sqrt{-1})
        (\LieagbdPartialbar \, \iota_{\basedualxi{\alpha^{'}}}
        +
        \iota_{\basedualxi{\alpha^{'}}}\,\LieagbdPartialbar)
        (\basexi{\indexI}\wedge\basedualxi{\indexJp})
        \\
        +
        \\
        (-\frac{\sqrt{-1}}{2})
        \displaystyle\sum_{h=1}^{n}
        \big(
            (\iota_{\basexi{h}} \, \LieagbdPartialbar \basexi{\alpha})
            \wedge
            \iota_{\basedualxi{h^{'}}}(\basexi{\indexI}\wedge\basedualxi{\indexJp})
            -
            (\iota_{\basedualxi{h^{'}}} \, \LieagbdPartialbar \basexi{\alpha})
            \wedge
            \iota_{\basexi{h}}(\basexi{\indexI}\wedge\basedualxi{\indexJp})
        \big)
    \end{pmatrix*}
    .
\end{align*}
We prove the lemma by substituting the expressions of $
(-\sqrt{-1})
(\LieagbdPartialbar \, \iota_{\basedualxi{\alpha^{'}}}
+
\iota_{\basedualxi{\alpha^{'}}}\,\LieagbdPartialbar)
(\basexi{\indexI}\wedge\basedualxi{\indexJp})
$ and $
(-\frac{\sqrt{-1}}{2})
\displaystyle\sum_{h=1}^{n}
\big(
    (\iota_{\basexi{h}} \, \LieagbdPartialbar \basexi{\alpha})
    \wedge
    \iota_{\basedualxi{h^{'}}}(\basexi{\indexI}\wedge\basedualxi{\indexJp})
    -
    (\iota_{\basedualxi{h^{'}}} \, \LieagbdPartialbar \basexi{\alpha})
    \wedge
    \iota_{\basexi{h}}(\basexi{\indexI}\wedge\basedualxi{\indexJp})
\big)
$ into the above formula.


Recall that Lemma \ref{lemma-For (alpha, I, J), calculation for LHS-extra 1]} states that $(-\sqrt{-1})
(\LieagbdPartialbar \, \iota_{\basedualxi{\alpha^{'}}}
+
\iota_{\basedualxi{\alpha^{'}}}\,\LieagbdPartialbar)
(\basexi{\indexI}\wedge\basedualxi{\indexJp})
$ is equal to
\begin{align}
    &
    (-2\sqrt{-1})
        \displaystyle\sum_{\indexi{k}\in\indexI}
        \begin{pmatrix*}[l]
            (-1)
            \coefB{\indexi{k}}{\indexi{k} \alpha^{'}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\indexJp}
        \end{pmatrix*}
\label{EQ-For (alpha, I, J), calculation for LHS, conclude-ref extra 1,1}
    \\
    +&\notag
    \\
    &
        (-2\sqrt{-1})
        \displaystyle\sum_{\indexi{k}\in\indexI}
        \displaystyle\sum_{s\in\indexIc}
        \begin{pmatrix*}[l]
            \sgn
                {s,\indexI}
                {\indexi{k},\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
            \coefB{\indexi{k}}{s \alpha^{'}}
            \basexi{\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
            \wedge
            \basedualxi{\indexJp}
        \end{pmatrix*}
\label{EQ-For (alpha, I, J), calculation for LHS, conclude-ref extra 1,2}
    \\
    +&\notag
    \\
    &
        (-2\sqrt{-1})
        \displaystyle\sum_{\indexj{l}\in\indexJp\backslash\{\alpha^{'}\}}
        \begin{pmatrix*}[l]
            \sgn
                {\order{\indexjp{l},\alpha^{'}}}
                {\alpha^{'},\indexjp{l}}
            \coefD{\indexjp{l}}{\order{\indexjp{l},\alpha^{'}}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\indexJp}
        \end{pmatrix*}
\label{EQ-For (alpha, I, J), calculation for LHS, conclude-ref extra 1,3}
    \\
    +&\notag
    \\
    &
        (-2\sqrt{-1})
        \displaystyle\sum_{\indexj{l}\in\indexJp}
        \displaystyle\sum_{t^{'}\in\indexJpc}
        \begin{pmatrix*}[l]
            \sgn
                {\order{\alpha^{'},t^{'}}}
                {t^{'},\alpha^{'}}
            \sgn
                {t^{'},\indexI,\indexJp}
                {\indexjp{l},\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
            \\
            \coefD{\indexjp{l}}{\order{\alpha^{'},t^{'}}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
        \end{pmatrix*}
    .
\label{EQ-For (alpha, I, J), calculation for LHS, conclude-ref extra 1,4}
\end{align}
Likewise, recall that Lemma \ref{lemma-For (alpha, I, J), calculation for LHS-extra 2]} states that $
(-\frac{\sqrt{-1}}{2})
\displaystyle\sum_{h=1}^{n}
\big(
    (\iota_{\basexi{h}} \, \LieagbdPartialbar \basexi{\alpha})
    \wedge
    \iota_{\basedualxi{h^{'}}}(\basexi{\indexI}\wedge\basedualxi{\indexJp})
    -
    (\iota_{\basedualxi{h^{'}}} \, \LieagbdPartialbar \basexi{\alpha})
    \wedge
    \iota_{\basexi{h}}(\basexi{\indexI}\wedge\basedualxi{\indexJp})
\big)
$  is equal to
\begin{align}
    &
        (-2\sqrt{-1})
        \displaystyle\sum_{\indexjp{l}\in\indexJp}
        \begin{matrix*}[l]
            \coefB{\alpha}{\indexj{l} \indexjp{l}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\indexJp}
        \end{matrix*}
\label{EQ-For (alpha, I, J), calculation for LHS, conclude-ref extra 2,1}
    \\
    +&\notag
    \\
    &
        (-2\sqrt{-1})
        \displaystyle\sum_{\indexjp{l}\in\indexJp}
        \displaystyle\sum_{t^{'}\in\indexJpc}
        \begin{matrix*}[l]
            (-1)
            \sgn
                {t^{'},\indexI,\indexJp}
                {\indexjp{l},\indexI,\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
            \coefB{\alpha}{\indexj{l} t^{'}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
        \end{matrix*}
\label{EQ-For (alpha, I, J), calculation for LHS, conclude-ref extra 2,2}
    \\
    +&\notag
    \\
    &
        (-2\sqrt{-1})
        \displaystyle\sum_{\indexi{k}\in\indexI}
        \begin{matrix*}[l]
            \coefB{\alpha}{\indexi{k} \indexip{k}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\indexJp}
        \end{matrix*}
\label{EQ-For (alpha, I, J), calculation for LHS, conclude-ref extra 2,3}
    \\
    +&\notag
    \\
    &
        (-2\sqrt{-1})
        \displaystyle\sum_{\indexi{k}\in\indexI}
        \displaystyle\sum_{s\in\indexIc}
        \begin{matrix*}[l]
            (-1)
            \sgn
                {s,\indexI}
                {\indexi{k},\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
            \coefB{\alpha}{s \indexip{k}}
            \basexi{\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
            \wedge
            \basedualxi{\indexJp}
        \end{matrix*}
    .
\label{EQ-For (alpha, I, J), calculation for LHS, conclude-ref extra 2,4}
\end{align}
We combine the similar terms in the above sums:
\begin{itemize}
    \item (\ref{EQ-For (alpha, I, J), calculation for LHS, conclude-ref extra 2,3}) + (\ref{EQ-For (alpha, I, J), calculation for LHS, conclude-ref extra 1,1}) is equal to
    \begin{align}
        (-2\sqrt{-1})
        \displaystyle\sum_{\indexi{k}\in\indexI}
            \bigg(
                \coefB{\alpha}{\indexi{k} \indexip{k}}
                -
                \coefB{\indexi{k}}{\indexi{k} \alpha^{'}}
            \bigg)
            \basexi{\indexI}
            \wedge
            \basedualxi{\indexJp}
        .
    \label{EQ-For (alpha, I, J), calculation for LHS, conclude-classified term 1}
    \end{align}
    Consider the constraint
    \begin{align*}
        \coefB{\alpha}{\indexi{k} \indexip{k}}
        -
        \coefB{\indexi{k}}{\indexi{k} \alpha}
        =
        \sgn
            {\order{\indexi{k}, \alpha}}
            {\indexi{k}, \alpha}
        \coefD{\indexi{k}}{\order{\indexi{k},\alpha}}
        .
    \end{align*}
    Applying it to the terms in (\ref{EQ-For (alpha, I, J), calculation for LHS, conclude-classified term 1}), we obtain the following simplified expression:
    \begin{align}
        (-2\sqrt{-1})
        \displaystyle\sum_{\indexi{k}\in\indexI}
            \sgn
                {\order{\indexi{k}, \alpha}}
                {\indexi{k}, \alpha}
            \coefD{\indexi{k}}{\order{\indexi{k},\alpha}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\indexJp}
        .
    \label{EQ-For (alpha, I, J), calculation for LHS, conclude-simplified term 1}   
    \end{align}
    
    

    \item We can add the case that $\indexjp{l}=\alpha^{'}$ to the summation inside (\ref{EQ-For (alpha, I, J), calculation for LHS, conclude-ref extra 1,3}) since $\coefD{\indexjp{l}}{\alpha^{'},\alpha^{'}}=0$. Then, 
    (\ref{EQ-For (alpha, I, J), calculation for LHS, conclude-ref extra 1,3}) + (\ref{EQ-For (alpha, I, J), calculation for LHS, conclude-ref extra 2,1}) is equal to
    \begin{align}
        (-2\sqrt{-1})
        \displaystyle\sum_{\indexjp{l}\in\indexJp}
        \begin{pmatrix*}[l]
            \sgn
                {\order{\indexjp{l},\alpha^{'}}}
                {\alpha^{'},\indexjp{l}}
            \coefD{\indexjp{l}}{\order{\indexjp{l},\alpha^{'}}}
            +
            \coefB{\alpha}{\indexj{l} \indexjp{l}}
        \end{pmatrix*}
        \basexi{\indexI}
        \wedge
        \basedualxi{\indexJp}
        .
    \label{EQ-For (alpha, I, J), calculation for LHS, conclude-classified term 2}
    \end{align}
    Recall the constraint
    \begin{align*}
        \coefB{\indexj{l}}{\indexj{l} \alpha}
        -
        \coefB{\alpha}{\indexj{l} \indexjp{l}}
        =
        \sgn
            {\order{\alpha,\indexjp{l}}}
            {\alpha,\indexj{l}}
        \coefD{\indexj{l}}{\order{\alpha,\indexjp{l}}}
        .
    \end{align*}
    Applying it to the terms in (\ref{EQ-For (alpha, I, J), calculation for LHS, conclude-classified term 2}), we obtain the following simplified expression:
    \begin{align}
        (-2\sqrt{-1})
        \displaystyle\sum_{\indexjp{l}\in\indexJp}
        \coefB{\indexj{l}}{\indexj{l} \alpha}
        \basexi{\indexI}
        \wedge
        \basedualxi{\indexJp}
        .
    \label{EQ-For (alpha, I, J), calculation for LHS, conclude-simplified term 2}
    \end{align}
    

    \item (\ref{EQ-For (alpha, I, J), calculation for LHS, conclude-ref extra 1,2}) + (\ref{EQ-For (alpha, I, J), calculation for LHS, conclude-ref extra 2,4}) is equal to
    \begin{align}
        (-2\sqrt{-1})
        \displaystyle\sum_{\indexi{k}\in\indexI}
        \displaystyle\sum_{s\in\indexIc}
        \begin{matrix*}[l]
            \sgn
                {s,\indexI}
                {\indexi{k},\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
            \big(
                \coefB{\indexi{k}}{s \alpha^{'}}
                -
                \coefB{\alpha}{s \indexip{k}}
            \big)
            \basexi{\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
            \wedge
            \basedualxi{\indexJp}
        \end{matrix*}
    .
    \label{EQ-For (alpha, I, J), calculation for LHS, conclude-classified term 3}
    \end{align}
    Recall the constraint
    \begin{align*}
        \coefB{\indexi{k}}{s \alpha^{'}}
        -
        \coefB{\alpha}{s \indexi{k}}
        =
        \sgn
            {\order{\alpha,\indexi{k}}}
            {\alpha,\indexi{k}}
        \coefD{s}{\order{\alpha,\indexi{k}}}
        .
    \end{align*}
    Applying it to the terms in (\ref{EQ-For (alpha, I, J), calculation for LHS, conclude-classified term 3}), we obtain the following simplified expression:
    \begin{align}
        (-2\sqrt{-1})
        \displaystyle\sum_{\indexi{k}\in\indexI}
        \displaystyle\sum_{s\in\indexIc}
        \begin{pmatrix*}[l]
            \sgn
                {s,\indexI}
                {\indexi{k},\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
            \sgn
                {\order{\alpha,\indexi{k}}}
                {\alpha,\indexi{k}}
            \\
            \coefD{s}{\order{\alpha,\indexi{k}}}
            \basexi{\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
            \wedge
            \basedualxi{\indexJp}
        \end{pmatrix*}
    .
    \label{EQ-For (alpha, I, J), calculation for LHS, conclude-simplified term 3}
    \end{align}
    To match the right-hand side, which we discuss later, we split the sum in (\ref{EQ-For (alpha, I, J), calculation for LHS, conclude-simplified term 3}) into two parts:
    \begin{align}
        &
        (-2\sqrt{-1})
        \displaystyle\sum_{\indexi{k}\in\indexI}
        \begin{pmatrix*}[l]
            (-1)
            \sgn
                {\indexI}
                {\indexi{k},\indexI\backslash\{\indexi{k}\}}
            \sgn
                {\order{\alpha,\indexi{k}}}
                {\alpha,\indexi{k}}
            \\
            \coefD{\alpha}{\order{\alpha,\indexi{k}}}
            \basexi{\alpha}
            \wedge
            \basexi{\indexI\backslash\{\indexi{k}\}}
            \wedge
            \basedualxi{\indexJp}
        \end{pmatrix*}
    \label{EQ-For (alpha, I, J), calculation for LHS, conclude-simplified term 3.1}
        \\
        +&\notag
        \\
        &
        (-2\sqrt{-1})
        \displaystyle\sum_{\indexi{k}\in\indexI}
        \displaystyle\sum_{s\in\indexIc\backslash\{\alpha\}}
        \begin{pmatrix*}[l]
            \sgn
                {s,\indexI}
                {\indexi{k},\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
            \sgn
                {\order{\alpha,\indexi{k}}}
                {\alpha,\indexi{k}}
            \\
            \coefD{s}{\order{\alpha,\indexi{k}}}
            \basexi{\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
            \wedge
            \basedualxi{\indexJp}
        \end{pmatrix*}
    ,
    \label{EQ-For (alpha, I, J), calculation for LHS, conclude-simplified term 3.2}
    \end{align}
    where (\ref{EQ-For (alpha, I, J), calculation for LHS, conclude-simplified term 3.1}) is obtained from
    \begin{align*}
        (-2\sqrt{-1})
        \displaystyle\sum_{\indexi{k}\in\indexI}
        \displaystyle\sum_{s=\alpha}
        \begin{pmatrix*}[l]
            \sgn
                {s,\indexI}
                {\indexi{k},\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
            \sgn
                {\order{\alpha,\indexi{k}}}
                {\alpha,\indexi{k}}
            \\
            \coefD{s}{\order{\alpha,\indexi{k}}}
            \basexi{\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
            \wedge
            \basedualxi{\indexJp}
        \end{pmatrix*}
    ,
    \end{align*}
    where $
    \order{(\indexI\backslash\{\indexi{k}\})\cup\{\alpha\}}
    =
    \{ \alpha,\indexI\backslash\{\indexi{k}\} \}
    $ since we assumed $\alpha<\indexi{1}$.
    

    \item (\ref{EQ-For (alpha, I, J), calculation for LHS, conclude-ref extra 1,4}) + (\ref{EQ-For (alpha, I, J), calculation for LHS, conclude-ref extra 2,2}) is equal to
    \begin{align}
        (-2\sqrt{-1})
        \displaystyle\sum_{\indexj{l}\in\indexJp}
        \displaystyle\sum_{t^{'}\in\indexJpc}
        \begin{pmatrix*}[l]
            \sgn
                {t^{'},\indexI,\indexJp}
                {\indexjp{l},\indexI,\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
            \\
            \bigg(
                \sgn
                    {\order{\alpha^{'},t^{'}}}
                    {t^{'},\alpha^{'}}
                \coefD{\indexjp{l}}{\order{\alpha^{'},t^{'}}}
                -
                \coefB{\alpha}{\indexj{l} t^{'}}
            \bigg)
            \\
            \basexi{\indexI}
            \wedge
            \basedualxi{\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
        \end{pmatrix*}
        .
    \label{EQ-For (alpha, I, J), calculation for LHS, conclude-classified term 4}
    \end{align}
    Recall the constraint
    \begin{align*}
        \coefB{\alpha}{\indexjp{l} t^{'}}
        -
        \coefB{t^{'}}{ \indexjp{l} \alpha }
        =
        \sgn
            {\order{t^{'},\alpha^{'}}}
            {t^{'},\alpha^{'}}
        \coefD{\indexjp{l}}{\order{t^{'},\alpha^{'}}}
        .
    \end{align*}
    Applying it to the terms in (\ref{EQ-For (alpha, I, J), calculation for LHS, conclude-classified term 4}), we obtain the following simplified expression:
    \begin{align}
        (-2\sqrt{-1})
        \displaystyle\sum_{\indexj{l}\in\indexJp}
        \displaystyle\sum_{t^{'}\in\indexJpc}
        \begin{pmatrix*}[l]
            \sgn
                {t^{'},\indexI,\indexJp}
                {\indexjp{l},\indexI,\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
            \\
            (-1)
            \coefB{t^{'}}{\indexjp{l} \alpha}
            \basexi{\indexI}
            \wedge
            \basedualxi{\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
        \end{pmatrix*}
        .
    \label{EQ-For (alpha, I, J), calculation for LHS, conclude-simplified term 4}
    \end{align}
\end{itemize}


We can now summarize the expression of $
[\LieagbdPartialbar,\iotaW]
(\basexi{\alpha}\wedge\basexi{\indexI}\wedge\basedualxi{\indexJp})
$ by summing up 
\begin{align*}
    \begin{pmatrix*}[l]
        [\LieagbdPartialbar,\iotaW]
        (\basexi{\alpha})
        \wedge
        \basexi{\indexI}\wedge\basedualxi{\indexJp}
        -
        \basexi{\alpha}
        \wedge
        [\LieagbdPartialbar,\iotaW]
        (\basexi{\indexI}\wedge\basedualxi{\indexJp})
    \end{pmatrix*}
\end{align*}
 with (\ref{EQ-For (alpha, I, J), calculation for LHS, conclude-simplified term 1}), (\ref{EQ-For (alpha, I, J), calculation for LHS, conclude-simplified term 2}), (\ref{EQ-For (alpha, I, J), calculation for LHS, conclude-simplified term 3.1}), (\ref{EQ-For (alpha, I, J), calculation for LHS, conclude-simplified term 3.2}), and (\ref{EQ-For (alpha, I, J), calculation for LHS, conclude-simplified term 4}):

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% state final result %%%%%%%%%%%%%%%%%%
\begin{align*}
    \begin{pmatrix*}[l]
            [\partialbar,\iotaW]
            \wedge
            \basexi{\indexI}\wedge\basedualxi{\indexJp}
            -
            \basexi{\alpha}
            \wedge
            [\partialbar,\iotaW]
            (\basexi{\indexI}\wedge\basedualxi{\indexJp})
            \\
            +
            \\
            (-2\sqrt{-1})
            \begin{pmatrix*}[l]
                \displaystyle\sum_{\indexi{k}\in\indexI}
                \begin{matrix*}[l]
                    \sgn
                        {\order{\indexi{k},\alpha}}
                        {\indexi{k},\alpha}
                    \coefD{\indexi{k}}{\order{\indexi{k},\alpha}}
                    \basexi{\indexI}
                    \wedge
                    \basedualxi{\indexJp}
                \end{matrix*}
                \\
                +
                \\
                \displaystyle\sum_{\indexj{l}\in\indexJp}
                \begin{matrix*}[l]
                    \coefB{\indexjp{l}}{\indexjp{l} \alpha}
                    \basexi{\indexI}
                    \wedge
                    \basedualxi{\indexJp}
                \end{matrix*}
                \\
                +
                \\
                \displaystyle\sum_{\indexi{k}\in\indexI}
                \begin{matrix*}[l]
                    \sgn
                        {\indexI}
                        {\indexi{k},\indexI\backslash\{\indexi{k}\}}
                    \sgn
                        {\order{\indexi{k},\alpha}}
                        {\indexi{k},\alpha}
                    \\
                    \coefD{\alpha}{\order{\indexi{k},\alpha}}
                    \basexi{\alpha}
                    \wedge
                    \basexi{(\indexI\backslash\{\indexi{k}\})}
                    \wedge
                    \basedualxi{\indexJp}
                \end{matrix*}
                \\
                +
                \\
                \displaystyle\sum_{\indexi{k}\in\indexI}
                \displaystyle\sum_{s\in\indexIc\backslash\{\alpha\}}
                \begin{matrix*}[l]
                    \sgn
                        {s,\indexI}
                        {\indexi{k},\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
                    \sgn
                        {\order{\alpha,\indexi{k}}}
                        {\alpha,\indexi{k}}  
                    \\
                    \coefD{s}{\order{\indexi{k},\alpha}}
                    \basexi{\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
                    \wedge
                    \basedualxi{\indexJp}
                \end{matrix*}
                \\
                +
                \\
                \displaystyle\sum_{\indexj{l}\in\indexJp}
                \displaystyle\sum_{t^{'}\in\indexJpc}
                \begin{matrix*}[l]
                    \sgn
                        {t^{'},\indexI,\indexJp}
                        {\indexjp{l},\indexI,\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
                    \\
                    (-1)
                    \coefB{t^{'}}{\indexjp{l} \alpha}
                    \basexi{\indexI}
                    \wedge
                    \basedualxi{\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
                \end{matrix*}
            \end{pmatrix*}
        \end{pmatrix*},
\end{align*}
which is the right-hand side in the statement of Lemma \ref{lemma-the final version of the LHS}.
\end{proof}











==> 4/For__alpha,_I,_J_,_calculation_for_LHS,_extra_1.tex <==
\newpage
\begin{lemma}
\label{lemma-For (alpha, I, J), calculation for LHS-extra 1]}
\begin{align*}
    (-\sqrt{-1})(\LieagbdPartialbar\,\contract{\basedualxi{\alpha^{'}}}
    +
    \contract{\basedualxi{\alpha^{'}}}\,\LieagbdPartialbar)
    (\basexi{\indexI}\wedge\basedualxi{\indexJp})
\end{align*}
is equal to
\begin{align}
    -2\sqrt{-1}
    \begin{pmatrix*}[l]
        \displaystyle\sum_{\indexi{k}\in\indexI}
        \begin{pmatrix*}[l]
            (-1)
            \coefB{\indexi{k}}{\indexi{k} \alpha^{'}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\indexJp}
        \end{pmatrix*}
    \\
    +
    \\
        \displaystyle\sum_{\indexi{k}\in\indexI}
        \displaystyle\sum_{s\in\indexIc}
        \begin{pmatrix*}[l]
            \sgn
                {s,\indexI,\indexJp}
                {\indexi{k},\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}},\indexJp}
            \coefB{\indexi{k}}{s \alpha^{'}}
            \basexi{\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
            \wedge
            \basedualxi{\indexJp}
        \end{pmatrix*}
    \\
    +
    \\
        \displaystyle\sum_{\indexj{l}\in\indexJp\backslash\{\alpha^{'}\}}
        \begin{pmatrix*}[l]
            \sgn
                {\order{\indexjp{l},\alpha^{'}}}
                {\alpha^{'},\indexjp{l}}
            \coefD{\indexjp{l}}{\order{\indexjp{l} \alpha^{'}}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\indexJp}
        \end{pmatrix*}
    \\
    +
    \\
        \displaystyle\sum_{\indexj{l}\in\indexJp}
        \displaystyle\sum_{t^{'}\in\indexJpc}
        \begin{pmatrix*}[l]
            \sgn
                {\order{\alpha^{'},t^{'}}}
                {t^{'},\alpha^{'}}
            \sgn
                {t^{'},\indexI,\indexJp}
                {\indexjp{l},\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
            \\
            \coefD{\indexjp{l}}{\order{\alpha^{'} t^{'}}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
        \end{pmatrix*}
    \end{pmatrix*}
    .
\label{EQ-For (alpha, I, J), calculation for LHS, extra 1-result}
\end{align}
\end{lemma}

\begin{proof}



%%%%%%%%%%%% finish calculate \LieagbdPartialbar (I,J) %%%%%%%%%%%%
The proof comprises the following steps.
\begin{enumerate}
    \item Calculate $
    \contract{\basedualxi{\alpha^{'}}}\,\LieagbdPartialbar
    (\basexi{\indexI}\wedge\basedualxi{\indexJp})
    $.

    \item Calculate $
    \LieagbdPartialbar\,\contract{\basedualxi{\alpha^{'}}}
    (\basexi{\indexI}\wedge\basedualxi{\indexJp})
    $.

    \item Combine the results from Steps 1–2.
\end{enumerate}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% start Step 1 %%%%%%%%%%%%
\keyword{Step 1:} The expression of $\LieagbdPartialbar(\basexi{\indexI} \wedge \basedualxi{\indexJp})$ is 
\begin{align}
    \begin{pmatrix*}[l]
        %?--1-1
        \displaystyle\sum_{\indexi{k}\in\indexI}
        \sgn
            {\indexI}
            {\indexi{k},\indexI\backslash\{\indexi{k}\}}
        \basexi{\indexi{1}}
        \wedge\cdots\wedge
        \LieagbdPartialbar \basexi{\indexi{k}}
        \wedge\cdots\wedge
        \basexi{\indexi{p}}
        \wedge
        \basedualxi{\indexJp}
        \\
        +
        \\
        %?--1-2
        \displaystyle\sum_{\indexjp{k}\in\indexJp}
        \sgn
            {\indexI,\indexJp}
            {\indexjp{k},\indexI,\indexJp\backslash\{\indexjp{k}\}}
        \basexi{\indexIp}
        \wedge
        \basedualxi{\indexjp{1}}
        \wedge\cdots\wedge
        \LieagbdPartialbar \basedualxi{\indexjp{k}}
        \wedge\cdots\wedge
        \basedualxi{\indexjp{q}}
    \end{pmatrix*}
    .
\label{EQ-For (alpha, I, J), calculation for LHS, extra 1-no1}
\end{align}
Recalling that $
    \LieagbdPartialbar \xi_i
    =
        \sum_{j,k}^n
        \coefB{i}{jk}
        \basexi{j} \wedge \basedualxi{k}
$
and
\begin{align*}
    \LieagbdPartialbar \basedualxi{i}
    =
        \sum_{j,k=1}^n
        \frac{1}{2}
        \coefD{i}{jk}
        \basedualxi{j} \wedge \basedualxi{k}
    =
        \sum_{j,k=1}^n
        \frac{1}{2}
        \sgn
            {\order{j,k}}
            {j,k}
        \coefD{i}{\order{j,k}}
        \basedualxi{j}\wedge\basedualxi{k}
    ,
\end{align*}
we plug these into (\ref{EQ-For (alpha, I, J), calculation for LHS, extra 1-no1}) and cancel out the terms containing repeated frame bases, then obtain
\begin{align}
    \begin{pmatrix*}[l]
        %1
        \displaystyle\sum_{\indexi{k}\in\indexI}
        \sgn
            {\indexI}
            {\indexi{k},\indexI\backslash\{\indexi{k}\}}
        \basexi{\indexi{1}}
        \wedge\cdots\wedge
        \basexi{\indexi{k-1}}
        \wedge
        \begin{pmatrix*}[l]
            %?--2-1-1
            \displaystyle\sum_{t^{'}\in\indexJpc}
            \coefB{\indexi{k}}{\indexi{k} t^{'}}
            \basexi{\indexi{k}}\wedge\basedualxi{t^{'}}
            \\
            +
            \\
            %?--2-1-2
            \displaystyle\sum_{s\in\indexIc}
            \displaystyle\sum_{t^{'}\in\indexJpc}
            \coefB{\indexi{k}}{s t^{'}}
            \basexi{s}\wedge\basedualxi{t^{'}}
        \end{pmatrix*}
        \wedge
        \basexi{\indexi{k+1}}
        \wedge\cdots\wedge
        \basexi{\indexi{p}}
        \wedge
        \basedualxi{\indexJp}
        \\
        +
        \\
        %2
        \displaystyle\sum_{\indexjp{l}\in\indexJp}
        \begin{pmatrix*}[l]
            \sgn
                {\indexI,\indexJp}
                {\indexjp{l},\indexI,\indexJp\backslash\{\indexjp{l}\}}
            \basexi{\indexI}
            \wedge
            \basexi{\indexjp{1}}
            \wedge\cdots\wedge
            \basedualxi{\indexjp{l-1}}
            \wedge
            \begin{pmatrix*}[l]
                %?--2-2-1
                \displaystyle\sum_{t^{'}\in\indexJpc}
                \frac{1}{2}
                (
                \coefD{\indexjp{l}}{\indexjp{l} t^{'}}
                \basedualxi{\indexjp{l}}\wedge\basedualxi{t^{'}}
                +
                \coefD{\indexjp{l}}{t^{'} \indexjp{l}}
                \basedualxi{t^{'}}\wedge\basedualxi{\indexjp{l}}
                )
                \\
                +
                \\
                %?--2-2-2
                \displaystyle\sum_{t^{'}\in\indexJpc}
                \displaystyle\sum_{u^{'}\in\indexJpc}
                \frac{1}{2}
                \coefD{\indexjp{l}}{u^{'} t^{'}}
                \basedualxi{u^{'}}\wedge\basedualxi{t^{'}}
            \end{pmatrix*}
            \\
            \wedge
            \basedualxi{\indexjp{l+1}}
            \wedge\cdots\wedge
            \basedualxi{\indexjp{q}}
        \end{pmatrix*}
    \end{pmatrix*}
    .
\label{EQ-For (alpha, I, J), calculation for LHS, extra 1-no2}
\end{align}
We reorder the above wedge product of frames as follows:
\begin{itemize}
    \item 
$   
        \qquad
        \basexi{\indexi{1}}
        \wedge\cdots\wedge
        \basexi{\indexi{k-1}}\wedge
        \bigg(
            \displaystyle\sum_{t^{'}\in\indexJpc}
            \coefB{\indexi{k}}{\indexi{k} t^{'}}
            \basexi{\indexi{k}}\wedge\basedualxi{t^{'}}
        \bigg)
        \wedge\basexi{\indexi{k+1}}
        \wedge\cdots\wedge
        \basexi{\indexi{p}}
        \wedge
        \basedualxi{\indexJp}
$
\\
$
        =
            \displaystyle\sum_{t^{'}\in\indexJpc}
            \sgn
                {\indexi{1},\cdots,\indexi{k},t^{'},\indexi{k+1},\cdots,\indexi{p},\indexJp}
                {\indexI,\order{\indexJp\cup\{t^{'}\}}}
            \coefB{\indexi{k}}{\indexi{k} t^{'}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\order{\indexJp\cup\{t^{'}\}}}
    % \end{matrix*}
$,
    \item 
$
        \qquad
        \basexi{\indexi{1}}
        \wedge\cdots\wedge
        \basexi{\indexi{k-1}}\wedge
        \bigg(
            \displaystyle\sum_{s\in\indexIc}
            \displaystyle\sum_{t^{'}\in\indexJpc}
            \coefB{\indexi{k}}{s t^{'}}
            \basexi{s}\wedge\basedualxi{t^{'}}
        \bigg)
        \wedge\basexi{\indexi{k+1}}
        \wedge\cdots\wedge
        \basexi{\indexi{p}}
        \wedge
        \basedualxi{\indexJp}
$
\\
$
        =
        \displaystyle\sum_{s\in\indexIc}
        \displaystyle\sum_{t^{'}\in\indexJpc}
        \sgn
            {\indexi{1},\cdots,\indexi{k},t^{'},\indexi{k+1},\cdots,\indexi{p},\indexJp}
            {\indexI,\order{\indexJp\cup\{t^{'}\}}}
        \coefB{\indexi{k}}{\indexi{k} t^{'}}
        \basexi{\indexI}
        \wedge
        \basedualxi{\order{\indexJp\cup\{t^{'}\}}}
$,
    \item
$
        \qquad
        \basexi{\indexI}
        \wedge
        \basexi{\indexjp{1}}
        \wedge\cdots\wedge
        \basedualxi{\indexjp{l-1}}
        \wedge
        \bigg(
            \displaystyle\sum_{t^{'}\in\indexJpc}
            \frac{1}{2}
            (
            \coefD{\indexjp{l}}{\indexjp{l} t^{'}}
            \basedualxi{\indexjp{l}}\wedge\basedualxi{t^{'}}
            +
            \coefD{\indexjp{l}}{t^{'} \indexjp{l}}
            \basedualxi{t^{'}}\wedge\basedualxi{\indexjp{l}}
            )
        \bigg)
        \wedge
        \basedualxi{\indexjp{l+1}}
        \wedge\cdots\wedge
        \basedualxi{\indexjp{q}}
$
\\
$
        =
        \basexi{\indexI}
        \wedge
        \basexi{\indexjp{1}}
        \wedge\cdots\wedge
        \basedualxi{\indexjp{l-1}}
        \wedge
        \bigg(
            \displaystyle\sum_{t^{'}\in\indexJpc}
            \coefD{\indexjp{l}}{\order{\indexjp{l} t^{'}}}
            \basedualxi{\order{ \indexjp{l} t^{'}}}
        \bigg)
        \wedge
        \basedualxi{\indexjp{l+1}}
        \wedge\cdots\wedge
        \basedualxi{\indexjp{q}}  
$
\\
$
        =
        \sgn
                {\indexjp{1},\cdots,\indexjp{l-1},\order{\indexjp{l},t^{'}},\indexjp{l+1},\cdots,\indexjp{q}}
                {\order{\indexJp\cup\{t^{'}\}}}
            \coefD{\indexjp{l}}{\order{\indexjp{l},t^{'}}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\order{\indexJp\cup\{t^{'}\}}}
$,
    \item
$
        \qquad
        \basexi{\indexI}
        \wedge
        \basexi{\indexjp{1}}
        \wedge\cdots\wedge
        \basedualxi{\indexjp{l-1}}
        \wedge
        \bigg(
            \displaystyle\sum_{t^{'}\in\indexJpc}
            \displaystyle\sum_{u^{'}\in\indexJpc}
            \frac{1}{2}
            \coefD{\indexjp{l}}{u^{'} t^{'}}
            \basedualxi{u^{'}}\wedge\basedualxi{t^{'}}
        \bigg)
        \wedge
        \basedualxi{\indexjp{l+1}}
        \wedge\cdots\wedge
        \basedualxi{\indexjp{q}}
$
\\
$
        =
        \basexi{\indexI}
        \wedge
        \basexi{\indexjp{1}}
        \wedge\cdots\wedge
        \basedualxi{\indexjp{l-1}}
        \wedge
        \bigg(
            \displaystyle\sum_{t^{'}\in\indexJpc}
            \displaystyle\sum_{u^{'}\in\indexJpc}
            \frac{1}{2}
            \coefD{\indexjp{l}}{\order{u^{'} t^{'}}}
            \basedualxi{\order{u^{'} t^{'}}}
        \bigg)
        \wedge
        \basedualxi{\indexjp{l+1}}
        \wedge\cdots\wedge
        \basedualxi{\indexjp{q}}
$
\\
$
        =
        \sgn
            {\indexjp{1},\cdots,\indexjp{l-1},\order{t^{'},u^{'}},\indexjp{l+1},\cdots,\indexjp{q}}
            {\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'},u^{'}\}}}
        \frac{1}{2}
        \coefD{\indexjp{l}}{\order{t^{'},u^{'}}}
        \basexi{\indexI}
        \wedge
        \basedualxi{\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'},u^{'}\}}}
$.
\end{itemize}
We then simplify (\ref{EQ-For (alpha, I, J), calculation for LHS, extra 1-no2}) to
\begin{align}
    \begin{pmatrix*}[l]
        %?--3-1
        \displaystyle\sum_{\indexi{k}\in\indexI}
        \displaystyle\sum_{t^{'}\in\indexJpc}
        \sgn
            {\indexI}
            {\indexi{k},\indexI\backslash\{\indexi{k}\}}
        \sgn
            {\indexi{1},\cdots,\indexi{k},t^{'},\indexi{k+1},\cdots,\indexi{p},\indexJp}
            {\indexI,\order{\indexJp\cup\{t^{'}\}}}
        \coefB{\indexi{k}}{\indexi{k} t^{'}}
        \basexi{\indexI}
        \wedge
        \basedualxi{\order{\indexJp\cup\{t^{'}\}}}
        \\
        +
        \\
        %?--3-2
        \displaystyle\sum_{\indexi{k}\in\indexI}
        \displaystyle\sum_{s\in\indexIc}
        \displaystyle\sum_{t^{'}\in\indexJpc}
        \begin{pmatrix*}[l]
            \sgn
                {\indexI}
                {\indexi{k},\indexI\backslash\{\indexi{k}\}}
            \sgn
                {\indexi{1},\cdots,\indexi{k-1},s,t^{'},\indexi{k+1},\cdots,\indexi{p},\indexJp}
                {\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}},\order{\indexJp\cup\{t^{'}\}}}
            \\
            \coefB{\indexi{k}}{s t^{'}}
            \basexi{\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
            \wedge
            \basedualxi{\order{\indexJp\cup\{t^{'}\}}}
        \end{pmatrix*}
        \\
        +
        \\
        %?--3-3
        \displaystyle\sum_{\indexjp{l}\in\indexJp}
        \displaystyle\sum_{t^{'}\in\indexJpc}
        \sgn
            {\indexI,\indexJp}
            {\indexjp{l},\indexI,\indexJp\backslash\{\indexjp{l}\}}
        \sgn
            {\indexjp{1},\cdots,\indexjp{l-1},\order{\indexjp{l},t^{'}},\indexjp{l+1},\cdots,\indexjp{q}}
            {\order{\indexJp\cup\{t^{'}\}}}
        \coefD{\indexjp{l}}{\order{\indexjp{l},t^{'}}}
        \basexi{\indexI}
        \wedge
        \basedualxi{\order{\indexJp\cup\{t^{'}\}}}
        \\
        +
        \\
        %?--3-4
        \displaystyle\sum_{\indexjp{l}\in\indexJp}
        \displaystyle\sum_{t^{'}\in\indexJpc}
        \displaystyle\sum_{u^{'}\in\indexJpc}
        \begin{pmatrix*}[l]
            \sgn
                {\indexI,\indexJp}
                {\indexjp{l},\indexI,\indexJp\backslash\{\indexjp{l}\}}
            \sgn
                {\indexjp{1},\cdots,\indexjp{l-1},\order{t^{'},u^{'}},\indexjp{l+1},\cdots,\indexjp{q}}
                {\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'},u^{'}\}}}
            \\
            \frac{1}{2}
            \coefD{\indexjp{l}}{\order{t^{'},u^{'}}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'},u^{'}\}}}
        \end{pmatrix*}
    \end{pmatrix*}
    ,
\label{EQ-For (alpha, I, J), calculation for LHS, extra 1-no3}
\end{align}
which is the expression of $\LieagbdPartialbar(\basexi{\indexI}\wedge\basedualxi{\indexJp})$.
%%%%%%%%%%%% finish calculate \LieagbdPartialbar (I,J) %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%% start calculate \iota alpha \,\LieagbdPartialbar (I,J) %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Next, we apply $\contract{\basedualxi{\alpha^{'}}}$ to (\ref{EQ-For (alpha, I, J), calculation for LHS, extra 1-no3}). Two cases, $\alpha\in\indexJ$ and $\alpha\in\indexJc$, must be considered. We observe that if $\alpha\in\indexJ$, then

%%%%%%%%%%%% start alpha not in J %%%%%%%%%%%%
\begin{itemize}
    \item 
$
    \contract{\basedualxi{\alpha^{'}}}
    \big(
    \basexi{\indexI}
    \wedge
    \basedualxi{\order{\indexJp\cup\{t^{'}\}}}
    \big)
    =
    \sgn
        {\indexI,\order{\indexJp\cup\{t^{'}\}}}
        {\alpha,\indexI,\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
    \basexi{\indexI}
    \wedge
    \basedualxi{\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
$,\\
    \item 
$
    \qquad
    \contract{\basedualxi{\alpha^{'}}}
    \big(
    \basexi{\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
    \wedge
    \basedualxi{\order{\indexJp\cup\{t^{'}\}}}
    \big)
$
\\
$
    =
    \sgn
        {\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}},\order{\indexJp\cup\{t^{'}\}}}
        {\alpha^{'},\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}},\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
    \basexi{\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
    \wedge
    \basedualxi{\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
$,\\
    \item 
$
    \contract{\basedualxi{\alpha^{'}}}
    \big(
    \basexi{\indexI}
    \wedge
    \basedualxi{\order{\indexJp\cup\{t^{'}\}}}
    \big)
    =
    \sgn
        {\indexI,\order{\indexJp\cup\{t^{'}\}}}
        {\alpha^{'},\indexI,\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
    \basexi{\indexI}
    \wedge
    \basedualxi{\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
$,\\
    \item 
$
    \qquad
    \contract{\basedualxi{\alpha^{'}}}
    \big(
    \basexi{\indexI}
    \wedge
    \basedualxi{\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'},u^{'}\}}}
    \big)
$
\\
$
    =
    \begin{cases}
        0       
        &
        \text{if }\alpha=\indexj{l}
        \\
        \sgn
            {\indexI,\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'},u^{'}\}}}
            {\alpha^{'},\indexI,\order{(\indexJp\backslash\{\indexjp{l},\alpha^{'}\})\cup\{t^{'},u^{'}\}}}
        \basexi{\indexI}
        \wedge
        \basedualxi{\order{(\indexJp\backslash\{\indexjp{l},\alpha^{'}\})\cup\{t^{'},u^{'}\}}}
        &
        \text{if }\alpha\neq\indexj{l}
    \end{cases}
$.
\end{itemize}
The above computation leads to
\begin{align}
    &
        \iota_{\basedualxi{\alpha}}\,\LieagbdPartialbar
        (\basexi{\indexI} \wedge \basedualxi{\indexJp})
    \notag\\
    =&
        2
        \begin{pmatrix*}[l]
            %?--1
            \displaystyle\sum_{\indexi{k}\in\indexI}
            \displaystyle\sum_{t^{'}\in\indexJpc}
            \begin{pmatrix*}[l]
                \sgn
                    {\indexI}
                    {\indexi{k},\indexI\backslash\{\indexi{k}\}}
                \sgn
                    {\indexi{1},\cdots,\indexi{k},t^{'},\indexi{k+1},\cdots,\indexi{p},\indexJp}
                    {\indexI,\order{\indexJp\cup\{t^{'}\}}}
                \sgn
                    {\indexI,\order{\indexJp\cup\{t^{'}\}}}
                    {\alpha,\indexI,\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
                \\
                \coefB{\indexi{k}}{\indexi{k} t^{'}}
                \basexi{\indexI}
                \wedge
                \basedualxi{\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
            \end{pmatrix*}
            \\
            +
            \\
            %?--2
            \displaystyle\sum_{\indexi{k}\in\indexI}
            \displaystyle\sum_{s\in\indexIc}
            \displaystyle\sum_{t^{'}\in\indexJpc}
            \begin{pmatrix*}[l]
                \sgn
                    {\indexI}
                    {\indexi{k},\indexI\backslash\{\indexi{k}\}}
                \sgn
                    {\indexi{1},\cdots,\indexi{k-1},s,t^{'},\indexi{k+1},\cdots,\indexi{p},\indexJp}
                    {\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}},\order{\indexJp\cup\{t^{'}\}}}
                \\
                \sgn
                    {\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}},\order{\indexJp\cup\{t^{'}\}}}
                    {\alpha^{'},\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}},\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
                \\
                \coefB{\indexi{k}}{s t^{'}}
                \basexi{\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
                \wedge
                \basedualxi{\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
            \end{pmatrix*}
            \\
            +
            \\
            %?--3
            \displaystyle\sum_{\indexjp{l}\in\indexJp}
            \displaystyle\sum_{t^{'}\in\indexJpc}
            \begin{pmatrix*}[l]
                \sgn
                    {\indexI,\indexJp}
                    {\indexjp{l},\indexI,\indexJp\backslash\{\indexjp{l}\}}
                \sgn
                    {\indexjp{1},\cdots,\indexjp{l-1},\order{\indexjp{l},t^{'}},\indexjp{l+1},\cdots,\indexjp{q}}
                    {\order{\indexJp\cup\{t^{'}\}}}
                \\
                \sgn
                    {\indexI,\order{\indexJp\cup\{t^{'}\}}}
                    {\alpha^{'},\indexI,\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
                \\
                \coefD{\indexjp{l}}{\order{\indexjp{l},t^{'}}}
                \basexi{\indexI}
                \wedge
                \basedualxi{\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
            \end{pmatrix*}
            \\
            +
            \\
            %?--4
            \displaystyle\sum_{\indexjp{l}\in\indexJp\backslash\{\alpha^{'}\}}
            \displaystyle\sum_{t^{'}\in\indexJpc}
            \displaystyle\sum_{u^{'}\in\indexJpc}
            \begin{pmatrix*}[l]
                \sgn
                    {\indexI,\indexJp}
                    {\indexjp{l},\indexI,\indexJp\backslash\{\indexjp{l}\}}
                \sgn
                    {\indexjp{1},\cdots,\indexjp{l-1},\order{t^{'},u^{'}},\indexjp{l+1},\cdots,\indexjp{q}}
                    {\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'},u^{'}\}}}
                \\
                \sgn
                    {\indexI,\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'},u^{'}\}}}
                    {\alpha^{'},\indexI,\order{(\indexJp\backslash\{\indexjp{l},\alpha^{'}\})\cup\{t^{'},u^{'}\}}}
                \\
                \frac{1}{2}
                \coefD{\indexjp{l}}{\order{t^{'},u^{'}}}
                \basexi{\indexI}
                \wedge
                \basedualxi{\order{(\indexJp\backslash\{\indexjp{l},\alpha^{'}\})\cup\{t^{'},u^{'}\}}}
            \end{pmatrix*}
        \end{pmatrix*}
\label{EQ-For (alpha, I, J), calculation for LHS, extra 1-unsimplified the first half, alpha in J}
\end{align}
for the case that $\alpha\in\indexJ$. 


The reader can find Lemmas \ref{lemma-simplification for LHS, extra 1, part 1-lemma 1}–\ref{lemma-simplification for LHS, extra 1, part 1-lemma 4} in Section \ref{apex-simplification for LHS, extra 1, part 1} for the calculation of the simplification of the signs of permutations. Thus, we conclude that when $\alpha\in\indexJ$ the expression of $
\iota_{\basedualxi{\alpha}}\,\LieagbdPartialbar
(\basexi{\indexI} \wedge \basedualxi{\indexJp})
$ is
\begin{align}
    2
    \begin{pmatrix*}[l]
        %?--1
        \displaystyle\sum_{\indexi{k}\in\indexI}
        \displaystyle\sum_{t^{'}\in\indexJpc}
        \begin{pmatrix*}[l]
            (-1)^{k}
            \sgn
                {\indexI}
                {\indexi{k},\indexI\backslash\{\indexi{k}\}}
            \sgn
                {t^{'},\indexI,\indexJp}
                {\alpha,\indexI,\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
            \\
            \coefB{\indexi{k}}{\indexi{k} t^{'}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
        \end{pmatrix*}
        \\
        +
        \\
        %?--2
        \displaystyle\sum_{\indexi{k}\in\indexI}
        \displaystyle\sum_{s\in\indexIc}
        \displaystyle\sum_{t^{'}\in\indexJpc}
        \begin{pmatrix*}[l]
            \sgn
                {s,t^{'},\indexI,\indexJp}
                {\indexi{k},\alpha^{'},\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}},\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
            \\
            \coefB{\indexi{k}}{s t^{'}}
            \basexi{\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
            \wedge
            \basedualxi{\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
        \end{pmatrix*}
        \\
        +
        \\
        %?--3
        \displaystyle\sum_{\indexjp{l}\in\indexJp}
        \displaystyle\sum_{t^{'}\in\indexJpc}
        \begin{pmatrix*}[l]
            \sgn
                {\order{\indexjp{l},t^{'}}}
                {t^{'},\indexjp{l}}
            \sgn
                {t^{'},\indexI,\indexJp}
                {\alpha^{'},\indexI,\order{(\indexJp\backslash\{\alpha^{'}\})\cup\    {t^{'}\}}}}
            \\
            \coefD{\indexjp{l}}{\order{\indexjp{l},t^{'}}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
        \end{pmatrix*}
        \\
        +
        \\
        %?--4
        \displaystyle\sum_{\indexjp{l}\in\indexJp\backslash\{\alpha^{'}\}}
        \displaystyle\sum_{t^{'}\in\indexJpc}
        \displaystyle\sum_{u^{'}\in\indexJpc}
        \begin{pmatrix*}[l]
            \sgn
                {\order{t^{'},u^{'}},\indexI,\indexJp}
                {\indexjp{l},\alpha^{'},\indexI,\order{(\indexJp\backslash\{\indexjp{l},\alpha^{'}\})\cup\{t^{'},u^{'}\}}}
            \\
            \frac{1}{2}
            \coefD{\indexjp{l}}{\order{t^{'},u^{'}}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\order{(\indexJp\backslash\{\indexjp{l},\alpha^{'}\})\cup\{t^{'},u^{'}\}}}
        \end{pmatrix*}
    \end{pmatrix*}
    .
\label{EQ-For (alpha, I, J), calculation for LHS, extra 1-simplified result of part 1, alpha in J}
\end{align}

%%%%%%%%%%%% finish alpha in J %%%%%%%%%%%%

%%%%%%%%%%%% start alpha not in J %%%%%%%%%%%%

Next, we observe that if $\alpha\notin\indexJ$, then the terms in (\ref{EQ-For (alpha, I, J), calculation for LHS, extra 1-no3}) are calculated as follows.
\begin{itemize}
    \item 
$
    \contract{\basedualxi{\alpha^{'}}}
    \big(
    \basexi{\indexI}
    \wedge
    \basedualxi{\order{\indexJp\cup\{t^{'}\}}}
    \big)
    =
    \begin{cases}
            0
            &
            \text{if }\alpha\neq t
        \\
            \sgn
                {\indexI,\order{\indexJp\cup\{\alpha^{'}\}}}
                {\alpha^{'},\indexI,\indexJp}
            \basexi{\indexI}
            \wedge
            \basedualxi{\indexJp}
            &
            \text{if }\alpha=t
    \end{cases}
$.
\\
    \item 
$
    \qquad
    \contract{\basedualxi{\alpha^{'}}}
    \big(
    \basexi{\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
    \wedge
    \basedualxi{\order{\indexJp\cup\{t^{'}\}}}
    \big)
$
\\
$
    =
    \begin{cases}
            0
            &
            \text{if }\alpha\neq t
        \\
            \sgn
                {\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}},\order{\indexJp\cup\{\alpha^{'}\}}}
                {\alpha^{'},\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}},\indexJp}
            \basexi{\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
            \wedge
            \basedualxi{\indexJp}
            &
            \text{if }\alpha=t
    \end{cases}
$.
\\
    \item 
$
    \contract{\basedualxi{\alpha^{'}}}
    \big(
    \basexi{\indexI}
    \wedge
    \basedualxi{\order{\indexJp\cup\{t^{'}\}}}
    \big)
    =
    \begin{cases}
            0
        &
            \text{if }\alpha\neq t
        \\
            \sgn
                {\indexI,\order{\indexJp\cup\{\alpha^{'}\}}}
                {\alpha^{'},\indexI,\indexJp}
            \basexi{\indexI}
            \wedge
            \basedualxi{\indexJp}
        &
            \text{if }\alpha=t
    \end{cases}
$.
    \item 
$
    \qquad
    \contract{\basedualxi{\alpha^{'}}}
    \big(
    \basexi{\indexI}
    \wedge
    \basedualxi{\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'},u^{'}\}}}
    \big)
$
\\
$
    =
    \begin{cases}
            0       
        &
            \text{if }\alpha\neq t,u
        \\
            \sgn
                {\indexI,\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'},\alpha^{'}\}}}
                {\alpha^{'},\indexI,\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
        &
            \text{if }\alpha=u
        \\
            \sgn
                {\indexI,\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{\alpha^{'},u^{'}\}}}
                {\alpha^{'},\indexI,\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{u^{'}\}}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{u^{'}\}}}
        &
            \text{if }\alpha=t
    \end{cases}
$ .
\end{itemize}
We use the above observation to calculate the expression of $
    \iota_{\basedualxi{\alpha}}\,\LieagbdPartialbar
    (\basexi{\indexI}\wedge\basedualxi{\indexJp})
$:
\begin{align}
    % &
    %     \iota_{\basedualxi{\alpha}}\,\LieagbdPartialbar
    %     (\basexi{\indexI}\wedge\basedualxi{\indexJp})
    % \notag
    % \\
    % =&
        2
        \begin{pmatrix*}[l]
            %?--1
            \displaystyle\sum_{\indexi{k}\in\indexI}
            \sgn
                {\indexI}
                {\indexi{k},\indexI\backslash\{\indexi{k}\}}
            \sgn
                {\indexi{1},\cdots,\indexi{k},\alpha^{'},\indexi{k+1},\cdots,\indexi{p},\indexJp}
                {\indexI,\order{\indexJp\cup\{\alpha^{'}\}}}
            \sgn
                {\indexI,\order{\indexJp\cup\{\alpha^{'}\}}}
                {\alpha^{'},\indexI,\indexJp}
            \coefB{\indexi{k}}{\indexi{k} \alpha^{'}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\indexJp}
            \\
            +
            \\
            %?--2
            \displaystyle\sum_{\indexi{k}\in\indexI}
            \displaystyle\sum_{s\in\indexIc}
            \begin{pmatrix*}[l]
                \sgn
                    {\indexI}
                    {\indexi{k},\indexI\backslash\{\indexi{k}\}}
                \sgn
                    {\indexi{1},\cdots,\indexi{k-1},s,\alpha^{'},\indexi{k+1},\cdots,\indexi{p},\indexJp}
                    {\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}},\order{\indexJp\cup\{\alpha^{'}\}}}
                \\
                \sgn
                    {\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}},\order{\indexJp\cup\{\alpha^{'}\}}}
                    {\alpha^{'},\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}},\indexJp}
                \\
                \coefB{\indexi{k}}{s \alpha^{'}}
                \basexi{\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
                \wedge
                \basedualxi{\indexJp}
            \end{pmatrix*}
            \\
            +
            \\
            %?--3
            \displaystyle\sum_{\indexjp{l}\in\indexJp}
                \begin{pmatrix*}[l]
                \sgn
                    {\indexI,\indexJp}
                    {\indexjp{l},\indexI,\indexJp\backslash\{\indexjp{l}\}}
                \sgn
                    {\indexjp{1},\cdots,\indexjp{l-1},\order{\indexjp{l},\alpha^{'}},\indexjp{l+1},\cdots,\indexjp{q}}
                    {\order{\indexJp\cup\{\alpha^{'}\}}}
                \sgn
                    {\indexI,\order{\indexJp\cup\{\alpha^{'}\}}}
                    {\alpha^{'},\indexI,\indexJp}
                \\
                \coefD{\indexjp{l}}{\order{\indexjp{l},\alpha^{'}}}
                \basexi{\indexI}
                \wedge
                \basedualxi{\indexJp}
            \end{pmatrix*}
            \\
            +
            \\
            %?--4
            \displaystyle\sum_{\indexjp{l}\in\indexJp}
            \displaystyle\sum_{t^{'}\in\indexJpc\backslash\{\alpha^{'}\}}
            \begin{pmatrix*}[l]
                \sgn
                    {\indexI,\indexJp}
                    {\indexjp{l},\indexI,\indexJp\backslash\{\indexjp{l}\}}
                \sgn
                    {\indexjp{1},\cdots,\indexjp{l-1},\order{t^{'},\alpha^{'}},\indexjp{l+1},\cdots,\indexjp{q}}
                    {\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'},\alpha^{'}\}}}
                \\
                \sgn
                    {\indexI,\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'},\alpha^{'}\}}}
                    {\alpha^{'},\indexI,\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
                \\
                \frac{1}{2}
                \coefD{\indexjp{l}}{\order{t^{'},\alpha^{'}}}
                \basexi{\indexI}
                \wedge
                \basedualxi{\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
            \end{pmatrix*}
            \\
            +
            \\
            %?--5
            \displaystyle\sum_{\indexjp{l}\in\indexJp}
            \displaystyle\sum_{u^{'}\in\indexJpc\backslash\{\alpha^{'}\}}
            \begin{pmatrix*}[l]
                \sgn
                    {\indexI,\indexJp}
                    {\indexjp{l},\indexI,\indexJp\backslash\{\indexjp{l}\}}
                \sgn
                    {\indexjp{1},\cdots,\indexjp{l-1},\order{\alpha^{'},u^{'}},\indexjp{l+1},\cdots,\indexjp{q}}
                    {\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{\alpha^{'},u^{'}\}}}
                \\
                \sgn
                    {\indexI,\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{\alpha^{'},u^{'}\}}}
                {\alpha^{'},\indexI,\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{u^{'}\}}}
                \\
                \frac{1}{2}
                \coefD{\indexjp{l}}{\order{\alpha^{'},u^{'}}}
                \basexi{\indexI}
                \wedge
                \basedualxi{\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{u^{'}\}}}
            \end{pmatrix*}
        \end{pmatrix*}
    .
\label{EQ-For (alpha, I, J), calculation for LHS, extra 1-no4}
\end{align}
The last two terms in (\ref{EQ-For (alpha, I, J), calculation for LHS, extra 1-no4}) are same if we identify $u$ with $t$. Therefore, we simplify (\ref{EQ-For (alpha, I, J), calculation for LHS, extra 1-no4}) to
\begin{align}
    &
        \iota_{\basedualxi{\alpha}}\,\LieagbdPartialbar
        (\basexi{\indexI}\wedge\basedualxi{\indexJp})
    \notag\\
    =&
        2
        \begin{pmatrix*}[l]
            %?--1
            \displaystyle\sum_{\indexi{k}\in\indexI}
            \begin{pmatrix*}[l]
                \sgn
                    {\indexI}
                    {\indexi{k},\indexI\backslash\{\indexi{k}\}}
                \sgn
                    {\indexi{1},\cdots,\indexi{k},\alpha^{'},\indexi{k+1},\cdots,\indexi{p},\indexJp}
                    {\indexI,\order{\indexJp\cup\{\alpha^{'}\}}}
                \sgn
                    {\indexI,\order{\indexJp\cup\{\alpha^{'}\}}}
                    {\alpha^{'},\indexI,\indexJp}
                \coefB{\indexi{k}}{\indexi{k} \alpha^{'}}
                \basexi{\indexI}
                \wedge
                \basedualxi{\indexJp}
            \end{pmatrix*}
            \\
            +
            \\
            %?--2
            \displaystyle\sum_{\indexi{k}\in\indexI}
            \displaystyle\sum_{s\in\indexIc}
            \begin{pmatrix*}[l]
                \sgn
                    {\indexI}
                    {\indexi{k},\indexI\backslash\{\indexi{k}\}}
                \sgn
                    {\indexi{1},\cdots,\indexi{k-1},s,\alpha^{'},\indexi{k+1},\cdots,\indexi{p},\indexJp}
                    {\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}},\order{\indexJp\cup\{\alpha^{'}\}}}
                \\
                \sgn
                    {\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}},\order{\indexJp\cup\{\alpha^{'}\}}}
                    {\alpha^{'},\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}},\indexJp}
                \\
                \coefB{\indexi{k}}{s \alpha^{'}}
                \basexi{\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
                \wedge
                \basedualxi{\indexJp}
            \end{pmatrix*}
            \\
            +
            \\
            %?--3
            \displaystyle\sum_{\indexjp{l}\in\indexJp}
                \begin{pmatrix*}[l]
                \sgn
                    {\indexI,\indexJp}
                    {\indexjp{l},\indexI,\indexJp\backslash\{\indexjp{l}\}}
                \sgn
                    {\indexjp{1},\cdots,\indexjp{l-1},\order{\indexjp{l},\alpha^{'}},\indexjp{l+1},\cdots,\indexjp{q}}
                    {\order{\indexJp\cup\{\alpha^{'}\}}}
                \\
                \sgn
                    {\indexI,\order{\indexJp\cup\{\alpha^{'}\}}}
                    {\alpha^{'},\indexI,\indexJp}
                \\
                \coefD{\indexjp{l}}{\order{\indexjp{l},\alpha^{'}}}
                \basexi{\indexI}
                \wedge
                \basedualxi{\indexJp}
            \end{pmatrix*}
            \\
            +
            \\
            %?--4
            \displaystyle\sum_{\indexjp{l}\in\indexJp}
            \displaystyle\sum_{t^{'}\in\indexJpc}
            \begin{pmatrix*}[l]
                \sgn
                    {\indexI,\indexJp}
                    {\indexjp{l},\indexI,\indexJp\backslash\{\indexjp{l}\}}
                \sgn
                    {\indexjp{1},\cdots,\indexjp{l-1},\order{t^{'},\alpha^{'}},\indexjp{l+1},\cdots,\indexjp{q}}
                    {\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'},\alpha^{'}\}}}
                \\
                \sgn
                    {\indexI,\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'},\alpha^{'}\}}}
                    {\alpha^{'},\indexI,\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
                \\
                \coefD{\indexjp{l}}{\order{t^{'},\alpha^{'}}}
                \basexi{\indexI}
                \wedge
                \basedualxi{\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
            \end{pmatrix*}
        \end{pmatrix*}.
\label{EQ-For (alpha, I, J), calculation for LHS, extra 1-unsimplified the first half, alpha not in J}
\end{align}
The reader can find the simplification of the signs of permutations in Lemmas \ref{lemma-simplification for LHS, extra 1, part 1-lemma 5}–\ref{lemma-simplification for LHS, extra 1, part 1-lemma 8} in Section \ref{apex-simplification for LHS, extra 1, part 1}. We conclude that when $\alpha\notin\indexJ$ the expression of $
\iota_{\basedualxi{\alpha}}\,\LieagbdPartialbar
(\basexi{\indexI} \wedge \basedualxi{\indexJp})
$ is
\begin{align}%simplified part 1
    &
        \iota_{\basedualxi{\alpha}}\,\LieagbdPartialbar
        (\basexi{\indexI}\wedge\basedualxi{\indexJp})
    \notag\\
    =&
        2
        \begin{pmatrix*}[l]
            %?--1
            \displaystyle\sum_{\indexi{k}\in\indexI}
                (-1)
                \coefB{\indexi{k}}{\indexi{k} \alpha^{'}}
                \basexi{\indexI}
                \wedge
                \basedualxi{\indexJp}
            \\
            +
            \\
            %?--2
            \displaystyle\sum_{\indexi{k}\in\indexI}
            \displaystyle\sum_{s\in\indexIc}
                \sgn
                    {s,\indexI,\indexJp}
                    {\indexi{k},\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}},\indexJp}
                \coefB{\indexi{k}}{s \alpha^{'}}
                \basexi{\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
                \wedge
                \basedualxi{\indexJp}
            \\
            +
            \\
            %?--3
            \displaystyle\sum_{\indexjp{l}\in\indexJp}
                \sgn
                    {\order{\indexjp{l},\alpha^{'}}}
                    {\alpha^{'},\indexjp{l}}
                \coefD{\indexjp{l}}{\order{\indexjp{l},\alpha^{'}}}
                \basexi{\indexI}
                \wedge
                \basedualxi{\indexJp}
            \\
            +
            \\
            %?--4
            \displaystyle\sum_{\indexjp{l}\in\indexJp}
            \displaystyle\sum_{t^{'}\in\indexJpc}
            \begin{pmatrix*}[l]
                \sgn
                    {\order{\alpha^{'},t^{'}}}
                    {t^{'},\alpha^{'}}
                \sgn
                    {t^{'},\indexI,\indexJp}
                    {\indexjp{l},\indexI,\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
            \\
                \coefD{\indexjp{l}}{\order{t^{'},\alpha^{'}}}
                \basexi{\indexI}
                \wedge
                \basedualxi{\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
            \end{pmatrix*}
        \end{pmatrix*}
        .
\label{EQ-For (alpha, I, J), calculation for LHS, extra 1-simplified the first half, alpha not in J}
\end{align}
%%%%%%%%%%%% finish calculate \iota alpha \,\LieagbdPartialbar (I,J) %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% start calculate partial \, \iota  (I,J) %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\keyword{Step 2:} Looking at $\contract{\basedualxi{\alpha}}(\basexi{\indexI}\wedge\basedualxi{\indexJp})$,
\begin{align}
    \contract{\basedualxi{\alpha}}
    (\basexi{\indexI}\wedge\basedualxi{\indexJp})
    =
    \begin{cases}
            0
        &
            \alpha\notin\indexJ
        \\
            2\sgn
                {\indexI,\indexJp}
                {\alpha^{'},\indexI,\indexJp\backslash\{\alpha^{'}\}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\indexJp\backslash\{\alpha^{'}\}}
        &
            \alpha\in\indexJ
    \end{cases}.
\label{EQ-For (alpha, I, J), calculation for LHS, extra 1-no5}
\end{align}
We just need to consider the case that $\alpha\in\indexJ$. Applying $\LieagbdPartialbar$ to the formula in (\ref{EQ-For (alpha, I, J), calculation for LHS, extra 1-no5}) such that $\alpha\in\indexJ$, we find that $
\LieagbdPartialbar\,\iota_{\basedualxi{\alpha}}(\basexi{\indexI}\wedge\basedualxi{\indexJp})
$ is equal to
\begin{align}
        2\sgn
            {\indexI,\indexJp}
            {\alpha^{'},\indexI,\indexJp\backslash\{\alpha^{'}\}}
        \begin{pmatrix*}[l]
            %?--2-1
            \displaystyle\sum_{\indexi{k}\in\indexI}
            \sgn
                {\indexI}
                {\indexi{k},\indexI\backslash\{\indexi{k}\}}
            \basexi{\indexi{1}}
            \wedge\cdots\wedge
            \LieagbdPartialbar\basexi{\indexi{k}}
            \wedge\cdots\wedge
            \basexi{\indexi{p}}
            \wedge
            \basedualxi{\indexJp\backslash\{\alpha^{'}\}}
            \\
            +
            \\
            %?--2-2
            \displaystyle\sum_{\indexj{l}\in\indexJp\backslash\{\alpha^{'}\}}
            \sgn
                {\indexI,\indexJp\backslash\{\alpha^{'}\}}
                {\indexjp{l},\indexI,\indexJp\backslash\{\alpha^{'},\indexjp{l}\}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\indexjp{1}}
            \wedge\cdots\wedge
            \LieagbdPartialbar\basedualxi{\indexjp{l}}
            \wedge\cdots\wedge
            \widehat{\basedualxi{\alpha^{'}}}
            \wedge\cdots\wedge
            \basedualxi{\indexjp{q}}
        \end{pmatrix*}
\label{EQ-For (alpha, I, J), calculation for LHS, extra 1-no6}
\end{align}
for $\alpha\in\indexJ$. Recalling that $
    \LieagbdPartialbar \xi_i
    =
        \sum_{j,k}^n
        \coefB{i}{jk}
        \basexi{j} \wedge \basedualxi{k}
$
and
\begin{align*}
    \LieagbdPartialbar \basedualxi{i}
    =
        \sum_{j,k=1}^n
        \frac{1}{2}
        \coefD{i}{jk}
        \basedualxi{j} \wedge \basedualxi{k}
    =
        \sum_{j,k=1}^n
        \frac{1}{2}
        \sgn
            {\order{j,k}}
            {j,k}
        \coefD{i}{\order{j,k}}
        \basedualxi{j}\wedge\basedualxi{k}
    ,
\end{align*}
we plug these into (\ref{EQ-For (alpha, I, J), calculation for LHS, extra 1-no6}) and cancel out the terms containing repeated frames. Thus, $
\LieagbdPartialbar\,\iota_{\basedualxi{\alpha}}(\basexi{\indexI}\wedge\basedualxi{\indexJp})
$ for $\alpha\in\indexJ$ has the following expression:
\begin{align*}
    2
    \begin{pmatrix*}[l]
        %?--3-1
        \displaystyle\sum_{\indexi{k}\in\indexI}
        \begin{pmatrix*}[l]
            \sgn
                {\indexI,\indexJp}
                {\alpha^{'},\indexI,\indexJp\backslash\{\alpha^{'}\}}
            \sgn
                {\indexI}
                {\indexi{k},\indexI\backslash\{\indexi{k}\}}
            \\
            \basexi{\indexi{1}}
            \wedge\cdots\wedge
            \basexi{\indexi{k-1}}\wedge
            \begin{pmatrix*}[l]
                %?--3-1-1
                \coefB{\indexi{k}}{\indexi{k} \alpha^{'}}
                \basexi{\indexi{k}}
                \wedge
                \basedualxi{\alpha^{'}}
                \\
                +
                \\
                %?--3-1-2
                \displaystyle\sum_{t^{'}\in \indexJpc}
                \coefB{\indexi{k}}{\indexi{k} t^{'}}
                \basexi{\indexi{k}}
                \wedge
                \basedualxi{t^{'}}
                \\
                +
                \\
                %?--3-1-3
                \displaystyle\sum_{s\in \indexIc}
                \coefB{\indexi{k}}{s \alpha^{'}}
                \basexi{s}
                \wedge
                \basedualxi{\alpha^{'}}
                \\
                +
                \\
                %?--3-1-4
                \displaystyle\sum_{s\in \indexIc}
                \displaystyle\sum_{t^{'}\in \indexJpc}
                \coefB{\indexi{k}}{s t^{'}}
                \basexi{s}
                \wedge
                \basedualxi{t^{'}}
            \end{pmatrix*}
            \wedge\basexi{\indexi{k+1}}
            \wedge\cdots\wedge
            \basexi{\indexi{p}}
            \wedge
            \basedualxi{\indexJp\backslash\{\alpha^{'}\}}
        \end{pmatrix*}
        \\
        +
        \\
        %?--3-2
        \displaystyle\sum_{\indexjp{l}\in\indexJp\backslash\{\alpha^{'}\}}
        \begin{pmatrix*}[l]
            \sgn
                {\indexI,\indexJp}
                {\alpha^{'},\indexI,\indexJp\backslash\{\alpha^{'}\}}
            \sgn
                {\indexI,\indexJp\backslash\{\alpha^{'}\}}
                {\indexjp{l},\indexI,\indexJp\backslash\{\alpha^{'},\indexjp{l}\}}
            \\
            \basexi{\indexI}
            \wedge
            \basedualxi{\indexjp{1}}
            \wedge\cdots\wedge
            \basedualxi{\indexjp{l-1}}\wedge
            \begin{pmatrix*}[l]
                %?--3-2-1
                \frac{1}{2}
                (
                \coefD{\indexjp{l}}{\indexjp{l} \alpha^{'}}
                \basedualxi{\indexjp{l}}
                \wedge
                \basedualxi{\alpha^{'}}
                +
                \coefD{\indexjp{l}}{\alpha^{'} \indexjp{l}}
                \basedualxi{\alpha^{'}}
                \wedge
                \basedualxi{\indexjp{l}}
                )
                \\
                +
                \\
                %?--3-2-2
                \frac{1}{2}
                \displaystyle\sum_{t^{'}\in\indexJpc}
                \coefD{\indexjp{l}}{\indexjp{l} t^{'}}
                \basedualxi{\indexjp{l}}
                \wedge
                \basedualxi{t^{'}}
                +
                \coefD{\indexjp{l}}{t^{'} \indexjp{l}}
                \basedualxi{t^{'}}
                \wedge
                \basedualxi{\indexjp{l}}
                \\
                +
                \\
                %?--3-2-3
                \frac{1}{2}
                \displaystyle\sum_{t^{'}\in\indexJpc}
                \coefD{\indexjp{l}}{\alpha^{'} t^{'}}
                \basedualxi{\alpha^{'}}
                \wedge
                \basedualxi{t^{'}}
                +
                \coefD{\indexjp{l}}{t^{'} \alpha^{'}}
                \basedualxi{t^{'}}
                \wedge
                \basedualxi{\alpha^{'}}
                \\
                +
                \\
                %?--3-2-4
                \frac{1}{2}
                \displaystyle\sum_{t^{'}\in\indexJpc}
                \displaystyle\sum_{u^{'}\in\indexJpc}
                \coefD{\indexjp{l}}{u^{'} t^{'}}
                \basedualxi{u^{'}}
                \wedge
                \basedualxi{t^{'}}
            \end{pmatrix*}
            \wedge\basedualxi{\indexjp{l+1}}
            \\
            \wedge\cdots\wedge
            \widehat{\basedualxi{\alpha^{'}}}
            \wedge\cdots\wedge
            \basedualxi{\indexjp{q}}
        \end{pmatrix*}
    \end{pmatrix*}.
\end{align*}


We reorder the wedge product of frames as follows:
\begin{itemize}
    \item %1
$
        \qquad
        \basexi{\indexi{1}}
        \wedge\cdots\wedge
        \basexi{\indexi{k-1}}\wedge
        \bigg(
            \coefB{\indexi{k}}{\indexi{k} \alpha^{'}}
            \basexi{\indexi{k}}
            \wedge
            \basedualxi{\alpha^{'}}
        \bigg)
        \wedge\basexi{\indexi{k+1}}
        \wedge\cdots\wedge
        \basexi{\indexi{p}}
        \wedge
        \basedualxi{\indexJp\backslash\{\alpha^{'}\}}
$
\\
$
    =
        \sgn        
            {\indexi{1},\cdots,\indexi{k},\alpha^{'},\indexi{k+1},\cdots,\indexi{p},\indexJp\backslash\{\alpha^{'}\}}
            {\indexI,\indexJp}
        \coefB{\indexi{k}}{\indexi{k} \alpha^{'}}
        \basexi{\indexI}
        \wedge
        \basedualxi{\indexJp}
$,
    \\
    \item %2
$
        \qquad
        \basexi{\indexi{1}}
        \wedge\cdots\wedge
        \basexi{\indexi{k-1}}\wedge
        \bigg(
            \displaystyle\sum_{t^{'}\in \indexJpc}
            \coefB{\indexi{k}}{\indexi{k} t^{'}}
            \basexi{\indexi{k}}
            \wedge
            \basedualxi{t^{'}}
        \bigg)
        \wedge\basexi{\indexi{k+1}}
        \wedge\cdots\wedge
        \basexi{\indexi{p}}
        \wedge
        \basedualxi{\indexJp\backslash\{\alpha^{'}\}}
$
\\
$
        =
        \displaystyle\sum_{t^{'}\in \indexJpc}
        \sgn
            {\indexi{1},\cdots,\indexi{k},t^{'},\indexi{k+1},\cdots,\indexi{p},\indexJp\backslash\{\alpha^{'}\}}
            {\indexI,\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
        \coefB{\indexi{k}}{\indexi{k} t^{'}}
        \basexi{\indexI}
        \wedge
        \basedualxi{\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}} 
$,
    \\
    \item %3
$
        \qquad
        \basexi{\indexi{1}}
        \wedge\cdots\wedge
        \basexi{\indexi{k-1}}\wedge
        \bigg(
            \displaystyle\sum_{s\in \indexIc}
            \coefB{\indexi{k}}{s \alpha^{'}}
            \basexi{s}
            \wedge
            \basedualxi{\alpha^{'}}
        \bigg)
        \wedge\basexi{\indexi{k+1}}
        \wedge\cdots\wedge
        \basexi{\indexi{p}}
        \wedge
        \basedualxi{\indexJp\backslash\{\alpha^{'}\}}
$
\\
$
        =
        \displaystyle\sum_{s\in \indexIc}
        \sgn
            {\indexi{1},\cdots,\indexi{k-1},s,\alpha^{'},\indexi{k+1},\cdots,\indexi{p},\indexJp\backslash\{\alpha^{'}\}}
            {\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}},\indexJp}
        \coefB{\indexi{k}}{s \alpha^{'}}
        \basexi{\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
        \wedge
        \basedualxi{\indexJp}
$,
    \\
    \item  %4
$
        \qquad
        \basexi{\indexi{1}}
            \wedge\cdots\wedge
            \basexi{\indexi{k-1}}\wedge
            \bigg(
                \displaystyle\sum_{s\in \indexIc}
                \displaystyle\sum_{t^{'}\in \indexJpc}
                \coefB{\indexi{k}}{s t^{'}}
                \basexi{s}
                \wedge
                \basedualxi{t^{'}}
            \bigg)
            \wedge\basexi{\indexi{k+1}}
            \wedge\cdots\wedge
            \basexi{\indexi{p}}
            \wedge
            \basedualxi{\indexJp\backslash\{\alpha^{'}\}}
$
\\
$
        =
        \displaystyle\sum_{s\in \indexIc}
        \displaystyle\sum_{t^{'}\in \indexJpc}
        \begin{pmatrix*}[l]
            \sgn
                {\indexi{1},\cdots,\indexi{k-1},s,t^{'},\indexi{k+1},\cdots,\indexi{p},\indexJp\backslash\{\alpha^{'}\}}
                {\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}},\order{(\indexJp\backslash\alpha^{'})\cup{t^{'}}}}
            \\
            \coefB{\indexi{k}}{s t^{'}}
            \basexi{\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
            \wedge
            \basedualxi{\order{(\indexJp\backslash\alpha^{'})\cup{t^{'}}}}
        \end{pmatrix*}   
$,
    \item %5
$
        \qquad
        \basexi{\indexI}
        \wedge
        \basedualxi{\indexjp{1}}
        \wedge\cdots\wedge
        \basedualxi{\indexjp{l-1}}\wedge
        \frac{1}{2}
        \begin{pmatrix*}[l]
            \coefD{\indexjp{l}}{\indexjp{l} \alpha^{'}}
            \basedualxi{\indexjp{l}}
            \wedge
            \basedualxi{\alpha^{'}}
            \\
            +
            \\
            \coefD{\indexjp{l}}{\alpha^{'} \indexjp{l}}
            \basedualxi{\alpha^{'}}
            \wedge
            \basedualxi{\indexjp{l}}
        \end{pmatrix*}
        \wedge\basedualxi{\indexjp{l+1}}
        \wedge\cdots\wedge
        \widehat{\basedualxi{\alpha^{'}}}
        \wedge\cdots\wedge
        \basedualxi{\indexjp{q}}
$
\\
$
        =
        \basexi{\indexI}
        \wedge
        \basedualxi{\indexjp{1}}
        \wedge\cdots\wedge
        \basedualxi{\indexjp{l-1}}\wedge
            \coefD{\indexjp{l}}{\order{\indexjp{l} \alpha^{'}}}
            \basedualxi{\order{\indexjp{l} \alpha^{'}}}
        \wedge\basedualxi{\indexjp{l+1}}
        \wedge\cdots\wedge
        \widehat{\basedualxi{\alpha^{'}}}
        \wedge\cdots\wedge
        \basedualxi{\indexjp{q}}
$
\\
$
        =
        \sgn
            {\indexjp{1},\cdots,\indexjp{l-1},\order{\indexjp{l},\alpha^{'}},\indexjp{l+1},\cdots,\widehat{\alpha^{'}},\cdots,\indexjp{q}}
            {\indexJp}
        \coefD{\indexjp{l}}{\order{\indexjp{l} \alpha^{'}}}
        \basexi{\indexI}
        \wedge
        \basedualxi{\indexJp}
$,
    \\
    \item %6
$
        \qquad
        \basexi{\indexI}
        \wedge
        \basedualxi{\indexjp{1}}
        \wedge\cdots\wedge
        \basedualxi{\indexjp{l-1}}\wedge
        \frac{1}{2}
        \displaystyle\sum_{t^{'}\in\indexJpc}
        \begin{pmatrix*}[l]
            \coefD{\indexjp{l}}{\indexjp{l} t^{'}}
            \basedualxi{\indexjp{l}}
            \wedge
            \basedualxi{t^{'}}
            \\
            +
            \\
            \coefD{\indexjp{l}}{t^{'} \indexjp{l}}
            \basedualxi{t^{'}}
            \wedge
            \basedualxi{\indexjp{l}}
        \end{pmatrix*}
        \wedge\basedualxi{\indexjp{l+1}}
        \wedge\cdots\wedge
        \widehat{\basedualxi{\alpha^{'}}}
        \wedge\cdots\wedge
        \basedualxi{\indexjp{q}}
$
\\
$
        =
        \basexi{\indexI}
            \wedge
            \basedualxi{\indexjp{1}}
            \wedge\cdots\wedge
            \basedualxi{\indexjp{l-1}}\wedge
                \displaystyle\sum_{t^{'}\in\indexJpc}
                \coefD{\indexjp{l}}{\order{ \indexjp{l} t^{'}} }
                \basedualxi{\order {\indexjp{l} t^{'}}}
            \wedge\basedualxi{\indexjp{l+1}}
            \wedge\cdots\wedge
            \widehat{\basedualxi{\alpha^{'}}}
            \wedge\cdots\wedge
            \basedualxi{\indexjp{q}}
$
\\
$
        =
        \displaystyle\sum_{t^{'}\in\indexJpc}
        \sgn
            {\indexjp{1},\cdots,\indexjp{l-1},\order{\indexjp{l},t^{'}},\indexjp{l+1},\cdots,\widehat{\alpha^{'}},\cdots,\indexjp{q}}
            {\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
        \coefD{\indexjp{l}}{\order{\indexjp{l} t^{'}}}
        \basexi{\indexI}
        \wedge
        \basedualxi{\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
$,
    \\
    \item %7
$
        \qquad
        \basexi{\indexI}
        \wedge
        \basedualxi{\indexjp{1}}
        \wedge\cdots\wedge
        \basedualxi{\indexjp{l-1}}\wedge
        \frac{1}{2}
        \displaystyle\sum_{t^{'}\in\indexJpc}
        \begin{pmatrix*}[l]
            \coefD{\indexjp{l}}{\alpha^{'} t^{'}}
            \basedualxi{\alpha^{'}}
            \wedge
            \basedualxi{t^{'}}
            \\
            +
            \\
            \coefD{\indexjp{l}}{t^{'} \alpha^{'}}
            \basedualxi{t^{'}}
            \wedge
            \basedualxi{\alpha^{'}}
        \end{pmatrix*}
        \wedge\basedualxi{\indexjp{l+1}}
        \wedge\cdots\wedge
        \widehat{\basedualxi{\alpha^{'}}}
        \wedge\cdots\wedge
        \basedualxi{\indexjp{q}}
$
\\
$
        =
        \basexi{\indexI}
        \wedge
        \basedualxi{\indexjp{1}}
        \wedge\cdots\wedge
        \basedualxi{\indexjp{l-1}}\wedge
            \displaystyle\sum_{t^{'}\in\indexJpc}
            \coefD{\indexjp{l}}{\order{\alpha^{'} t^{'}}}
            \basedualxi{\order{ \alpha^{'}  t^{'}}}
        \wedge\basedualxi{\indexjp{l+1}}
        \wedge\cdots\wedge
        \widehat{\basedualxi{\alpha^{'}}}
        \wedge\cdots\wedge
        \basedualxi{\indexjp{q}}
$
\\
$
        =
        \displaystyle\sum_{t^{'}\in\indexJpc}
        \sgn
            {\indexjp{1},\cdots,\indexjp{l-1},\order{\alpha^{'},t^{'}},\indexjp{l+1},\cdots,\widehat{\alpha^{'}},\cdots,\indexjp{q}}
            {\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
        \coefD{\indexjp{l}}{\order{\alpha^{'} t^{'}}}
        \basexi{\indexI}
        \wedge
        \basedualxi{\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
$,
    \\
    \item %8
$
        \qquad
        \begin{matrix*}[l]
            \basexi{\indexI}
            \wedge
            \basedualxi{\indexjp{1}}
            \wedge\cdots\wedge
            \basedualxi{\indexjp{l-1}}\wedge
            \frac{1}{2}
            \bigg(
                \displaystyle\sum_{t^{'}\in\indexJpc}
                \displaystyle\sum_{u^{'}\in\indexJpc}
                \coefD{\indexjp{l}}{u^{'} t^{'}}
                \basedualxi{u^{'}}
                \wedge
                \basedualxi{t^{'}}
            \bigg)
            \wedge\basedualxi{\indexjp{l+1}}
            \wedge\cdots\wedge
            \widehat{\basedualxi{\alpha^{'}}}
            \wedge\cdots
            \\
            \wedge\basedualxi{\indexjp{q}}
        \end{matrix*}
$
\\
$
        =
        \displaystyle\sum_{t^{'}\in\indexJpc}
        \displaystyle\sum_{u^{'}\in\indexJpc}
        \begin{pmatrix*}[l]
            \sgn
                {\indexjp{1},\cdots,\indexjp{l-1},\order{t^{'},u^{'}},\indexjp{l+1},\cdots,\widehat{\alpha^{'}},\cdots,\indexjp{q}}
                {\order{(\indexJp\backslash\{\indexjp{l},\alpha^{'}\})\cup\{t^{'},u^{'}\}}}
            \\
            \frac{1}{2}
            \coefD{\indexjp{l}}{\order{t^{'} u^{'}}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\order{(\indexJp\backslash\{\indexjp{l}, \alpha^{'}\})\cup\{t^{'},u^{'}\}}}
        \end{pmatrix*}
$.
    \\
\end{itemize}
Using the above properties, we calculate $\LieagbdPartialbar\,\contract{\basedualxi{\alpha}}(\basexi{\indexI}\wedge\basedualxi{\indexJp})$ for $\alpha\in\indexJ$ as a sum of eight groups of terms:
\begin{flalign}
    &
        %?--4-1
        \displaystyle\sum_{\indexi{k}\in\indexI}
        2
        \begin{pmatrix*}[l]
            \sgn
                {\indexI,\indexJp}
                {\alpha^{'},\indexI,\indexJp\backslash\{\alpha^{'}\}}
            \sgn
                {\indexI}
                {\indexi{k},\indexI\backslash\{\indexi{k}\}}
            \sgn
                {\indexi{1},\cdots,\indexi{k},\alpha^{'},\indexi{k+1},\cdots,\indexi{p},\indexJp\backslash\{\alpha^{'}\}}
                {\indexI,\indexJp}
            \\
            \coefB{\indexi{k}}{\indexi{k} \alpha^{'}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\indexJp}
        \end{pmatrix*}
        &&
        \notag\\
    &   +&&
        \notag\\
    &       %?--4-2
        \displaystyle\sum_{\indexi{k}\in\indexI}
        \displaystyle\sum_{t^{'}\in\indexJpc}
        2
        \begin{pmatrix*}[l]
            \sgn
                {\indexI,\indexJp}
                {\alpha^{'},\indexI,\indexJp\backslash\{\alpha^{'}\}}
            \sgn
                {\indexI}
                {\indexi{k},\indexI\backslash\{\indexi{k}\}}
            \sgn
                {\indexi{1},\cdots,\indexi{k},t^{'},\indexi{k+1},\cdots,\indexi{p},\indexJp\backslash\{\alpha^{'}\}}
                {\indexI,\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
            \\
            \coefB{\indexi{k}}{\indexi{k} t^{'}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
        \end{pmatrix*}
        &&
        \notag\\
    &   +&&
        \notag\\
    &       %?--4-3
        \displaystyle\sum_{\indexi{k}\in\indexI}
        \displaystyle\sum_{s\in\indexIc}
        2
        \begin{pmatrix*}[l]
            \sgn
                {\indexI,\indexJp}
                {\alpha^{'},\indexI,\indexJp\backslash\{\alpha^{'}\}}
            \sgn
                {\indexI}
                {\indexi{k},\indexI\backslash\{\indexi{k}\}}
            \sgn
                {\indexi{1},\cdots,\indexi{k-1},s,\alpha^{'},\indexi{k+1},\cdots,\indexi{p},\indexJp\backslash\{\alpha^{'}\}}
                {\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}},\indexJp}
            \\
            \coefB{\indexi{k}}{s \alpha^{'}}
            \basexi{\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
            \wedge
            \basedualxi{\indexJp}
        \end{pmatrix*}
        &&
        \notag\\
    &   +&&
        \notag\\
    &   %?--4-4
        \displaystyle\sum_{\indexi{k}\in\indexI}
        \displaystyle\sum_{s\in\indexIc}
        \displaystyle\sum_{t^{'}\in\indexJpc}
        2
        \begin{pmatrix*}[l]
            \sgn
                {\indexI,\indexJp}
                {\alpha^{'},\indexI,\indexJp\backslash\{\alpha^{'}\}}
            \sgn
                {\indexI}
                {\indexi{k},\indexI\backslash\{\indexi{k}\}}
            \sgn
                {\indexi{1},\cdots,\indexi{k-1},s,t^{'},\indexi{k+1},\cdots,\indexi{p},\indexJp\backslash\{\alpha^{'}\}}
                {\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}},\order{(\indexJp\backslash\alpha^{'})\cup{t^{'}}}}
            \\
            \coefB{\indexi{k}}{s t^{'}}
            \basexi{\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
            \wedge
            % \basedualxi{\indexJp}??
            \basedualxi{\order{(\indexJp\backslash\alpha^{'})\cup{t^{'}}}}
        \end{pmatrix*}
        &&
        \notag\\
    &   +&&
        \notag\\
    &        %?--4-5
        \displaystyle\sum_{\indexjp{l}\in\indexJp\backslash\{\alpha^{'}\}}
        2
        \begin{pmatrix*}[l]
            \sgn
                {\indexI,\indexJp}
                {\alpha^{'},\indexI,\indexJp\backslash\{\alpha^{'}\}}
            \sgn
                {\indexI,\indexJp\backslash\{\alpha^{'}\}}
                {\indexjp{l},\indexI,\indexJp\backslash\{\alpha^{'},\indexjp{l}\}}
            \sgn
                {\indexjp{1},\cdots,\indexjp{l-1},\order{\indexjp{l},\alpha^{'}},\indexjp{l+1},\cdots,\widehat{\alpha^{'}},\cdots,\indexjp{q}}
                {\indexJp}
            \\
            \coefD{\indexjp{l}}{\order{\indexjp{l} \alpha^{'}}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\indexJp}
        \end{pmatrix*}
        &&
        \notag\\
    &   +&&
        \notag\\
    &        %?--4-6
        \displaystyle\sum_{\indexjp{l}\in\indexJp\backslash\{\alpha^{'}\}}
        \displaystyle\sum_{t^{'}\in\indexJpc}
        2
        \begin{pmatrix*}[l]
            \sgn
                {\indexI,\indexJp}
                {\alpha^{'},\indexI,\indexJp\backslash\{\alpha^{'}\}}
            \sgn
                {\indexI,\indexJp\backslash\{\alpha^{'}\}}
                {\indexjp{l},\indexI,\indexJp\backslash\{\alpha^{'},\indexjp{l}\}}
            \sgn
                {\indexjp{1},\cdots,\indexjp{l-1},\order{\indexjp{l},t^{'}},\indexjp{l+1},\cdots,\widehat{\alpha^{'}},\cdots,\indexjp{q}}
                {\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
            \\
            \coefD{\indexjp{l}}{\order{\indexjp{l} t^{'}}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
        \end{pmatrix*}
        &&
        \notag\\
    &   +&&
        \notag\\
    &       %?--4-7
        \displaystyle\sum_{\indexjp{l}\in\indexJp\backslash\{\alpha^{'}\}}
        \displaystyle\sum_{t^{'}\in\indexJpc}
        2
        \begin{pmatrix*}[l]
            \sgn
                {\indexI,\indexJp}
                {\alpha^{'},\indexI,\indexJp\backslash\{\alpha^{'}\}}
            \sgn
                {\indexI,\indexJp\backslash\{\alpha^{'}\}}
                {\indexjp{l},\indexI,\indexJp\backslash\{\alpha^{'},\indexjp{l}\}}
            \sgn
                {\indexjp{1},\cdots,\indexjp{l-1},\order{\alpha^{'},t^{'}},\indexjp{l+1},\cdots,\widehat{\alpha^{'}},\cdots,\indexjp{q}}
                {\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
            \\
            \coefD{\indexjp{l}}{\order{\alpha^{'} t^{'}}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
        \end{pmatrix*}
        &&
        \notag\\
    &   +&&
        \notag\\
    &        %?--4-8
        \displaystyle\sum_{\indexjp{l}\in\indexJp\backslash\{\alpha^{'}\}}
        \displaystyle\sum_{t^{'}\in\indexJpc}
        \displaystyle\sum_{u^{'}\in\indexJpc}
        2
        \begin{pmatrix*}[l]
            \sgn
                {\indexI,\indexJp}
                {\alpha^{'},\indexI,\indexJp\backslash\{\alpha^{'}\}}
            \sgn
                {\indexI,\indexJp\backslash\{\alpha^{'}\}}
                {\indexjp{l},\indexI,\indexJp\backslash\{\alpha^{'},\indexjp{l}\}}
            \\
            \sgn
                {\indexjp{1},\cdots,\indexjp{l-1},\order{t^{'},u^{'}},\indexjp{l+1},\cdots,\widehat{\alpha^{'}},\cdots,\indexjp{q}}
                {\order{(\indexJp\backslash\{\indexjp{l},\alpha^{'}\})\cup\{t^{'},u^{'}\}}}
            \\
            \frac{1}{2}
            \coefD{\indexjp{l}}{\order{t^{'} u^{'}}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\order{(\indexJp\backslash\{\indexjp{l}, \alpha^{'}\})\cup\{t^{'},u^{'}\}}}
        \end{pmatrix*}.
        &&
    \label{EQ-For (alpha, I, J), calculation for LHS, extra 1-unsimplified result of part 2, alpha in J}
\end{flalign}


We simplify the coefficients in Lemmas \ref{lemma-simplification for LHS, extra 1, part 2-lemma 1}–\ref{lemma-simplification for LHS, extra 1, part 2-lemma 8} in Section $\ref{apex-simplification for LHS, extra 1, part 2}$. The simplified expression of $\LieagbdPartialbar\,\contract{\basedualxi{\alpha}}(\basexi{\indexI}\wedge\basedualxi{\indexJp})$ for $\alpha\in\indexJ$ is:


\begin{flalign}
    &
        %?--4-1
        \displaystyle\sum_{\indexi{k}\in\indexI}
        2
        \begin{pmatrix*}[l]
            (-1)
            \coefB{\indexi{k}}{\indexi{k} \alpha^{'}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\indexJp}
        \end{pmatrix*}
        &&
        \notag\\
    &   +&&
        \notag\\
    &       %?--4-2
        \displaystyle\sum_{\indexi{k}\in\indexI}
        \displaystyle\sum_{t^{'}\in\indexJpc}
        2
        \begin{pmatrix*}[l]
            -(-1)^{k}
            \sgn
                {\indexI}
                {\indexi{k},\indexI\backslash\{\indexi{k}\}}
            \sgn
                {t^{'},\indexI,\indexJp}
                {\alpha,\indexI,\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
            \coefB{\indexi{k}}{\indexi{k} t^{'}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
        \end{pmatrix*}
        &&
        \notag\\
    &   +&&
        \notag\\
    &       %?--4-3
        \displaystyle\sum_{\indexi{k}\in\indexI}
        \displaystyle\sum_{s\in\indexIc}
        2
        \begin{pmatrix*}[l]
            \sgn
                {s,\indexI,\indexJp}
                {\indexi{k},\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}},\indexJp}
            \coefB{\indexi{k}}{s \alpha^{'}}
            \basexi{\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
            \wedge
            \basedualxi{\indexJp}
        \end{pmatrix*}
        &&
        \notag\\
    &   +&&
        \notag\\
    &   %?--4-4
        \displaystyle\sum_{\indexi{k}\in\indexI}
        \displaystyle\sum_{s\in\indexIc}
        \displaystyle\sum_{t^{'}\in\indexJpc}
        2
        \begin{pmatrix*}[l]
            (-1)
            \sgn
                {s,t^{'},\indexI,\indexJp}
                {\indexi{k},\alpha^{'},\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}},\order{(\indexJp\backslash\alpha^{'})\cup{t^{'}}}}
            \\
            \coefB{\indexi{k}}{s t^{'}}
            \basexi{\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
            \wedge
            % \basedualxi{\indexJp}??
            \basedualxi{\order{(\indexJp\backslash\alpha^{'})\cup{t^{'}}}}
        \end{pmatrix*}
        &&
        \notag\\
    &   +&&
        \notag\\
    &        %?--4-5
        \displaystyle\sum_{\indexjp{l}\in\indexJp\backslash\{\alpha^{'}\}}
        2
        \begin{pmatrix*}[l]
            \sgn
                {\order{\indexjp{l},\alpha^{'}}}
                {\alpha^{'},\indexjp{l}}
            \coefD{\indexjp{l}}{\order{\indexjp{l} \alpha^{'}}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\indexJp}
        \end{pmatrix*}
        &&
        \notag\\
    &   +&&
        \notag\\
    &        %?--4-6
        \displaystyle\sum_{\indexjp{l}\in\indexJp\backslash\{\alpha^{'}\}}
        \displaystyle\sum_{t^{'}\in\indexJpc}
        2
        \begin{pmatrix*}[l]
            (-1)
            \sgn
                {\order{\indexjp{l},t^{'}}}
                {t^{'},\indexjp{l}}
            \sgn
                {t^{'},\indexI,\indexJp}
                {\alpha^{'},\indexI,\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
            \\
            \coefD{\indexjp{l}}{\order{\indexjp{l} t^{'}}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
        \end{pmatrix*}
        &&
        \notag\\
    &   +&&
        \notag\\
    &       %?--4-7
        \displaystyle\sum_{\indexjp{l}\in\indexJp\backslash\{\alpha^{'}\}}
        \displaystyle\sum_{t^{'}\in\indexJpc}
        2
        \begin{pmatrix*}[l]
            \sgn
                {\order{\alpha^{'},t^{'}}}
                {t^{'},\alpha^{'}}
            \sgn
                {t^{'},\indexI,\indexJp}
                {\indexjp{l},\indexI,\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
            \\
            \coefD{\indexjp{l}}{\order{\alpha^{'} t^{'}}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
        \end{pmatrix*}
        &&
        \notag\\
    &   +&&
        \notag\\
    &        %?--4-8
        \displaystyle\sum_{\indexjp{l}\in\indexJp\backslash\{\alpha^{'}\}}
        \displaystyle\sum_{t^{'}\in\indexJpc}
        \displaystyle\sum_{u^{'}\in\indexJpc}
        2
        \begin{pmatrix*}[l]
            (-1)
            \sgn
                {\order{t^{'},u^{'}},\indexI,\indexJp}
                {\indexjp{l},\alpha^{'},\indexI,\order{(\indexJp\backslash\{\indexjp{l},\alpha^{'}\})\cup\{t^{'},u^{'}\}}}
            \\
            \frac{1}{2}
            \coefD{\indexjp{l}}{\order{t^{'} u^{'}}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\order{(\indexJp\backslash\{\indexjp{l}, \alpha^{'}\})\cup\{t^{'},u^{'}\}}}
        \end{pmatrix*}.
        &&
    \label{EQ-For (alpha, I, J), calculation for LHS, extra 1-simplified result of part 2, alpha in J}
\end{flalign}
%%%%%%%%%%%% finish calculate partial \, \iota  (I,J) %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% start combine  \iota \, partial + parital \, \iota  (I,J) %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\keyword{Step 3:} We combine the computations of $
\LieagbdPartialbar\,\contract{\basedualxi{\alpha^{'}}}
(\basexi{\indexI}\wedge\basedualxi{\indexJp})
$ and $
\contract{\basedualxi{\alpha^{'}}}\,\LieagbdPartialbar
(\basexi{\indexI}\wedge\basedualxi{\indexJp})
$. The first step is to consider the case that $\alpha\in\indexJ$. The expression of $
(
\LieagbdPartialbar\,\contract{\basedualxi{\alpha^{'}}}
+
\contract{\basedualxi{\alpha^{'}}}\,\LieagbdPartialbar
)
(\basexi{\indexI}\wedge\basedualxi{\indexJp})
$ is equal to (\ref{EQ-For (alpha, I, J), calculation for LHS, extra 1-simplified result of part 1, alpha in J}) + (\ref{EQ-For (alpha, I, J), calculation for LHS, extra 1-simplified result of part 2, alpha in J}):

\begin{align*}
    %%%%froam part 1
    &2
    \begin{pmatrix*}[l]
        %part 1--1
        \displaystyle\sum_{\indexi{k}\in\indexI}
        \displaystyle\sum_{t^{'}\in\indexJpc}
        \begin{pmatrix*}[l]
            (-1)^{k}
            \sgn
                {\indexI}
                {\indexi{k},\indexI\backslash\{\indexi{k}\}}
            \sgn
                {t^{'},\indexI,\indexJp}
                {\alpha,\indexI,\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
            \\
            \coefB{\indexi{k}}{\indexi{k} t^{'}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
        \end{pmatrix*}
        \\
        +
        \\
        %part 1--2
        \displaystyle\sum_{\indexi{k}\in\indexI}
        \displaystyle\sum_{s\in\indexIc}
        \displaystyle\sum_{t^{'}\in\indexJpc}
        \begin{pmatrix*}[l]
            \sgn
                {s,t^{'},\indexI,\indexJp}
                {\indexi{k},\alpha^{'},\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}},\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
            \\
            \coefB{\indexi{k}}{s t^{'}}
            \basexi{\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
            \wedge
            \basedualxi{\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
        \end{pmatrix*}
        \\
        +
        \\
        %part 1--3
        \displaystyle\sum_{\indexjp{l}\in\indexJp}
        \displaystyle\sum_{t^{'}\in\indexJpc}
        \begin{pmatrix*}[l]
            \sgn
                {\order{\indexjp{l},t^{'}}}
                {t^{'},\indexjp{l}}
            \sgn
                {t^{'},\indexI,\indexJp}
                {\alpha^{'},\indexI,\order{(\indexJp\backslash\{\alpha^{'}\})\cup\    {t^{'}\}}}}
            \\
            \coefD{\indexjp{l}}{\order{\indexjp{l},t^{'}}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
        \end{pmatrix*}
        \\
        +
        \\
        %part 1--4
        \displaystyle\sum_{\indexjp{l}\in\indexJp\backslash\{\alpha^{'}\}}
        \displaystyle\sum_{t^{'}\in\indexJpc}
        \displaystyle\sum_{u^{'}\in\indexJpc}
        \begin{pmatrix*}[l]
            \sgn
                {\order{t^{'},u^{'}},\indexI,\indexJp}
                {\indexjp{l},\alpha^{'},\indexI,\order{(\indexJp\backslash\{\indexjp{l},\alpha^{'}\})\cup\{t^{'},u^{'}\}}}
            \\
            \frac{1}{2}
            \coefD{\indexjp{l}}{\order{t^{'},u^{'}}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\order{(\indexJp\backslash\{\indexjp{l},\alpha^{'}\})\cup\{t^{'},u^{'}\}}}
        \end{pmatrix*}
    \end{pmatrix*}
    \\
    +&%%%%part 2 start
    \\
        &
        %part 2-1
        \displaystyle\sum_{\indexi{k}\in\indexI}
        2
        \begin{pmatrix*}[l]
            (-1)
            \coefB{\indexi{k}}{\indexi{k} \alpha^{'}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\indexJp}
        \end{pmatrix*}
    \\
    +&
    \\
    &   %part 2-2
        \displaystyle\sum_{\indexi{k}\in\indexI}
        \displaystyle\sum_{t^{'}\in\indexJpc}
        2
        \begin{pmatrix*}[l]
            -(-1)^{k}
            \sgn
                {\indexI}
                {\indexi{k},\indexI\backslash\{\indexi{k}\}}
            \sgn
                {t^{'},\indexI,\indexJp}
                {\alpha,\indexI,\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
            \coefB{\indexi{k}}{\indexi{k} t^{'}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
        \end{pmatrix*}
    \\
    +&
    \\
    &   %part 2-3
        \displaystyle\sum_{\indexi{k}\in\indexI}
        \displaystyle\sum_{s\in\indexIc}
        2
        \begin{pmatrix*}[l]
            \sgn
                {s,\indexI,\indexJp}
                {\indexi{k},\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}},\indexJp}
            \coefB{\indexi{k}}{s \alpha^{'}}
            \basexi{\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
            \wedge
            \basedualxi{\indexJp}
        \end{pmatrix*}
    \\
    +&
    \\
    &   %part 2-4
        \displaystyle\sum_{\indexi{k}\in\indexI}
        \displaystyle\sum_{s\in\indexIc}
        \displaystyle\sum_{t^{'}\in\indexJpc}
        2
        \begin{pmatrix*}[l]
            (-1)
            \sgn
                {s,t^{'},\indexI,\indexJp}
                {\indexi{k},\alpha^{'},\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}},\order{(\indexJp\backslash\alpha^{'})\cup{t^{'}}}}
            \\
            \coefB{\indexi{k}}{s t^{'}}
            \basexi{\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
            \wedge
            \basedualxi{\order{(\indexJp\backslash\alpha^{'})\cup{t^{'}}}}
        \end{pmatrix*}
    \\
    +&
    \\
    &   %part 2-5
        \displaystyle\sum_{\indexjp{l}\in\indexJp\backslash\{\alpha^{'}\}}
        2
        \begin{pmatrix*}[l]
            \sgn
                {\order{\indexjp{l},\alpha^{'}}}
                {\alpha^{'},\indexjp{l}}
            \coefD{\indexjp{l}}{\order{\indexjp{l} \alpha^{'}}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\indexJp}
        \end{pmatrix*}
    \\
    +&
    \\
    &   %part 2-6
        \displaystyle\sum_{\indexjp{l}\in\indexJp\backslash\{\alpha^{'}\}}
        \displaystyle\sum_{t^{'}\in\indexJpc}
        2
        \begin{pmatrix*}[l]
            (-1)
            \sgn
                {\order{\indexjp{l},t^{'}}}
                {t^{'},\indexjp{l}}
            \sgn
                {t^{'},\indexI,\indexJp}
                {\alpha^{'},\indexI,\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
            \\
            \coefD{\indexjp{l}}{\order{\indexjp{l} t^{'}}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
        \end{pmatrix*}
    \\
    +&
    \\
    &   %part 2-7
        \displaystyle\sum_{\indexjp{l}\in\indexJp\backslash\{\alpha^{'}\}}
        \displaystyle\sum_{t^{'}\in\indexJpc}
        2
        \begin{pmatrix*}[l]
            \sgn
                {\order{\alpha^{'},t^{'}}}
                {t^{'},\alpha^{'}}
            \sgn
                {t^{'},\indexI,\indexJp}
                {\indexjp{l},\indexI,\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
            \\
            \coefD{\indexjp{l}}{\order{\alpha^{'} t^{'}}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
        \end{pmatrix*}
    \\
    +&
    \\
    &   %part 2-8
        \displaystyle\sum_{\indexjp{l}\in\indexJp\backslash\{\alpha^{'}\}}
        \displaystyle\sum_{t^{'}\in\indexJpc}
        \displaystyle\sum_{u^{'}\in\indexJpc}
        2
        \begin{pmatrix*}[l]
            (-1)
            \sgn
                {\order{t^{'},u^{'}},\indexI,\indexJp}
                {\indexjp{l},\alpha^{'},\indexI,\order{(\indexJp\backslash\{\indexjp{l},\alpha^{'}\})\cup\{t^{'},u^{'}\}}}
            \\
            \frac{1}{2}
            \coefD{\indexjp{l}}{\order{t^{'} u^{'}}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\order{(\indexJp\backslash\{\indexjp{l}, \alpha^{'}\})\cup\{t^{'},u^{'}\}}}
        \end{pmatrix*}
    .
\end{align*}
We merge the terms that have the same wedge product of frames and simplify the expression of $
(
\LieagbdPartialbar\,\contract{\basedualxi{\alpha^{'}}}
+
\contract{\basedualxi{\alpha^{'}}}\,\LieagbdPartialbar
)
(\basexi{\indexI}\wedge\basedualxi{\indexJp})
$ for $\alpha\in\indexJ$ to the following one:
\begin{align}
    %%%%     1,3,5,7,
    &
        2
        \begin{pmatrix*}[l]% part 1-1 + part 2-2
            \displaystyle\sum_{\indexi{k}\in\indexI}
            \displaystyle\sum_{t^{'}\in\indexJpc}
            \begin{pmatrix*}[l]
                (-1)^{k}
                \sgn
                    {\indexI}
                    {\indexi{k},\indexI\backslash\{\indexi{k}\}}
                \sgn
                    {t^{'},\indexI,\indexJp}
                    {\alpha,\indexI,\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
                \\
                \coefB{\indexi{k}}{\indexi{k} t^{'}}
                \basexi{\indexI}
                \wedge
                \basedualxi{\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
            \end{pmatrix*}
        \\
        +
        \\
            \displaystyle\sum_{\indexi{k}\in\indexI}
            \displaystyle\sum_{t^{'}\in\indexJpc}
            \begin{pmatrix*}[l]
                -1(-1)^{k}
                \sgn
                    {\indexI}
                    {\indexi{k},\indexI\backslash\{\indexi{k}\}}
                \sgn
                    {t^{'},\indexI,\indexJp}
                    {\alpha,\indexI,\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
                \\
                \coefB{\indexi{k}}{\indexi{k} t^{'}}
                \basexi{\indexI}
                \wedge
                \basedualxi{\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
            \end{pmatrix*}
        \end{pmatrix*}
\label{EQ-For (alpha, I, J), calculation for LHS-together-block 1}
    \\
    +&\notag
    \\
    &
        2
        \begin{pmatrix*}[l]%%%part 1-2 + part 2-4
            \displaystyle\sum_{\indexi{k}\in\indexI}
            \displaystyle\sum_{s\in\indexIc}
            \displaystyle\sum_{t^{'}\in\indexJpc}
            \begin{pmatrix*}[l]
                \sgn
                    {s,t^{'},\indexI,\indexJp}
                    {\indexi{k},\alpha^{'},\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}},\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
                \\
                \coefB{\indexi{k}}{s t^{'}}
                \basexi{\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
                \wedge
                \basedualxi{\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
            \end{pmatrix*}
        \\
        +
        \\
            \displaystyle\sum_{\indexi{k}\in\indexI}
            \displaystyle\sum_{s\in\indexIc}
            \displaystyle\sum_{t^{'}\in\indexJpc}
            \begin{pmatrix*}[l]
                (-1)
                \sgn
                    {s,t^{'},\indexI,\indexJp}
                    {\indexi{k},\alpha^{'},\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}},\order{(\indexJp\backslash\alpha^{'})\cup{t^{'}}}}
                \\
                \coefB{\indexi{k}}{s t^{'}}
                \basexi{\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
                \wedge
                \basedualxi{\order{(\indexJp\backslash\alpha^{'})\cup{t^{'}}}}
            \end{pmatrix*}
        \end{pmatrix*}
\label{EQ-For (alpha, I, J), calculation for LHS-together-block 2}
    \\
    +&\notag
    \\
    &
        2
        \begin{pmatrix*}[l] %part 1-3   part 2-6
            \displaystyle\sum_{\indexjp{l}\in\indexJp}
            \displaystyle\sum_{t^{'}\in\indexJpc}
            \begin{pmatrix*}[l]
                \sgn
                    {\order{\indexjp{l},t^{'}}}
                    {t^{'},\indexjp{l}}
                \sgn
                    {t^{'},\indexI,\indexJp}
                    {\alpha^{'},\indexI,\order{(\indexJp\backslash\{\alpha^{'}\})\cup\    {t^{'}\}}}}
                \\
                \coefD{\indexjp{l}}{\order{\indexjp{l},t^{'}}}
                \basexi{\indexI}
                \wedge
                \basedualxi{\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
            \end{pmatrix*}
        \\
        +
        \\
            \displaystyle\sum_{\indexjp{l}\in\indexJp\backslash\{\alpha^{'}\}}
            \displaystyle\sum_{t^{'}\in\indexJpc}
            \begin{pmatrix*}[l]
                (-1)
                \sgn
                    {\order{\indexjp{l},t^{'}}}
                    {t^{'},\indexjp{l}}
                \sgn
                    {t^{'},\indexI,\indexJp}
                    {\alpha^{'},\indexI,\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
                \\
                \coefD{\indexjp{l}}{\order{\indexjp{l} t^{'}}}
                \basexi{\indexI}
                \wedge
                \basedualxi{\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
            \end{pmatrix*}
        \end{pmatrix*}
\label{EQ-For (alpha, I, J), calculation for LHS-together-block 3}
    \\
    +&\notag
    \\
    &
        2
        \begin{pmatrix*}[l] %%%% part 1-4+part 2-8
            \displaystyle\sum_{\indexjp{l}\in\indexJp\backslash\{\alpha^{'}\}}
            \displaystyle\sum_{t^{'}\in\indexJpc}
            \displaystyle\sum_{u^{'}\in\indexJpc}
            \begin{pmatrix*}[l]
                \sgn
                    {\order{t^{'},u^{'}},\indexI,\indexJp}
                    {\indexjp{l},\alpha^{'},\indexI,\order{(\indexJp\backslash\{\indexjp{l},\alpha^{'}\})\cup\{t^{'},u^{'}\}}}
                \\
                \frac{1}{2}
                \coefD{\indexjp{l}}{\order{t^{'},u^{'}}}
                \basexi{\indexI}
                \wedge
                \basedualxi{\order{(\indexJp\backslash\{\indexjp{l},\alpha^{'}\})\cup\{t^{'},u^{'}\}}}
            \end{pmatrix*}
        \\
        +
        \\
            \displaystyle\sum_{\indexjp{l}\in\indexJp\backslash\{\alpha^{'}\}}
            \displaystyle\sum_{t^{'}\in\indexJpc}
            \displaystyle\sum_{u^{'}\in\indexJpc}
            \begin{pmatrix*}[l]
                (-1)
                \sgn
                    {\order{t^{'},u^{'}},\indexI,\indexJp}
                    {\indexjp{l},\alpha^{'},\indexI,\order{(\indexJp\backslash\{\indexjp{l},\alpha^{'}\})\cup\{t^{'},u^{'}\}}}
                \\
                \frac{1}{2}
                \coefD{\indexjp{l}}{\order{t^{'} u^{'}}}
                \basexi{\indexI}
                \wedge
                \basedualxi{\order{(\indexJp\backslash\{\indexjp{l}, \alpha^{'}\})\cup\{t^{'},u^{'}\}}}
            \end{pmatrix*}
        \end{pmatrix*}
\label{EQ-For (alpha, I, J), calculation for LHS-together-block 4}
    \\
    +&\notag
    \\
    &
        2
        \begin{pmatrix*}[l]%%%% part2-1 + part2-4 + part2-5 + part2-7
            \displaystyle\sum_{\indexi{k}\in\indexI}
            \begin{pmatrix*}[l]
                (-1)
                \coefB{\indexi{k}}{\indexi{k} \alpha^{'}}
                \basexi{\indexI}
                \wedge
                \basedualxi{\indexJp}
            \end{pmatrix*}
        \\
        +
        \\
            \displaystyle\sum_{\indexi{k}\in\indexI}
            \displaystyle\sum_{s\in\indexIc}
            \begin{pmatrix*}[l]
                \sgn
                    {s,\indexI}
                    {\indexi{k},\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
                \coefB{\indexi{k}}{s \alpha^{'}}
                \basexi{\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
                \wedge
                \basedualxi{\indexJp}
            \end{pmatrix*}
        \\
        +
        \\
            \displaystyle\sum_{\indexjp{l}\in\indexJp\backslash\{\alpha^{'}\}}
            \begin{pmatrix*}[l]
                \sgn
                    {\order{\indexjp{l},\alpha^{'}}}
                    {\alpha^{'},\indexjp{l}}
                \coefD{\indexjp{l}}{\order{\indexjp{l} \alpha^{'}}}
                \basexi{\indexI}
                \wedge
                \basedualxi{\indexJp}
            \end{pmatrix*}
        \\
        +
        \\
            \displaystyle\sum_{\indexjp{l}\in\indexJp\backslash\{\alpha^{'}\}}
            \displaystyle\sum_{t^{'}\in\indexJpc}
            \begin{pmatrix*}[l]
                \sgn
                    {\order{\alpha^{'},t^{'}}}
                    {t^{'},\alpha^{'}}
                \sgn
                    {t^{'},\indexI,\indexJp}
                    {\indexjp{l},\indexI,\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
                \\
                \coefD{\indexjp{l}}{\order{\alpha^{'} t^{'}}}
                \basexi{\indexI}
                \wedge
                \basedualxi{\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
            \end{pmatrix*}
        \end{pmatrix*}
\label{EQ-For (alpha, I, J), calculation for LHS-together-block 5}
    .
\end{align}
We can easily check that:
\begin{itemize}
    \item (\ref{EQ-For (alpha, I, J), calculation for LHS-together-block 1}) is equal to 0.
    \item (\ref{EQ-For (alpha, I, J), calculation for LHS-together-block 2}) is equal to 0.
    \item (\ref{EQ-For (alpha, I, J), calculation for LHS-together-block 3}) is equal to
\begin{align}
        2
        \displaystyle\sum_{t^{'}\in\indexJpc}
        \begin{pmatrix*}[l]
            \sgn
                {\order{\alpha^{'},t^{'}}}
                {t^{'},\alpha^{'}}
            \sgn
                {t^{'},\indexI,\indexJp}
                {\alpha^{'},\indexI,\order{(\indexJp\backslash\{\alpha^{'}\})\cup\    {t^{'}\}}}}
            \\
            \coefD{\alpha^{'}}{\order{\alpha^{'},t^{'}}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\order{(\indexJp\backslash\{\alpha^{'}\})\cup\{t^{'}\}}}
        \end{pmatrix*}
    ,
\label{EQ-For (alpha, I, J), calculation for LHS-together-simplified block 3}
\end{align}
    since it can be viewed as 
\begin{align*}
        2
        \displaystyle\sum_{\indexjp{l}=\alpha^{'}}
        \displaystyle\sum_{t^{'}\in\indexJpc}
        \begin{pmatrix*}[l]
            \sgn
                {\order{\alpha^{'},t^{'}}}
                {t^{'},\alpha^{'}}
            \sgn
                {t^{'},\indexI,\indexJp}
                {\indexjp{l},\indexI,\order{(\indexJp\backslash\{\indexjp{l}\})\cup\    {t^{'}\}}}}
            \\
            \coefD{\alpha^{'}}{\order{\alpha^{'},t^{'}}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
        \end{pmatrix*}
    .
\end{align*}
    \item (\ref{EQ-For (alpha, I, J), calculation for LHS-together-block 4}) is equal to 0.
\end{itemize}
Thus, (\ref{EQ-For (alpha, I, J), calculation for LHS-together-simplified block 3}) + (\ref{EQ-For (alpha, I, J), calculation for LHS-together-block 5}) is the simplified expression of $
(
\LieagbdPartialbar\,\contract{\basedualxi{\alpha^{'}}}
+
\contract{\basedualxi{\alpha^{'}}}\,\LieagbdPartialbar
)
(\basexi{\indexI}\wedge\basedualxi{\indexJp})
$ for $\alpha\in\indexJ$. Multiplying this by $-\sqrt{-1}$, we conclude that the expression of $
-\sqrt{-1}
(
\LieagbdPartialbar\,\contract{\basedualxi{\alpha^{'}}}
+
\contract{\basedualxi{\alpha^{'}}}\,\LieagbdPartialbar
)
(\basexi{\indexI}\wedge\basedualxi{\indexJp})
$ for $\alpha\in\indexJ$ is equal to
\begin{align}
    -2\sqrt{-1}
    \begin{pmatrix*}[l]
        \displaystyle\sum_{\indexi{k}\in\indexI}
        \begin{pmatrix*}[l]
            (-1)
            \coefB{\indexi{k}}{\indexi{k} \alpha^{'}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\indexJp}
        \end{pmatrix*}
    \\
    +
    \\
        \displaystyle\sum_{\indexi{k}\in\indexI}
        \displaystyle\sum_{s\in\indexIc}
        \begin{pmatrix*}[l]
            \sgn
                {s,\indexI,}
                {\indexi{k},\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}},}
            \coefB{\indexi{k}}{s \alpha^{'}}
            \basexi{\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
            \wedge
            \basedualxi{\indexJp}
        \end{pmatrix*}
    \\
    +
    \\
        \displaystyle\sum_{\indexj{l}\in\indexJp\backslash\{\alpha^{'}\}}
        \begin{pmatrix*}[l]
            \sgn
                {\order{\indexjp{l},\alpha^{'}}}
                {\alpha^{'},\indexjp{l}}
            \coefD{\indexjp{l}}{\order{\indexjp{l} \alpha^{'}}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\indexJp}
        \end{pmatrix*}
    \\
    +
    \\
        \displaystyle\sum_{\indexj{l}\in\indexJp}
        \displaystyle\sum_{t^{'}\in\indexJpc}
        \begin{pmatrix*}[l]
            \sgn
                {\order{\alpha^{'},t^{'}}}
                {t^{'},\alpha^{'}}
            \sgn
                {t^{'},\indexI,\indexJp}
                {\indexjp{l},\indexI,\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
            \\
            \coefD{\indexjp{l}}{\order{\alpha^{'} t^{'}}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
        \end{pmatrix*}
    \end{pmatrix*}
    .
\label{EQ-For (alpha, I, J), calculation for LHS, extra 1-result, alpha in J}
\end{align}



Next, we look at the case that $\alpha\notin\indexJ$. We observe that $
-\sqrt{-1}(
\LieagbdPartialbar\,\contract{\basedualxi{\alpha^{'}}}
+
\contract{\basedualxi{\alpha^{'}}}\,\LieagbdPartialbar
)
(\basexi{\indexI}\wedge\basedualxi{\indexJp})
$ is equal to 0 + (\ref{EQ-For (alpha, I, J), calculation for LHS, extra 1-simplified the first half, alpha not in J}) multiplied by $-\sqrt{-1}$, which is computed as follows:
\begin{align}
    -2\sqrt{-1}
    \begin{pmatrix*}[l]
        %?--1
        \displaystyle\sum_{\indexi{k}\in\indexI}
            (-1)
            \coefB{\indexi{k}}{\indexi{k} \alpha^{'}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\indexJp}
        \\
        +
        \\
        %?--2
        \displaystyle\sum_{\indexi{k}\in\indexI}
        \displaystyle\sum_{s\in\indexIc}
            \sgn
                {s,\indexI}
                {\indexi{k},\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
            \coefB{\indexi{k}}{s \alpha^{'}}
            \basexi{\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
            \wedge
            \basedualxi{\indexJp}
        \\
        +
        \\
        %?--3
        \displaystyle\sum_{\indexjp{l}\in\indexJp}
            \sgn
                {\order{\indexjp{l},\alpha^{'}}}
                {\alpha^{'},\indexjp{l}}
            \coefD{\indexjp{l}}{\order{\indexjp{l},\alpha^{'}}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\indexJp}
        \\
        +
        \\
        %?--4
        \displaystyle\sum_{\indexjp{l}\in\indexJp}
        \displaystyle\sum_{t^{'}\in\indexJpc}
        \begin{pmatrix*}
            \sgn
                {\order{\alpha^{'},t^{'}}}
                {t^{'},\alpha^{'}}
            \sgn
                {t^{'},\indexI,\indexJp}
                {\indexjp{l},\indexI,\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
            \\
            \coefD{\indexjp{l}}{\order{t^{'},\alpha^{'}}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
        \end{pmatrix*}
    \end{pmatrix*}
    ,
\label{EQ-For (alpha, I, J), calculation for LHS, extra 1-result, alpha not in J}
\end{align}
since $\LieagbdPartialbar\,\contract{\basedualxi{\alpha^{'}}}=0$ when $\alpha\notin\indexJ$. 


%%%%%%%%%%%% finish combine  \iota \, partial + parital \, \iota  (I,J) %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


We see that (\ref{EQ-For (alpha, I, J), calculation for LHS, extra 1-result, alpha in J}) and (\ref{EQ-For (alpha, I, J), calculation for LHS, extra 1-result, alpha not in J}) are same, which implies that the expression of $
(-\sqrt{-1})(\LieagbdPartialbar\,\contract{\basedualxi{\alpha^{'}}}
+
\contract{\basedualxi{\alpha^{'}}}\,\LieagbdPartialbar)
(\basexi{\indexI}\wedge\basedualxi{\indexJp})
$ does not depend on $\alpha\in\indexJ$ or $\alpha\notin\indexJ$.

\end{proof}

==> 4/For__alpha,_I,_J_,_calculation_for_LHS,_extra_2.tex <==
\begin{lemma}
\label{lemma-For (alpha, I, J), calculation for LHS-extra 2]}
\begin{align}
&
    (-\frac{\sqrt{-1}}{2})
    \displaystyle\sum_{h=1}^{n}
    \big(
        (\iota_{\basexi{h}} \, \LieagbdPartialbar \basexi{\alpha})
        \wedge
        \iota_{\basedualxi{h^{'}}}(\basexi{\indexI}\wedge\basedualxi{\indexJp})
        -
        (\iota_{\basedualxi{h^{'}}} \, \LieagbdPartialbar \basexi{\alpha})
        \wedge
        \iota_{\basexi{h}}
        (\basexi{\indexI}\wedge\basedualxi{\indexJp})
    \big)
\notag    
\\
=&
    -2\sqrt{-1}
    \begin{pmatrix*}[l]
        \displaystyle\sum_{\indexjp{l}\in\indexJp}
        \begin{matrix*}[l]
            \coefB{\alpha}{\indexj{l} \indexjp{l}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\indexJp}
        \end{matrix*}
        \\
        +
        \\
        \displaystyle\sum_{\indexjp{l}\in\indexJp}
        \displaystyle\sum_{t^{'}\in\indexJpc}
        \begin{matrix*}[l]
            (-1)
            \sgn
                {t^{'},\indexI,\indexJp}
                {\indexjp{l},\indexI,\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
            \coefB{\alpha}{\indexj{l} t^{'}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
        \end{matrix*}
        \\
        +
        \\
        \displaystyle\sum_{\indexi{k}\in\indexI}
        \begin{matrix*}[l]
            \coefB{\alpha}{\indexi{k} \indexip{k}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\indexJp}
        \end{matrix*}
        \\
        +
        \\
        \displaystyle\sum_{\indexi{k}\in\indexI}
        \displaystyle\sum_{s\in\indexIc}
        \begin{matrix*}[l]
            (-1)
            \sgn
                {s,\indexI}
                {\indexi{k},\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
            \coefB{\alpha}{s \indexip{k}}
            \basexi{\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
            \wedge
            \basedualxi{\indexJp}
        \end{matrix*}
    \end{pmatrix*}
    .
\label{EQ-For (alpha, I, J), calculation for LHS, extra 2-result}
\end{align}
\end{lemma}




\begin{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%% start the first part %%%%%%%%%%%%%%%%%
Let us calculate the first half,
\begin{align}
    (-\frac{\sqrt{-1}}{2})
    \displaystyle\sum_{h=1}^{n}
    (\iota_{\basexi{h}}\,\LieagbdPartialbar\basexi{\alpha})
    \wedge
    \iota_{\basedualxi{h^{'}}}(\basexi{\indexI}\wedge\basedualxi{\indexJp})
    .
\label{EQ-For (alpha, I, J), calculation for LHS, extra 2-first part, target}
\end{align}
With the contraction computation
\begin{align*}
    \iota_{\basedualxi{h}}(\basexi{\indexI}\wedge\basedualxi{\indexJp})
    =
    \begin{cases}
        0       & \,h\notin\indexJ \\
        2
        \sgn
            {\indexI,\indexJp}
            {h^{'},\indexI,\indexJp\backslash\{h^{'}\}}
        \basexi{\indexI}
        \wedge
        \basedualxi{\indexJp\backslash\{h^{'}\}}
                & \,h\in\indexJ
    \end{cases},
\end{align*}
we use $\indexj{l}$ to replace $h$ and simplify (\ref{EQ-For (alpha, I, J), calculation for LHS, extra 2-first part, target}) to
\begin{align}
    (-\frac{\sqrt{-1}}{2})
    \displaystyle\sum_{\indexj{l}\in\indexJ}
    (\iota_{\basexi{\indexj{l}}}\,\LieagbdPartialbar\basexi{\alpha})
    \wedge
    \bigg(
    2\,
        \sgn
            {\indexI,\indexJp}
            {\indexjp{l},\indexI,\indexJp\backslash\{\indexjp{l}\}}
        \basexi{\indexI}
        \wedge
        \basedualxi{\indexJp\backslash\{\indexjp{l}\}}
    \bigg).
\label{EQ-For (alpha, I, J), calculation for LHS, extra 2-first part, no 1}
\end{align}

Recall that $
\LieagbdPartialbar \basexi{\alpha}
=
\displaystyle\sum_{s,t}
\coefB{\alpha}{s t^{'}}
\basexi{s}\wedge\basedualxi{t^{'}}
$. We plug this into (\ref{EQ-For (alpha, I, J), calculation for LHS, extra 2-first part, no 1}) and cancel out the terms containing repeated wedge product of frames, obtaining
\begin{align}
    (-\frac{\sqrt{-1}}{2})
    \displaystyle\sum_{\indexjp{l}\in\indexJp}
    (
    \iota_{\basexi{\indexj{l}}}
    \begin{pmatrix*}[l]
        \coefB{\alpha}{\indexj{l} \indexjp{l}}
        \basexi{\indexj{l}}
        \wedge
        \basedualxi{\indexjp{l}}
        \\
        +
        \\
        \displaystyle\sum_{t^{'}\in\indexJpc}
        \coefB{\alpha}{\indexj{l} t^{'}}
        \basexi{\indexj{l}}
        \wedge
        \basedualxi{t^{'}}
    \end{pmatrix*}
    )
    \wedge
    \bigg(
    2
        \sgn
            {\indexI,\indexJp}
            {\indexjp{l},\indexI,\indexJp\backslash\{\indexjp{l}\}}
        \basexi{\indexI}
        \wedge
        \basedualxi{\indexJp\backslash\{\indexjp{l}\}}
    \bigg)
    .
\label{EQ-For (alpha, I, J), calculation for LHS, extra 2-first part, no 2}
\end{align}
The contractions in the first parenthesis are computed as follows:
\begin{align*}
    \iota_{\basexi{\indexj{l}}}
    (\basexi{\indexj{l}}\wedge\basedualxi{\indexjp{l}})
    =
    2\basedualxi{\indexjp{l}}
    \qquad \text{and} \qquad 
    \iota_{\basexi{\indexj{l}}}
    (\basexi{\indexj{l}}\wedge\basedualxi{t^{'}})
    =
    2\basedualxi{t^{'}}
    .
\end{align*}
Thus, we simplify (\ref{EQ-For (alpha, I, J), calculation for LHS, extra 2-first part, no 2}) to
\begin{align}
    (-\frac{\sqrt{-1}}{2})
    \displaystyle\sum_{\indexjp{l}\in\indexJp}
    2
    \begin{pmatrix*}[l]
        \coefB{\alpha}{\indexj{l} \indexjp{l}}
        \basedualxi{\indexjp{l}}
        \\
        +
        \\
        \displaystyle\sum_{t^{'}\in\indexJpc}
        \coefB{\alpha}{\indexj{l} t^{'}}
        \basedualxi{t^{'}}
    \end{pmatrix*}
    \wedge
    \big(
        2
        \sgn
            {\indexI,\indexJp}
            {\indexjp{l},\indexI,\indexJp\backslash\{\indexjp{l}\}}
        \basexi{\indexI}
        \wedge
        \basedualxi{\indexJp\backslash\{\indexjp{l}\}}
    \big)
    .
\label{EQ-For (alpha, I, J), calculation for LHS, extra 2-first part, no 3}
\end{align}
We observe that
\begin{itemize}
    \item 
$
    \basedualxi{\indexjp{l}}
    \wedge
    \basexi{\indexI}\wedge\basedualxi{\indexJp\backslash\{\indexjp{l}\}}
    =
    \sgn
        {\indexjp{l},\indexI,\indexJp\backslash\{\indexjp{l}\}}
        {\indexI,\indexJp}
    \basexi{\indexI}\wedge\basedualxi{\indexJp}    
$,
    \item 
$
    \basedualxi{t^{'}}
    \wedge
    \basexi{\indexI}\wedge\basedualxi{\indexJp\backslash\{\indexjp{l}\}}
    =
    \sgn
        {t^{'},\indexI,\indexJp\backslash\{\indexjp{l}\}}
        {\indexI,\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
    \basexi{\indexI}
    \wedge
    \basedualxi{\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
$.
\end{itemize}
After ordering the wedge product of frames, we can simplify (\ref{EQ-For (alpha, I, J), calculation for LHS, extra 2-first part, no 3}) to
\begin{align}
    -2\sqrt{-1}
    \begin{pmatrix*}[l]
        \displaystyle\sum_{\indexjp{l}\in\indexJp}
        \sgn
            {\indexjp{l},\indexI,\indexJp\backslash\{\indexjp{l}\}}
            {\indexI,\indexJp}
        \sgn
            {\indexI,\indexJp}
            {\indexjp{l},\indexI,\indexJp\backslash\{\indexjp{l}\}}
        \coefB{\alpha}{\indexj{l} \indexjp{l}}
        \basexi{\indexI}
        \wedge
        \basedualxi{\indexJp}
        \\
        +
        \\
        \displaystyle\sum_{\indexjp{l}\in\indexJp}
        \displaystyle\sum_{t^{'}\in\indexJpc}
        \begin{matrix*}[l]
            \sgn
                {\indexI,\indexJp}
                {\indexjp{l},\indexI,\indexJp\backslash\{\indexjp{l}\}}
            \sgn
                {t^{'},\indexI,\indexJp\backslash\{\indexjp{l}\}}
                {\indexI,\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
            \\
            \coefB{\alpha}{\indexj{l} t^{'}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
        \end{matrix*}
    \end{pmatrix*}.
\label{EQ-For (alpha, I, J), calculation for LHS, extra 2-first part, no 4}
\end{align}
We then calculate the sign of permutations:
\begin{itemize}
    \item 
$
    \sgn
        {\indexjp{l},\indexI,\indexJp\backslash\{\indexjp{l}\}}
        {\indexI,\indexJp}
    \sgn
        {\indexI,\indexJp}
        {\indexjp{l},\indexI,\indexJp\backslash\{\indexjp{l}\}}
    =
    1,
$
    \item 
$
    \sgn
        {\indexI,\indexJp}
        {\indexjp{l},\indexI,\indexJp\backslash\{\indexjp{l}\}}
    \sgn
        {t^{'},\indexI,\indexJp\backslash\{\indexjp{l}\}}
        {\indexI,\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
    =
    \sgn
        {\indexI,\indexJp}
        {\indexjp{l},\indexI,\indexJp\backslash\{\indexjp{l}\}}
    \sgn
        {\indexjp{l},t^{'},\indexI,\indexJp\backslash\{\indexjp{l}\}}
        {\indexjp{l},\indexI,\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
    \\
    =
    \sgn
        {\indexI,\indexJp}
        {\indexjp{l},\indexI,\indexJp\backslash\{\indexjp{l}\}}
    (-1)
    \sgn
        {t^{'},\indexjp{l},\indexI,\indexJp\backslash\{\indexjp{l}\}}
        {\indexjp{l},\indexI,\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
    =
    (-1)
    \sgn
        {t^{'},\indexI,\indexJp}
        {\indexjp{l},\indexI,\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}.
$
\end{itemize}




Rearranging (\ref{EQ-For (alpha, I, J), calculation for LHS, extra 2-first part, no 4}), we conclude that the simplified expression of the first half is:
\begin{align}
    -2\sqrt{-1}
    \begin{pmatrix*}[l]
        \displaystyle\sum_{\indexjp{l}\in\indexJp}
        \coefB{\alpha}{\indexj{l} \indexjp{l}}
        \basexi{\indexI}
        \wedge
        \basedualxi{\indexJp}
        \\
        +
        \\
        \displaystyle\sum_{\indexjp{l}\in\indexJp}
        \displaystyle\sum_{t^{'}\in\indexJpc}
        \begin{matrix*}[l]
            (-1)
            \sgn
                {t^{'},\indexI,\indexJp}
                {\indexjp{l},\indexI,\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
            \coefB{\alpha}{\indexj{l} t^{'}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
        \end{matrix*}
    \end{pmatrix*}.
\label{EQ-For (alpha, I, J), calculation for LHS, extra 2-first part, simplified result}
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%% finish the first part %%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%% start the second part %%%%%%%%%%%%%%%%
We then look at the second part,
\begin{align}
    -\frac{\sqrt{-1}}{2}
    \displaystyle\sum_{h=1}^{n}
    (\iota_{\basedualxi{h}}\,\LieagbdPartialbar\basexi{\alpha})
    \wedge
    \iota_{\basexi{h}}(\basexi{\indexI}\wedge\basedualxi{\indexJp})
.
\label{EQ-For (alpha, I, J), calculation for LHS, extra 2-second part, target}
\end{align}
Using the contraction computation
\begin{align}
    \iota_{\basexi{h}}(\basexi{\indexI}\wedge\basedualxi{\indexJp})
    =
    \begin{cases}
        0       & \,h\notin\indexI \\
        2
        \sgn
            {\indexI}
            {h,\indexI\backslash\{h\}}
        \basexi{\indexI\backslash\{h\}}
        \wedge
        \basedualxi{\indexJp}
                & \,h\in\indexI
    \end{cases},
\end{align}
we use $\indexi{k}$ to replace h and simplify (\ref{EQ-For (alpha, I, J), calculation for LHS, extra 2-second part, target}) to
\begin{align}
    -\frac{\sqrt{-1}}{2}
    \displaystyle\sum_{\indexi{k}\in\indexI}
    (\iota_{\basedualxi{k^{'}}}\,\LieagbdPartialbar\basexi{\alpha})
    \wedge
    \bigg(
        2
        \sgn
            {\indexI}
            {\indexi{k},\indexI\backslash\{\indexi{k}\}}
        \basexi{\indexI\backslash\{\indexi{k}\}}
        \wedge
        \basedualxi{\indexJp}
    \bigg)
    .
\label{EQ-For (alpha, I, J), calculation for LHS, extra 2-second part, no 1}
\end{align}
We plug $
\LieagbdPartialbar \basexi{\alpha}
=
\displaystyle\sum_{s,t}
\coefB{\alpha}{s t^{'}}
\basexi{s}\wedge\basedualxi{t^{'}}
$ into (\ref{EQ-For (alpha, I, J), calculation for LHS, extra 2-second part, no 1}) and cancel out the terms containing repeated wedge product of frames, obtaining
\begin{align}
    -\frac{\sqrt{-1}}{2}
    \displaystyle\sum_{\indexi{k}\in\indexI}
    (
    \iota_{\basedualxi{k^{'}}}
    \begin{pmatrix*}[l]
        \coefB{\alpha}{\indexi{k} \indexip{k}}
        \basexi{\indexi{k}}
        \wedge
        \basedualxi{\indexip{k}}
        \\
        +
        \\
        \displaystyle\sum_{s\in\indexIc}
        \coefB{\alpha}{s \indexip{k}}
        \basexi{s}
        \wedge
        \basedualxi{\indexip{k}}
    \end{pmatrix*}
    )
    \wedge
    \bigg(
        2
        \sgn
            {\indexI}
            {\indexi{k},\indexI\backslash\{\indexi{k}\}}
        \basexi{\indexI\backslash\{\indexi{k}\}}
        \wedge
        \basedualxi{\indexJp}
    \bigg)
    .
\label{EQ-For (alpha, I, J), calculation for LHS, extra 2-second part, no 2}
\end{align}
The contractions in the first parenthesis are computed as follows:
\begin{align*}
    \iota_{\basedualxi{\indexip{k}}}
    (\basexi{\indexi{k}}\wedge\basedualxi{\indexip{k}})
    =
    -2\basexi{\indexi{k}}
    \qquad \text{and} \qquad 
    \iota_{\basedualxi{\indexip{k}}}
    (\basexi{s}\wedge\basedualxi{\indexip{k}})
    =
    -2\basexi{s}
    .
\end{align*}
Thus, we simplify (\ref{EQ-For (alpha, I, J), calculation for LHS, extra 2-second part, no 2}) to
\begin{align}
    -\frac{\sqrt{-1}}{2}
    \displaystyle\sum_{\indexi{k}\in\indexI}
    \begin{pmatrix*}[l]
        -2
        \coefB{\alpha}{\indexi{k} \indexip{k}}
        \basexi{\indexi{k}}
        \\
        +
        \\
        \displaystyle\sum_{s\in\indexIc}
        -2
        \coefB{\alpha}{s \indexip{k}}
        \basexi{s}
    \end{pmatrix*}
    \wedge
    \bigg(
        2
        \sgn
            {\indexI}
            {\indexi{k},\indexI\backslash\{\indexi{k}\}}
        \basexi{\indexI\backslash\{\indexi{k}\}}
        \wedge
        \basedualxi{\indexJp}
    \bigg)
    ,
\label{EQ-For (alpha, I, J), calculation for LHS, extra 2-second part, no 3}
\end{align}
in which
\begin{itemize}
    \item 
$
    \basexi{\indexi{k}}
    \wedge\basexi{\indexI\backslash\{\indexi{k}\}}    
    \wedge\basedualxi{\indexJp}
    =
    \sgn
        {\indexI}
        {\indexi{k},\indexI\backslash\{\indexi{k}\}}
    \basexi{\indexI}\wedge\basedualxi{\indexJp}
$,
    \item 
$
    \basexi{s}
    \wedge\basexi{\indexI\backslash\{\indexi{k}\}}    
    \wedge\basedualxi{\indexJp}
    =
    \sgn
        {s,\indexI\backslash\{\indexi{k}\}}
        {\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
    \basexi{\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
    \wedge
    \basedualxi{\indexJp}
$.
\end{itemize}
Thus, after ordering the wedge product of frames, we simplify (\ref{EQ-For (alpha, I, J), calculation for LHS, extra 2-second part, no 3}) to
\begin{align}
    -2\sqrt{-1}
    \begin{pmatrix*}[l]
        \displaystyle\sum_{\indexi{k}\in\indexI}
        (-1)
        \sgn
            {\indexI}
            {\indexi{k},\indexI\backslash\{\indexi{k}\}}
        \sgn
            {\indexI}
            {\indexi{k},\indexI\backslash\{\indexi{k}\}}
        \coefB{\alpha}{\indexi{k} \indexip{k}}
        \basexi{\indexI}
        \wedge
        \basedualxi{\indexJp}
        \\
        +
        \\
        \displaystyle\sum_{\indexi{k}\in\indexI}
        \displaystyle\sum_{s\in\indexIc}
        \begin{matrix*}[l]
            \sgn
                {\indexI}
                {\indexi{k},\indexI\backslash\{\indexi{k}\}}
            \sgn
                {s,\indexI\backslash\{\indexi{k}\}}
                {\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
            (-1)
            \coefB{\alpha}{s \indexip{k}}
            \basexi{\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
            \wedge
            \basedualxi{\indexJp}
        \end{matrix*}
    \end{pmatrix*}
    .
\label{EQ-For (alpha, I, J), calculation for LHS, extra 2-second part, no 4}
\end{align}
We calculate the sign of permutations:
\begin{itemize}
    \item 
$
    \sgn
        {\indexI}
        {\indexi{k},\indexI\backslash\{\indexi{k}\}}
    \sgn
        {\indexI}
        {\indexi{k},\indexI\backslash\{\indexi{k}\}}
    =
    1
$,
    \item 
$
    \sgn
        {\indexI}
        {\indexi{k},\indexI\backslash\{\indexi{k}\}}
    \sgn
        {s,\indexI\backslash\{\indexi{k}\}}
        {\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
    =
    \sgn
        {\indexI}
        {\indexi{k},\indexI\backslash\{\indexi{k}\}}
    \sgn
        {\indexi{k},s,\indexI\backslash\{\indexi{k}\}}
        {\indexi{k},\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
    \\
    =
    \sgn
        {\indexI}
        {\indexi{k},\indexI\backslash\{\indexi{k}\}}
    (-1)
    \sgn
        {s,\indexi{k},\indexI\backslash\{\indexi{k}\}}
        {\indexi{k},\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
    =
    (-1)
    \sgn
        {s,\indexI}
        {\indexi{k},\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
$.
\end{itemize}
We then calculate (\ref{EQ-For (alpha, I, J), calculation for LHS, extra 2-second part, no 4}):
\begin{align}
    -2\sqrt{-1}
    \begin{pmatrix*}[l]
        \displaystyle\sum_{\indexi{k}\in\indexI}
        (-1)
        \coefB{\alpha}{\indexi{k} \indexip{k}}
        \basexi{\indexI}
        \wedge
        \basedualxi{\indexJp}
        \\
        +
        \\
        \displaystyle\sum_{\indexi{k}\in\indexI}
        \displaystyle\sum_{s\in\indexIc}
        \begin{matrix*}[l]
            \sgn
                {s,\indexI}
                {\indexi{k},\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
            \coefB{\alpha}{s \indexip{k}}
            \basexi{\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
            \wedge
            \basedualxi{\indexJp}
        \end{matrix*}
    \end{pmatrix*}.
\label{EQ-For (alpha, I, J), calculation for LHS, extra 2-second part, simplified result}
\end{align}



Finally, we assemble (\ref{EQ-For (alpha, I, J), calculation for LHS, extra 2-first part, simplified result}) and (\ref{EQ-For (alpha, I, J), calculation for LHS, extra 2-second part, simplified result}) and complete the proof of Lemma \ref{lemma-For (alpha, I, J), calculation for LHS-extra 2]}:
\begin{align*}
    &
    (-\frac{\sqrt{-1}}{2})
    \displaystyle\sum_{k=1}^{n}
    \bigg(
        (\iota_{\basexi{k}}\,\LieagbdPartialbar\basexi{\alpha})
        \wedge
        \iota_{\basedualxi{k}}(\basexi{\indexI}\wedge\basedualxi{\indexJp})
        -
        (\iota_{\basedualxi{k}}\,\LieagbdPartialbar\basexi{\alpha})
        \wedge
        \iota_{\basexi{k}}(\basexi{\indexI}\wedge\basedualxi{\indexJp})
    \bigg)
    \\
    =&
    -2\sqrt{-1}
    \begin{pmatrix*}[l]
        \displaystyle\sum_{\indexjp{l}\in\indexJp}
        \begin{matrix*}[l]
            \coefB{\alpha}{\indexj{l} \indexjp{l}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\indexJp}
        \end{matrix*}
        \\
        +
        \\
        \displaystyle\sum_{\indexjp{l}\in\indexJp}
        \displaystyle\sum_{t^{'}\in\indexJpc}
        \begin{matrix*}[l]
            (-1)
            \sgn
                {t^{'},\indexI,\indexJp}
                {\indexjp{l},\indexI,\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
            \coefB{\alpha}{\indexj{l} t^{'}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\order{(\indexJp\backslash\{\indexjp{l}\})\cup\{t^{'}\}}}
        \end{matrix*}
        \\
        +
        \\
        \displaystyle\sum_{\indexi{k}\in\indexI}
        \begin{matrix*}[l]
            \coefB{\alpha}{\indexi{k} \indexip{k}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\indexJp}
        \end{matrix*}
        \\
        +
        \\
        \displaystyle\sum_{\indexi{k}\in\indexI}
        \displaystyle\sum_{s\in\indexIc}
        \begin{matrix*}[l]
            (-1)
            \sgn
                {s,\indexI}
                {\indexi{k},\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
            \coefB{\alpha}{s \indexip{k}}
            \basexi{\order{(\indexI\backslash\{\indexi{k}\})\cup\{s\}}}
            \wedge
            \basedualxi{\indexJp}
        \end{matrix*}
    \end{pmatrix*}.
\end{align*}

\end{proof}

==> 4/For__alpha,_I,_J_,_calculation_for_LHS.tex <==


\begin{lemma}
\label{lemma-For (alpha, I, J), calculation for LHS-initial resutl]}
    The expression of $
    [\LieagbdPartialbar,\iotaW]
    (\basexi{\alpha}\wedge\basexi{\indexI}\wedge\basedualxi{\indexJp})
    $ is    
\begin{align}
    \begin{pmatrix*}[l]
        [\LieagbdPartialbar,\iotaW]
        (\basexi{\alpha})
        \wedge
        \basexi{\indexI}\wedge\basedualxi{\indexJp}
        \\
        -
        \\
        \basexi{\alpha}
        \wedge
        [\LieagbdPartialbar,\iotaW]
        (\basexi{\indexI}\wedge\basedualxi{\indexJp})
        \\
        +
        \\
        (-\sqrt{-1})
        (\LieagbdPartialbar \, \iota_{\basedualxi{\alpha^{'}}}
        +
        \iota_{\basedualxi{\alpha^{'}}}\,\LieagbdPartialbar)
        (\basexi{\indexI}\wedge\basedualxi{\indexJp})
        \\
        +
        \\
        (-\frac{\sqrt{-1}}{2})
        \displaystyle\sum_{h=1}^{n}
        \big(
            (\iota_{\basexi{h}} \, \LieagbdPartialbar \basexi{\alpha})
            \wedge
            \iota_{\basedualxi{h^{'}}}(\basexi{\indexI}\wedge\basedualxi{\indexJp})
            -
            (\iota_{\basedualxi{h^{'}}} \, \LieagbdPartialbar \basexi{\alpha})
            \wedge
            \iota_{\basexi{h}}(\basexi{\indexI}\wedge\basedualxi{\indexJp})
        \big)
    \end{pmatrix*}
.
\label{EQ-For (alpha, I, J), calculation for LHS-half summary}
\end{align}
\end{lemma}


\begin{proof}
Observe that
\begin{align*}
    [\LieagbdPartialbar,\iotaW]
    (
        \basexi{\alpha}\wedge\basexi{\indexI}\wedge\basedualxi{\indexJp}
    )
    =
    \LieagbdPartialbar\,\iotaW
    (
        \basexi{\alpha}\wedge\basexi{\indexI}\wedge\basedualxi{\indexJp}
    )
    -
    \iotaW\,\LieagbdPartialbar
    (
        \basexi{\alpha}\wedge\basexi{\indexI}\wedge\basedualxi{\indexJp}
    ).
\end{align*}
Recalling that $
\iotaW
=
-\frac{\sqrt{-1}}{2}
\displaystyle\sum_{h=1}^{n}
\iota_{\basedualxi{h^{'}}} \, \iota_{\basexi{h}}
$, we apply this to $\basexi{\alpha}\wedge\basexi{\indexI}\wedge\basedualxi{\indexJp}$ and obtain
\begin{align}
        \iotaW
        (\basexi{\alpha}\wedge\basexi{\indexI}\wedge\basedualxi{\indexJp})
    =&
        -\frac{\sqrt{-1}}{2}
        \displaystyle\sum_{h=1}^{n}
        \iota_{\basedualxi{h^{'}}} \, \iota_{\basexi{h}}
        (\basexi{\alpha}\wedge\basexi{\indexI}\wedge\basedualxi{\indexJp})
\notag
    \\
    =&
        -\frac{\sqrt{-1}}{2}
        \displaystyle\sum_{h=1}^{n}
        \iota_{\basedualxi{h^{'}}}
        \begin{pmatrix*}[l]
            (\iota_{\basexi{h}}\basexi{\alpha})
            \wedge\basexi{\indexI}\wedge\basedualxi{\indexJp}
            \\
            -
            \\
            \basexi{\alpha}
            \wedge
            \iota_{\basexi{h}}(\basexi{\indexI}\wedge\basedualxi{\indexJp})
        \end{pmatrix*}
\notag
    \\
    =&
        -\frac{\sqrt{-1}}{2}
        \LieagbdPartialbar
        \displaystyle\sum_{h=1}^{n}
        \begin{pmatrix*}[l]
            \begin{pmatrix*}[l]
                (\iota_{\basedualxi{h^{'}}} \, \iota_{\basexi{h}}\basexi{\alpha})
                \wedge
                \basexi{\indexI}\wedge\basedualxi{\indexJp}
                \\
                +
                \\
                (\iota_{\basexi{h}}\basexi{\alpha})
                \wedge
                \iota_{\basedualxi{h^{'}}} (\basexi{\indexI}\wedge\basedualxi{\indexJp})
            \end{pmatrix*}
            \\
            -
            \\
            \begin{pmatrix*}[l]
                (\iota_{\basedualxi{h^{'}}} \basexi{\alpha})
                \wedge
                \iota_{\basexi{h}}(\basexi{\indexI}\wedge\basedualxi{\indexJp})
                \\
                -
                \\
                \basexi{\alpha}
                \wedge
                \iota_{\basedualxi{h^{'}}} \, \iota_{\basexi{h}}
                (\basexi{\indexI}\wedge\basedualxi{\indexJp})
            \end{pmatrix*}
        \end{pmatrix*}.
\label{EQ-For (alpha, I, J), calculation for LHS-No 1}
\end{align}
We note that $\contract{\basexi{h}}\basexi{\alpha}=2 \delta_{\alpha,h}$, $\contract{h}\basexi{\alpha}=2 \delta_{\alpha,h}$, and $\contract{\basedualxi{h^{'}}}\basexi{\alpha}=0$ are constant functions. Thus, the formula 
$\contract{\basedualxi{h^{'}}}\,\contract{\basexi{h}}\basexi{\alpha}=0$ as the contraction on a constant function is zero. Plugging these into (\ref{EQ-For (alpha, I, J), calculation for LHS-No 1}), we obtain
\begin{align}
        -\frac{\sqrt{-1}}{2}
        \displaystyle\sum_{h=1}^{n}
        \begin{pmatrix*}[l]
            \begin{pmatrix*}[l]
                (0)
                \wedge
                \basexi{\indexI}\wedge\basedualxi{\indexJp}
                \\
                +
                \\
                (2\delta_{\alpha, h})
                \wedge
                \iota_{\basedualxi{h^{'}}} (\basexi{\indexI}\wedge\basedualxi{\indexJp})
            \end{pmatrix*}
            \\
            -
            \\
            \begin{pmatrix*}[l]
                (0)
                \wedge
                \iota_{\basexi{h}}(\basexi{\indexI}\wedge\basedualxi{\indexJp})
                \\
                -
                \\
                \basexi{\alpha}
                \wedge
                \iota_{\basedualxi{h^{'}}} \, \iota_{\basexi{h}}
                (\basexi{\indexI}\wedge\basedualxi{\indexJp})
            \end{pmatrix*}
        \end{pmatrix*}
    =
        -\frac{\sqrt{-1}}{2}
        \begin{pmatrix*}[l]
            2\iota_{\basedualxi{\alpha^{'}}} (\basexi{\indexI}\wedge\basedualxi{\indexJp})
            \\
            +
            \\
            \displaystyle\sum_{h=1}^{n}
            \basexi{\alpha}
            \wedge
            \iota_{\basedualxi{h}} \, \iota_{\basexi{h}}
            (\basexi{\indexI}\wedge\basedualxi{\indexJp})
        \end{pmatrix*}.
\label{EQ-For (alpha, I, J), calculation for LHS-No 2}
\end{align}
The next step is to apply $\LieagbdPartialbar$ on $\basexi{\alpha}\wedge\basexi{\indexI}\wedge\basedualxi{\indexJp}$: 
\begin{align}
        \LieagbdPartialbar\,\iotaW
        (\basexi{\alpha}\wedge\basexi{\indexI}\wedge\basedualxi{\indexJp})
    =
        -\frac{\sqrt{-1}}{2}
        \begin{pmatrix*}[l]
            2\LieagbdPartialbar \, \iota_{\basedualxi{\alpha^{'}}}
            (\basexi{\indexI}\wedge\basedualxi{\indexJp})
            \\
            +
            \\
            \displaystyle\sum_{h=1}^{n}
            (\LieagbdPartialbar \basexi{\alpha})
            \wedge
            \iota_{\basedualxi{h}} \, \iota_{\basexi{h}}
            (\basexi{\indexI}\wedge\basedualxi{\indexJp})
            \\
            -
            \\
            \displaystyle\sum_{h=1}^{n}
            \basexi{\alpha}
            \wedge
            \LieagbdPartialbar \, \iota_{\basedualxi{h}} \, \iota_{\basexi{h}}
            (\basexi{\indexI}\wedge\basedualxi{\indexJp})
        \end{pmatrix*}.
    \label{EQ-For (alpha, I, J), calculation for LHS-No 3}
\end{align}
It is not necessary to calculate the expressions of $
\LieagbdPartialbar \, \iota_{\basedualxi{h}} \, \iota_{\basexi{h}}(\basexi{\indexI}\wedge\basedualxi{\indexJp})
$
and 
$
(\LieagbdPartialbar \basexi{\alpha})\wedge \iota_{\basedualxi{h}} \, \iota_{\basexi{h}}(\basexi{\indexI}\wedge\basedualxi{\indexJp})
$ 
as they may represent 
$
[\LieagbdPartialbar,\iotaW]
(\basexi{\alpha}\wedge\basexi{\indexI}\wedge\basedualxi{\indexJp})
$.


Next, we compute $\iotaW\,\LieagbdPartialbar(\basexi{\alpha}\wedge\basexi{\indexI}\wedge\basedualxi{\indexJp})$. Applying $\LieagbdPartialbar$ to $\basexi{\alpha}\wedge\basexi{\indexI}\wedge\basedualxi{\indexJp}$, we obtain
\begin{align*}
    (\LieagbdPartialbar \basexi{\alpha})
    \wedge
    \basexi{\indexI}\wedge\basedualxi{\indexJp}
    -
    \basexi{\alpha}
    \wedge
    \LieagbdPartialbar(\basexi{\indexI}\wedge\basedualxi{\indexJp}).
\end{align*}
We then apply $
\iotaW
=
-\frac{\sqrt{-1}}{2}
\displaystyle\sum_{h=1}^{n}
\iota_{\basedualxi{h^{'}}} \, \iota_{\basexi{h}}
$ to $\LieagbdPartialbar(\basexi{\alpha}\wedge\basexi{\indexI}\wedge\basedualxi{\indexJp})$ and obtain 
\begin{align}
    &
        \iotaW\,\LieagbdPartialbar
        (\basexi{\alpha}\wedge\basexi{\indexI}\wedge\basedualxi{\indexJp})
    \notag
    \\
    =&
        -\frac{\sqrt{-1}}{2}
        \displaystyle\sum_{h=1}^{n}
        \iota_{\basedualxi{h^{'}}} \, \iota_{\basexi{h}}
        \begin{pmatrix*}[l]
            (\LieagbdPartialbar \basexi{\alpha})
            \wedge
            \basexi{\indexI}\wedge\basedualxi{\indexJp}
            -
            \basexi{\alpha}
            \wedge
            \LieagbdPartialbar(\basexi{\indexI}\wedge\basedualxi{\indexJp})
        \end{pmatrix*}
\notag
    \\
    =&
        -\frac{\sqrt{-1}}{2}
        \displaystyle\sum_{h=1}^{n}
        \iota_{\basedualxi{h^{'}}}
        \begin{pmatrix*}[l]
            \begin{pmatrix*}
                (\iota_{\basexi{h}} \, \LieagbdPartialbar \basexi{\alpha})
                \wedge
                \basexi{\indexI}\wedge\basedualxi{\indexJp}
                \\
                +
                \\
                (\LieagbdPartialbar \basexi{\alpha})
                \wedge
                \iota_{\basexi{h}}(\basexi{\indexI}\wedge\basedualxi{\indexJp})
            \end{pmatrix*}   
            -
            \begin{pmatrix*}
                (\iota_{\basexi{h}}\basexi{\alpha})
                \wedge
                \LieagbdPartialbar(\basexi{\indexI}\wedge\basedualxi{\indexJp})
                \\
                -
                \\
                \basexi{\alpha}
                \wedge
                \iota_{\basexi{h}}\,\LieagbdPartialbar
                (\basexi{\indexI}\wedge\basedualxi{\indexJp})
            \end{pmatrix*} 
        \end{pmatrix*}
\notag
    \\
    =&
        -\frac{\sqrt{-1}}{2}
        \displaystyle\sum_{h=1}^{n}
        \begin{pmatrix*}[l]
            \begin{pmatrix*}
                \begin{pmatrix*}                                    
                    (\iota_{\basedualxi{h^{'}}}\,\iota_{\basexi{h}} \, \LieagbdPartialbar \basexi{\alpha})
                    \wedge
                    \basexi{\indexI}\wedge\basedualxi{\indexJp}
                    \\
                    -
                    \\
                    (\iota_{\basexi{h}} \, \LieagbdPartialbar \basexi{\alpha})
                    \wedge
                    \iota_{\basedualxi{h^{'}}}(\basexi{\indexI}\wedge\basedualxi{\indexJp})
                \end{pmatrix*}
                \\
                +
                \\
                \begin{pmatrix*}
                    (\iota_{\basedualxi{h^{'}}} \, \LieagbdPartialbar \basexi{\alpha})
                    \wedge
                    \iota_{\basexi{h}}(\basexi{\indexI}\wedge\basedualxi{\indexJp})
                    \\
                    +
                    \\
                    (\LieagbdPartialbar \basexi{\alpha})
                    \wedge
                    \iota_{\basedualxi{h^{'}}} \, \iota_{\basexi{h}}
                    (\basexi{\indexI}\wedge\basedualxi{\indexJp})
                \end{pmatrix*}
            \end{pmatrix*}
            -
            \begin{pmatrix*}
                \begin{pmatrix*}
                    (\iota_{\basedualxi{h^{'}}}\,\iota_{\basexi{h}}\basexi{\alpha})
                    \wedge
                    \LieagbdPartialbar
                    (\basexi{\indexI}\wedge\basedualxi{\indexJp})
                    \\
                    +
                    \\
                    (\iota_{\basexi{h}}\basexi{\alpha})
                    \wedge
                    \iota_{\basedualxi{h^{'}}}\,\LieagbdPartialbar
                    (\basexi{\indexI}\wedge\basedualxi{\indexJp})
                \end{pmatrix*}
                \\
                -
                \\
                \begin{pmatrix*}  
                    (\iota_{\basedualxi{h^{'}}}\basexi{\alpha})
                    \wedge
                    \iota_{\basexi{h}}\,\LieagbdPartialbar
                    (\basexi{\indexI}\wedge\basedualxi{\indexJp})
                    \\
                    -
                    \\
                    \basexi{\alpha}
                    \wedge
                    \iota_{\basedualxi{h^{'}}}\,\iota_{\basexi{h}}\,\LieagbdPartialbar
                    (\basexi{\indexI}\wedge\basedualxi{\indexJp})
                \end{pmatrix*}
            \end{pmatrix*}
        \end{pmatrix*}.
\label{EQ-For (alpha, I, J), calculation for LHS-No 4}
\end{align}
Using the property that $\contract{\basexi{h}}\basexi{\alpha}=2\delta_{h,\alpha}$, $\contract{\basedualxi{h^{'}}}\basexi{\alpha}=0$ and $(\iota_{\basedualxi{h^{'}}}\,\iota_{\basexi{h}}\basexi{\alpha})=0$, we can simplify the terms in (\ref{EQ-For (alpha, I, J), calculation for LHS-No 4}) to
\begin{align*}
    &
        -\frac{\sqrt{-1}}{2}
        \displaystyle\sum_{h=1}^{n}
        \begin{pmatrix*}[l]
            \begin{pmatrix*}
                \begin{pmatrix*}                                    
                    (\iota_{\basedualxi{h^{'}}}\,\iota_{\basexi{h}} \, \LieagbdPartialbar \basexi{\alpha})
                    \wedge
                    \basexi{\indexI}\wedge\basedualxi{\indexJp}
                    \\
                    -
                    \\
                    (\iota_{\basexi{h}} \, \LieagbdPartialbar \basexi{\alpha})
                    \wedge
                    \iota_{\basedualxi{h^{'}}}(\basexi{\indexI}\wedge\basedualxi{\indexJp})
                \end{pmatrix*}
                \\
                +
                \\
                \begin{pmatrix*}
                    (\iota_{\basedualxi{h^{'}}} \, \LieagbdPartialbar \basexi{\alpha})
                    \wedge
                    \iota_{\basexi{h}}(\basexi{\indexI}\wedge\basedualxi{\indexJp})
                    \\
                    +
                    \\
                    (\LieagbdPartialbar \basexi{\alpha})
                    \wedge
                    \iota_{\basedualxi{h^{'}}} \, \iota_{\basexi{h}}
                    (\basexi{\indexI}\wedge\basedualxi{\indexJp})
                \end{pmatrix*}
            \end{pmatrix*}
            -
            \begin{pmatrix*}
                \begin{pmatrix*}
                    0
                    \wedge
                    \LieagbdPartialbar
                    (\basexi{\indexI}\wedge\basedualxi{\indexJp})
                    \\
                    +
                    \\
                    2\delta_{h,\alpha}
                    \wedge
                    \iota_{\basedualxi{h^{'}}}\,\LieagbdPartialbar
                    (\basexi{\indexI}\wedge\basedualxi{\indexJp})
                \end{pmatrix*}
                \\
                -
                \\
                \begin{pmatrix*}  
                    0
                    \wedge
                    \iota_{\basexi{h}}\,\LieagbdPartialbar
                    (\basexi{\indexI}\wedge\basedualxi{\indexJp})
                    \\
                    -
                    \\
                    \basexi{\alpha}
                    \wedge
                    \iota_{\basedualxi{h^{'}}}\,\iota_{\basexi{h}}\,\LieagbdPartialbar
                    (\basexi{\indexI}\wedge\basedualxi{\indexJp})
                \end{pmatrix*}
            \end{pmatrix*}
        \end{pmatrix*}
    \\
    =&
        -\frac{\sqrt{-1}}{2}
        \displaystyle\sum_{h=1}^{n}
        \begin{pmatrix*}[l]
            (\iota_{\basedualxi{h^{'}}}\,\iota_{\basexi{h}} \, \LieagbdPartialbar \basexi{\alpha})
            \wedge
            \basexi{\indexI}\wedge\basedualxi{\indexJp}
            \\
            -
            \\
            (\iota_{\basexi{h}} \, \LieagbdPartialbar \basexi{\alpha})
            \wedge
            \iota_{\basedualxi{h^{'}}}(\basexi{\indexI}\wedge\basedualxi{\indexJp})
            \\
            +
            \\
            (\iota_{\basedualxi{h^{'}}} \, \LieagbdPartialbar \basexi{\alpha})
            \wedge
            \iota_{\basexi{h}}(\basexi{\indexI}\wedge\basedualxi{\indexJp})
            \\
            +
            \\
            (\LieagbdPartialbar \basexi{\alpha})
            \wedge
            \iota_{\basedualxi{h^{'}}} \, \iota_{\basexi{h}}
            (\basexi{\indexI}\wedge\basedualxi{\indexJp})
            \\
            -
            \\
            2\delta_{h,\alpha}
            \wedge
            \iota_{\basedualxi{h^{'}}}\,\LieagbdPartialbar
            (\basexi{\indexI}\wedge\basedualxi{\indexJp})
            \\
            -
            \\
            \basexi{\alpha}
            \wedge
            \iota_{\basedualxi{h^{'}}}\,\iota_{\basexi{h}}\,\LieagbdPartialbar
            (\basexi{\indexI}\wedge\basedualxi{\indexJp})
        \end{pmatrix*}.
\end{align*}
Taking $
-2\delta_{h,\alpha}\wedge\iota_{\basedualxi{h^{'}}}
\,\LieagbdPartialbar
(\basexi{\indexI}\wedge\basedualxi{\indexJp})
=-2\iota_{\basedualxi{\alpha^{'}}}
\,\LieagbdPartialbar
(\basexi{\indexI}\wedge\basedualxi{\indexJp})
$, we conclude that
\begin{align}
    \iotaW \, \LieagbdPartialbar
    (\basexi{\alpha}\wedge\basexi{\indexI}\wedge\basedualxi{\indexJp})
    =&
        -\frac{\sqrt{-1}}{2}
        (
        \displaystyle\sum_{h=1}^{n}
        \begin{pmatrix*}[l]
            (\iota_{\basedualxi{h^{'}}}\iota_{\basexi{h}} \, \LieagbdPartialbar \basexi{\alpha})
            \wedge
            \basexi{\indexI}\wedge\basedualxi{\indexJp}
            \\
            -
            \\
            (\iota_{\basexi{h}} \, \LieagbdPartialbar \basexi{\alpha})
            \wedge
            \iota_{\basedualxi{h^{'}}}(\basexi{\indexI}\wedge\basedualxi{\indexJp})
            \\
            +
            \\
            (\iota_{\basedualxi{h^{'}}} \, \LieagbdPartialbar \basexi{\alpha})
            \wedge
            \iota_{\basexi{h}}(\basexi{\indexI}\wedge\basedualxi{\indexJp})
            \\
            +
            \\
            (\LieagbdPartialbar \basexi{\alpha})
            \wedge
            \iota_{\basedualxi{h^{'}}} \, \iota_{\basexi{h}}
            (\basexi{\indexI}\wedge\basedualxi{\indexJp})
            \\
            -
            \\
            2\iota_{\basedualxi{\alpha^{'}}}\,\LieagbdPartialbar
            (\basexi{\indexI}\wedge\basedualxi{\indexJp})
            \\
            -
            \\
            \basexi{\alpha}
            \wedge
            \iota_{\basedualxi{h^{'}}}\,\iota_{\basexi{h}}\,\LieagbdPartialbar
            (\basexi{\indexI}\wedge\basedualxi{\indexJp})
        \end{pmatrix*}
        .
\label{EQ-For (alpha, I, J), calculation for LHS-No 5}
\end{align}


Combining (\ref{EQ-For (alpha, I, J), calculation for LHS-No 3}) and (\ref{EQ-For (alpha, I, J), calculation for LHS-No 5}), we find that 
\begin{align*}
    [\LieagbdPartialbar,\iotaW]
    (\basexi{\alpha}\wedge\basexi{\indexI}\wedge\basedualxi{\indexJp})
    =
        \LieagbdPartialbar\,\iotaW
        (\basexi{\alpha}\wedge\basexi{\indexI}\wedge\basedualxi{\indexJp})
        -
        \iotaW\,\LieagbdPartialbar
        (\basexi{\alpha}\wedge\basexi{\indexI}\wedge\basedualxi{\indexJp})
\end{align*}
is equal to
\begin{align*}
        (-\frac{\sqrt{-1}}{2})
        \Big(
        \begin{pmatrix*}[l]
            2\LieagbdPartialbar \, \iota_{\basedualxi{\alpha^{'}}}
            (\basexi{\indexI}\wedge\basedualxi{\indexJp})
            \\
            +
            \\
            \displaystyle\sum_{h=1}^{n}
            (\LieagbdPartialbar \basexi{\alpha})
            \wedge
            \iota_{\basedualxi{h}} \, \iota_{\basexi{h}}
            (\basexi{\indexI}\wedge\basedualxi{\indexJp})
            \\
            -
            \\
            \displaystyle\sum_{h=1}^{n}
            \basexi{\alpha}
            \wedge
            \LieagbdPartialbar \, \iota_{\basedualxi{h}} \, \iota_{\basexi{h}}
            (\basexi{\indexI}\wedge\basedualxi{\indexJp})
        \end{pmatrix*}
        -
        \begin{pmatrix*}[l]
            (\iota_{\basedualxi{h^{'}}}\iota_{\basexi{h}} \, \LieagbdPartialbar \basexi{\alpha})
            \wedge
            \basexi{\indexI}\wedge\basedualxi{\indexJp}
            \\
            -
            \\
            (\iota_{\basexi{h}} \, \LieagbdPartialbar \basexi{\alpha})
            \wedge
            \iota_{\basedualxi{h^{'}}}(\basexi{\indexI}\wedge\basedualxi{\indexJp})
            \\
            +
            \\
            (\iota_{\basedualxi{h^{'}}} \, \LieagbdPartialbar \basexi{\alpha})
            \wedge
            \iota_{\basexi{h}}(\basexi{\indexI}\wedge\basedualxi{\indexJp})
            \\
            +
            \\
            (\LieagbdPartialbar \basexi{\alpha})
            \wedge
            \iota_{\basedualxi{h^{'}}} \, \iota_{\basexi{h}}
            (\basexi{\indexI}\wedge\basedualxi{\indexJp})
            \\
            -
            \\
            2\iota_{\basedualxi{\alpha^{'}}}\,\LieagbdPartialbar
            (\basexi{\indexI}\wedge\basedualxi{\indexJp})
            \\
            -
            \\
            \basexi{\alpha}
            \wedge
            \iota_{\basedualxi{h^{'}}}\,\iota_{\basexi{h}}\,\LieagbdPartialbar
            (\basexi{\indexI}\wedge\basedualxi{\indexJp})
        \end{pmatrix*}
        \Big)
    ,
    \notag\\
\end{align*}
which can be simplified to
\begin{align*}
        (-\frac{\sqrt{-1}}{2})
        \begin{pmatrix*}[l]
            (0-\iota_{\basedualxi{h^{'}}}\iota_{\basexi{h}} \, \LieagbdPartialbar \basexi{\alpha})
            \wedge
            \basexi{\indexI}\wedge\basedualxi{\indexJp}
            \\
            -
            \\
            \basexi{\alpha}
            \wedge
            (\LieagbdPartialbar \, \iota_{\basedualxi{h}} \, \iota_{\basexi{h}}
            -
            \iota_{\basedualxi{h^{'}}}\,\iota_{\basexi{h}}\,\LieagbdPartialbar)
            (\basexi{\indexI}\wedge\basedualxi{\indexJp})
            \\
            +
            \\
            2(
            \LieagbdPartialbar \, \iota_{\basedualxi{\alpha^{'}}}
            +
            \iota_{\basedualxi{\alpha^{'}}}\,\LieagbdPartialbar
            )
            (\basexi{\indexI}\wedge\basedualxi{\indexJp})
            \\
            +
            \\
            \displaystyle\sum_{h=1}^{n}
            \big(
                (\iota_{\basexi{h}} \, \LieagbdPartialbar \basexi{\alpha})
                \wedge
                \iota_{\basedualxi{h^{'}}}(\basexi{\indexI}\wedge\basedualxi{\indexJp})
                -
                (\iota_{\basedualxi{h^{'}}} \, \LieagbdPartialbar \basexi{\alpha})
                \wedge
                \iota_{\basexi{h}}(\basexi{\indexI}\wedge\basedualxi{\indexJp})
            \big)
        \end{pmatrix*}
    .
\end{align*}
Observing that $
(0-\iota_{\basedualxi{h^{'}}}\iota_{\basexi{h}} \, \LieagbdPartialbar \basexi{\alpha})
=
[\LieagbdPartialbar,\iotaW](\basexi{\alpha})
$ and $
(\LieagbdPartialbar \, \iota_{\basedualxi{h}} \, \iota_{\basexi{h}}
-
\iota_{\basedualxi{h^{'}}}\,\iota_{\basexi{h}}\,\LieagbdPartialbar)
=
[\LieagbdPartialbar,\iotaW]
$, we have completed the proof.

\end{proof}

==> 4/For__alpha,_I,_J_,_calculation_for_RHS.tex <==
\begin{lemma}
\label{EQ-Kahler identity on Lie agbd-For (alpha,I,J), calculation for RHS-final target part 2}
$
\sqrt{-1}\LieagbdPartial^{*}
(\basexi{\alpha}\wedge\basexi{\indexI}\wedge\basedualxi{\indexJp})
$ is equal to (a) + (b) + (c) where
\\
    (a):
\begin{align}% The first part
    -2\sqrt{-1}
    \begin{pmatrix*}[l]
        \displaystyle\sum_{\indexic{k}\in\indexIc\backslash\{\alpha\}}
        \begin{matrix*}[l]
            \sgn
                {\order{\indexic{k},\alpha}}
                {\alpha,\indexic{k}}
            \coefD{\indexic{k}}{\order{\indexic{k}, \alpha}}
            \basexi{\indexI}
            \wedge
            \basedualxi{\indexJp}
        \end{matrix*}
        \\
        +
        \\
        \displaystyle\sum_{\indexjpc{l}\in\indexJpc}
        \begin{matrix*}[l]
            (-1)
            \coefB{\indexjpc{l}}{\indexjpc{l} \alpha}
            \basexi{\indexI}
            \wedge
            \basedualxi{\indexJp}
        \end{matrix*}
    \end{pmatrix*}
\label{EQ-Kahler identity on Lie agbd-For (alpha,I,J), calculation for RHS-final target part 1}
\end{align}
\\
    (b):
\begin{align}% The second part
    -2\sqrt{-1}
    \begin{pmatrix*}[l]
        \displaystyle\sum_{\indexic{k}\in\indexIc\backslash\{\alpha\}}
        \displaystyle\sum_{r\in\indexI}
        \begin{matrix*}[l]
            (-1)
            \sgn
                {r,\indexI\backslash\{r\}}
                {\indexI}
            \sgn
                {\order{\indexic{k},r}}
                {r,\indexic{k}}
            \coefD{\indexic{k}}{\order{\indexic{k}, r}}
            \basexi{\alpha}
            \wedge
            \basexi{\indexI\backslash\{r\}}
            \wedge
            \basedualxi{\indexJp}
        \end{matrix*}
        \\
        +
        \\
        \displaystyle\sum_{\indexic{k}\in\indexIc\backslash\{\alpha\}}
        \displaystyle\sum_{r_1\in\indexI}
        \displaystyle\sum_{r_2\in\indexI}
        \begin{matrix*}[l]
            \sgn
                {\order{r_1,r_2},\indexI\backslash\{r_1,r_2\}}
                {\indexI}
            \sgn
                {\order{(\indexI\backslash\{r_1,r_2\})\cup\{\indexic{k}\}}}
                {\indexic{k},(\indexI\backslash\{r_1,r_2\})}
        \\
            \frac{1}{2}
            \coefD{\indexic{k}}{\order{r_1,r_2}}
            \basexi{\alpha}
            \wedge
            \basexi{\order{(\indexI\backslash\{r_1,r_2\})\cup\{\indexic{k}\}}}
            \wedge
            \basedualxi{\indexJp}
        \end{matrix*}
        \\
        +
        \\
        \displaystyle\sum_{\indexjpc{l}\in\indexJpc}
        \displaystyle\sum_{r\in\indexI}
        \begin{matrix*}[l]
            \sgn
                {r,\indexI\backslash\{r\}}
                {\indexI}
            \coefB{\indexjpc{l}}{\indexjpc{l} r}
            \basexi{\alpha}
            \wedge
            \basexi{\indexI\backslash\{r\}}
            \wedge
            \basedualxi{\indexJp}
    \end{matrix*}
        \\
        +
        \\
        \displaystyle\sum_{\indexjpc{l}\in\indexJpc}
        \displaystyle\sum_{r\in\indexI}
        \displaystyle\sum_{u^{'}\in\indexJp}
        \begin{matrix*}[l]    
            (-1)^{p+1}
            \sgn
                {u^{'},r,\indexI\backslash\{r\},\indexJp\backslash\{u^{'}\}}
                {\indexI,\indexJp}
            \sgn
                {\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
                {\indexjpc{l},\indexJp\backslash\{u^{'}\}}
        \\
            \coefB{\indexjpc{l}}{u^{'} r}
            \basexi{\alpha}
            \wedge
            \basexi{\indexI\backslash\{r\}}
            \wedge
            \basedualxi{\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
        \end{matrix*}
    \end{pmatrix*}
\end{align}
\\
    (c): 
\begin{align} %The third part
    -2\sqrt{-1}
    \begin{pmatrix*}[l]
        \displaystyle\sum_{\indexic{k}\in\indexIc\backslash\{\alpha\}}
        \displaystyle\sum_{r\in\indexI}
        \begin{matrix*}[l]
            (-1)
            \sgn
                {r,\indexI\backslash\{r\}}
                {\indexI}
            \sgn
                {\order{(\indexI\backslash\{r\})\cup\{\indexic{k}\}}}
                {\indexic{k},\indexI\backslash\{r\}}
            \sgn
                {\order{\alpha,r}}
                {\alpha,r}
        \\
            \coefD{\indexic{k}}{\order{\alpha, r}}
            \basexi{\order{(\indexI\backslash\{r\})\cup\{\indexic{k}\}}}
            \wedge
            \basedualxi{\indexJp}
        \end{matrix*}
        \\
        +
        \\   
        \displaystyle\sum_{\indexjpc{l}\in\indexJpc}
        \displaystyle\sum_{u^{'}\in\indexJp}
        \begin{matrix*}[l]
            (-1)
            \sgn
                {u^{'},\indexI,\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
                {\indexjpc{l},\indexI,\indexJp}
            \coefB{\indexjpc{l}}{u^{'} \alpha}
            \basexi{\indexI}
            \wedge
            \basedualxi{\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
        \end{matrix*}
    \end{pmatrix*}
    .
\label{EQ-Kahler identity on Lie agbd-For (alpha,I,J), calculation for RHS-final target part 3}
\end{align}
\end{lemma}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
Recall that  $\LieagbdPartial^{*}=-(-1)^{n^{2}}\star\,\LieagbdPartialbar\,\star$. Our calculation comprises four steps:
\begin{enumerate}
    \item Calculate 
$
    \star(\basexi{\alpha}\wedge\basexi{\indexI}\wedge\basedualxi{\indexJp})
$.
    \item Calculate
$
    \LieagbdPartialbar\,\star(\basexi{\alpha}\wedge\basexi{\indexI}\wedge\basedualxi{\indexJp})
$.
    \item Calculate
$
    -(-1)^{n^{2}}\sqrt{-1}\star\,\LieagbdPartialbar\,\star
    (\basexi{\alpha}\wedge\basexi{\indexI}\wedge\basedualxi{\indexJp})
$.
    \item Decompose the result from Step 3 into three parts, where the first part is related to the expression of $
    (\sqrt{-1}\LieagbdPartial^{*}\basexi{\alpha})
    \wedge\basexi{\indexI}\wedge\basedualxi{\indexJp})
    $ and the second part is related to the expression of $
    \basexi{\alpha}\wedge
    \sqrt{-1}\LieagbdPartial^{*}(\basexi{\indexI}\wedge\basedualxi{\indexJp})
    $.
\end{enumerate}
Completing Step 4 gives the formulas in the statement of Lemma \ref{EQ-Kahler identity on Lie agbd-For (alpha,I,J), calculation for RHS-final target part 2}.
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% start Step 1 %%%%%%%%%%%%%%%%%%
\keyword{Step 1:} Using the definition of the Hodge star, we obtain
\begin{align}
    \star
    (\basexi{\alpha}\wedge\basexi{\indexI}\wedge\basedualxi{\indexJp})
    =
    2^{p+1+q-n}
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJc}
    \basedualxi{\indexIc\backslash\{\alpha\}}
    \wedge
    \basexi{\indexJpc},
\label{EQ-For (alpha, I, J), calculation for RHS-Step 1, No1}
\end{align}
where $\{\indexic{1},\cdots,\indexic{n-p}\}=\indexIc$ and $\{\indexjpc{1},\cdots,\indexjpc{n-q}\}=\indexJpc$ are the complement sets of $\indexI$ and $\indexJp$.
%%%%%%%%%%%%%%%%%% finish Step 1 %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% start Step 2 %%%%%%%%%%%%%%%%%%
\keyword{Step 2:}
We apply $\LieagbdPartialbar$ to (\ref{EQ-For (alpha, I, J), calculation for RHS-Step 1, No1}):
\begin{align}
    \LieagbdPartialbar\,\star
    (\basexi{\alpha}\wedge\basexi{\indexI}\wedge\basedualxi{\indexJp})
    =
        2^{p+1+q-n}
        \begin{pmatrix*}[l]
        %%%--1-2-1
        \displaystyle\sum_{\indexic{k}\in\indexIc\backslash\{\alpha\}}
        \begin{matrix*}[l]
            \sgn
                {1,\cdots,n,1^{'},\cdots,n^{'}}
                {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJc}
            \sgn
                {\indexIc\backslash\{\alpha\}}
                {\indexic{k},\indexIc\backslash\{\alpha,\indexic{k}\}}
            \\
            \basedualxi{\indexic{1}}
            \wedge\cdots\wedge
            \LieagbdPartialbar\basedualxi{\indexic{k}}
            \wedge\cdots\wedge
            \widehat{\basedualxi{\alpha}}
            \wedge\cdots\wedge
            \basedualxi{\indexic{n-p}}
            \wedge
            \basexi{\indexJpc}
        \end{matrix*}
        \\
        +
        \\
        %%%--1-2-2
        \displaystyle\sum_{\indexjpc{l}\in\indexJpc}
        \begin{matrix*}[l]
            \sgn
                {1,\cdots,n,1^{'},\cdots,n^{'}}
                {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJc}
            \sgn
                {\indexIc\backslash\{\alpha\},\indexJpc}
                {\indexjpc{l},\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\}}
            \\
            \basedualxi{\indexIc\backslash\{\alpha\}}
            \wedge
            \basexi{\indexjpc{1}}
            \wedge\cdots\wedge
            \LieagbdPartialbar\basexi{\indexjpc{l}}
            \wedge\cdots\wedge
            \basexi{\indexjpc{n-q}}
        \end{matrix*}
    \end{pmatrix*}.
\label{EQ-For (alpha, I, J), calculation for RHS, calculation for RHS-Step 2, No1}
\end{align}
Recalling that 
\begin{align*}
    \LieagbdPartialbar \xi_i
    =
    \sum_{j,k}^n
    \coefB{i}{jk}
    \basexi{j} \wedge \basedualxi{k}
    \qquad\text{and}\qquad
    \LieagbdPartialbar \basedualxi{i}
    =
    \sum_{j<k}^n
    \coefD{i}{jk}
    \basedualxi{j} \wedge \basedualxi{k}
    ,
\end{align*}
we plug these into (\ref{EQ-For (alpha, I, J), calculation for RHS, calculation for RHS-Step 2, No1}) and obtain
\begin{align}
    2^{p+1+q-n}
    \begin{pmatrix*}[l]
        \displaystyle\sum_{\indexic{k}\in\indexIc\backslash\{\alpha\}}
        \begin{pmatrix*}[l]
            \sgn
                {1,\cdots,n,1^{'},\cdots,n^{'}}
                {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJc}
            \sgn
                {\indexIc\backslash\{\alpha\}}
                {\indexic{k},\indexIc\backslash\{\alpha,\indexic{k}\}}
            \\
            \basedualxi{\indexic{1}}
            \wedge\cdots\wedge
            \basedualxi{\indexic{k-1}}\wedge
            \begin{pmatrix*}[l]
                \frac{1}{2}
                (
                \coefD{\indexic{k}}{\indexic{k} \alpha}
                \basedualxi{\indexic{k}}\wedge\basedualxi{\alpha}
                +
                \coefD{\indexic{k}}{\alpha \indexic{k}}
                \basedualxi{\alpha}\wedge\basedualxi{\indexic{k}}
                )
                \\
                +
                \\
                \frac{1}{2}
                \displaystyle\sum_{r \in \indexI}
                \coefD{\indexic{k}}{\indexic{k} r}
                \basedualxi{\indexic{k}}\wedge\basedualxi{r}
                +
                \coefD{\indexic{k}}{r \indexic{k}}
                \basedualxi{r}\wedge\basedualxi{\indexic{k}}
                \\
                +
                \\
                \frac{1}{2}
                \displaystyle\sum_{r \in \indexI}
                \coefD{\indexic{k}}{r \alpha}
                \basedualxi{r}\wedge\basedualxi{\alpha}
                +
                \coefD{\indexic{k}}{\alpha r}
                \basedualxi{\alpha}\wedge\basedualxi{r}
                \\
                +
                \\
                \frac{1}{2}
                \displaystyle\sum_{r_1 \in \indexI}
                \displaystyle\sum_{r_2 \in \indexI}
                \coefD{\indexic{k}}{r_1 r_2}
                \basedualxi{r_1}\wedge\basedualxi{r_2}
            \end{pmatrix*}
            \wedge\basedualxi{\indexic{k+1}}
            \\
            \wedge\cdots\wedge
            \widehat{\basedualxi{\alpha}}
            \wedge\cdots\wedge
            \basedualxi{\indexic{n-p}}
            \wedge
            \basexi{\indexJpc}
        \end{pmatrix*}
        \\
        +
        \\
        \displaystyle\sum_{\indexjpc{l}\in\indexJpc}
        \begin{pmatrix*}[l]
            \sgn
                {1,\cdots,n,1^{'},\cdots,n^{'}}
                {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJc}
            \sgn
                {\indexIc\backslash\{\alpha\},\indexJpc}
                {\indexjpc{l},\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\}}
            \\
            \basedualxi{\indexIc\backslash\{\alpha\}}
            \wedge
            \basexi{\indexjpc{1}}
            \wedge\cdots\wedge
            \basexi{\indexjpc{l-1}}\wedge
            \begin{pmatrix*}[l]
                \coefB{\indexjpc{l}}{\indexjpc{l} \alpha}
                \basexi{\indexjpc{l}}\wedge\basedualxi{\alpha}
                \\
                +
                \\
                \displaystyle\sum_{r\in\indexI}
                \coefB{\indexjpc{l}}{\indexjpc{l} r}
                \basexi{\indexjpc{l}}\wedge\basedualxi{r}
                \\
                +
                \\
                \displaystyle\sum_{u^{'}\in\indexJp}
                \coefB{\indexjpc{l}}{u^{'} \alpha}
                \basexi{u^{'}}\wedge\basedualxi{\alpha}
                \\
                +
                \\
                \displaystyle\sum_{r\in\indexI}
                \displaystyle\sum_{u\in\indexJp}
                \coefB{\indexjpc{l}}{u r}
                \basexi{u}\wedge\basedualxi{r}
            \end{pmatrix*}
            \wedge\basexi{\indexjpc{l+1}}
            \\
            \wedge\cdots\wedge
            \basexi{\indexjpc{n-q}}
        \end{pmatrix*}
    \end{pmatrix*}.
\label{EQ-For (alpha, I, J), calculation for RHS, calculation for RHS-Step 2, No2}
\end{align}


Recall that $\coefD{i}{j k}=-\coefD{i}{k j}$. Let us use the notation
$
    \basedualxi{\order{j k}}=
    \begin{cases}
        \basedualxi{j}\wedge\basedualxi{k}
        \qquad\text{if }j<k
        \\
        \basedualxi{k}\wedge\basedualxi{j}
        \qquad\text{if }k<j
    \end{cases}
$ and obtain the following expression:
\begin{align*}
        \coefD{i}{j k}
        \basedualxi{j}\wedge\basedualxi{k}
    =
        \coefD{i}{k j}
        \basedualxi{k}\wedge\basedualxi{j}
    =  
        \coefD{i}{\order{j k}}
        \basedualxi{\order{j k}}
    .
\end{align*}
Using this trick, we can simplify the terms in (\ref{EQ-For (alpha, I, J), calculation for RHS, calculation for RHS-Step 2, No2}) as follows:
\begin{align*}
    \begin{pmatrix*}[l]
        \frac{1}{2}
        (
        \coefD{\indexic{k}}{\indexic{k} \alpha}
        \basedualxi{\indexic{k}}\wedge\basedualxi{\alpha}
        +
        \coefD{\indexic{k}}{\alpha \indexic{k}}
        \basedualxi{\alpha}\wedge\basedualxi{\indexic{k}}
        )
        \\
        +
        \\
        \frac{1}{2}
        \displaystyle\sum_{r \in \indexI}
        \coefD{\indexic{k}}{\indexic{k} r}
        \basedualxi{\indexic{k}}\wedge\basedualxi{r}
        +
        \coefD{\indexic{k}}{r \indexic{k}}
        \basedualxi{r}\wedge\basedualxi{\indexic{k}}
        \\
        +
        \\
        \frac{1}{2}
        \displaystyle\sum_{r \in \indexI}
        \coefD{\indexic{k}}{r \alpha}
        \basedualxi{r}\wedge\basedualxi{\alpha}
        +
        \coefD{\indexic{k}}{\alpha r}
        \basedualxi{\alpha}\wedge\basedualxi{r}
        \\
        +
        \\
        \frac{1}{2}
        \displaystyle\sum_{r_1 \in \indexI}
        \displaystyle\sum_{r_2 \in \indexI}
        \coefD{\indexic{k}}{r_1 r_2}
        \basedualxi{r_1}\wedge\basedualxi{r_2}
    \end{pmatrix*}
    =
    \begin{pmatrix*}[l]
        \coefD{\indexic{k}}{\order{\indexic{k} \alpha}}
        \basedualxi{\order{\indexic{k} \alpha}}
        \\
        +
        \\
        \displaystyle\sum_{r \in \indexI}
        \coefD{\indexic{k}}{\order{\indexic{k} r}}
        \basedualxi{\order{\indexic{k} r}}
        \\
        +
        \\
        \displaystyle\sum_{r \in \indexI}
        \coefD{\indexic{k}}{\order{r \alpha}}
        \basedualxi{\order{r \alpha}}
        \\
        +
        \\
        \frac{1}{2}
        \displaystyle\sum_{r_1 \in \indexI}
        \displaystyle\sum_{r_2 \in \indexI}
        \coefD{\indexic{k}}{\order{r_1 r_2}}
        \basedualxi{\order{r_1 r_2}}
    \end{pmatrix*}.
\end{align*}


Next, we rearrange the terms in (\ref{EQ-For (alpha, I, J), calculation for RHS, calculation for RHS-Step 2, No2}). The calculation for ordering the wedge product of frames is as follows. In the first parenthesis, we have:
\begin{itemize}
    \item %1
$
    \quad
        \basedualxi{\indexic{1}}
        \wedge\cdots\wedge
        \basedualxi{\indexic{k-1}}\wedge
        \coefD{\indexic{k}}{\order{\indexic{k} \alpha}}
        \basedualxi{\order{\indexic{k} \alpha}}
        \wedge\basedualxi{\indexic{k+1}}
        \wedge\cdots\wedge
        \widehat{\basedualxi{\alpha}}
        \wedge\cdots\wedge
        \basedualxi{\indexic{n-p}}
        \wedge
        \basexi{\indexJpc}
    \\
    =
        \sgn
            {\indexic{1},\cdots,\indexic{k-1},\order{\indexic{k},\alpha},\indexic{k+1},\cdots,\indexic{n-p}}
            {\indexIc}
        \coefD{\indexic{k}}{\order{\indexic{k}, \alpha}}
        \basedualxi{\indexIc}
        \wedge
        \basexi{\indexJpc}
$,

    \item %2
$
    \quad
        \basedualxi{\indexic{1}}
        \wedge\cdots\wedge
        \basedualxi{\indexic{k-1}}\wedge
            \coefD{\indexic{k}}{\order{\indexic{k} r}}
            \basedualxi{\order{\indexic{k} r}}
        \wedge\basedualxi{\indexic{k+1}}
        \wedge\cdots\wedge
        \widehat{\basedualxi{\alpha}}
        \wedge\cdots\wedge
        \basedualxi{\indexic{n-p}}
        \wedge
        \basexi{\indexJpc}
    \\
    =
        \sgn
            {\indexic{1},\cdots,\indexic{k-1},\order{\indexic{k},r},\indexic{k+1},\cdots,\widehat{\alpha},\cdots,\indexic{n-p}}
            {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}}}
        \coefD{\indexic{k}}{\order{\indexic{k}, r}}
        \basedualxi{\order{(\indexIc\backslash\{\alpha\})\cup\{r\}}}
        \wedge
        \basexi{\indexJpc}
$,
    \item %3
$
    \quad
        \basedualxi{\indexic{1}}
        \wedge\cdots\wedge
        \basedualxi{\indexic{k-1}}\wedge
            \coefD{\indexic{k}}{\order{r \alpha}}
            \basedualxi{\order{r \alpha}}
        \wedge\basedualxi{\indexic{k+1}}
        \wedge\cdots\wedge
        \widehat{\basedualxi{\alpha}}
        \wedge\cdots\wedge
        \basedualxi{\indexic{n-p}}
        \wedge
        \basexi{\indexJpc}
    \\
    =
        \sgn
            {\indexic{1},\cdots,\indexic{k-1},\order{\alpha,r},\indexic{k+1},\cdots,\indexic{n-p}}
            {\order{(\indexIc\backslash\{\indexic{k}\})\cup\{r\}}}
        \coefD{\indexic{k}}{\order{\alpha, r}}
        \basedualxi{\order{(\indexIc\backslash\{\indexic{k}\})\cup\{r\}}}
        \wedge
        \basexi{\indexJpc}
$,
    \item %4
$
    \quad
        \basedualxi{\indexic{1}}
        \wedge\cdots\wedge
        \basedualxi{\indexic{k-1}}\wedge
        \frac{1}{2}
            \coefD{\indexic{k}}{\order{r_1 r_2}}
            \basedualxi{\order{r_1 r_2}}
        \wedge\basedualxi{\indexic{k+1}}
        \wedge\cdots\wedge
        \widehat{\basedualxi{\alpha}}
        \wedge\cdots\wedge
        \basedualxi{\indexic{n-p}}
        \wedge
        \basexi{\indexJpc}
    \\
    =
        \sgn
            {\indexic{1},\cdots,\indexic{k-1},\order{r_1,r_2},\indexic{k+1},\cdots,\widehat{\alpha},\cdots,\indexic{n-p}}
            {\order{(\indexIc\backslash\{\indexic{k},\alpha\})\cup\{r_1,r_2\}}}
        \frac{1}{2}
        \coefD{\indexic{k}}{\order{r_1,r_2}}
        \basedualxi{\order{(\indexIc\backslash\{\indexic{k},\alpha\})\cup\{r_1,r_2\}}}
        \wedge
        \basexi{\indexJpc}
$.
\end{itemize}
In the second parenthesis, we have:
\begin{itemize}
    \item %5
$
    \quad
        \basedualxi{\indexIc\backslash\{\alpha\}}
        \wedge
        \basexi{\indexjpc{1}}
        \wedge\cdots\wedge
        \basexi{\indexjpc{l-1}}\wedge
            \coefB{\indexjpc{l}}{\indexjpc{l} \alpha}
            \basexi{\indexjpc{l}}\wedge\basedualxi{\alpha}
        \wedge\basexi{\indexjpc{l+1}}
        \wedge\cdots\wedge
        \basexi{\indexjpc{n-q}}
    \\
    =
        \sgn
            {\indexIc\backslash\{\alpha\},\indexjpc{1},\cdots,\indexjpc{l-1},\indexjpc{l},\alpha,\indexjpc{l+1},\cdots,\indexjpc{n-q}}
            {\indexIc,\indexJpc}
        \coefB{\indexjpc{l}}{\indexjpc{l} \alpha}
        \basedualxi{\indexIc}
        \wedge
        \basexi{\indexJpc}
$,
    \item %6
$
    \quad
        \basedualxi{\indexIc\backslash\{\alpha\}}
        \wedge
        \basexi{\indexjpc{1}}
        \wedge\cdots\wedge
        \basexi{\indexjpc{l-1}}\wedge
            \coefB{\indexjpc{l}}{\indexjpc{l} r}
            \basexi{\indexjpc{l}}\wedge\basedualxi{r}
        \wedge\basexi{\indexjpc{l+1}}
        \wedge\cdots\wedge
        \basexi{\indexjpc{n-q}}
    \\
    =
        \sgn
            {\indexIc\backslash\{\alpha\},\indexjpc{1},\cdots,\indexjpc{l-1},\indexjpc{l},r,\indexjpc{l+1},\cdots,\indexjpc{n-q}}
            {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}},\indexJpc}
        \coefB{\indexjpc{l}}{\indexjpc{l} r}
        \basedualxi{\order{(\indexIc\backslash\{\alpha\})\cup\{r\}}}
        \wedge
        \basexi{\indexJpc}
$,
    \item %7
$
    \quad
        \basedualxi{\indexIc\backslash\{\alpha\}}
        \wedge
        \basexi{\indexjpc{1}}
        \wedge\cdots\wedge
        \basexi{\indexjpc{l-1}}\wedge
            \coefB{\indexjpc{l}}{u^{'} \alpha}
            \basexi{u^{'}}\wedge\basedualxi{\alpha}
        \wedge\basexi{\indexjpc{l+1}}
        \wedge\cdots\wedge
        \basexi{\indexjpc{n-q}}
    \\
    =   
        \sgn
            {\indexIc\backslash\{\alpha\},\indexjpc{1},\cdots,\indexjpc{l-1},u^{'},\alpha,\indexjpc{l+1},\cdots,\indexjpc{n-q}}
            {\indexIc,\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}}}
        \coefB{\indexjpc{l}}{u^{'} \alpha}
        \basedualxi{\indexIc}
        \wedge
        \basexi{\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}}}
$,
    \item 
$
    \quad
        \basedualxi{\indexIc\backslash\{\alpha\}}
        \wedge
        \basexi{\indexjpc{1}}
        \wedge\cdots\wedge
        \basexi{\indexjpc{l-1}}\wedge
            \coefB{\indexjpc{l}}{u r}
            \basexi{u}\wedge\basedualxi{r}
        \wedge\basexi{\indexjpc{l+1}}
        \wedge\cdots\wedge
        \basexi{\indexjpc{n-q}}
    \\
    =
        \sgn
            {\indexIc\backslash\{\alpha\},\indexjpc{1},\cdots,\indexjpc{l-1},u^{'},r,\indexjpc{l+1},\cdots,\indexjpc{n-q}}
            {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}},\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}}}
        \coefB{\indexjpc{l}}{u^{'} r}
        \basedualxi{\order{(\indexIc\backslash\{\alpha\})\cup\{r\}}}
        \wedge
        \basexi{\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}}}
$.
\end{itemize}


We conclude that $
\LieagbdPartialbar\,\star
(\basexi{\alpha}\wedge\basexi{\indexI}\wedge\basedualxi{\indexJp})
$ is equal to
\begin{align}
    %%%#1
    &
    2^{p+1+q-n}
    \displaystyle\sum_{\indexic{k}\in\indexIc\backslash\{\alpha\}}
    \begin{pmatrix*}[l]
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJc}
        \sgn
            {\indexIc\backslash\{\alpha\}}
            {\indexic{k},\indexIc\backslash\{\alpha,\indexic{k}\}}
        \sgn
            {\indexic{1},\cdots,\indexic{k-1},\order{\indexic{k},\alpha},\indexic{k+1},\cdots,\indexic{n-p}}
            {\indexIc}
        \\
        \coefD{\indexic{k}}{\order{\indexic{k}, \alpha}}
        \basedualxi{\indexIc}
        \wedge
        \basexi{\indexJpc}
    \end{pmatrix*}
\label{EQ-For (alpha, I, J), calculation for RHS, calculation for RHS-Step 2, result-term 1}
    \\
    &+\notag
    \\
    %%%#2
    &
    2^{p+1+q-n}
    \displaystyle\sum_{\indexic{k}\in\indexIc\backslash\{\alpha\}}
    \displaystyle\sum_{r\in\indexI}
    \begin{pmatrix*}[l]
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJc}
        \sgn
            {\indexIc\backslash\{\alpha\}}
            {\indexic{k},\indexIc\backslash\{\alpha,\indexic{k}\}}
        \\
        \sgn
            {\indexic{1},\cdots,\indexic{k-1},\order{\indexic{k},r},\indexic{k+1},\cdots,\widehat{\alpha},\cdots,\indexic{n-p}}
            {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}}}
        \\
        \coefD{\indexic{k}}{\order{\indexic{k}, r}}
        \basedualxi{\order{(\indexIc\backslash\{\alpha\})\cup\{r\}}}
        \wedge
        \basexi{\indexJpc}
    \end{pmatrix*}
\label{EQ-For (alpha, I, J), calculation for RHS, calculation for RHS-Step 2, result-term 2}
    \\
    &+\notag
    \\
    %%%#3
    &
    2^{p+1+q-n}
    \displaystyle\sum_{\indexic{k}\in\indexIc\backslash\{\alpha\}}
    \displaystyle\sum_{r\in\indexI}
    \begin{pmatrix*}[l]
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJc}
        \sgn
            {\indexIc\backslash\{\alpha\}}
            {\indexic{k},\indexIc\backslash\{\alpha,\indexic{k}\}}
        \\
        \sgn
            {\indexic{1},\cdots,\indexic{k-1},\order{\alpha,r},\indexic{k+1},\cdots,\indexic{n-p}}
            {\order{(\indexIc\backslash\{\indexic{k}\})\cup\{r\}}}
        \\
        \coefD{\indexic{k}}{\order{\alpha, r}}
        \basedualxi{\order{(\indexIc\backslash\{\indexic{k}\})\cup\{r\}}}
        \wedge
        \basexi{\indexJpc}
    \end{pmatrix*}
\label{EQ-For (alpha, I, J), calculation for RHS, calculation for RHS-Step 2, result-term 3}
    \\
    &+\notag
    \\
    %%%#4
    &
    2^{p+1+q-n}
    \displaystyle\sum_{\indexic{k}\in\indexIc\backslash\{\alpha\}}
    \displaystyle\sum_{r_1\in\indexI}
    \displaystyle\sum_{r_2\in\indexI}
    \begin{pmatrix*}[l]
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJc}
        \sgn
            {\indexIc\backslash\{\alpha\}}
            {\indexic{k},\indexIc\backslash\{\alpha,\indexic{k}\}}
        \\
        \sgn
            {\indexic{1},\cdots,\indexic{k-1},\order{r_1,r_2},\indexic{k+1},\cdots,\widehat{\alpha},\cdots,\indexic{n-p}}
            {\order{(\indexIc\backslash\{\indexic{k},\alpha\})\cup\{r_1,r_2\}}}
        \\
        \frac{1}{2}
        \coefD{\indexic{k}}{\order{r_1,r_2}}
        \basedualxi{\order{(\indexIc\backslash\{\indexic{k},\alpha\})\cup\{r_1,r_2\}}}
        \wedge
        \basexi{\indexJpc}
    \end{pmatrix*}
\label{EQ-For (alpha, I, J), calculation for RHS, calculation for RHS-Step 2, result-term 4}
    \\
    &+\notag
    \\
    %%%#5
    &
    2^{p+1+q-n}
    \displaystyle\sum_{\indexjpc{l}\in\indexJpc}
    \begin{pmatrix*}[l]
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJc}
        \sgn
            {\indexIc\backslash\{\alpha\},\indexJpc}
            {\indexjpc{l},\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\}}
        \\
        \sgn
            {\indexIc\backslash\{\alpha\},\indexjpc{1},\cdots,\indexjpc{l-1},\indexjpc{l},\alpha,\indexjpc{l+1},\cdots,\indexjpc{n-q}}
            {\indexIc,\indexJpc}
        \\
        \coefB{\indexjpc{l}}{\indexjpc{l} \alpha}
        \basedualxi{\indexIc}
        \wedge
        \basexi{\indexJpc}
    \end{pmatrix*}
\label{EQ-For (alpha, I, J), calculation for RHS, calculation for RHS-Step 2, result-term 5}
    \\
    &+\notag
    \\
    %%%#6
    &
    2^{p+1+q-n}
    \displaystyle\sum_{\indexjpc{l}\in\indexJpc}
    \displaystyle\sum_{r\in\indexI}
    \begin{pmatrix*}[l]
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJc}
        \sgn
            {\indexIc\backslash\{\alpha\},\indexJpc}
            {\indexjpc{l},\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\}}
        \\
        \sgn
            {\indexIc\backslash\{\alpha\},\indexjpc{1},\cdots,\indexjpc{l-1},\indexjpc{l},r,\indexjpc{l+1},\cdots,\indexjpc{n-q}}
            {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}},\indexJpc}
        \\
        \coefB{\indexjpc{l}}{\indexjpc{l} r}
        \basedualxi{\order{(\indexIc\backslash\{\alpha\})\cup\{r\}}}
        \wedge
        \basexi{\indexJpc}
    \end{pmatrix*}
\label{EQ-For (alpha, I, J), calculation for RHS, calculation for RHS-Step 2, result-term 6}
    \\
    &+\notag
    \\
    %%%#7
    &
    2^{p+1+q-n}
    \displaystyle\sum_{\indexjpc{l}\in\indexJpc}
    \displaystyle\sum_{u^{'}\in\indexJp}
    \begin{pmatrix*}[l]
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJc}
        \sgn
            {\indexIc\backslash\{\alpha\},\indexJpc}
            {\indexjpc{l},\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\}}
        \\
        \sgn
            {\indexIc\backslash\{\alpha\},\indexjpc{1},\cdots,\indexjpc{l-1},u^{'},\alpha,\indexjpc{l+1},\cdots,\indexjpc{n-q}}
            {\indexIc,\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}}}
        \\
        \coefB{\indexjpc{l}}{u^{'} \alpha}
        \basedualxi{\indexIc}
        \wedge
        \basexi{\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}}}
    \end{pmatrix*}
\label{EQ-For (alpha, I, J), calculation for RHS, calculation for RHS-Step 2, result-term 7}
    \\
    &+\notag
    \\
    %%%#8
    &
    2^{p+1+q-n}
    \displaystyle\sum_{\indexjpc{l}\in\indexJpc}
    \displaystyle\sum_{r\in\indexI}
    \displaystyle\sum_{u^{'}\in\indexJp}
    \begin{pmatrix*}[l]
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJc}
        \sgn
            {\indexIc\backslash\{\alpha\},\indexJpc}
            {\indexjpc{l},\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\}}
        \\
        \sgn
            {\indexIc\backslash\{\alpha\},\indexjpc{1},\cdots,\indexjpc{l-1},u^{'},r,\indexjpc{l+1},\cdots,\indexjpc{n-q}}
            {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}},\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}}}
        \\
        \coefB{\indexjpc{l}}{u^{'} r}
        \basedualxi{\order{(\indexIc\backslash\{\alpha\})\cup\{r\}}}
        \wedge
        \basexi{\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}}}
    \end{pmatrix*}
    .
\label{EQ-For (alpha, I, J), calculation for RHS, calculation for RHS-Step 2, result-term 8}
\end{align}
%%%%%%%%%%%%%% finish step 2 %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% start step 3 %%%%%%%%%%%%%%
\keyword{Step 3:}
Recall that
\begin{align*}
    \star
    (\basedualxi{\indexIc}\wedge\basexi{\indexJpc})
    =
    2^{(|\indexIc|+|\indexJpc|-n)}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}{\indexIc,\indexJpc,\indexI,\indexJp}\basexi{\indexI}\wedge\basedualxi{\indexJp}.
\end{align*}
Let us take $\star$ on $
\LieagbdPartialbar\,\star
(\basexi{\alpha}\wedge\basexi{\indexI}\wedge\basedualxi{\indexJp})
$. Each term in $
\LieagbdPartialbar\,\star
(\basexi{\alpha}\wedge\basexi{\indexI}\wedge\basedualxi{\indexJp})
$ is as follows: 
\begin{itemize}
    %%%% 1
    \item applying $\star$ to (\ref{EQ-For (alpha, I, J), calculation for RHS, calculation for RHS-Step 2, result-term 1}), we calculate
\begin{align*}
        \star
        (\basedualxi{\indexIc}\wedge\basexi{\indexJpc})
    =
        2^{n-p-q}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\indexIc,\indexJpc,\indexI,\indexJp}
        \basexi{\indexI}\wedge\basedualxi{\indexJp}
    ;
\end{align*}  

    %%%% 2
    \item applying $\star$ to (\ref{EQ-For (alpha, I, J), calculation for RHS, calculation for RHS-Step 2, result-term 2}), we calculate
\begin{align*}
        \star
        (
        \basedualxi{\order{(\indexIc\backslash\{\alpha\})\cup\{r\}}}
        \wedge
        \basexi{\indexJpc}
        )
    =
        2^{n-p-q}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}},\indexJpc,\alpha,\indexI\backslash\{r\},\indexJp}
        \basexi{\alpha}
        \wedge
        \basexi{\indexI\backslash\{r\}}
        \wedge
        \basedualxi{\indexJp}
    ,
\end{align*}
    where $\basexi{\alpha}$ is at the head of the wedge product of frames since we use the assumption that $\alpha<\indexi{1}$;

    %%%% 3
    \item applying $\star$ to (\ref{EQ-For (alpha, I, J), calculation for RHS, calculation for RHS-Step 2, result-term 3}), we calculate
\begin{align*}
    &
        \star
        (
        \basedualxi{\order{(\indexIc\backslash\{\indexic{k}\})\cup\{r\}}}
        \wedge
        \basexi{\indexJpc}
        )
    \\
    =&
        2^{n-p-q}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\order{(\indexIc\backslash\{\indexic{k}\})\cup\{r\}},\indexJpc,\order{(\indexI\backslash\{r\})\cup\{\indexic{k}\}},\indexJp}
        \basexi{\order{(\indexI\backslash\{r\})\cup\{\indexic{k}\}}}
        \wedge
        \basedualxi{\indexJp}
    ;
\end{align*}  

    %%%% 4
    \item applying $\star$ to (\ref{EQ-For (alpha, I, J), calculation for RHS, calculation for RHS-Step 2, result-term 4}), we calculate
\begin{align*}
    &
        \star
        (
        \basedualxi{\order{(\indexIc\backslash\{\indexic{k},\alpha\})\cup\{r_1,r_2\}}}
        \wedge
        \basexi{\indexJpc}
        )
    \\
    =&
        2^{n-p-q}
        \begin{pmatrix*}[l]
            \sgn
                {1^{'},\cdots,n^{'},1,\cdots,n}
                {\order{(\indexIc\backslash\{\indexic{k},\alpha\})\cup\{r_1,r_2\}},\indexJpc,\alpha,\order{(\indexI\backslash\{r_1,r_2\})\cup\{\indexic{k}\}},\indexJp} 
            \\
            \basexi{\alpha}
            \wedge
            \basexi{\order{(\indexI\backslash\{r_1,r_2\})\cup\{\indexic{k}\}}}
            \wedge
            \basedualxi{\indexJp}
        \end{pmatrix*}
    ;
\end{align*}  
    
    %%%% 5
    \item applying $\star$ to (\ref{EQ-For (alpha, I, J), calculation for RHS, calculation for RHS-Step 2, result-term 5}), we calculate
\begin{align*}
        \star
        (
        \basedualxi{\indexIc}
        \wedge
        \basexi{\indexJpc}
        )
    =
        2^{n-p-q}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\indexIc,\indexJpc,\indexI,\indexJp}
        \basexi{\indexI}
        \wedge
        \basedualxi{\indexJp}
    ;
\end{align*}  
    
    %%%% 6
    \item applying $\star$ to (\ref{EQ-For (alpha, I, J), calculation for RHS, calculation for RHS-Step 2, result-term 6}), we calculate
\begin{align*}
        \star
        (
        \basedualxi{\order{(\indexIc\backslash\{\alpha\})\cup\{r\}}}
        \wedge
        \basexi{\indexJpc}
        )
    =
        2^{n-p-q}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}},\indexJpc,\alpha,\indexI\backslash\{r\},\indexJp}
        \basexi{\alpha}
        \wedge
        \basexi{\indexI\backslash\{r\}}
        \wedge
        \basedualxi{\indexJp}
    ,
\end{align*}  
    where $\basexi{\alpha}$ is at the head of the wedge product of frames since we use the assumption that $\alpha<\indexi{1}$;
    
    %%%% 7
    \item applying $\star$ to (\ref{EQ-For (alpha, I, J), calculation for RHS, calculation for RHS-Step 2, result-term 7}), we calculate
\begin{align*}
    &
        \star
        (
        \basedualxi{\indexIc}
        \wedge
        \basexi{\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}}}
        )
    \\
    =&
        2^{n-p-q}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\indexIc,\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}},\indexI,\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
        \basexi{\indexI}
        \wedge
        \basedualxi{\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
    ;
\end{align*}  
    
    %%%% 8
    \item applying $\star$ to (\ref{EQ-For (alpha, I, J), calculation for RHS, calculation for RHS-Step 2, result-term 8}), we calculate
\begin{align*}
    &
        \star
        (
        \basedualxi{\order{(\indexIc\backslash\{\alpha\})\cup\{r\}}}
        \wedge
        \basexi{\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}}}
        )
    \\
    =&
        2^{n-p-q}
        \begin{pmatrix*}
            \sgn
                {1^{'},\cdots,n^{'},1,\cdots,n}
                {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}},\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}},\alpha,\indexI\backslash\{r\},\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
            \\
            \basexi{\alpha}
            \wedge
            \basexi{\indexI\backslash\{r\}}
            \wedge
            \basedualxi{\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
        \end{pmatrix*}
    ,
\end{align*}  
    where $\basexi{\alpha}$ is at the head of the wedge product of frames since we use the assumption that $\alpha<\indexi{1}$.
\end{itemize}


Recall that 
\begin{align*}
    \sqrt{-1}\LieagbdPartial^{*}(\basexi{\alpha}\wedge\basexi{\indexI}\wedge\basedualxi{\indexJp})
    =
    -\sqrt{-1}(-1)^{n^2}
    \star\,\LieagbdPartialbar\,\star
    (\basexi{\alpha}\wedge\basexi{\indexI}\wedge\basedualxi{\indexJp})
    .
\end{align*}
As we have already applied $\star$ to each term in $
\LieagbdPartialbar\,\star
(\basexi{\alpha}\wedge\basexi{\indexI}\wedge\basedualxi{\indexJp})
$, we just need to multiply by $-\sqrt{-1}(-1)^{n^2}$ to obtain the expression of $
\sqrt{-1}\LieagbdPartial^{*}
(\basexi{\alpha}\wedge\basexi{\indexI}\wedge\basedualxi{\indexJp})
$:
\begin{align}
    %%%#1
    &
    % -2\sqrt{-1}(-1)^{n^2}
    % \displaystyle\sum_{\indexic{k}\in\indexIc\backslash\{\alpha\}}
    \begin{pmatrix*}[l]
        -2\sqrt{-1}(-1)^{n^2}
        \displaystyle\sum_{\indexic{k}\in\indexIc\backslash\{\alpha\}}
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJc}
        \sgn
            {\indexIc\backslash\{\alpha\}}
            {\indexic{k},\indexIc\backslash\{\alpha,\indexic{k}\}}
        \\
        \sgn
            {\indexic{1},\cdots,\indexic{k-1},\order{\indexic{k},\alpha},\indexic{k+1},\cdots,\indexic{n-p}}
            {\indexIc}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\indexIc,\indexJpc,\indexI,\indexJp}
        \coefD{\indexic{k}}{\order{\indexic{k}, \alpha}}
        \basexi{\indexI}
        \wedge
        \basedualxi{\indexJp}
    \end{pmatrix*}
\label{EQ-For (alpha, I, J), calculation for RHS-Step 3, unsimplfied term 1}
    \\
    &+
    \notag\\
    %%%#2
    &
    \begin{pmatrix*}[l]
        -2\sqrt{-1}(-1)^{n^2}
        \displaystyle\sum_{\indexic{k}\in\indexIc\backslash\{\alpha\}}
        \displaystyle\sum_{r\in\indexI}
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJc}
        \sgn
            {\indexIc\backslash\{\alpha\}}
            {\indexic{k},\indexIc\backslash\{\alpha,\indexic{k}\}}
        \\
        \sgn
            {\indexic{1},\cdots,\indexic{k-1},\order{\indexic{k},r},\indexic{k+1},\cdots,\widehat{\alpha},\cdots,\indexic{n-p}}
            {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}}}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}},\indexJpc,\alpha,\indexI\backslash\{r\},\indexJp}
        \coefD{\indexic{k}}{\order{\indexic{k}, r}}
        \\
        \basexi{\alpha}
        \wedge
        \basexi{\indexI\backslash\{r\}}
        \wedge
        \basedualxi{\indexJp}
    \end{pmatrix*}
\label{EQ-For (alpha, I, J), calculation for RHS-Step 3, unsimplfied term 2}
    \\
    &+
    \notag\\
    %%%#3
    &
    \begin{pmatrix*}[l]
        -2\sqrt{-1}(-1)^{n^2}
        \displaystyle\sum_{\indexic{k}\in\indexIc\backslash\{\alpha\}}
        \displaystyle\sum_{r\in\indexI}
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJc}
        \sgn
            {\indexIc\backslash\{\alpha\}}
            {\indexic{k},\indexIc\backslash\{\alpha,\indexic{k}\}}
        \\
        \sgn
            {\indexic{1},\cdots,\indexic{k-1},\order{\alpha,r},\indexic{k+1},\cdots,\indexic{n-p}}
            {\order{(\indexIc\backslash\{\indexic{k}\})\cup\{r\}}}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\order{(\indexIc\backslash\{\indexic{k}\})\cup\{r\}},\indexJpc,\order{(\indexI\backslash\{r\})\cup\{\indexic{k}\}},\indexJp}
        \\
        \coefD{\indexic{k}}{\order{\alpha, r}}
        \basexi{\order{(\indexI\backslash\{r\})\cup\{\indexic{k}\}}}
        \wedge
        \basedualxi{\indexJp}
    \end{pmatrix*}
\label{EQ-For (alpha, I, J), calculation for RHS-Step 3, unsimplfied term 3}
    \\
    &+
    \notag\\
    &
    %%%#4
    \begin{pmatrix*}[l]
        -2\sqrt{-1}(-1)^{n^2}
        \displaystyle\sum_{\indexic{k}\in\indexIc\backslash\{\alpha\}}
        \displaystyle\sum_{r_1\in\indexI}
        \displaystyle\sum_{r_2\in\indexI}
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJc}
        \sgn
            {\indexIc\backslash\{\alpha\}}
            {\indexic{k},\indexIc\backslash\{\alpha,\indexic{k}\}}
        \\
        \sgn
            {\indexic{1},\cdots,\indexic{k-1},\order{r_1,r_2},\indexic{k+1},\cdots,\widehat{\alpha},\cdots,\indexic{n-p}}
            {\order{(\indexIc\backslash\{\indexic{k},\alpha\})\cup\{r_1,r_2\}}}
        \\
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\order{(\indexIc\backslash\{\indexic{k},\alpha\})\cup\{r_1,r_2\}},\indexJpc,\alpha,\order{(\indexI\backslash\{r_1,r_2\})\cup\{\indexic{k}\}},\indexJp} 
        \\
        \frac{1}{2}
        \coefD{\indexic{k}}{\order{r_1,r_2}}
        \basexi{\alpha}
        \wedge
        \basexi{\order{(\indexI\backslash\{r_1,r_2\})\cup\{\indexic{k}\}}}
        \wedge
        \basedualxi{\indexJp}
    \end{pmatrix*}
\label{EQ-For (alpha, I, J), calculation for RHS-Step 3, unsimplfied term 4}
    \\
    &+
    \notag\\
    &
    %%%#5
    \begin{pmatrix*}[l]
        -2\sqrt{-1}(-1)^{n^2}
        \displaystyle\sum_{\indexjpc{l}\in\indexJpc}
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJc}
        \sgn
            {\indexIc\backslash\{\alpha\},\indexJpc}
            {\indexjpc{l},\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\}}
        \\
        \sgn
            {\indexIc\backslash\{\alpha\},\indexjpc{1},\cdots,\indexjpc{l-1},\indexjpc{l},\alpha,\indexjpc{l+1},\cdots,\indexjpc{n-q}}
            {\indexIc,\indexJpc}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\indexIc,\indexJpc,\indexI,\indexJp}
        \coefB{\indexjpc{l}}{\indexjpc{l} \alpha}
        \basexi{\indexI}
        \wedge
        \basedualxi{\indexJp}
    \end{pmatrix*}
\label{EQ-For (alpha, I, J), calculation for RHS-Step 3, unsimplfied term 5}
    \\
    &+
    \notag\\
    &
    %%%#6
    \begin{pmatrix*}[l]
        -2\sqrt{-1}(-1)^{n^2}
        \displaystyle\sum_{\indexjpc{l}\in\indexJpc}
        \displaystyle\sum_{r\in\indexI}
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJc}
        \sgn
            {\indexIc\backslash\{\alpha\},\indexJpc}
            {\indexjpc{l},\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\}}
        \\
        \sgn
            {\indexIc\backslash\{\alpha\},\indexjpc{1},\cdots,\indexjpc{l-1},\indexjpc{l},r,\indexjpc{l+1},\cdots,\indexjpc{n-q}}
            {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}},\indexJpc}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}},\indexJpc,\alpha,\indexI\backslash\{r\},\indexJp}
        \\
        \coefB{\indexjpc{l}}{\indexjpc{l} r}
        \basexi{\alpha}
        \wedge
        \basexi{\indexI\backslash\{r\}}
        \wedge
        \basedualxi{\indexJp}
    \end{pmatrix*}
\label{EQ-For (alpha, I, J), calculation for RHS-Step 3, unsimplfied term 6}
    \\
    &+
    \notag\\
    &
    %%%#7
    \begin{pmatrix*}[l]
        -2\sqrt{-1}(-1)^{n^2}
        \displaystyle\sum_{\indexjpc{l}\in\indexJpc}
        \displaystyle\sum_{u^{'}\in\indexJp}
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJc}
        \sgn
            {\indexIc\backslash\{\alpha\},\indexJpc}
            {\indexjpc{l},\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\}}
        \\
        \sgn
            {\indexIc\backslash\{\alpha\},\indexjpc{1},\cdots,\indexjpc{l-1},u^{'},\alpha,\indexjpc{l+1},\cdots,\indexjpc{n-q}}
            {\indexIc,\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}}}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\indexIc,\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}},\indexI,\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
        \\
        \coefB{\indexjpc{l}}{u^{'} \alpha}
        \basexi{\indexI}
        \wedge
        \basedualxi{\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
    \end{pmatrix*}
\label{EQ-For (alpha, I, J), calculation for RHS-Step 3, unsimplfied term 7}
    \\
    &+
    \notag\\
    &
    %%%#8
    \begin{pmatrix*}[l]
        -2\sqrt{-1}(-1)^{n^2}
        \displaystyle\sum_{\indexjpc{l}\in\indexJpc}
        \displaystyle\sum_{r\in\indexI}
        \displaystyle\sum_{u^{'}\in\indexJp}
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJc}
        \sgn
            {\indexIc\backslash\{\alpha\},\indexJpc}
            {\indexjpc{l},\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\}}
        \\
        \sgn
            {\indexIc\backslash\{\alpha\},\indexjpc{1},\cdots,\indexjpc{l-1},u^{'},r,\indexjpc{l+1},\cdots,\indexjpc{n-q}}
            {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}},\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}}}
        \\
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}},\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}},\alpha,\indexI\backslash\{r\},\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
        \\
        \coefB{\indexjpc{l}}{u^{'} r}
        \basexi{\alpha}
        \wedge
        \basexi{\indexI\backslash\{r\}}
        \wedge
        \basedualxi{\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
    \end{pmatrix*}.
\label{EQ-For (alpha, I, J), calculation for RHS-Step 3, unsimplfied term 8}
\end{align}
We simplify the sign of permutations in Section \ref{apex-simplification for RHs of (alpha,I,J)}. The reader can check Lemmas \ref{Lemma-simplification for RHS of (alpha,I,J)-lemma 1}–\ref{Lemma-simplification for RHS of (alpha,I,J)-lemma 8} for details. Thus, we conclude that the simplified expression of $
\sqrt{-1}\LieagbdPartial^{*}
(\basedualxi{\indexIc}\wedge\basexi{\indexJpc})
$ is
\begin{align}
    %%%#1
    &
    -2\sqrt{-1}(-1)^{n^2}
    \displaystyle\sum_{\indexic{k}\in\indexIc\backslash\{\alpha\}}
    \begin{matrix*}[l]
        (-1)^{n^2}
        \sgn
            {\order{\indexic{k},\alpha}}
            {\alpha,\indexic{k}}
        \coefD{\indexic{k}}{\order{\indexic{k}, \alpha}}
        \basexi{\indexI}
        \wedge
        \basedualxi{\indexJp}
    \end{matrix*}
\label{EQ-Kahler identity on Lie agbd-For (alpha,I,J), calculation for RHS-simplified half target no1}
    \\
    &+
    \notag\\
    %%%#2
    &
    \begin{pmatrix*}[l]
    -2\sqrt{-1}(-1)^{n^2}
    \displaystyle\sum_{\indexic{k}\in\indexIc\backslash\{\alpha\}}
    \displaystyle\sum_{r\in\indexI}
        -(-1)^{n^2}
        \begin{pmatrix*}[l]
            \sgn
                {r,\indexI\backslash\{r\}}
                {\indexI}
            \sgn
                {\order{\indexic{k},r}}
                {r,\indexic{k}}
        \end{pmatrix*}
        \coefD{\indexic{k}}{\order{\indexic{k}, r}}
        \\
        \basexi{\alpha}
        \wedge
        \basexi{\indexI\backslash\{r\}}
        \wedge
        \basedualxi{\indexJp}
    \end{pmatrix*}
\label{EQ-Kahler identity on Lie agbd-For (alpha,I,J), calculation for RHS-simplified half target no2}
    \\
    &+
    \notag\\
    %%%#3
    &
    \begin{pmatrix*}[l]
    -2\sqrt{-1}(-1)^{n^2}
    \displaystyle\sum_{\indexic{k}\in\indexIc\backslash\{\alpha\}}
    \displaystyle\sum_{r\in\indexI}
        (-1)^{n^2}
        \sgn
            {r,\order{(\indexI\backslash\{r\})\cup\{\indexic{k}\}}}
            {\indexic{k},\indexI}
        \sgn
            {\order{\alpha,r}}
            {\alpha,r}
        \\
        \coefD{\indexic{k}}{\order{\alpha, r}}
        \basexi{\order{(\indexI\backslash\{r\})\cup\{\indexic{k}\}}}
        \wedge
        \basedualxi{\indexJp}
    \end{pmatrix*}
\label{EQ-Kahler identity on Lie agbd-For (alpha,I,J), calculation for RHS-simplified half target no3}
    \\
    &+
    \notag\\
    &
    %%%#4
    \begin{pmatrix*}[l]
    -2\sqrt{-1}(-1)^{n^2}
    \displaystyle\sum_{\indexic{k}\in\indexIc\backslash\{\alpha\}}
    \displaystyle\sum_{r_1\in\indexI}
    \displaystyle\sum_{r_2\in\indexI}
        (-1)^{n^2}
        \sgn
            {\order{r_1,r_2},\indexI\backslash\{r_1,r_2\}}
            {\indexI}
        \sgn
            {\order{(\indexI\backslash\{r_1,r_2\})\cup\{\indexic{k}\}}}
            {\indexic{k},(\indexI\backslash\{r_1,r_2\})}
        \\
        \frac{1}{2}
        \coefD{\indexic{k}}{\order{r_1,r_2}}
        \basexi{\alpha}
        \wedge
        \basexi{\order{(\indexI\backslash\{r_1,r_2\})\cup\{\indexic{k}\}}}
        \wedge
        \basedualxi{\indexJp}
    \end{pmatrix*}
\label{EQ-Kahler identity on Lie agbd-For (alpha,I,J), calculation for RHS-simplified half target no4}
    \\
    &+
    \notag\\
    &
    %%%#5
    -2\sqrt{-1}(-1)^{n^2}
    \displaystyle\sum_{\indexjpc{l}\in\indexJpc}
    \displaystyle\sum_{r\in\indexI}
    \begin{matrix*}[l]
        -(-1)^{n^2}
        \coefB{\indexjpc{l}}{\indexjpc{l} \alpha}
        \basexi{\indexI}
        \wedge
        \basedualxi{\indexJp}
    \end{matrix*}
\label{EQ-Kahler identity on Lie agbd-For (alpha,I,J), calculation for RHS-simplified half target no5}
    \\
    &+
    \notag\\
    &
    %%%#6
    -2\sqrt{-1}(-1)^{n^2}
    \displaystyle\sum_{\indexjpc{l}\in\indexJpc}
    \displaystyle\sum_{r\in\indexI}
    \begin{matrix*}[l]
        (-1)^{n^2}
        \sgn
            {r,\indexI\backslash\{r\}}
            {\indexI}
        \coefB{\indexjpc{l}}{\indexjpc{l} r}
        \basexi{\alpha}
        \wedge
        \basexi{\indexI\backslash\{r\}}
        \wedge
        \basedualxi{\indexJp}
    \end{matrix*}
\label{EQ-Kahler identity on Lie agbd-For (alpha,I,J), calculation for RHS-simplified half target no6}
    \\
    &+
    \notag\\
    &
    %%%#7
    -2\sqrt{-1}(-1)^{n^2}
    \displaystyle\sum_{\indexjpc{l}\in\indexJpc}
    \displaystyle\sum_{u^{'}\in\indexJp}
    \begin{matrix*}[l]
        -(-1)^{n^2}
        \sgn
            {u^{'},\indexI,\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
            {\indexjpc{l},\indexI,\indexJp}
        \coefB{\indexjpc{l}}{u^{'} \alpha}
        \basexi{\indexI}
        \wedge
        \basedualxi{\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
    \end{matrix*}
\label{EQ-Kahler identity on Lie agbd-For (alpha,I,J), calculation for RHS-simplified half target no7}
    \\
    &+
    \notag\\
    &
    %%%#8
    \begin{pmatrix*}[l]
        -2\sqrt{-1}(-1)^{n^2}
        \displaystyle\sum_{\indexjpc{l}\in\indexJpc}
        \displaystyle\sum_{r\in\indexI}
        \displaystyle\sum_{u^{'}\in\indexJp}
        (-1)^{p+1}
        (-1)^{n^2}
        \sgn
            {u^{'},r,\indexI\backslash\{r\},\indexJp\backslash\{u^{'}\}}
            {\indexI,\indexJp}
        \sgn
            {\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
            {\indexjpc{l},\indexJp\backslash\{u^{'}\}}
        \\
        \coefB{\indexjpc{l}}{u^{'} r}
        \basexi{\alpha}
        \wedge
        \basexi{\indexI\backslash\{r\}}
        \wedge
        \basedualxi{\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
    \end{pmatrix*}
    .
\label{EQ-Kahler identity on Lie agbd-For (alpha,I,J), calculation for RHS-simplified half target no8}
\end{align}
%%%%%%%%%%%%%% finish step 3 %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% start step 4 %%%%%%%%%%%%%%
\keyword{Step 4:}
Cancel out $(-1)^{n^2}$ and rearrange the expression according to the expressions of $
\sqrt{-1}(\LieagbdPartial^{*}\basexi{\alpha})
\wedge\basexi{\indexI}\wedge\basedualxi{\indexJp}
$ and $
\basexi{\alpha}\wedge
\sqrt{-1}\LieagbdPartial^{*}(\basexi{\indexI}\wedge\basedualxi{\indexJp})
$. The expression of $
\sqrt{-1}
\LieagbdPartial^{*}(
\basexi{\alpha}\wedge
\basexi{\indexI}\wedge\basedualxi{\indexJp})
$ is a sum of three parts.
\begin{itemize}
    \item The first part is (\ref{EQ-Kahler identity on Lie agbd-For (alpha,I,J), calculation for RHS-simplified half target no1}) + (\ref{EQ-Kahler identity on Lie agbd-For (alpha,I,J), calculation for RHS-simplified half target no5}), whose expression is
    \begin{align}% no1 + no5
        -2\sqrt{-1}
        \begin{pmatrix*}[l]
            \displaystyle\sum_{\indexic{k}\in\indexIc\backslash\{\alpha\}}
            \begin{matrix*}[l]
                \sgn
                    {\order{\indexic{k},\alpha}}
                    {\alpha,\indexic{k}}
                \coefD{\indexic{k}}{\order{\indexic{k}, \alpha}}
                \basexi{\indexI}
                \wedge
                \basedualxi{\indexJp}
            \end{matrix*}
            \\
            +
            \\
            \displaystyle\sum_{\indexjpc{l}\in\indexJpc}
            \begin{matrix*}[l]
                (-1)
                \coefB{\indexjpc{l}}{\indexjpc{l} \alpha}
                \basexi{\indexI}
                \wedge
                \basedualxi{\indexJp}
            \end{matrix*}
        \end{pmatrix*}
        .
    \label{EQ-Kahler identity on Lie agbd-For (alpha,I,J), the first part}
    \end{align}
    This part is related to the expression of $
    \sqrt{-1}(\LieagbdPartial^{*}\basexi{\alpha})
    \wedge\basexi{\indexI}\wedge\basedualxi{\indexJp}
    $.

    \item The second part is
    (\ref{EQ-Kahler identity on Lie agbd-For (alpha,I,J), calculation for RHS-simplified half target no2})
    +
    (\ref{EQ-Kahler identity on Lie agbd-For (alpha,I,J), calculation for RHS-simplified half target no4})
    +
    (\ref{EQ-Kahler identity on Lie agbd-For (alpha,I,J), calculation for RHS-simplified half target no6})
    +
    (\ref{EQ-Kahler identity on Lie agbd-For (alpha,I,J), calculation for RHS-simplified half target no8}), which is equal to the sum of the following terms:
    \begin{align}% no2 + no4 + no6 + no8
        -2\sqrt{-1}
        \begin{pmatrix*}[l]
            \displaystyle\sum_{\indexic{k}\in\indexIc\backslash\{\alpha\}}
            \displaystyle\sum_{r\in\indexI}
            \begin{matrix*}[l]
                (-1)
                    \sgn
                        {r,\indexI\backslash\{r\}}
                        {\indexI}
                    \sgn
                        {\order{\indexic{k},r}}
                        {r,\indexic{k}}
            \\
                \coefD{\indexic{k}}{\order{\indexic{k}, r}}
                \basexi{\alpha}
                \wedge
                \basexi{\indexI\backslash\{r\}}
                \wedge
                \basedualxi{\indexJp}
            \end{matrix*}
            \\
            +
            \\
            \displaystyle\sum_{\indexic{k}\in\indexIc\backslash\{\alpha\}}
            \displaystyle\sum_{r_1\in\indexI}
            \displaystyle\sum_{r_2\in\indexI}
            \begin{matrix*}[l]
                \sgn
                    {\order{r_1,r_2},\indexI\backslash\{r_1,r_2\}}
                    {\indexI}
                \sgn
                    {\order{(\indexI\backslash\{r_1,r_2\})\cup\{\indexic{k}\}}}
                    {\indexic{k},(\indexI\backslash\{r_1,r_2\})}
            \\
                \frac{1}{2}
                \coefD{\indexic{k}}{\order{r_1,r_2}}
                \basexi{\alpha}
                \wedge
                \basexi{\order{(\indexI\backslash\{r_1,r_2\})\cup\{\indexic{k}\}}}
                \wedge
                \basedualxi{\indexJp}
            \end{matrix*}
            \\
            +
            \\
            \displaystyle\sum_{\indexjpc{l}\in\indexJpc}
            \displaystyle\sum_{r\in\indexI}
            \begin{matrix*}[l]
                \sgn
                    {r,\indexI\backslash\{r\}}
                    {\indexI}
                \coefB{\indexjpc{l}}{\indexjpc{l} r}
                \basexi{\alpha}
                \wedge
                \basexi{\indexI\backslash\{r\}}
                \wedge
                \basedualxi{\indexJp}
        \end{matrix*}
            \\
            +
            \\
            \displaystyle\sum_{\indexjpc{l}\in\indexJpc}
            \displaystyle\sum_{r\in\indexI}
            \displaystyle\sum_{u^{'}\in\indexJp}
            \begin{matrix*}[l]    
                (-1)^{p+1}
                \sgn
                    {u^{'},r,\indexI\backslash\{r\},\indexJp\backslash\{u^{'}\}}
                    {\indexI,\indexJp}
                \sgn
                    {\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
                    {\indexjpc{l},\indexJp\backslash\{u^{'}\}}
            \\
                \coefB{\indexjpc{l}}{u^{'} r}
                \basexi{\alpha}
                \wedge
                \basexi{\indexI\backslash\{r\}}
                \wedge
                \basedualxi{\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
            \end{matrix*}
        \end{pmatrix*}
        .
    \label{EQ-Kahler identity on Lie agbd-For (alpha,I,J), the second part}
    \end{align}
    This part is related to $
    \basexi{\alpha}\wedge
    \sqrt{-1}\LieagbdPartial^{*}(\basexi{\indexI}\wedge\basedualxi{\indexJp})
    $.

    \item The third part is 
    (\ref{EQ-Kahler identity on Lie agbd-For (alpha,I,J), calculation for RHS-simplified half target no3})
    +
    (\ref{EQ-Kahler identity on Lie agbd-For (alpha,I,J), calculation for RHS-simplified half target no7}), which is equal to
    \begin{align}% no3 + no7
        (-2\sqrt{-1})
        \begin{pmatrix*}[l]
            \displaystyle\sum_{\indexic{k}\in\indexIc\backslash\{\alpha\}}
            \displaystyle\sum_{r\in\indexI}
            \begin{matrix*}[l]
                \sgn
                    {r,\order{(\indexI\backslash\{r\})\cup\{\indexic{k}\}}}
                    {\indexic{k},\indexI}
                \sgn
                    {\order{\alpha,r}}
                    {\alpha,r}
                \\
                \coefD{\indexic{k}}{\order{\alpha, r}}
                \basexi{\order{(\indexI\backslash\{r\})\cup\{\indexic{k}\}}}
                \wedge
                \basedualxi{\indexJp}
            \end{matrix*}
            \\
            +
            \\   
            \displaystyle\sum_{\indexjpc{l}\in\indexJpc}
            \displaystyle\sum_{u^{'}\in\indexJp}
            \begin{matrix*}[l]
                (-1)
                \sgn
                    {u^{'},\indexI,\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
                    {\indexjpc{l},\indexI,\indexJp}
                \\
                \coefB{\indexjpc{l}}{u^{'} \alpha}
                \basexi{\indexI}
                \wedge
                \basedualxi{\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
            \end{matrix*}
        \end{pmatrix*}
        .
    \label{EQ-Kahler identity on Lie agbd-For (alpha,I,J), the third part}
    \end{align}
\end{itemize}


\end{proof}

==> 4/For__alpha_,_I_,J,_calculation_for_RHS.tex <==
\begin{lemma}
\label{lemma-Kahler identity on Lie agbd-For (alpha),I,J, calculation for RHS}
    \begin{align}                                                       
        (\sqrt{-1}\LieagbdPartial^{*}\basexi{\alpha})
        \wedge\basexi{\indexI}\wedge\basedualxi{\indexJp}
        =
        -2\sqrt{-1}
        \begin{pmatrix*}[l]
            \displaystyle\sum_{k\neq\alpha}
            \begin{matrix*}[l]
                \sgn
                    {\order{k,\alpha}}
                    {\alpha,k}
                \coefD{k}{\order{k,\alpha}}
                \basexi{\indexI}\wedge\basedualxi{\indexJp}
            \end{matrix*}
            \\
            +
            \\
            \displaystyle\sum_{l^{'}=1}^{n}
            \begin{matrix*}[l]
                (-1)\coefB{l^{'}}{l^{'} \alpha}
                \basexi{\indexI}\wedge\basedualxi{\indexJp}
            \end{matrix*}
        \end{pmatrix*}.
    \label{EQ-Kahler identity on Lie agbd-For (alpha),I,J, calculation for RHS-target}
    \end{align}
\end{lemma}


\begin{proof}
Recall that $\LieagbdPartial^{*}=-(-1)^{n^2}\star\,\LieagbdPartialbar\,\star$. Our proof comprises the following steps:
\begin{enumerate}
    \item Calculate $\star(\basexi{\alpha})$.
    \item Calculate $
    \LieagbdPartialbar\,\star
    (\basexi{\alpha})
    $.
    \item Calculate $
    \star\,\LieagbdPartialbar\,\star
    (\basexi{\alpha})
    $ and conclude the expression of $
    (\sqrt{-1}\LieagbdPartial^{*}\basexi{\alpha})
    \wedge\basexi{\indexI}\wedge\basedualxi{\indexJp}
    $.
\end{enumerate}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% start Step 1 %%%%%%%%%%%%%%%%%%
\keyword{Step 1:} We take $\star$ on $\basexi{\alpha}$ and obtain
\begin{align}
    \star(\basexi{\alpha})
    =
    2^{1+0-n}
    \sgn
        {1,\cdots,n}
        {\alpha,1,\cdots,\widehat{\alpha},\cdots,n}
    \basedualxi{1,\cdots,\widehat{\alpha},\cdots,n}
    \wedge
    \basexi{1^{'},\cdots,n^{'}}
    .
    \label{EQ-Kahler identity on Lie agbd-For (alpha),I,J, calculation for RHS-No1}
\end{align}
%%%%%%%%%%%%%%%%%% finish Step 1 %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% start Step 2 %%%%%%%%%%%%%%%%%%
\keyword{Step 2:} We apply $\LieagbdPartialbar$ to (\ref{EQ-Kahler identity on Lie agbd-For (alpha),I,J, calculation for RHS-No1}) and obtain
\begin{align}
    &
    2^{1-n}
    \begin{pmatrix*}[l]
        \displaystyle\sum_{k\neq\alpha}
        \begin{matrix*}[l]
            \sgn
                {1,\cdots,n}
                {\alpha,1,\cdots,\widehat{\alpha},\cdots,n}
            \sgn
                {1,\cdots,\widehat{\alpha},\cdots,n}
                {k,1,\cdots,\widehat{k},\cdots,\widehat{\alpha},\cdots,n}
            \\
            \basedualxi{1}
            \wedge\cdots\wedge
            \LieagbdPartialbar\basedualxi{k}
            \wedge\cdots\wedge
            \widehat{\basedualxi{\alpha}}
            \wedge\cdots\wedge
            \basedualxi{n}
            \wedge
            \basexi{1^{'},\cdots,n^{'}}
        \end{matrix*}
        \\
        +
        \\
        \displaystyle\sum_{l^{'}=1}^{n}
        \begin{matrix*}[l]
            \sgn
                {1,\cdots,n}
                {\alpha,1,\cdots,\widehat{\alpha},\cdots,n}
            \sgn
                {1,\cdots,\widehat{\alpha},\cdots,n,1^{'},\cdots,n^{'}}
                {l^{'},1,\cdots,\widehat{\alpha},\cdots,n,1^{'},\cdots,\widehat{l^{'}},\cdots,n^{'}}
            \\
            \basedualxi{1}
            \wedge\cdots\wedge
            \widehat{\basedualxi{\alpha}}
            \wedge\cdots\wedge
            \basedualxi{n}
            \wedge
            \basexi{1^{'}}
            \wedge\cdots\wedge
            \LieagbdPartialbar\basexi{l^{'}}
            \wedge\cdots\wedge
            \basexi{n^{'}}
        \end{matrix*}
    \end{pmatrix*}
    .
\label{EQ-Kahler identity on Lie agbd-For (alpha),I,J, calculation for RHS-No1.5}
\end{align}
Recalling that $
\LieagbdPartialbar\basedualxi{k}
=
\frac{1}{2}\displaystyle\sum_{s,t}
\coefD{k}{s t}\basedualxi{s}\wedge\basedualxi{t}
$ and $
\LieagbdPartialbar\basexi{l^{'}}
=
\displaystyle\sum_{s,t}
\coefB{l^{'}}{s t}\basexi{s}\wedge\basedualxi{t}
$, we cancel out the terms containing repeated frame bases. The formula of (\ref{EQ-Kahler identity on Lie agbd-For (alpha),I,J, calculation for RHS-No1.5}) is simplified to
\begin{align}
    2^{1-n}
    \begin{pmatrix*}[l]
        \displaystyle\sum_{k\neq\alpha}
        \begin{matrix*}[l]
            \sgn
                {1,\cdots,n}
                {\alpha,1,\cdots,\widehat{\alpha},\cdots,n}
            \sgn
                {1,\cdots,\widehat{\alpha},\cdots,n}
                {k,1,\cdots,\widehat{k},\cdots,\widehat{\alpha},\cdots,n}
            \\
            \basedualxi{1}
            \wedge\cdots\wedge
            \begin{pmatrix*}[l]
                \frac{1}{2}
                (
                \coefD{k}{k \alpha}
                \basedualxi{k}\wedge\basedualxi{\alpha}
                +
                \coefD{k}{\alpha k}
                \basedualxi{\alpha}\wedge\basedualxi{k}
                )
            \end{pmatrix*}
            \wedge\cdots\wedge
            \widehat{\basedualxi{\alpha}}
            \wedge\cdots\wedge
            \basedualxi{n}
            \wedge
            \basexi{1^{'},\cdots,n^{'}}
        \end{matrix*}
        \\
        +
        \\
        \displaystyle\sum_{l^{'}=1}^{n}
        \begin{matrix*}[l]
            \sgn
                {1,\cdots,n}
                {\alpha,1,\cdots,\widehat{\alpha},\cdots,n}
            \sgn
                {1,\cdots,\widehat{\alpha},\cdots,n,1^{'},\cdots,n^{'}}
                {l^{'},1,\cdots,\widehat{\alpha},\cdots,n,1^{'},\cdots,\widehat{l^{'}},\cdots,n^{'}}
            \\
            \basedualxi{1}
            \wedge\cdots\wedge
            \widehat{\basedualxi{\alpha}}
            \wedge\cdots\wedge
            \basedualxi{n}
            \wedge
            \basexi{1^{'}}
            \wedge\cdots\wedge
            \begin{pmatrix*}[l]
                \coefB{l^{'}}{l^{'} \alpha}
                \basexi{l^{'}}\wedge\basedualxi{\alpha}
            \end{pmatrix*}
            \wedge\cdots\wedge
            \basexi{n^{'}}
        \end{matrix*}
    \end{pmatrix*}.
\label{EQ-Kahler identity on Lie agbd-For (alpha),I,J, calculation for RHS-No2}
\end{align}


We use the notation
\begin{align*}
    \basedualxi{\order{j k}}
    =
    \begin{cases}
        \basedualxi{j}\wedge\basedualxi{k}
        \qquad\text{if }j<k
        \\
        \basedualxi{k}\wedge\basedualxi{j}
        \qquad\text{if }k<j
    \end{cases}
\end{align*}
to simplify the formula
\begin{align*}
        \coefD{i}{j k}
        \basedualxi{j}\wedge\basedualxi{k}
    =
        \coefD{i}{k j}
        \basedualxi{k}\wedge\basedualxi{j}
    =  
        \coefD{i}{\order{j k}}
        \basedualxi{\order{j k}},
\end{align*}
where $\coefD{i}{j k}=-\coefD{i}{k j}$. Thus, the wedge product of frames in (\ref{EQ-Kahler identity on Lie agbd-For (alpha),I,J, calculation for RHS-No2}) can be simplified to
\begin{align}
    &
        \basedualxi{1}
        \wedge\cdots\wedge
        \begin{pmatrix*}[l]
            \frac{1}{2}
            (
            \coefD{k}{k \alpha}
            \basedualxi{k}\wedge\basedualxi{\alpha}
            +
            \coefD{k}{\alpha k}
            \basedualxi{\alpha}\wedge\basedualxi{k}
            )
        \end{pmatrix*}
        \wedge\cdots\wedge
        \widehat{\basedualxi{\alpha}}
        \wedge\cdots\wedge
        \basedualxi{n}
        \wedge
        \basexi{1^{'},\cdots,n^{'}}
    \notag
    \\
    =&
        \basedualxi{1}
        \wedge\cdots\wedge  
            \coefD{k}{\order{k \alpha}}
            \basedualxi{\order{k \alpha}}
        \wedge\cdots\wedge
        \widehat{\basedualxi{\alpha}}
        \wedge\cdots\wedge
        \basedualxi{n}
        \wedge
        \basexi{1^{'},\cdots,n^{'}}
    \notag
    \\
    =&
        \sgn
            {1,\cdots,k-1,\order{k,\alpha},k+1,\cdots,\widehat{\alpha},\cdots,n}
            {1,\cdots,n}
        \coefD{k}{\order{k,\alpha}}
        \basedualxi{1,\cdots,n}
        \wedge
        \basexi{1^{'},\cdots,n^{'}}
\label{EQ-Kahler identity on Lie agbd-For (alpha),I,J, calculation for RHS-No3}
\end{align}
and
\begin{align}
    &
        \basedualxi{1}
        \wedge\cdots\wedge
        \widehat{\basedualxi{\alpha}}
        \wedge\cdots\wedge
        \basedualxi{n}
        \wedge
        \basexi{1^{'}}
        \wedge\cdots\wedge
        \begin{pmatrix*}[l]
            \coefB{l^{'}}{l^{'} \alpha}
            \basexi{l^{'}}\wedge\basedualxi{\alpha}
        \end{pmatrix*}
        \wedge\cdots\wedge
        \basexi{n^{'}}
    \notag
    \\
    =&
        \sgn
            {1,\cdots,\widehat{\alpha},\cdots,n,1^{'},\cdots,l^{'},\alpha,l+1^{'},\cdots,n^{'}}
            {1,\cdots,n,1^{'},\cdots,n^{'}}
        \coefB{l^{'}}{l^{'} \alpha}
        \basedualxi{1,\cdots,n}
        \wedge
        \basexi{1^{'},\cdots,n^{'}}
    .
    \label{EQ-Kahler identity on Lie agbd-For (alpha),I,J, calculation for RHS-No4}
\end{align}
Using (\ref{EQ-Kahler identity on Lie agbd-For (alpha),I,J, calculation for RHS-No3}) and
(\ref{EQ-Kahler identity on Lie agbd-For (alpha),I,J, calculation for RHS-No4}) to replace the corresponding terms in (\ref{EQ-Kahler identity on Lie agbd-For (alpha),I,J, calculation for RHS-No2}), we obtain the expression of $\LieagbdPartialbar\,\star(\basexi{\alpha})$:
\begin{align}
    2^{1-n}
    \begin{pmatrix*}[l]
        \displaystyle\sum_{k\neq\alpha}
        \begin{matrix*}[l]
            \sgn
                {1,\cdots,n}
                {\alpha,1,\cdots,\widehat{\alpha},\cdots,n}
            \sgn
                {1,\cdots,\widehat{\alpha},\cdots,n}
                {k,1,\cdots,\widehat{k},\cdots,\widehat{\alpha},\cdots,n}
            \sgn
                {1,\cdots,k-1,\order{k,\alpha},k+1,\cdots,\widehat{\alpha},\cdots,n}
                {1,\cdots,n}
            \\
            \coefD{k}{\order{k,\alpha}}
            \basedualxi{1,\cdots,n}
            \wedge
            \basexi{1^{'},\cdots,n^{'}}
        \end{matrix*}
        \\
        +
        \\
        \displaystyle\sum_{l^{'}=1}^{n}
        \begin{matrix*}[l]
            \sgn
                {1,\cdots,n}
                {\alpha,1,\cdots,\widehat{\alpha},\cdots,n}
            \sgn
                {1,\cdots,\widehat{\alpha},\cdots,n,1^{'},\cdots,n^{'}}
                {l^{'},1,\cdots,\widehat{\alpha},\cdots,n,1^{'},\cdots,\widehat{l^{'}},\cdots,n^{'}}
            \sgn
                {1,\cdots,\widehat{\alpha},\cdots,n,1^{'},\cdots,l^{'},\alpha,l+1^{'},\cdots,n^{'}}
                {1,\cdots,n,1^{'},\cdots,n^{'}}
            \\
            \coefB{l^{'}}{l^{'} \alpha}
            \basedualxi{1,\cdots,n}
            \wedge
            \basexi{1^{'},\cdots,n^{'}}
        \end{matrix*}
    \end{pmatrix*}.
\label{EQ-Kahler identity on Lie agbd-For (alpha),I,J, calculation for RHS-No5}
\end{align}
%%%%%%%%%%%%%%%%%% finish Step 2 %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% start Step 3 %%%%%%%%%%%%%%%%%%
\keyword{Step 3:} Take $\star$ on (\ref{EQ-Kahler identity on Lie agbd-For (alpha),I,J, calculation for RHS-No5}). Using the formula
\begin{align*}
    \star
    (
    \basedualxi{1,\cdots,n}
    \wedge
    \basexi{1^{'},\cdots,n^{'}}
    )
    =
    2^{n+n-n}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {1,\cdots,n,1^{'},\cdots,n^{'}}
    =
    2^{n}(-1)^{n^2}
    ,
\end{align*}
we compute $\star\,\LieagbdPartialbar\,\star(\basexi{\alpha})$ as
\begin{align}
    &
        2^{1-n}
        \begin{pmatrix*}[l]
            2^{n}(-1)^{n^2}
            \displaystyle\sum_{k\neq\alpha}
            \begin{pmatrix*}[l]
                \sgn
                    {1,\cdots,n}
                    {\alpha,1,\cdots,\widehat{\alpha},\cdots,n}
                \sgn
                    {1,\cdots,\widehat{\alpha},\cdots,n}
                    {k,1,\cdots,\widehat{k},\cdots,\widehat{\alpha},\cdots,n}
                \\
                \sgn
                    {1,\cdots,k-1,\order{k,\alpha},k+1,\cdots,\widehat{\alpha},\cdots,n}
                    {1,\cdots,n}
                \coefD{k}{\order{k,\alpha}}
            \end{pmatrix*}
            \\
            +
            \\
            2^{n}(-1)^{n^2}
            \displaystyle\sum_{l^{'}=1}^{n}
            \begin{pmatrix*}[l]
                \sgn
                    {1,\cdots,n}
                    {\alpha,1,\cdots,\widehat{\alpha},\cdots,n}
                \sgn
                    {1,\cdots,\widehat{\alpha},\cdots,n,1^{'},\cdots,n^{'}}
                    {l^{'},1,\cdots,\widehat{\alpha},\cdots,n,1^{'},\cdots,\widehat{l^{'}},\cdots,n^{'}}
                \\
                \sgn
                    {1,\cdots,\widehat{\alpha},\cdots,n,1^{'},\cdots,l^{'},\alpha,l+1^{'},\cdots,n^{'}}
                    {1,\cdots,n,1^{'},\cdots,n^{'}}
                \coefB{l^{'}}{l^{'} \alpha}
            \end{pmatrix*}
        \end{pmatrix*}
    \notag
    \\
    =&
        (-1)^{n^2}2
        \begin{pmatrix*}[l]
            \displaystyle\sum_{k\neq\alpha}
            \begin{pmatrix*}[l]
                \sgn
                    {1,\cdots,n}
                    {\alpha,1,\cdots,\widehat{\alpha},\cdots,n}
                \sgn
                    {1,\cdots,\widehat{\alpha},\cdots,n}
                    {k,1,\cdots,\widehat{k},\cdots,\widehat{\alpha},\cdots,n}
                \\
                \sgn
                    {1,\cdots,k-1,\order{k,\alpha},k+1,\cdots,\widehat{\alpha},\cdots,n}
                    {1,\cdots,n}
                \coefD{k}{\order{k,\alpha}}
            \end{pmatrix*}
            \\
            +
            \\
            \displaystyle\sum_{l^{'}=1}^{n}
            \begin{pmatrix*}[l]
                \sgn
                    {1,\cdots,n}
                    {\alpha,1,\cdots,\widehat{\alpha},\cdots,n}
                \sgn
                    {1,\cdots,\widehat{\alpha},\cdots,n,1^{'},\cdots,n^{'}}
                    {l^{'},1,\cdots,\widehat{\alpha},\cdots,n,1^{'},\cdots,\widehat{l^{'}},\cdots,n^{'}}]
                \\
                \sgn
                    {1,\cdots,\widehat{\alpha},\cdots,n,1^{'},\cdots,l^{'},\alpha,l+1^{'},\cdots,n^{'}}
                    {1,\cdots,n,1^{'},\cdots,n^{'}}
                \coefB{l^{'}}{l^{'} \alpha}
            \end{pmatrix*}
        \end{pmatrix*}
    .
\label{EQ-Kahler identity on Lie agbd-For (alpha),I,J, calculation for RHS-No6}
\end{align}
The signs of permutation in (\ref{EQ-Kahler identity on Lie agbd-For (alpha),I,J, calculation for RHS-No6}) can be simplified as follows:
\begin{align}
    &
        \sgn
            {1,\cdots,n}
            {\alpha,1,\cdots,\widehat{\alpha},\cdots,n}
        \sgn
            {1,\cdots,\widehat{\alpha},\cdots,n}
            {k,1,\cdots,\widehat{k},\cdots,\widehat{\alpha},\cdots,n}
        \sgn
            {1,\cdots,k-1,\order{k,\alpha},k+1,\cdots,\widehat{\alpha},\cdots,n}
            {1,\cdots,n}
    \notag
    \\
    =&
        \sgn
            {1,\cdots,n}
            {\alpha,k,1,\cdots,\widehat{k},\cdots,\widehat{\alpha},\cdots,z}
        \sgn
            {1,\cdots,k-1,\order{k,\alpha},k+1,\cdots,\widehat{\alpha},\cdots,n}
            {1,\cdots,n}
    \notag
    \\
    =&
        \sgn
            {1,\cdots,n}
            {\alpha,k,1,\cdots,\widehat{k},\cdots,\widehat{\alpha},\cdots,z}
        \sgn
            {\order{k,\alpha},1,\cdots,\widehat{k},\cdots,\widehat{\alpha},\cdots,n}
            {1,\cdots,n}
    \notag
    \\
    =&
        \sgn
            {1,\cdots,n}
            {\alpha,k,1,\cdots,\widehat{k},\cdots,\widehat{\alpha},\cdots,z}
        \sgn
            {\order{k,\alpha}}
            {\alpha,k}
        \sgn
            {\alpha,k,1,\cdots,\widehat{k},\cdots,\widehat{\alpha},\cdots,n}
            {1,\cdots,n}
    \notag
    \\
    =&
        \sgn
            {\order{k,\alpha}}
            {\alpha,k}
\label{EQ-Kahler identity on Lie agbd-For (alpha),I,J, calculation for RHS-No7}
\end{align}
and
\begin{align}
    &
        \sgn
            {1,\cdots,n}
            {\alpha,1,\cdots,\widehat{\alpha},\cdots,n}
        \sgn
            {1,\cdots,\widehat{\alpha},\cdots,n,1^{'},\cdots,n^{'}}
            {l^{'},1,\cdots,\widehat{\alpha},\cdots,n,1^{'},\cdots,\widehat{l^{'}},\cdots,n^{'}}
        \sgn
            {1,\cdots,\widehat{\alpha},\cdots,n,1^{'},\cdots,l^{'},\alpha,l+1^{'},\cdots,n^{'}}
            {1,\cdots,n,1^{'},\cdots,n^{'}}
    \notag
    \\
    =&
        \sgn
            {1,\cdots,n}
            {\alpha,1,\cdots,\widehat{\alpha},\cdots,n}
        \sgn
            {1,\cdots,\widehat{\alpha},\cdots,n,1^{'},\cdots,n^{'}}
            {l^{'},1,\cdots,\widehat{\alpha},\cdots,n,1^{'},\cdots,\widehat{l^{'}},\cdots,n^{'}}
        \sgn
            {l^{'},\alpha,1,\cdots,\widehat{\alpha},\cdots,n,1^{'},\cdots,\widehat{l},\cdots,n^{'}}
            {1,\cdots,n,1^{'},\cdots,n^{'}}
    \notag
    \\
    =&
        \sgn
            {1,\cdots,n}
            {\alpha,1,\cdots,\widehat{\alpha},\cdots,n}
        (-1)
        \sgn
            {\alpha,1,\cdots,\widehat{\alpha},\cdots,n,1^{'},\cdots,n^{'}}
            {l^{'},\alpha,1,\cdots,\widehat{\alpha},\cdots,n,1^{'},\cdots,\widehat{l^{'}},\cdots,n^{'}}
        \sgn
            {l^{'},\alpha,1,\cdots,\widehat{\alpha},\cdots,n,1^{'},\cdots,\widehat{l},\cdots,n^{'}}
            {1,\cdots,n,1^{'},\cdots,n^{'}}
    \notag
    \\
    =&
        (-1)
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {l^{'},\alpha,1,\cdots,\widehat{\alpha},\cdots,n,1^{'},\cdots,\widehat{l^{'}},\cdots,n^{'}}
        \sgn
            {l^{'},\alpha,1,\cdots,\widehat{\alpha},\cdots,n,1^{'},\cdots,\widehat{l},\cdots,n^{'}}
            {1,\cdots,n,1^{'},\cdots,n^{'}}
    \notag
    \\
    =&
        (-1)
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {1,\cdots,n,1^{'},\cdots,n^{'}}
    \notag
    \\
    =&
        (-1)
    .
\label{EQ-Kahler identity on Lie agbd-For (alpha),I,J, calculation for RHS-No8}
\end{align}
We plug (\ref{EQ-Kahler identity on Lie agbd-For (alpha),I,J, calculation for RHS-No7}) and (\ref{EQ-Kahler identity on Lie agbd-For (alpha),I,J, calculation for RHS-No8}) into (\ref{EQ-Kahler identity on Lie agbd-For (alpha),I,J, calculation for RHS-No6}) and simplify the expression of $\star\,\LieagbdPartial\,\star(\basexi{\alpha})$ to
\begin{align*}
    2(-1)^{n^2}
    \begin{pmatrix*}[l]
        \displaystyle\sum_{k\neq\alpha}
        \begin{matrix*}[l]
            \sgn
                {\order{k,\alpha}}
                {\alpha,k}
            \coefD{k}{\order{k,\alpha}}
        \end{matrix*}
        \\
        +
        \\
        \displaystyle\sum_{l^{'}=1}^{n}
        \begin{matrix*}[l]
            (-1)\coefB{l^{'}}{l^{'} \alpha}
        \end{matrix*}
    \end{pmatrix*}.
\end{align*}
Thus, we arrive at the final expression:
\begin{align*}
    (\sqrt{-1}\LieagbdPartial^{*}\basexi{\alpha})
    \wedge
    \basexi{\indexI}\wedge\basedualxi{\indexJp}
    =&
        \sqrt{-1}
        \big(
        -(-1)^{n^2}\star\,\LieagbdPartialbar\star
        (\basexi{\alpha})
        \big)
        \wedge
        \basexi{\indexI}\wedge\basedualxi{\indexJp}
    \\
    =&
    -2\sqrt{-1}
    \begin{pmatrix*}[l]
        \displaystyle\sum_{k\neq\alpha}
        \begin{matrix*}[l]
            \sgn
                {\order{k,\alpha}}
                {\alpha,k}
            \coefD{k}{\order{k,\alpha}}
            \basexi{\indexI}\wedge\basedualxi{\indexJp}
        \end{matrix*}
        \\
        +
        \\
        \displaystyle\sum_{l^{'}=1}^{n}
        \begin{matrix*}[l]
            (-1)\coefB{l^{'}}{l^{'} \alpha}
            \basexi{\indexI}\wedge\basedualxi{\indexJp}
        \end{matrix*}
    \end{pmatrix*}.
\end{align*}

\end{proof}

==> 4/For_alpha,__I_,J_,_calculation_for_RHS.tex <==
\begin{lemma}
\label{lemma-Kahler identity on Lie agbd-For alpha,(I,J), calculation for RHS}
    \begin{align}
        &
        \basexi{\alpha}\wedge
        \sqrt{-1}\LieagbdPartial^{*}
        (\basexi{\indexI}\wedge\basedualxi{\indexJp})
    \\
    =&
        -2\sqrt{-1}
        \begin{pmatrix*}[l]
            %%%1
            \displaystyle\sum_{\indexic{k}\in\indexIc}
            \displaystyle\sum_{r\in\indexI}
            \begin{matrix*}[l]
                \sgn
                    {r,\indexic{k}}
                    {\order{\indexic{k},r}}
                \sgn
                    {r,\indexI\backslash\{r\}}                    
                    {\indexI}
                \coefD{\indexic{k}}{\order{\indexic{k},r}}
                \basexi{\alpha}
                \wedge
                \basexi{\indexI\backslash\{r\}}
                \wedge
                \basedualxi{\indexJp} 
            \end{matrix*}
            \\
            +
            \\
            %%%2
            \displaystyle\sum_{\indexic{k}\in\indexIc\backslash\{\alpha\}}
            \displaystyle\sum_{r_1\in\indexI}
            \displaystyle\sum_{r_2\in\indexI}
            \begin{pmatrix*}[l]
                (-1)
                \sgn
                    {\order{r_1,r_2},\order{(\indexI\backslash\{r_1,r_2\})}}
                    {\indexI}
                \\
                \sgn
                    {\order{(\indexI\backslash\{r_1,r_2\})\cup\{\indexic{k}\}}}
                    {\indexic{k},\indexI\backslash\{r_1,r_2\})}
                \\
                \frac{1}{2}
                \coefD{\indexic{k}}{\order{r_1,r_2}}
                \basexi{\alpha}
                \wedge
                \basexi{\order{(\indexI\backslash\{r_1,r_2\})\cup\{\indexic{k}\}}}
                \wedge
                \basedualxi{\indexJp} 
            \end{pmatrix*}
            \\
            +
            \\
            %%%3
            \displaystyle\sum_{\indexjpc{l}\in\indexJpc}
            \displaystyle\sum_{r\in\indexI}
            \begin{matrix*}[l]
                (-1)
                \sgn
                    {r,\indexI\backslash\{r\}}
                    {\indexI}
                \coefB{\indexjpc{l}}{\indexjpc{l} r}
                \basexi{\alpha}
                \wedge
                \basexi{\indexI\backslash\{r\}}
                \wedge
                \basedualxi{\indexJp} 
            \end{matrix*}
            \\
            +
            \\
            %%%4
            \displaystyle\sum_{\indexjpc{l}\in\indexJpc}
            \displaystyle\sum_{r\in\indexI}
            \displaystyle\sum_{u^{'}\in\indexJp}
            \begin{pmatrix*}[l]
                (-1)^{p}
                \sgn
                    {u^{'},r,\indexI\backslash\{r\},\order{(\indexJp\backslash\{u^{'}\})}}
                    {\indexI,\indexJp}
                \\
                \sgn
                    {\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
                    {\indexjpc{l},(\indexJp\backslash\{u^{'}\})}
                \\
                \coefB{\indexjpc{l}}{u^{'} r}
                \basexi{\alpha}
                \wedge
                \basexi{\indexI\backslash\{r\}}
                \wedge
                \basedualxi{\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}} 
            \end{pmatrix*}
        \end{pmatrix*}.
    \label{EQ-Kahler identity on Lie agbd-For alpha,(I,J), calculation for RHS-target}
    \end{align}
\end{lemma}


\begin{proof}
Recall that $\LieagbdPartial^{\star}=-(-1)^{n^2}\star\,\LieagbdPartialbar\,\star$. Our proof comprises the following steps:
\begin{enumerate}
    \item Calculate $\star(\basexi{\indexI}\wedge\basedualxi{\indexJp})$.
    \item Calculate $
    \LieagbdPartialbar\,\star
    (\basexi{\indexI}\wedge\basedualxi{\indexJp})
    $.
    \item Calculate $
    \star\,\LieagbdPartialbar\,\star
    (\basexi{\indexI}\wedge\basedualxi{\indexJp})
    $ and conclude the expression of $
    \basexi{\alpha}\wedge
    \sqrt{-1}\LieagbdPartial^{*}
    (\basexi{\indexI}\wedge\basedualxi{\indexJp})
    $.
\end{enumerate}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% start step 1 %%%%%%%%%%%%%%%%%%
\keyword{Step 1:} We take $\star$ on $\basexi{\indexI}\wedge\basedualxi{\indexJp}$ and obtain
\begin{align}
    \star(\basexi{\indexI}\wedge\basedualxi{\indexJp})
    =
    2^{p+q-n}
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\indexI,\indexJp,\indexIc,\indexJpc}
    \basedualxi{\indexIc}
    \wedge
    \basexi{\indexJpc}
    .
    \label{EQ-Kahler identity on Lie agbd-For alpha,(I,J), calculation for RHS-no1}
\end{align}
%%%%%%%%%%%%%%%%%% finish step 1 %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% start step 2 %%%%%%%%%%%%%%%%%%
\keyword{Step 2:} We apply $\LieagbdPartialbar$ to (\ref{EQ-Kahler identity on Lie agbd-For alpha,(I,J), calculation for RHS-no1}):
\begin{align}
    2^{p+q-n}
    \begin{pmatrix*}[l]
        \displaystyle\sum_{\indexic{k}\in\indexIc}
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\indexI,\indexJp,\indexIc,\indexJpc}
        \sgn
            {\indexIc}
            {\indexic{k},\indexIc\backslash\{\indexic{k}\}}
        \basedualxi{\indexic{1}}
        \wedge\cdots\wedge
        \LieagbdPartialbar\basedualxi{\indexic{k}}
        \wedge\cdots\wedge
        \basedualxi{\indexic{n-p}}
        \wedge
        \basexi{\indexJpc} 
        \\
        +
        \\
        \displaystyle\sum_{\indexjpc{l}\in\indexJpc}
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\indexI,\indexJp,\indexIc,\indexJpc}
        \sgn
            {\indexIc,\indexJpc}
            {\indexjpc{l},\indexIc,\indexJpc\backslash\{\indexjpc{l}\}}
        \basedualxi{\indexIc}
        \wedge
        \basexi{\indexjpc{1}} 
        \wedge\cdots\wedge
        \LieagbdPartialbar\basexi{\indexjpc{l}}
        \wedge\cdots\wedge
        \basexi{\indexjpc{n-q}} 
        \\
    \end{pmatrix*}
    .
    \label{EQ-Kahler identity on Lie agbd-For alpha,(I,J), calculation for RHS-no2}
\end{align}
Recall that
\begin{align*}
    \LieagbdPartialbar\basedualxi{k}
    =
    \frac{1}{2}\displaystyle\sum_{s,t}
    \coefD{k}{s t}\basedualxi{s}\wedge\basedualxi{t}
    \qquad\text{and}\qquad
    \LieagbdPartialbar\basexi{l^{'}}
    =
    \displaystyle\sum_{s,t}
    \coefB{l^{'}}{s t}\basexi{s}\wedge\basedualxi{t}
    .
\end{align*} 
We plug these into (\ref{EQ-Kahler identity on Lie agbd-For alpha,(I,J), calculation for RHS-no2}) and cancel out the terms containing repeated frames in the wedge product, obtaining the following expression of $\LieagbdPartialbar\star(\basexi{\indexI}\wedge\basedualxi{\indexJp})$:
\begin{align}
     2^{p+q-n}
    \begin{pmatrix*}[l]
        %%%--1-3-1
        \displaystyle\sum_{\indexic{k}\in\indexIc}
        \begin{pmatrix*}[l]
            \sgn
                {1,\cdots,n,1^{'},\cdots,n^{'}}
                {\indexI,\indexJp,\indexIc,\indexJpc}
            \sgn
                {\indexIc}
                {\indexic{k},\indexIc\backslash\{\indexic{k}\}}
            \\
            \basedualxi{\indexic{1}}
            \wedge\cdots\wedge
            \basedualxi{\indexic{k-1}}
            \wedge
            \begin{pmatrix*}[l]
                \frac{1}{2}
                \displaystyle\sum_{r\in\indexI}
                \coefD{\indexic{k}}{\indexic{k} r}
                \basedualxi{\indexic{k}}
                \wedge
                \basedualxi{r}
                +
                \coefD{\indexic{k}}{r \indexic{k}}
                \basedualxi{r}
                \wedge
                \basedualxi{\indexic{k}}
                \\
                +
                \\
                \frac{1}{2}
                \displaystyle\sum_{r_1\in\indexI}
                \displaystyle\sum_{r_2\in\indexI}
                \coefD{\indexic{k}}{r_1 r_2}
                \basedualxi{r_1}
                \wedge
                \basedualxi{r_2}
            \end{pmatrix*}
            \wedge
            \basedualxi{\indexic{k+1}}
            \wedge\cdots\wedge
            \\
            \basedualxi{\indexic{n-p}}
            \wedge
            \basexi{\indexJpc} 
        \end{pmatrix*}
        \\
        +
        \\
        %%%--1-3-2
        \displaystyle\sum_{\indexjpc{l}\in\indexJpc}
        \begin{pmatrix*}[l]
            \sgn
                {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\indexI,\indexJp,\indexIc,\indexJpc}
            \sgn
                {\indexIc,\indexJpc}
                {\indexjpc{l},\indexIc,\indexJpc\backslash\{\indexjpc{l}\}}
            \\
            \basedualxi{\indexIc}
            \wedge
            \basexi{\indexjpc{1}} 
            \wedge\cdots\wedge
            \basexi{\indexjpc{l-1}}
            \wedge
            \begin{pmatrix*}
                \displaystyle\sum_{r\in\indexI}
                \coefB{\indexjpc{l}}{\indexjpc{l} r}
                \basexi{\indexjpc{l}}
                \wedge
                \basedualxi{r}
                \\
                +
                \\
                \displaystyle\sum_{r\in\indexI}
                \displaystyle\sum_{u^{'}\in\indexJp}
                \coefB{\indexjpc{l}}{u^{'} r}
                \basexi{u^{'}}
                \wedge
                \basedualxi{r}
            \end{pmatrix*}
            \wedge
            \basexi{\indexjpc{l+1}}
            \wedge\cdots\wedge
            \basexi{\indexjpc{n-q}} 
        \end{pmatrix*}
    \end{pmatrix*}.
\label{EQ-Kahler identity on Lie agbd-For alpha,(I,J), calculation for RHS-no3}
\end{align}
We use the notation
$
    \basedualxi{\order{j k}}=
    \begin{cases}
        \basedualxi{j}\wedge\basedualxi{k}
        \qquad\text{if }j<k
        \\
        \basedualxi{k}\wedge\basedualxi{j}
        \qquad\text{if }k<j
    \end{cases}
$ 
to rewrite the formula
\begin{align*}
        \coefD{i}{j k}
        \basedualxi{j}\wedge\basedualxi{k}
    =
        \coefD{i}{k j}
        \basedualxi{k}\wedge\basedualxi{j}
    =  
        \coefD{i}{\order{j k}}
        \basedualxi{\order{j k}}
    ,
\end{align*}
where $\coefD{i}{j k}=-\coefD{i}{k j}$. Thus, the wedge product of frames in (\ref{EQ-Kahler identity on Lie agbd-For alpha,(I,J), calculation for RHS-no3}) can be simplified as follows.
\begin{itemize}
    \item 
\begin{align}
    &
        \basedualxi{\indexic{1}}
        \wedge\cdots\wedge
        \basedualxi{\indexic{k-1}}
        \wedge
        \frac{1}{2}
        \bigg(
            \displaystyle\sum_{r\in\indexI}
            \coefD{\indexic{k}}{\indexic{k} r}
            \basedualxi{\indexic{k}}
            \wedge
            \basedualxi{r}
            +
            \coefD{\indexic{k}}{r \indexic{k}}
            \basedualxi{r}
            \wedge
            \basedualxi{\indexic{k}}
        \bigg)
        \wedge
        \basedualxi{\indexic{k+1}}
        \wedge\cdots\wedge
        \basedualxi{\indexic{n-p}}
        \wedge
        \basexi{\indexJpc} 
\notag
    \\
    =&
        \basedualxi{\indexic{1}}
        \wedge\cdots\wedge
        \basedualxi{\indexic{k-1}}
        \wedge
        \bigg(
            \displaystyle\sum_{r\in\indexI}
            \coefD{\indexic{k}}{\order{\indexic{k} r}}
            \basedualxi{\order{\indexic{k} r}}
            \bigg)
        \wedge
        \basedualxi{\indexic{k+1}}
        \wedge\cdots\wedge
        \basedualxi{\indexic{n-p}}
        \wedge
        \basexi{\indexJpc} 
\notag
    \\
    =&
        \displaystyle\sum_{r\in\indexI}
        \sgn
            {\indexic{1},\cdots,\indexic{k-1},\order{\indexic{k},r},\indexic{k+1},\cdots,\indexic{n-p}}
            {\order{\indexIc\cup\{r\}}}
        \coefD{\indexic{k}}{\order{\indexic{k},r}}
        \basedualxi{\order{\indexIc\cup\{r\}}}
        \wedge
        \basexi{\indexJpc} 
    .
\label{EQ-Kahler identity on Lie agbd-For alpha,(I,J), calculation for RHS-no4}
\end{align}

\item
\begin{align}
    &
        \basedualxi{\indexic{1}}
        \wedge\cdots\wedge
        \basedualxi{\indexic{k-1}}
        \wedge
        \bigg(
            \frac{1}{2}
            \displaystyle\sum_{r_1\in\indexI}
            \displaystyle\sum_{r_2\in\indexI}
            \coefD{\indexic{k}}{r_1 r_2}
            \basedualxi{r_1}
            \wedge
            \basedualxi{r_2}
        \bigg)
        \wedge
        \basedualxi{\indexic{k+1}}
        \wedge\cdots\wedge
        \basedualxi{\indexic{n-p}}
        \wedge
        \basexi{\indexJpc} 
\notag
    \\
    =&
        \basedualxi{\indexic{1}}
        \wedge\cdots\wedge
        \basedualxi{\indexic{k-1}}
        \wedge
        \bigg(
            \frac{1}{2}
            \displaystyle\sum_{r_1\in\indexI}
            \displaystyle\sum_{r_2\in\indexI}
            \coefD{\indexic{k}}{\order{r_1 r_2}}
            \basedualxi{\order{r_1 r_2}}
        \bigg)
        \wedge
        \basedualxi{\indexic{k+1}}
        \wedge\cdots\wedge
        \basedualxi{\indexic{n-p}}
        \wedge
        \basexi{\indexJpc} 
\notag
    \\
    =&
        \displaystyle\sum_{r_1\in\indexI}
        \displaystyle\sum_{r_2\in\indexI}
        \frac{1}{2}
        \sgn
            {\indexic{1},\cdots,\indexic{k-1},\order{r_1,r_2},\indexic{k+1},\cdots,\indexic{n-p}}
            {\order{(\indexIc\backslash\{\indexic{k}\})\cup\{r_1,r_2\}}}
        \coefD{\indexic{k}}{\order{r_1,r_2}}
        \basedualxi{\order{(\indexIc\backslash\{\indexic{k}\})\cup\{r_1,r_2\}}}
        \wedge
        \basexi{\indexJpc}
    .
\label{EQ-Kahler identity on Lie agbd-For alpha,(I,J), calculation for RHS-no5}
\end{align}

\item
\begin{align}
    &
        \basedualxi{\indexIc}
        \wedge
        \basexi{\indexjpc{1}} 
        \wedge\cdots\wedge
        \basexi{\indexjpc{l-1}}
        \wedge
        \bigg(
            \displaystyle\sum_{r\in\indexI}
            \coefB{\indexjpc{l}}{\indexjpc{l} r}
            \basexi{\indexjpc{l}}
            \wedge
            \basedualxi{r}
        \bigg)
        \wedge
        \basexi{\indexjpc{l+1}}
        \wedge\cdots\wedge
        \basexi{\indexjpc{n-q}} 
\notag
    \\
    =&
        \displaystyle\sum_{r\in\indexI}
        \sgn
            {\indexIc,\indexjpc{1},\cdots,\indexjpc{l-1},\indexjpc{l},r,\indexjpc{l+1},\cdots,\indexjpc{n-1}}
            {\order{\indexIc\cup\{r\}},\indexJpc}
        \coefB{\indexjpc{l}}{\indexjpc{l} r}
        \basedualxi{\order{\indexIc\cup\{r\}}}
        \wedge
        \basexi{\indexJpc} 
    .
\label{EQ-Kahler identity on Lie agbd-For alpha,(I,J), calculation for RHS-no6}
\end{align}

\item
\begin{align}
    &
        \basedualxi{\indexIc}
        \wedge
        \basexi{\indexjpc{1}} 
        \wedge\cdots\wedge
        \basexi{\indexjpc{l-1}}
        \wedge
        \bigg(
            \displaystyle\sum_{r\in\indexI}
            \displaystyle\sum_{u^{'}\in\indexJp}
            \coefB{\indexjpc{l}}{u^{'} r}
            \basexi{u^{'}}
            \wedge
            \basedualxi{r}
        \bigg)
        \wedge
        \basexi{\indexjpc{l+1}}
        \wedge\cdots\wedge
        \basexi{\indexjpc{n-q}} 
\notag
    \\
    =&
        \displaystyle\sum_{r\in\indexI}
        \displaystyle\sum_{u^{'}\in\indexJp}
        \begin{matrix*}[l]
            \sgn
                {\indexIc,\indexjpc{1},\cdots,\indexjpc{l-1},u^{'},r,\indexjpc{l+1},\cdots,\indexjpc{n-1}}
                {\order{\indexIc\cup\{r\}},\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}}}
            \\
            \coefB{\indexjpc{l}}{u^{'} r}
            \basedualxi{\order{\indexIc\cup\{r\}}}
            \wedge
            \basexi{\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}}} 
        \end{matrix*}
    .
\label{EQ-Kahler identity on Lie agbd-For alpha,(I,J), calculation for RHS-no7}
\end{align}

\end{itemize}
Using (\ref{EQ-Kahler identity on Lie agbd-For alpha,(I,J), calculation for RHS-no4}), (\ref{EQ-Kahler identity on Lie agbd-For alpha,(I,J), calculation for RHS-no5}), (\ref{EQ-Kahler identity on Lie agbd-For alpha,(I,J), calculation for RHS-no6}), and (\ref{EQ-Kahler identity on Lie agbd-For alpha,(I,J), calculation for RHS-no7}) to simplify the corresponding terms in (\ref{EQ-Kahler identity on Lie agbd-For alpha,(I,J), calculation for RHS-no3}), we obtain the expression of $\LieagbdPartialbar\,\star(\basexi{\indexI}\wedge\basedualxi{\indexJp})$:
\begin{align}
    2^{p+q-n}
    \begin{pmatrix*}[l]
        %%%--1-4-1
        \displaystyle\sum_{\indexic{k}\in\indexIc}
        \displaystyle\sum_{r\in\indexI}
        \begin{pmatrix*}[l]
            \sgn
                {1,\cdots,n,1^{'},\cdots,n^{'}}
                {\indexI,\indexJp,\indexIc,\indexJpc}                
            \sgn
                {\indexIc}
                {\indexic{k},\indexIc\backslash\{\indexic{k}\}}
            \\
            \sgn
                {\indexic{1},\cdots,\indexic{k-1},\order{\indexic{k},r},\indexic{k+1},\cdots,\indexic{n-p}}
                {\order{\indexIc\cup\{r\}}}
            \\
            \coefD{\indexic{k}}{\order{\indexic{k},r}}
            \basedualxi{\order{\indexIc\cup\{r\}}}
            \wedge
            \basexi{\indexJpc} 
        \end{pmatrix*}
        \\
        +
        \\
        %--1-4-2
        \displaystyle\sum_{\indexic{k}\in\indexIc}
        \displaystyle\sum_{r_1\in\indexI}
        \displaystyle\sum_{r_2\in\indexI}
        \begin{pmatrix*}[l]
            \sgn
                {1,\cdots,n,1^{'},\cdots,n^{'}}
                {\indexI,\indexJp,\indexIc,\indexJpc}
            \sgn
                {\indexIc}
                {\indexic{k},\indexIc\backslash\{\indexic{k}\}}
            \\
            \sgn
                {\indexic{1},\cdots,\indexic{k-1},\order{r_1,r_2},\indexic{k+1},\cdots,\indexic{n-p}}
                {\order{(\indexIc\backslash\{\indexic{k}\})\cup\{r_1,r_2\}}}
            \\
            \frac{1}{2}
            \coefD{\indexic{k}}{\order{r_1,r_2}}
            \basedualxi{\order{(\indexIc\backslash\{\indexic{k}\})\cup\{r_1,r_2\}}}
            \wedge
            \basexi{\indexJpc} 
        \end{pmatrix*}
        \\
        +
        \\
        %%%--1-4-3
        \displaystyle\sum_{\indexjpc{l}\in\indexJpc}
        \displaystyle\sum_{r\in\indexI}
        \begin{pmatrix*}[l]
            \sgn
                {1,\cdots,n,1^{'},\cdots,n^{'}}
                {\indexI,\indexJp,\indexIc,\indexJpc}
            \sgn
                {\indexIc,\indexJpc}
                {\indexjpc{l},\indexIc,\indexJpc\backslash\{\indexjpc{l}\}}
            \\
            \sgn
                {\indexIc,\indexjpc{1},\cdots,\indexjpc{l-1},\indexjpc{l},r,\indexjpc{l+1},\cdots,\indexjpc{n-1}}
                {\order{\indexIc\cup\{r\}},\indexJpc}
            \\
            \coefB{\indexjpc{l}}{\indexjpc{l} r}
            \basedualxi{\order{\indexIc\cup\{r\}}}
            \wedge
            \basexi{\indexJpc} 
        \end{pmatrix*}
        \\
        +
        \\
        %%%--1-4-4
        \displaystyle\sum_{\indexjpc{l}\in\indexJpc}
        \displaystyle\sum_{r\in\indexI}
        \displaystyle\sum_{u^{'}\in\indexJp}
        \begin{pmatrix*}[l]
            \sgn
                {1,\cdots,n,1^{'},\cdots,n^{'}}
                {\indexI,\indexJp,\indexIc,\indexJpc}
            \sgn
                {\indexIc,\indexJpc}
                {\indexjpc{l},\indexIc,\indexJpc\backslash\{\indexjpc{l}\}}
            \\
            \sgn
                {\indexIc,\indexjpc{1},\cdots,\indexjpc{l-1},u^{'},r,\indexjpc{l+1},\cdots,\indexjpc{n-1}}
                {\order{\indexIc\cup\{r\}},\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}}}
            \\
            \coefB{\indexjpc{l}}{u^{'} r}
            \basedualxi{\order{\indexIc\cup\{r\}}}
            \wedge
            \basexi{\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}}} 
        \end{pmatrix*}
    \end{pmatrix*}.
\label{EQ-Kahler identity on Lie agbd-For alpha,(I,J), calculation for RHS-no8}
\end{align}
%%%%%%%%%%%%%%%%%% finish step 2 %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% start step 3 %%%%%%%%%%%%%%%%%%
\keyword{Step 3:} We apply $\star$ to (\ref{EQ-Kahler identity on Lie agbd-For alpha,(I,J), calculation for RHS-no8}). Recall that
\begin{align*}
    \star
    (\basedualxi{\indexIc}\wedge\basexi{\indexJpc})
    =
    2^{(|\indexIc|+|\indexJpc|-n)}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}{\indexIc,\indexJpc,\indexI,\indexJp}\basexi{\indexI}\wedge\basedualxi{\indexJp}.
\end{align*}
The expression of $
\star\,\LieagbdPartialbar\,\star
(\basexi{\indexI}\wedge\basedualxi{\indexJp})
$ is:
\begin{align}
    2
    \begin{pmatrix*}[l]
            %%%#1
            \displaystyle\sum_{\indexic{k}\in\indexIc}
            \displaystyle\sum_{r\in\indexI}
            \begin{pmatrix*}[l]
                \sgn
                    {1,\cdots,n,1^{'},\cdots,n^{'}}
                    {\indexI,\indexJp,\indexIc,\indexJpc}
                \sgn
                    {\indexIc}
                    {\indexic{k},\indexIc\backslash\{\indexic{k}\}}
                \sgn
                    {\indexic{1},\cdots,\indexic{k-1},\order{\indexic{k},r},\indexic{k+1},\cdots,\indexic{n-p}}
                    {\order{\indexIc\cup\{r\}}}
                \\
                \sgn
                    {1^{'},\cdots,n^{'},1,\cdots,n}
                    {\order{\indexIc\cup\{r\}},\indexJpc,\indexI\backslash\{r\},\indexJp}
                \\
                \coefD{\indexic{k}}{\order{\indexic{k},r}}
                \basexi{\indexI\backslash\{r\}}
                \wedge
                \basedualxi{\indexJp} 
            \end{pmatrix*}
            \\
            +
            \\
            %%%#2
            \displaystyle\sum_{\indexic{k}\in\indexIc}
            \displaystyle\sum_{r_1\in\indexI}
            \displaystyle\sum_{r_2\in\indexI}
            \begin{pmatrix*}[l]
                \sgn
                    {1,\cdots,n,1^{'},\cdots,n^{'}}
                    {\indexI,\indexJp,\indexIc,\indexJpc}
                \sgn
                    {\indexIc}
                    {\indexic{k},\indexIc\backslash\{\indexic{k}\}}
                \sgn
                    {\indexic{1},\cdots,\indexic{k-1},\order{r_1,r_2},\indexic{k+1},\cdots,\indexic{n-p}}
                    {\order{(\indexIc\backslash\{\indexic{k}\})\cup\{r_1,r_2\}}}
                \\
                \sgn
                    {1^{'},\cdots,n^{'},1,\cdots,n}
                    {\order{(\indexIc\backslash\{\indexic{k}\})\cup\{r_1,r_2\}},\indexJpc,\order{(\indexI\backslash\{r_1,r_2\})\cup\{\indexic{k}\}},\indexJp}
                \\
                \frac{1}{2}
                \coefD{\indexic{k}}{\order{r_1,r_2}}
                \basexi{\order{(\indexI\backslash\{r_1,r_2\})\cup\{\indexic{k}\}}}
                \wedge
                \basedualxi{\indexJp} 
            \end{pmatrix*}
            \\
            +
            \\
            %%%#3
            \displaystyle\sum_{\indexjpc{l}\in\indexJpc}
            \displaystyle\sum_{r\in\indexI}
            \begin{pmatrix*}[l]
                \sgn
                    {1,\cdots,n,1^{'},\cdots,n^{'}}
                    {\indexI,\indexJp,\indexIc,\indexJpc}
                \sgn
                    {\indexIc,\indexJpc}
                    {\indexjpc{l},\indexIc,\indexJpc\backslash\{\indexjpc{l}\}}
                \\
                \sgn
                    {\indexIc,\indexjpc{1},\cdots,\indexjpc{l-1},\indexjpc{l},r,\indexjpc{l+1},\cdots,\indexjpc{n-1}}
                    {\order{\indexIc\cup\{r\}},\indexJpc}
                \sgn
                    {1^{'},\cdots,n^{'},1,\cdots,n}
                    {\order{\indexIc\cup\{r\}},\indexJpc,\indexI\backslash\{r\},\indexJp}
                \\
                \coefB{\indexjpc{l}}{\indexjpc{l} r}
                \basexi{\indexI\backslash\{r\}}
                \wedge
                \basedualxi{\indexJp} 
            \end{pmatrix*}
            \\
            +
            \\
            %%%#4
            \displaystyle\sum_{\indexjpc{l}\in\indexJpc}
            \displaystyle\sum_{r\in\indexI}
            \displaystyle\sum_{u^{'}\in\indexJp}
            \begin{pmatrix*}[l]
                \sgn
                    {1,\cdots,n,1^{'},\cdots,n^{'}}
                    {\indexI,\indexJp,\indexIc,\indexJpc}
                \sgn
                    {\indexIc,\indexJpc}
                    {\indexjpc{l},\indexIc,\indexJpc\backslash\{\indexjpc{l}\}}
                \\
                \sgn
                    {\indexIc,\indexjpc{1},\cdots,\indexjpc{l-1},u^{'},r,\indexjpc{l+1},\cdots,\indexjpc{n-1}}
                    {\order{\indexIc\cup\{r\}},\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}}}
                \\
                \sgn
                    {1^{'},\cdots,n^{'},1,\cdots,n}
                    {\order{\indexIc\cup\{r\}},\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}},\indexI\backslash\{r\},\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
                \\
                \coefB{\indexjpc{l}}{u^{'} r}
                \basexi{\indexI\backslash\{r\}}
                \wedge
                \basedualxi{\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}} 
            \end{pmatrix*}
        \end{pmatrix*}.
\label{EQ-For alpha, (I ,J), calculation for RHS-step 3,unsimplified close to the target}
\end{align}


We simplify the signs of permutation in Section \ref{apex-simplification for RHS of alpha,(I,J)}. The details can be found in Lemmas \ref{Lemma-simplification for RHS of alpha,(I,J)-lemma 1}–\ref{Lemma-simplification for RHS of alpha,(I,J)-lemma 4}. We simplify the expression of $
\star\,\LieagbdPartialbar\,\star
(\basexi{\indexI}\wedge\basedualxi{\indexJp})
$ to
\begin{align*}
    2(-1)^{n^2}
    \begin{pmatrix*}[l]
        %%%1
        \displaystyle\sum_{\indexic{k}\in\indexIc}
        \displaystyle\sum_{r\in\indexI}
        \begin{matrix*}[l]
            \sgn
                {r,\indexic{k}}
                {\order{\indexic{k},r}}
            \sgn
                {r,\indexI\backslash\{r\}}                    
                {\indexI}
            \coefD{\indexic{k}}{\order{\indexic{k},r}}
            \basexi{\indexI\backslash\{r\}}
            \wedge
            \basedualxi{\indexJp} 
        \end{matrix*}
        \\
        +
        \\
        %%%2
        \displaystyle\sum_{\indexic{k}\in\indexIc\backslash\{\alpha\}}
        \displaystyle\sum_{r_1\in\indexI}
        \displaystyle\sum_{r_2\in\indexI}
        \begin{matrix*}[l]
            (-1)
            \sgn
                {\order{r_1,r_2},\order{(\indexI\backslash\{r_1,r_2\})}}
                {\indexI}
            \sgn
                {\order{(\indexI\backslash\{r_1,r_2\})\cup\{\indexic{k}\}}}
                {\indexic{k},\indexI\backslash\{r_1,r_2\})}
            \\
            \frac{1}{2}
            \coefD{\indexic{k}}{\order{r_1,r_2}}
            \basexi{\order{(\indexI\backslash\{r_1,r_2\})\cup\{\indexic{k}\}}}
            \wedge
            \basedualxi{\indexJp} 
        \end{matrix*}
        \\
        +
        \\
        %%%3
        \displaystyle\sum_{\indexjpc{l}\in\indexJpc}
        \displaystyle\sum_{r\in\indexI}
        \begin{matrix*}[l]
            (-1)
            \sgn
                {r,\indexI\backslash\{r\}}
                {\indexI}
            \coefB{\indexjpc{l}}{\indexjpc{l} r}
            \basexi{\indexI\backslash\{r\}}
            \wedge
            \basedualxi{\indexJp} 
        \end{matrix*}
        \\
        +
        \\
        %%%4
        \displaystyle\sum_{\indexjpc{l}\in\indexJpc}
        \displaystyle\sum_{r\in\indexI}
        \displaystyle\sum_{u^{'}\in\indexJp}
        \begin{matrix*}[l]
            (-1)^{p}
            \sgn
                {u^{'},r,\indexI\backslash\{r\},\order{(\indexJp\backslash\{u^{'}\})}}
                {\indexI,\indexJp}
            \sgn
                {\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
                {\indexjpc{l},(\indexJp\backslash\{u^{'}\})}
            \\
            \coefB{\indexjpc{l}}{u^{'} r}
            \basexi{\indexI\backslash\{r\}}
            \wedge
            \basedualxi{\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}} 
        \end{matrix*}
    \end{pmatrix*}.
\end{align*}
We can now calculate $
    \sqrt{-1}
    \basexi{\alpha}
    \wedge
    \big(
    -(-1)^{n^2}
    \star\,\LieagbdPartialbar\,\star
    \big)
    (\basexi{\indexI}\wedge\basedualxi{\indexJp})
$ as
\begin{align*}
    -2\sqrt{-1}
    \begin{pmatrix*}[l]
        %%%1
        \displaystyle\sum_{\indexic{k}\in\indexIc}
        \displaystyle\sum_{r\in\indexI}
        \begin{matrix*}[l]
            \sgn
                {r,\indexic{k}}
                {\order{\indexic{k},r}}
            \sgn
                {r,\indexI\backslash\{r\}}                    
                {\indexI}
            \coefD{\indexic{k}}{\order{\indexic{k},r}}
            \basexi{\alpha}
            \wedge
            \basexi{\indexI\backslash\{r\}}
            \wedge
            \basedualxi{\indexJp} 
        \end{matrix*}
        \\
        +
        \\
        %%%2
        \displaystyle\sum_{\indexic{k}\in\indexIc\backslash\{\alpha\}}
        \displaystyle\sum_{r_1\in\indexI}
        \displaystyle\sum_{r_2\in\indexI}
        \begin{matrix*}[l]
            (-1)
            \sgn
                {\order{r_1,r_2},\order{(\indexI\backslash\{r_1,r_2\})}}
                {\indexI}
            \sgn
                {\order{(\indexI\backslash\{r_1,r_2\})\cup\{\indexic{k}\}}}
                {\indexic{k},\indexI\backslash\{r_1,r_2\})}
            \\
            \frac{1}{2}
            \coefD{\indexic{k}}{\order{r_1,r_2}}
            \basexi{\alpha}
            \wedge
            \basexi{\order{(\indexI\backslash\{r_1,r_2\})\cup\{\indexic{k}\}}}
            \wedge
            \basedualxi{\indexJp} 
        \end{matrix*}
        \\
        +
        \\
        %%%3
        \displaystyle\sum_{\indexjpc{l}\in\indexJpc}
        \displaystyle\sum_{r\in\indexI}
        \begin{matrix*}[l]
            (-1)
            \sgn
                {r,\indexI\backslash\{r\}}
                {\indexI}
            \coefB{\indexjpc{l}}{\indexjpc{l} r}
            \basexi{\alpha}
            \wedge
            \basexi{\indexI\backslash\{r\}}
            \wedge
            \basedualxi{\indexJp} 
        \end{matrix*}
        \\
        +
        \\
        %%%4
        \displaystyle\sum_{\indexjpc{l}\in\indexJpc}
        \displaystyle\sum_{r\in\indexI}
        \displaystyle\sum_{u^{'}\in\indexJp}
        \begin{matrix*}[l]
            (-1)^{p}
            \sgn
                {u^{'},r,\indexI\backslash\{r\},\order{(\indexJp\backslash\{u^{'}\})}}
                {\indexI,\indexJp}
            \sgn
                {\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
                {\indexjpc{l},(\indexJp\backslash\{u^{'}\})}
            \\
            \coefB{\indexjpc{l}}{u^{'} r}
            \basexi{\alpha}
            \wedge
            \basexi{\indexI\backslash\{r\}}
            \wedge
            \basedualxi{\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}} 
        \end{matrix*}
    \end{pmatrix*}
    ,
\end{align*}
which completes the proof of Lemma \ref{lemma-Kahler identity on Lie agbd-For alpha,(I,J), calculation for RHS}.
\end{proof}

==> 5/simplification_for_RHS_of__alpha,I,J_.tex <==
In this section we calculate the following formulas:
\begin{itemize}
    %%% 1
    \item 
$
    \begin{pmatrix*}[l]
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJpc}
        \sgn
            {\indexIc\backslash\{\alpha\}}
            {\indexic{k},\indexIc\backslash\{\alpha,\indexic{k}\}}
        \\
        \sgn
            {\indexic{1},\cdots,\indexic{k-1},\order{\indexic{k},\alpha},\indexic{k+1},\cdots,\indexic{n-p}}
            {\indexIc}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\indexIc,\indexJpc,\indexI,\indexJp}
    \end{pmatrix*}
$,
    %%% 2
    \item 
$
    \begin{pmatrix*}[l]
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJpc}
    \sgn
        {\indexIc\backslash\{\alpha\}}
        {\indexic{k},\indexIc\backslash\{\alpha,\indexic{k}\}}
    \\
    \sgn
        {\indexic{1},\cdots,\indexic{k-1},\order{\indexic{k},r},\indexic{k+1},\cdots,\widehat{\alpha},\cdots,\indexic{n-p}}
        {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}}}
    \\
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}},\indexJpc,\alpha,\indexI\backslash\{r\},\indexJp}
    \end{pmatrix*}
$,
    %%% 3
    \item 
$
    \begin{pmatrix*}[l]
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJpc}
        \sgn
            {\indexIc\backslash\{\alpha\}}
            {\indexic{k},\indexIc\backslash\{\alpha,\indexic{k}\}}
        \\
        \sgn
            {\indexic{1},\cdots,\indexic{k-1},\order{\alpha,r},\indexic{k+1},\cdots,\widehat{\alpha},\cdots,\indexic{n-p}}
            {\order{(\indexIc\backslash\{\indexic{k}\})\cup\{r\}}}
        \\
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\order{(\indexIc\backslash\{\indexic{k}\})\cup\{r\}},\indexJpc,\order{(\indexI\backslash\{r\})\cup\{\indexic{k}\}},\indexJp}
    \end{pmatrix*}
$,
    %%% 4
    \item 
$
    \begin{pmatrix*}[l]
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJpc}
        \sgn
            {\indexIc\backslash\{\alpha\}}
            {\indexic{k},\indexIc\backslash\{\alpha,\indexic{k}\}}
        \\
        \sgn
            {\indexic{1},\cdots,\indexic{k-1},\order{r_1,r_2},\indexic{k+1},\cdots,\widehat{\alpha},\cdots,\indexic{n-p}}
            {\order{(\indexIc\backslash\{\indexic{k},\alpha\})\cup\{r_1,r_2\}}}
        \\
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\order{(\indexIc\backslash\{\indexic{k},\alpha\})\cup\{r_1,r_2\}},\indexJpc,\alpha,\order{(\indexI\backslash\{r_1,r_2\})\cup\{\indexic{k}\}},\indexJp}
    \end{pmatrix*}    
$,
    %%% 5
    \item 
$
    \begin{pmatrix*}[l]
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJpc}
        \sgn
            {\indexIc\backslash\{\alpha\},\indexJpc}
            {\indexjpc{l},\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\}}
        \\
        \sgn
            {\indexIc\backslash\{\alpha\},\indexjpc{1},\cdots,\indexjpc{l-1},\indexjpc{l},\alpha,\indexjpc{l+1},\cdots,\indexjpc{n-q}}
            {\indexIc,\indexJpc}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\indexIc,\indexJpc,\indexI,\indexJp}
    \end{pmatrix*}
$,
    %%% 6
    \item 
$
    \begin{pmatrix*}[l]
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJpc}
        \sgn
            {\indexIc\backslash\{\alpha\},\indexJpc}
            {\indexjpc{l},\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\}}
        \\
        \sgn
            {\indexIc\backslash\{\alpha\},\indexjpc{1},\cdots,\indexjpc{l-1},\indexjpc{l},r,\indexjpc{l+1},\cdots,\indexjpc{n-q}}
            {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}},\indexJpc}
        \\
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}},\indexJpc,\alpha,\indexI\backslash\{r\},\indexJp}
    \end{pmatrix*}
$,
    %%% 7
    \item 
$
    \begin{pmatrix*}[l]
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJpc}
        \sgn
            {\indexIc\backslash\{\alpha\},\indexJpc}
            {\indexjpc{l},\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\}}
        \\
        \sgn
            {\indexIc\backslash\{\alpha\},\indexjpc{1},\cdots,\indexjpc{l-1},u^{'},\alpha,\indexjpc{l+1},\cdots,\indexjpc{n-q}}
            {\indexIc,\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}}}
        \\
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\indexIc,\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}},\indexI,\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
    \end{pmatrix*}
$,
    %%% 8
    \item 
$
    \begin{pmatrix*}[l]
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJpc}
        \sgn
            {\indexIc\backslash\{\alpha\},\indexJpc}
            {\indexjpc{l},\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\}}
        \\
        \sgn
            {\indexIc\backslash\{\alpha\},\indexjpc{1},\cdots,\indexjpc{l-1},u^{'},r,\indexjpc{l+1},\cdots,\indexjpc{n-q}}
            {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}},\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}}}
        \\
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}},\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}},\alpha,\indexI\backslash\{r\},\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
    \end{pmatrix*}
$,
\end{itemize}
which are from (\ref{EQ-For (alpha, I, J), calculation for RHS-Step 3, unsimplfied term 1}) to (\ref{EQ-For (alpha, I, J), calculation for RHS-Step 3, unsimplfied term 8}) in Section \ref{subsection-For (alpha, I, J), calculation for RHS}. The purpose is to simplify the expression of $
\sqrt{-1}\LieagbdPartial^{*}
(\basexi{\alpha}\wedge\basexi{\indexI}\wedge\basedualxi{\indexJp})
$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%      start Lemma 1      %%%%%%%%%
\begin{lemma}
\label{Lemma-simplification for RHS of (alpha,I,J)-lemma 1}
\begin{align*}
    \begin{pmatrix*}[l]
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJpc}
        \sgn
            {\indexIc\backslash\{\alpha\}}
            {\indexic{k},\indexIc\backslash\{\alpha,\indexic{k}\}}
        \\
        \sgn
            {\indexic{1},\cdots,\indexic{k-1},\order{\indexic{k},\alpha},\indexic{k+1},\cdots,\indexic{n-p}}
            {\indexIc}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\indexIc,\indexJpc,\indexI,\indexJp}
    \end{pmatrix*}
    =
    (-1)^{n^2}
    \sgn
        {\order{\indexic{k},\alpha}}
        {\alpha,\indexic{k}}
    .
\end{align*}
\end{lemma}
\begin{proof}
We use the following properties of the sign of permutation:
\begin{itemize}
    \item 
$
    \sgn
        {\indexic{1},\cdots,\indexic{k-1},\order{\indexic{k},\alpha},\indexic{k+1},\cdots,\indexic{n-p}}
        {\indexIc}
    =
    \sgn
        {\order{\indexic{k},\alpha},\indexIc\backslash\{\indexic{k},\alpha\}}
        {\indexIc}
$,
    \item 
$
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJpc}
    \sgn
        {\indexIc\backslash\{\alpha\}}
        {\indexic{k},\indexIc\backslash\{\alpha,\indexic{k}\}}
    =
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexI,\indexJp,\indexic{k},\indexIc\backslash\{\alpha,\indexic{k}\},\indexJpc}
$.
\end{itemize}
We simplify the left-hand side of the equation in Lemma \ref{Lemma-simplification for RHS of (alpha,I,J)-lemma 1} to
\begin{align}
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexI,\indexJp,\indexic{k},\indexIc\backslash\{\alpha,\indexic{k}\},\indexJpc}
    \sgn
        {\order{\indexic{k},\alpha},\indexIc\backslash\{\indexic{k}\}}
        {\indexIc}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\indexIc,\indexJpc,\indexI,\indexJp}.
\label{EQ-simplification for RHS of (alpha,I,J)-lemma 1-no1}
\end{align}
We use the following properties of the sign of permutation:
\begin{itemize}
    \item 
$
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexI,\indexJp,\indexic{k},\indexIc\backslash\{\alpha,\indexic{k}\},\indexJpc}
    =
    (-1)^{p+q}
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\indexI,\indexJp,\alpha,\indexic{k},\indexIc\backslash\{\alpha,\indexic{k}\},\indexJpc}
$,
    \item 
$
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\indexI,\indexJp,\alpha,\indexic{k},\indexIc\backslash\{\alpha,\indexic{k}\},\indexJpc}
    \sgn
        {\alpha,\indexic{k},\indexIc\backslash\{\indexic{k}\}}
        {\indexIc}
    =
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\indexI,\indexJp,\indexIc,\indexJpc}
$,
    \item
$
    \sgn
        {\order{\indexic{k},\alpha},\indexIc\backslash\{\indexic{k}\}}
        {\indexIc}
    =
    \sgn
        {\alpha,\indexic{k},\indexIc\backslash\{\indexic{k}\}}
        {\indexIc}
    \sgn
        {\order{\indexic{k},\alpha}}
        {\alpha,\indexic{k}}
$.
\end{itemize}
We simplify (\ref{EQ-simplification for RHS of (alpha,I,J)-lemma 1-no1}) to
\begin{align}
    (-1)^{p+q}
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\indexI,\indexJp,\indexIc,\indexJpc}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\indexIc,\indexJpc,\indexI,\indexJp}
    \sgn
        {\order{\indexic{k},\alpha}}
        {\alpha,\indexic{k}}
    .
\label{EQ-simplification for RHS of (alpha,I,J)-lemma 1-no2}
\end{align}
We use the following properties of the sign of permutation:
\begin{itemize}
    \item 
$
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\indexIc,\indexJpc,\indexI,\indexJp}
    =
    (-1)^{(p+q)(n-p+n-q)}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\indexI,\indexJp,\indexIc,\indexJpc}
    \\
    =
    (-1)^{(p+q)^2}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\indexI,\indexJp,\indexIc,\indexJpc}
$,
    \item 
$
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\indexI,\indexJp,\indexIc,\indexJpc}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\indexI,\indexJp,\indexIc,\indexJpc}
    =
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {1^{'},\cdots,n^{'},1,\cdots,n}
    =
    (-1)^{n^2}
$.
\end{itemize}
We simplify (\ref{EQ-simplification for RHS of (alpha,I,J)-lemma 1-no2}) to
\begin{align*}
    (-1)^{(p+q)(p+q+1)}
    (-1)^{n^2}
    \sgn
        {\order{\indexic{k},\alpha}}
        {\alpha,\indexic{k}}
=
    (-1)^{n^2}
    \sgn
        {\order{\indexic{k},\alpha}}
        {\alpha,\indexic{k}}
    ,
\end{align*}
which completes the proof of Lemma \ref{Lemma-simplification for RHS of (alpha,I,J)-lemma 1}.
\end{proof}
%%%%%%%%%      finish Lemma 1      %%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%      start Lemma 2      %%%%%%%%%
\begin{lemma}
\label{Lemma-simplification for RHS of (alpha,I,J)-lemma 2}
\begin{align*} 
    \begin{pmatrix*}[l]
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJpc}
    \sgn
        {\indexIc\backslash\{\alpha\}}
        {\indexic{k},\indexIc\backslash\{\alpha,\indexic{k}\}}
    \\
    \sgn
        {\indexic{1},\cdots,\indexic{k-1},\order{\indexic{k},r},\indexic{k+1},\cdots,\widehat{\alpha},\cdots,\indexic{n-p}}
        {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}}}
    \\
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}},\indexJpc,\alpha,\indexI\backslash\{r\},\indexJp}
    \end{pmatrix*}
    =
    -(-1)^{n^2}
    \sgn
        {r,\indexI\backslash\{r\}}
        {\indexI}
    \sgn
        {\order{\indexic{k},r}}
        {r,\indexic{k}}
    .
\end{align*}
\end{lemma}

\begin{proof}
We use the following properties of the sign of permutation:
\begin{itemize}
    \item 
$
    \sgn
        {\indexic{1},\cdots,\indexic{k-1},\order{\indexic{k},r},\indexic{k+1},\cdots,\widehat{\alpha},\cdots,\indexic{n-p}}
        {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}}}
    =
    \sgn
        {\order{\indexic{k},r},\indexIc\backslash\{\indexic{k},\alpha\}}
        {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}}}
$,
    \item 
$
    \sgn
        {\order{\indexic{k},r},\indexIc\backslash\{\indexic{k},\alpha\}}
        {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}}}
    =
    \sgn
        {r,\indexic{k},\indexIc\backslash\{\indexic{k},\alpha\}}
        {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}}}
    \sgn
        {\order{\indexic{k},r}}
        {r,\indexic{k}}
$,
    \item
$
    \sgn
        {\indexIc\backslash\{\alpha\}}
        {\indexic{k},\indexIc\backslash\{\alpha,\indexic{k}\}}
    \sgn
        {r,\indexic{k},\indexIc\backslash\{\indexic{k},\alpha\}}
        {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}}}
    =
    \sgn
        {r,\indexIc\backslash\{\alpha\}}
        {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}}}
$.
\end{itemize}
We simplify the left-hand side of the equation in Lemma \ref{Lemma-simplification for RHS of (alpha,I,J)-lemma 2} to
\begin{align}
    \begin{pmatrix*}[l]
        \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJpc}
    \sgn
        {r,\indexIc\backslash\{\alpha\}}
        {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}}}
    \\
    \sgn
        {\order{\indexic{k},r}}
        {r,\indexic{k}}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}},\indexJpc,\alpha,\indexI\backslash\{r\},\indexJp}
    \end{pmatrix*}
    .
\label{EQ-simplification for RHS of (alpha,I,J)-lemma 2-no1}
\end{align}
We use the following properties of the sign of permutation:
\begin{itemize}
    \item 
$
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJpc}
    =
    \sgn
        {r,\indexI\backslash\{r\}}
        {\indexI}
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,r,\indexI\backslash\{r\},\indexJp,\indexIc\backslash\{\alpha\},\indexJpc}
$,
    \item 
$
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,r,\indexI\backslash\{r\},\indexJp,\indexIc\backslash\{\alpha\},\indexJpc}
    =
    (-1)^{p-1+q}
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexI\backslash\{r\},\indexJp,r,\indexIc\backslash\{\alpha\},\indexJpc}
    \\
    =
    -(-1)^{p+q}
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexI\backslash\{r\},\indexJp,r,\indexIc\backslash\{\alpha\},\indexJpc}
$,
    \item 
$
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexI\backslash\{r\},\indexJp,r,\indexIc\backslash\{\alpha\},\indexJpc}
    \sgn
        {r,\indexIc\backslash\{\alpha\}}
        {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}}}
    =
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexI\backslash\{r\},\indexJp,\order{(\indexIc\backslash\{\alpha\})\cup\{r\}},\indexJpc}
$.
\end{itemize}
We simplify (\ref{EQ-simplification for RHS of (alpha,I,J)-lemma 2-no1}) to
\begin{align}
    -(-1)^{p+q}
    \begin{pmatrix*}[l]
        \sgn
            {r,\indexI\backslash\{r\}}
            {\indexI}
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\alpha,\indexI\backslash\{r\},\indexJp,\order{(\indexIc\backslash\{\alpha\})\cup\{r\}},\indexJpc}
        \\
        \sgn
            {\order{\indexic{k},r}}
            {r,\indexic{k}}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}},\indexJpc,\alpha,\indexI\backslash\{r\},\indexJp}
    \end{pmatrix*}
    .
\label{EQ-simplification for RHS of (alpha,I,J)-lemma 2-no2}
\end{align}
We use the following properties of the sign of permutation:
\begin{itemize}
    \item 
$  
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexI\backslash\{r\},\indexJp,\order{(\indexIc\backslash\{\alpha\})\cup\{r\}},\indexJpc}
    \\
    =
    (-1)^{(p+q)(n-p+n-q)}
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}},\indexJpc,\alpha,\indexI\backslash\{r\},\indexJp}
    \\
    =
    (-1)^{(p+q)^2}
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}},\indexJpc,\alpha,\indexI\backslash\{r\},\indexJp}
$,
    \item 
$
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}},\indexJpc,\alpha,\indexI\backslash\{r\},\indexJp}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}},\indexJpc,\alpha,\indexI\backslash\{r\},\indexJp}
    \\
    =
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {1^{'},\cdots,n^{'},1,\cdots,n}
    =(-1)^{n^2}
$.
\end{itemize}
We simplify (\ref{EQ-simplification for RHS of (alpha,I,J)-lemma 2-no2}) to
\begin{align*}
    &
        -(-1)^{p+q}
        (-1)^{(p+q)^2}
        (-1)^{n^2}
        \sgn
            {r,\indexI\backslash\{r\}}
            {\indexI}
        \sgn
            {\order{\indexic{k},r}}
            {r,\indexic{k}}
    \\
    =&
        -(-1)^{n^2}
        \sgn
            {r,\indexI\backslash\{r\}}
            {\indexI}
        \sgn
            {\order{\indexic{k},r}}
            {r,\indexic{k}}
    ,
\end{align*}
which completes the proof of Lemma \ref{Lemma-simplification for RHS of (alpha,I,J)-lemma 2}.
\end{proof}
%%%%%%%%%      finish Lemma 2      %%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%      start Lemma 3      %%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}
\label{Lemma-simplification for RHS of (alpha,I,J)-lemma 3}
\begin{align*}
    \begin{pmatrix*}[l]
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJpc}
        \sgn
            {\indexIc\backslash\{\alpha\}}
            {\indexic{k},\indexIc\backslash\{\alpha,\indexic{k}\}}
        \\
        \sgn
            {\indexic{1},\cdots,\indexic{k-1},\order{\alpha,r},\indexic{k+1},\cdots,\widehat{\alpha},\cdots,\indexic{n-p}}
            {\order{(\indexIc\backslash\{\indexic{k}\})\cup\{r\}}}
        \\
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\order{(\indexIc\backslash\{\indexic{k}\})\cup\{r\}},\indexJpc,\order{(\indexI\backslash\{r\})\cup\{\indexic{k}\}},\indexJp}
    \end{pmatrix*}
    =
    (-1)^{n^2}
    \begin{pmatrix*}[l]
        \sgn
            {r,\order{(\indexI\backslash\{r\})\cup\{\indexic{k}\}}}
            {\indexic{k},\indexI}
        \\
        \sgn
            {\order{\alpha,r}}
            {\alpha,r}
    \end{pmatrix*}
    .
\end{align*}
\end{lemma}
\begin{proof}
We use the following properties of the sign of permutation:
\begin{itemize}
    \item 
$
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJpc}
    \sgn
        {\indexIc\backslash\{\alpha\}}
        {\indexic{k},\indexIc\backslash\{\alpha,\indexic{k}\}}
    =
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexI,\indexJp,\indexic{k},\indexIc\backslash\{\alpha,\indexic{k}\},\indexJpc}
$,
    \item 
$
    \sgn
        {\indexic{1},\cdots,\indexic{k-1},\order{\alpha,r},\indexic{k+1},\cdots,\widehat{\alpha},\cdots,\indexic{n-p}}
        {\order{(\indexIc\backslash\{\indexic{k}\})\cup\{r\}}}
    =
    \sgn
        {\order{\alpha,r},\indexIc\backslash\{\indexic{k},\alpha\}}
        {\order{(\indexIc\backslash\{\indexic{k}\})\cup\{r\}}}
$,
    \item 
$
    \begin{pmatrix*}[l]
        \sgn
        {\order{\alpha,r},\indexIc\backslash\{\indexic{k},\alpha\}}
        {\order{(\indexIc\backslash\{\indexic{k}\})\cup\{r\}}}
    \\
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\order{(\indexIc\backslash\{\indexic{k}\})\cup\{r\}},\indexJpc,\order{(\indexI\backslash\{r\})\cup\{\indexic{k}\}},\indexJp}
    \end{pmatrix*}
    \\
    =
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\order{\alpha,r},\indexIc\backslash\{\indexic{k},\alpha\},\indexJpc,\order{(\indexI\backslash\{r\})\cup\{\indexic{k}\}},\indexJp}
$.
\end{itemize}
We simplify the left-hand side of the equation in Lemma \ref{Lemma-simplification for RHS of (alpha,I,J)-lemma 3} to
\begin{align}
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexI,\indexJp,\indexic{k},\indexIc\backslash\{\alpha,\indexic{k}\},\indexJpc}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\order{\alpha,r},\indexIc\backslash\{\indexic{k},\alpha\},\indexJpc,\order{(\indexI\backslash\{r\})\cup\{\indexic{k}\}},\indexJp}
    .
\label{EQ-simplification for RHS of (alpha,I,J)-lemma 3-no1}
\end{align}


We use the following properties of the sign of permutation:
\begin{itemize}
    \item 
$
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexI,\indexJp,\indexic{k},\indexIc\backslash\{\alpha,\indexic{k}\},\indexJpc}
    =
    \sgn
        {r,\indexI\backslash\{r\}}
        {\indexI}
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,r,\indexI\backslash\{r\},\indexJp,\indexic{k},\indexIc\backslash\{\alpha,\indexic{k}\},\indexJpc}
$,
    \item 
$
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\order{\alpha,r},\indexIc\backslash\{\indexic{k},\alpha\},\indexJpc,\order{(\indexI\backslash\{r\})\cup\{\indexic{k}\}},\indexJp}
    \\
    =
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\alpha,r,\indexIc\backslash\{\indexic{k},\alpha\},\indexJpc,\order{(\indexI\backslash\{r\})\cup\{\indexic{k}\}},\indexJp}
    \sgn
        {\order{\alpha,r}}
        {\alpha,r}
$.
\end{itemize}
We simplify (\ref{EQ-simplification for RHS of (alpha,I,J)-lemma 3-no1}) to
\begin{align}
    \begin{pmatrix*}[l]
        \sgn
            {r,\indexI\backslash\{r\}}
            {\indexI}
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\alpha,r,\indexI\backslash\{r\},\indexJp,\indexic{k},\indexIc\backslash\{\alpha,\indexic{k}\},\indexJpc}
        \\
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\alpha,r,\indexIc\backslash\{\indexic{k},\alpha\},\indexJpc,\order{(\indexI\backslash\{r\})\cup\{\indexic{k}\}},\indexJp}
        \sgn
            {\order{\alpha,r}}
            {\alpha,r}
    \end{pmatrix*}
    .
\label{EQ-simplification for RHS of (alpha,I,J)-lemma 3-no2}
\end{align}


We use the following properties of the sign of permutation:
\begin{itemize}
    \item 
$
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,r,\indexI\backslash\{r\},\indexJp,\indexic{k},\indexIc\backslash\{\alpha,\indexic{k}\},\indexJpc}
    =
    (-1)^{p-1+q}
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,r,\indexic{k},\indexI\backslash\{r\},\indexJp,\indexIc\backslash\{\alpha,\indexic{k}\},\indexJpc}
$,
    \item 
$
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\alpha,r,\indexIc\backslash\{\indexic{k},\alpha\},\indexJpc,\order{(\indexI\backslash\{r\})\cup\{\indexic{k}\}},\indexJp}
    \\
    =
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\alpha,r,\indexIc\backslash\{\indexic{k},\alpha\},\indexJpc,\indexic{k},\indexI\backslash\{r\},\indexJp}
    \sgn
        {\order{(\indexI\backslash\{r\})\cup\{\indexic{k}\}}}
        {\indexic{k},\indexI\backslash\{r\}}
$,
    \item 
$
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\alpha,r,\indexIc\backslash\{\indexic{k},\alpha\},\indexJpc,\indexic{k},\indexI\backslash\{r\},\indexJp}
    =
    (-1)^{n-p-2+n-q}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\alpha,r,\indexic{k},\indexIc\backslash\{\indexic{k},\alpha\},\indexJpc,\indexI\backslash\{r\},\indexJp}
$.
\end{itemize}
We simplify (\ref{EQ-simplification for RHS of (alpha,I,J)-lemma 3-no2}) to
\begin{align}
    \begin{pmatrix*}[l]
        (-1)
        \sgn
            {r,\indexI\backslash\{r\}}
            {\indexI}
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\alpha,r,\indexic{k},\indexI\backslash\{r\},\indexJp,\indexIc\backslash\{\alpha,\indexic{k}\},\indexJpc}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\alpha,r,\indexic{k},\indexIc\backslash\{\indexic{k},\alpha\},\indexJpc,\indexI\backslash\{r\},\indexJp}
        \\
        \sgn
            {\order{(\indexI\backslash\{r\})\cup\{\indexic{k}\}}}
            {\indexic{k},\indexI\backslash\{r\}}
        \sgn
            {\order{\alpha,r}}
            {\alpha,r}
    \end{pmatrix*}
    .
\label{EQ-simplification for RHS of (alpha,I,J)-lemma 3-no3}
\end{align}
We use the following properties of the sign of permutation:
\begin{itemize}
    \item 
$
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\alpha,r,\indexic{k},\indexIc\backslash\{\indexic{k},\alpha\},\indexJpc,\indexI\backslash\{r\},\indexJp}
    =
        (-1)^{(n-p-2+n-q)(p-1+q)}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\alpha,r,\indexic{k},\indexI\backslash\{r\},\indexJp,\indexIc\backslash\{\indexic{k},\alpha\},\indexJpc}
    \\
    =
        (-1)^{(p+q)(p+q+1)}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\alpha,r,\indexic{k},\indexI\backslash\{r\},\indexJp,\indexIc\backslash\{\indexic{k},\alpha\},\indexJpc}
    =
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\alpha,r,\indexic{k},\indexI\backslash\{r\},\indexJp,\indexIc\backslash\{\indexic{k},\alpha\},\indexJpc}
$,
    \item 
$
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,r,\indexic{k},\indexI\backslash\{r\},\indexJp,\indexIc\backslash\{\alpha,\indexic{k}\},\indexJpc}
    \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\alpha,r,\indexic{k},\indexI\backslash\{r\},\indexJp,\indexIc\backslash\{\indexic{k},\alpha\},\indexJpc}
    \\
    =
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {1^{'},\cdots,n^{'},1,\cdots,n}
    =
    (-1)^{n^2}
$.
\end{itemize}
We simplify (\ref{EQ-simplification for RHS of (alpha,I,J)-lemma 3-no3}) to
\begin{align}
    -(-1)^{n^2}
    \sgn
        {r,\indexI\backslash\{r\}}
        {\indexI}
    \sgn
        {\order{(\indexI\backslash\{r\})\cup\{\indexic{k}\}}}
        {\indexic{k},\indexI\backslash\{r\}}
    \sgn
        {\order{\alpha,r}}
        {\alpha,r}
    .
\label{EQ-simplification for RHS of (alpha,I,J)-lemma 3-no4}
\end{align}

We use the following properties of the sign of permutation:
\begin{itemize}
    \item 
$
    \sgn
        {\order{(\indexI\backslash\{r\})\cup\{\indexic{k}\}}}
        {\indexic{k},\indexI\backslash\{r\}}
    =
    \sgn
        {r,\order{(\indexI\backslash\{r\})\cup\{\indexic{k}\}}}
        {r,\indexic{k},\indexI\backslash\{r\}}
    =
    (-1)
    \sgn
        {r,\order{(\indexI\backslash\{r\})\cup\{\indexic{k}\}}}
        {\indexic{k},r,\indexI\backslash\{r\}}
$,
    \item 
$
    \sgn
        {r,\indexI\backslash\{r\}}
        {\indexI}
    \sgn
        {r,\order{(\indexI\backslash\{r\})\cup\{\indexic{k}\}}}
        {\indexic{k},r,\indexI\backslash\{r\}}
    =
    \sgn
        {r,\order{(\indexI\backslash\{r\})\cup\{\indexic{k}\}}}
        {\indexic{k},\indexI}
$.
\end{itemize}
We simplify (\ref{EQ-simplification for RHS of (alpha,I,J)-lemma 3-no4}) to
\begin{align*}
    &
        -(-1)^{n^2}
        (-1)
        \sgn
            {r,\order{(\indexI\backslash\{r\})\cup\{\indexic{k}\}}}
            {\indexic{k},\indexI}
        \sgn
            {\order{\alpha,r}}
            {\alpha,r}
    \\
    =&
        (-1)^{n^2}
        \sgn
            {r,\order{(\indexI\backslash\{r\})\cup\{\indexic{k}\}}}
            {\indexic{k},\indexI}
        \sgn
            {\order{\alpha,r}}
            {\alpha,r}
    ,
\end{align*}
which completes the proof of Lemma \ref{Lemma-simplification for RHS of (alpha,I,J)-lemma 3}.
\end{proof}
%%%%%%%%%      finish Lemma 3      %%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%      start Lemma 4      %%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}
\label{Lemma-simplification for RHS of (alpha,I,J)-lemma 4}
\begin{align*}
    &
    \begin{pmatrix*}[l]
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJpc}
        \sgn
            {\indexIc\backslash\{\alpha\}}
            {\indexic{k},\indexIc\backslash\{\alpha,\indexic{k}\}}
        \\
        \sgn
            {\indexic{1},\cdots,\indexic{k-1},\order{r_1,r_2},\indexic{k+1},\cdots,\widehat{\alpha},\cdots,\indexic{n-p}}
            {\order{(\indexIc\backslash\{\indexic{k},\alpha\})\cup\{r_1,r_2\}}}
        \\
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\order{(\indexIc\backslash\{\indexic{k},\alpha\})\cup\{r_1,r_2\}},\indexJpc,\alpha,\order{(\indexI\backslash\{r_1,r_2\})\cup\{\indexic{k}\}},\indexJp}
    \end{pmatrix*}   
    \\
    =&
    (-1)^{n^2}
    \begin{pmatrix*}[l]
        \sgn
            {\order{r_1,r_2},\indexI\backslash\{r_1,r_2\}}
            {\indexI}
        \\
        \sgn
            {\order{(\indexI\backslash\{r_1,r_2\})\cup\{\indexic{k}\}}}
            {\indexic{k},(\indexI\backslash\{r_1,r_2\})}
    \end{pmatrix*}
    .
\end{align*}
\end{lemma}
\begin{proof}
We use the following properties of the sign of permutation:
\begin{itemize}
    \item 
$
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJpc}
    \sgn
        {\indexIc\backslash\{\alpha\}}
        {\indexic{k},\indexIc\backslash\{\alpha,\indexic{k}\}}
    =
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexI,\indexJp,\indexic{k},\indexIc\backslash\{\alpha,\indexic{k}\},\indexJpc}
$,
    \item 
$
    \sgn
        {\indexic{1},\cdots,\indexic{k-1},\order{r_1,r_2},\indexic{k+1},\cdots,\widehat{\alpha},\cdots,\indexic{n-p}}
        {\order{(\indexIc\backslash\{\indexic{k},\alpha\})\cup\{r_1,r_2\}}}
    =
    \sgn
        {\order{r_1,r_2},\indexIc\backslash\{\indexic{k},\alpha\}}
        {\order{(\indexIc\backslash\{\indexic{k},\alpha\})\cup\{r_1,r_2\}}}
$,
    \item 
$
    \sgn
        {\order{r_1,r_2},\indexIc\backslash\{\indexic{k},\alpha\}}
        {\order{(\indexIc\backslash\{\indexic{k},\alpha\})\cup\{r_1,r_2\}}}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\order{(\indexIc\backslash\{\indexic{k},\alpha\})\cup\{r_1,r_2\}},\indexJpc,\alpha,\order{(\indexI\backslash\{r_1,r_2\})\cup\{\indexic{k}\}},\indexJp}
    \\
    =
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\order{r_1,r_2},\indexIc\backslash\{\indexic{k},\alpha\},\indexJpc,\alpha,\order{(\indexI\backslash\{r_1,r_2\})\cup\{\indexic{k}\}},\indexJp}
$.
\end{itemize}
We simplify the left-hand side of the equation in Lemma \ref{Lemma-simplification for RHS of (alpha,I,J)-lemma 4} to
\begin{align}
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexI,\indexJp,\indexic{k},\indexIc\backslash\{\alpha,\indexic{k}\},\indexJpc}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\order{r_1,r_2},\indexIc\backslash\{\indexic{k},\alpha\},\indexJpc,\alpha,\order{(\indexI\backslash\{r_1,r_2\})\cup\{\indexic{k}\}},\indexJp}
    .
\label{EQ-simplification for RHS of (alpha,I,J)-lemma 4-no1}
\end{align}


We use the following properties of the sign of permutation:
\begin{itemize}
    \item 
$
    \sgn
    {1^{'},\cdots,n^{'},1,\cdots,n}
    {\order{r_1,r_2},\indexIc\backslash\{\indexic{k},\alpha\},\indexJpc,\alpha,\order{(\indexI\backslash\{r_1,r_2\})\cup\{\indexic{k}\}},\indexJp}
    \\
    =
    \begin{pmatrix*}[l]
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\order{r_1,r_2},\indexIc\backslash\{\indexic{k},\alpha\},\indexJpc,\alpha,\indexic{k},\indexI\backslash\{r_1,r_2\},\indexJp}
        \\
        \sgn
            {\order{(\indexI\backslash\{r_1,r_2\})\cup\{\indexic{k}\}}}
            {\indexic{k},\indexI\backslash\{r_1,r_2\}}
    \end{pmatrix*}
$,
    \item 
$
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\order{r_1,r_2},\indexIc\backslash\{\indexic{k},\alpha\},\indexJpc,\alpha,\indexic{k},\indexI\backslash\{r_1,r_2\},\indexJp}
        =
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\indexIc\backslash\{\indexic{k},\alpha\},\indexJpc,\alpha,\indexic{k},\order{r_1,r_2},\indexI\backslash\{r_1,r_2\},\indexJp}
        \\
        =
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\indexIc\backslash\{\indexic{k},\alpha\},\indexJpc,\alpha,\indexic{k},\indexI,\indexJp}
        \sgn
            {\order{r_1,r_2},\indexI\backslash\{r_1,r_2\}}
            {\indexI}  
$.
\end{itemize}
We simplify (\ref{EQ-simplification for RHS of (alpha,I,J)-lemma 4-no1}) to
\begin{align}
    \begin{pmatrix*}[l]
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\alpha,\indexI,\indexJp,\indexic{k},\indexIc\backslash\{\alpha,\indexic{k}\},\indexJpc}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\indexIc\backslash\{\indexic{k},\alpha\},\indexJpc,\alpha,\indexic{k},\indexI,\indexJp}
        \\
        \sgn
            {\order{r_1,r_2},\indexI\backslash\{r_1,r_2\}}
            {\indexI}
        \sgn
            {\order{(\indexI\backslash\{r_1,r_2\})\cup\{\indexic{k}\}}}
            {\indexic{k},(\indexI\backslash\{r_1,r_2\})}
    \end{pmatrix*}
    .
\label{EQ-simplification for RHS of (alpha,I,J)-lemma 4-no2}
\end{align}


We use the following properties of the sign of permutation:
\begin{itemize}
    \item 
$
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexI,\indexJp,\indexic{k},\indexIc\backslash\{\alpha,\indexic{k}\},\indexJpc}
    =
    (-1)^{p+q}
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexic{k},\indexI,\indexJp,\indexIc\backslash\{\alpha,\indexic{k}\},\indexJpc}
$,
    \item 
$
        \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\indexIc\backslash\{\indexic{k},\alpha\},\indexJpc,\alpha,\indexic{k},\indexI,\indexJp}
        =
        (-1)^{(p+q+2)(n-p-2+n-q)}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\alpha,\indexic{k},\indexI,\indexJp,\indexIc\backslash\{\indexic{k},\alpha\},\indexJpc}
        \\
        =
        (-1)^{(p+q)}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\alpha,\indexic{k},\indexI,\indexJp,\indexIc\backslash\{\indexic{k},\alpha\},\indexJpc}
$,
    \item
$
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexic{k},\indexI,\indexJp,\indexIc\backslash\{\alpha,\indexic{k}\},\indexJpc}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\alpha,\indexic{k},\indexI,\indexJp,\indexIc\backslash\{\indexic{k},\alpha\},\indexJpc}
    =
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {1^{'},\cdots,n^{'},1,\cdots,n}
    =
    (-1)^{n^2}
$.
\end{itemize}
We simplify (\ref{EQ-simplification for RHS of (alpha,I,J)-lemma 4-no2}) to
\begin{align*}
    (-1)^{n^2}
    \sgn
        {\order{r_1,r_2},\indexI\backslash\{r_1,r_2\}}
        {\indexI}
    \sgn
        {\order{(\indexI\backslash\{r_1,r_2\})\cup\{\indexic{k}\}}}
        {\indexic{k},(\indexI\backslash\{r_1,r_2\})}
    ,
\end{align*}
which completes the proof of Lemma \ref{Lemma-simplification for RHS of (alpha,I,J)-lemma 4}.
\end{proof}
%%%%%%%%%      finish Lemma 4      %%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%      start Lemma 5      %%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}
\label{Lemma-simplification for RHS of (alpha,I,J)-lemma 5}
\begin{align*}
    \begin{pmatrix*}[l]
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJpc}
        \sgn
            {\indexIc\backslash\{\alpha\},\indexJpc}
            {\indexjpc{l},\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\}}
        \\
        \sgn
            {\indexIc\backslash\{\alpha\},\indexjpc{1},\cdots,\indexjpc{l-1},\indexjpc{l},\alpha,\indexjpc{l+1},\cdots,\indexjpc{n-q}}
            {\indexIc,\indexJpc}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\indexIc,\indexJpc,\indexI,\indexJp}
    \end{pmatrix*}
    =
    -(-1)^{n^2}
    .
\end{align*}
\end{lemma}


\begin{proof}
We use the following properties of the sign of permutation:
\begin{itemize}
    \item 
$
        \sgn
            {\indexIc\backslash\{\alpha\},\indexJpc}
            {\indexjpc{l},\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\}}
        =
        \sgn
            {\alpha,\indexIc\backslash\{\alpha\},\indexJpc}
            {\alpha,\indexjpc{l},\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\}}
        \\
        =
        (-1)
        \sgn
            {\alpha,\indexIc\backslash\{\alpha\},\indexJpc}
            {\indexjpc{l},\alpha,\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\}}
        =
        (-1)
        \sgn
            {\alpha,\indexIc\backslash\{\alpha\},\indexJpc}
            {\indexIc\backslash\{\alpha\},\indexjpc{1},\cdots,\indexjpc{l-1},\indexjpc{l},\alpha,\indexjpc{l+1},\cdots,\indexjpc{n-q}}
$,
    \item 
$
        \sgn
            {\alpha,\indexIc\backslash\{\alpha\},\indexJpc}
            {\indexIc\backslash\{\alpha\},\indexjpc{1},\cdots,\indexjpc{l-1},\indexjpc{l},\alpha,\indexjpc{l+1},\cdots,\indexjpc{n-q}}
        \sgn
            {\indexIc\backslash\{\alpha\},\indexjpc{1},\cdots,\indexjpc{l-1},\indexjpc{l},\alpha,\indexjpc{l+1},\cdots,\indexjpc{n-q}}
            {\indexIc,\indexJpc}
        \\
        =
        \sgn
            {\alpha,\indexIc\backslash\{\alpha\},\indexJpc}
            {\indexIc,\indexJpc}
$.
\end{itemize}
We simplify the left-hand side of the equation in Lemma \ref{Lemma-simplification for RHS of (alpha,I,J)-lemma 5} to
\begin{align}
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJpc}
    (-1)
    \sgn
        {\alpha,\indexIc\backslash\{\alpha\},\indexJpc}
        {\indexIc,\indexJpc}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\indexIc,\indexJpc,\indexI,\indexJp}
    .
\label{EQ-simplification for RHS of (alpha,I,J)-lemma 5-no1}
\end{align}


We use the following properties of the sign of permutation:
\begin{itemize}
    \item 
$
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJpc}
    =
    (-1)^{p+q}
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\indexI,\indexJp,\alpha,\indexIc\backslash\{\alpha\},\indexJpc}
$,
    \item 
$
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\indexI,\indexJp,\alpha,\indexIc\backslash\{\alpha\},\indexJpc}
    \sgn
        {\alpha,\indexIc\backslash\{\alpha\},\indexJpc}
        {\indexIc,\indexJpc}
    =
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\indexI,\indexJp,\indexIc,\indexJpc}
    \\
    =
    (-1)^{(p+q)(n-p+n-q)}
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\indexIc,\indexJpc,\indexI,\indexJp}
$,
    \item 
$
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\indexIc,\indexJpc,\indexI,\indexJp}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\indexIc,\indexJpc,\indexI,\indexJp}
    =
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {1^{'},\cdots,n^{'},1,\cdots,n}
    =
    (-1)^{n^2}
$.
\end{itemize}
We simplify (\ref{EQ-simplification for RHS of (alpha,I,J)-lemma 5-no1}) to
\begin{align*}
    (-1)^{p+q}
    (-1)^{(p+q)(n-p+n-q)}
    (-1)^{n^2}
    =
    (-1)^{(p+q)(p+q+1)}
    (-1)^{n^2}
    =
    -(-1)^{n^2}
    ,
\end{align*}
which completes the proof of Lemma \ref{Lemma-simplification for RHS of (alpha,I,J)-lemma 5}.
\end{proof}
%%%%%%%%%      finish Lemma 5      %%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%      start Lemma 6      %%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}
\label{Lemma-simplification for RHS of (alpha,I,J)-lemma 6}
\begin{align*}
    \begin{pmatrix*}[l]
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJpc}
        \sgn
            {\indexIc\backslash\{\alpha\},\indexJpc}
            {\indexjpc{l},\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\}}
        \\
        \sgn
            {\indexIc\backslash\{\alpha\},\indexjpc{1},\cdots,\indexjpc{l-1},\indexjpc{l},r,\indexjpc{l+1},\cdots,\indexjpc{n-q}}
            {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}},\indexJpc}
        \\
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}},\indexJpc,\alpha,\indexI\backslash\{r\},\indexJp}
    \end{pmatrix*}
    =
    (-1)^{n^2}
    \sgn
        {r,\indexI\backslash\{r\}}
        {\indexI}
    .
\end{align*}
\end{lemma}


\begin{proof}
We use the following properties of the sign of permutation:
\begin{itemize}
    \item 
$
    \sgn
        {\indexIc\backslash\{\alpha\},\indexjpc{1},\cdots,\indexjpc{l-1},\indexjpc{l},r,\indexjpc{l+1},\cdots,\indexjpc{n-q}}
        {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}},\indexJpc}
    =
    \sgn
        {\indexjpc{l},r,\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\}}
        {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}},\indexJpc}
    \\
    =
    (-1)
    \sgn
        {r,\indexjpc{l},\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\}}
        {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}},\indexJpc}
$,
    \item 
$
    \sgn
        {\indexIc\backslash\{\alpha\},\indexJpc}
        {\indexjpc{l},\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\}}
    \sgn
        {r,\indexjpc{l},\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\}}
        {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}},\indexJpc}
    =
    \sgn
        {r,\indexIc\backslash\{\alpha\},\indexJpc}
        {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}},\indexJpc}
$.
\end{itemize}
We simplify the left-hand side of the equation in Lemma \ref{Lemma-simplification for RHS of (alpha,I,J)-lemma 6} to
\begin{align}
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJpc}
    (-1)
    \sgn
        {r,\indexIc\backslash\{\alpha\},\indexJpc}
        {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}},\indexJpc}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}},\indexJpc,\alpha,\indexI\backslash\{r\},\indexJp}
    .
\label{EQ-simplification for RHS of (alpha,I,J)-lemma 6-no1}
\end{align}


We use the following properties of the sign of permutation:
\begin{itemize}
    \item 
$
    \sgn
        {r,\indexIc\backslash\{\alpha\},\indexJpc}
        {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}},\indexJpc}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}},\indexJpc,\alpha,\indexI\backslash\{r\},\indexJp}
    \\
    =
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {r,\indexIc\backslash\{\alpha\},\indexJpc,\alpha,\indexI\backslash\{r\},\indexJp}
$,
    \item 
$
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {r,\indexIc\backslash\{\alpha\},\indexJpc,\alpha,\indexI\backslash\{r\},\indexJp}
    =
    (-1)
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\alpha,\indexIc\backslash\{\alpha\},\indexJpc,r,\indexI\backslash\{r\},\indexJp}
$,
    \item 
$
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\alpha,\indexIc\backslash\{\alpha\},\indexJpc,r,\indexI\backslash\{r\},\indexJp}
    =
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\alpha,\indexIc\backslash\{\alpha\},\indexJpc,\indexI,\indexJp}
    \sgn
        {r,\indexI\backslash\{r\}}
        {\indexI}
$.
\end{itemize}
We simplify (\ref{EQ-simplification for RHS of (alpha,I,J)-lemma 6-no1}) to
\begin{align}
    &
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJpc}
    (-1)(-1)
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\alpha,\indexIc\backslash\{\alpha\},\indexJpc,\indexI,\indexJp}
    \sgn
        {r,\indexI\backslash\{r\}}
        {\indexI}
    \notag
    \\
    =&
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJpc}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\alpha,\indexIc\backslash\{\alpha\},\indexJpc,\indexI,\indexJp}
    \sgn
        {r,\indexI\backslash\{r\}}
        {\indexI}
    .
\label{EQ-simplification for RHS of (alpha,I,J)-lemma 6-no2}
\end{align}


We use the following properties of the sign of permutation:
\begin{itemize}
    \item 
$
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJpc}
    =
    (-1)^{(p+q)(n-p-1+n-q)}
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexIc\backslash\{\alpha\},\indexJpc,\indexI,\indexJp}
$,
    \item 
$
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexIc\backslash\{\alpha\},\indexJpc,\indexI,\indexJp}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\alpha,\indexIc\backslash\{\alpha\},\indexJpc,\indexI,\indexJp}
    =
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {1^{'},\cdots,n^{'},1,\cdots,n}
    =
    (-1)^{n^2}
$.
\end{itemize}
We simplify (\ref{EQ-simplification for RHS of (alpha,I,J)-lemma 6-no2}) to
\begin{align*}
    &
    (-1)^{(p+q)(n-p-1+n-q)}
    (-1)^{n^2}
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexIc\backslash\{\alpha\},\indexJpc,\indexI,\indexJp}
    \\
    =&
    (-1)^{n^2}
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexIc\backslash\{\alpha\},\indexJpc,\indexI,\indexJp}
    ,
\end{align*}
which completes the proof of Lemma \ref{Lemma-simplification for RHS of (alpha,I,J)-lemma 6}.
\end{proof}
%%%%%%%%%      finish Lemma 6      %%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%      start Lemma 7      %%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}
\label{Lemma-simplification for RHS of (alpha,I,J)-lemma 7}
\begin{align*}
    \begin{pmatrix*}[l]
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJpc}
        \sgn
            {\indexIc\backslash\{\alpha\},\indexJpc}
            {\indexjpc{l},\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\}}
        \\
        \sgn
            {\indexIc\backslash\{\alpha\},\indexjpc{1},\cdots,\indexjpc{l-1},u^{'},\alpha,\indexjpc{l+1},\cdots,\indexjpc{n-q}}
            {\indexIc,\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}}}
        \\
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\indexIc,\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}},\indexI,\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
    \end{pmatrix*}
    =
    -(-1)^{n^2}
    \sgn
        {u^{'},\indexI,\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
        {\indexjpc{l},\indexI,\indexJp}
    .
\end{align*}
\end{lemma}


\begin{proof}
We use the following properties of the sign of permutation:
\begin{itemize}
    \item 
$
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJpc}
    \sgn
        {\indexIc\backslash\{\alpha\},\indexJpc}
        {\indexjpc{l},\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\}}
    =
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexI,\indexJp,\indexjpc{l},\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\}}
$,
    \item 
$
    \sgn
        {\indexIc\backslash\{\alpha\},\indexjpc{1},\cdots,\indexjpc{l-1},u^{'},\alpha,\indexjpc{l+1},\cdots,\indexjpc{n-q}}
        {\indexIc,\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}}}
    =
    \sgn
        {u^{'},\alpha,\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\}}
        {\indexIc,\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}}}
$,
    \item 
$
    \sgn
        {u^{'},\alpha,\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\}}
        {\indexIc,\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}}}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\indexIc,\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}},\indexI,\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
    \\
    =
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {u^{'},\alpha,\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\},\indexI,\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
$.
\end{itemize}
We simplify the left-hand side of the equation in Lemma \ref{Lemma-simplification for RHS of (alpha,I,J)-lemma 7} to
\begin{align}
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexI,\indexJp,\indexjpc{l},\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\}}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {u^{'},\alpha,\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\},\indexI,\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
    .
\label{EQ-simplification for RHS of (alpha,I,J)-lemma 7-no1}
\end{align}


We use the following properties of the sign of permutation:
\begin{itemize}
    \item 
$
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexI,\indexJp,\indexjpc{l},\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\}}
    =
    (-1)^{p+q}
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexjpc{l},\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\}}
$,
    \item 
$
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {u^{'},\alpha,\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\},\indexI,\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
    \\
    =
    (-1)^{n-p+n-q-1}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\alpha,\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\},u^{'},\indexI,\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
$,
    \item 
$
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\alpha,\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\},u^{'},\indexI,\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
    \\
    =
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\alpha,\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\},\indexjpc{l},\indexI,\indexJp}
    \sgn
        {u^{'},\indexI,\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
        {\indexjpc{l},\indexI,\indexJp}
$.
\end{itemize}
We simplify (\ref{EQ-simplification for RHS of (alpha,I,J)-lemma 7-no1}) to
\begin{align}
    &
    \begin{pmatrix*}
        (-1)^{p+q}
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexjpc{l},\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\}}
    \\
    (-1)^{n-p+n-q-1}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\alpha,\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\},\indexjpc{l},\indexI,\indexJp}
    \sgn
        {u^{'},\indexI,\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
        {\indexjpc{l},\indexI,\indexJp}
    \end{pmatrix*}
    \notag
    \\
    =&
    (-1)
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexjpc{l},\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\}}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\alpha,\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\},\indexjpc{l},\indexI,\indexJp}
    \sgn
        {u^{'},\indexI,\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
        {\indexjpc{l},\indexI,\indexJp}    
    .
\label{EQ-simplification for RHS of (alpha,I,J)-lemma 7-no2}
\end{align}


We use the following properties of the sign of permutation:
\begin{itemize}
    \item 
$
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\alpha,\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\},\indexjpc{l},\indexI,\indexJp}
    =
    (-1)^{(n-p-1+n-q-1)(p+q+1)}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\alpha,\indexjpc{l},\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\}}
$,
    \item
$
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexjpc{l},\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\}}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\alpha,\indexjpc{l},\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\}}
    \\
    =
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {1^{'},\cdots,n^{'},1,\cdots,n}
    =
    (-1)^{n^2}
$.
\end{itemize}
We simplify (\ref{EQ-simplification for RHS of (alpha,I,J)-lemma 7-no2}) to
\begin{align*}
    &
    (-1)
    (-1)^{(p+q)(p+q+1)}
    (-1)^{n^2}
    \sgn
        {u^{'},\indexI,\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
        {\indexjpc{l},\indexI,\indexJp}
    \\
    =&
    -(-1)^{n^2}
    \sgn
        {u^{'},\indexI,\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
        {\indexjpc{l},\indexI,\indexJp}
    ,
\end{align*}
which completes the proof of Lemma \ref{Lemma-simplification for RHS of (alpha,I,J)-lemma 7}.
\end{proof}
%%%%%%%%%      finish Lemma 7      %%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%      start Lemma 8      %%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}
\label{Lemma-simplification for RHS of (alpha,I,J)-lemma 8}
\begin{align*}
    &
    \begin{pmatrix*}[l]
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJpc}
        \sgn
            {\indexIc\backslash\{\alpha\},\indexJpc}
            {\indexjpc{l},\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\}}
        \\
        \sgn
            {\indexIc\backslash\{\alpha\},\indexjpc{1},\cdots,\indexjpc{l-1},u^{'},r,\indexjpc{l+1},\cdots,\indexjpc{n-q}}
            {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}},\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}}}
        \\
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}},\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}},\alpha,\indexI\backslash\{r\},\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
    \end{pmatrix*}
    \\
    =&
    \begin{pmatrix*}
        (-1)^{p+1}
        (-1)^{n^2}
        \\
        \sgn
            {u^{'},r,\indexI\backslash\{r\},\indexJp\backslash\{u^{'}\}}
            {\indexI,\indexJp}
        \\
        \sgn
            {\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
            {\indexjpc{l},\indexJp\backslash\{u^{'}\}}
    \end{pmatrix*}
    .
\end{align*}
\end{lemma}
\begin{proof}
We use the following properties of the sign of permutation:
\begin{itemize}
    \item 
$
    \sgn
        {\indexIc\backslash\{\alpha\},\indexjpc{1},\cdots,\indexjpc{l-1},u^{'},r,\indexjpc{l+1},\cdots,\indexjpc{n-q}}
        {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}},\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}}}
    =
    \sgn
        {u^{'},r,\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\}}
        {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}},\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}}}
$,
    \item 
$
    \begin{pmatrix*}
        \sgn
            {u^{'},r,\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\}}
            {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}},\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}}}
        \\
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\order{(\indexIc\backslash\{\alpha\})\cup\{r\}},\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}},\alpha,\indexI\backslash\{r\},\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
    \end{pmatrix*}
    \\
    =
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {u^{'},r,\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\},\alpha,\indexI\backslash\{r\},\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
$.
\end{itemize}
We simplify the left-hand side of the equation in Lemma \ref{Lemma-simplification for RHS of (alpha,I,J)-lemma 8} to
\begin{align}
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJpc}
    \sgn
        {\indexIc\backslash\{\alpha\},\indexJpc}
        {\indexjpc{l},\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\}}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {u^{'},r,\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\},\alpha,\indexI\backslash\{r\},\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
    .
\label{EQ-simplification for RHS of (alpha,I,J)-lemma 8-no1}
\end{align}


We use the following properties of the sign of permutation:
\begin{itemize}
    \item 
$
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {u^{'},r,\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\},\alpha,\indexI\backslash\{r\},\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
    \\
    =
    \begin{pmatrix*}[l]
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {u^{'},r,\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\},\alpha,\indexI\backslash\{r\},\indexjpc{l},\indexJp\backslash\{u^{'}\}}
        \\
        \sgn
            {\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
            {\indexjpc{l},\indexJp\backslash\{u^{'}\}}
    \end{pmatrix*}
$,
    \item 
$
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {u^{'},r,\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\},\alpha,\indexI\backslash\{r\},\indexjpc{l},\indexJp\backslash\{u^{'}\}}
    \\
    =
    (-1)^{p+n-q-1+n-p-1}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {u^{'},r,\indexIc\backslash\{\alpha\},\indexjpc{l},\indexJpc\backslash\{\indexjpc{l}\},\alpha,\indexI\backslash\{r\},\indexJp\backslash\{u^{'}\}}
$,
    \item 
$
    \sgn
        {\indexIc\backslash\{\alpha\},\indexJpc}
        {\indexjpc{l},\indexIc\backslash\{\alpha\},\indexJpc\backslash\{\indexjpc{l}\}}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {u^{'},r,\indexIc\backslash\{\alpha\},\indexjpc{l},\indexJpc\backslash\{\indexjpc{l}\},\alpha,\indexI\backslash\{r\},\indexJp\backslash\{u^{'}\}}
    \\
    =
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {u^{'},r,\indexIc\backslash\{\alpha\},\indexJpc,\alpha,\indexI\backslash\{r\},\indexJp\backslash\{u^{'}\}}
$.
\end{itemize}
We simplify (\ref{EQ-simplification for RHS of (alpha,I,J)-lemma 8-no1}) to
\begin{align}
    &
    \begin{pmatrix*}[l]
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJpc}
        (-1)^{p+n-q-1+n-p-1}
        \\
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {u^{'},r,\indexIc\backslash\{\alpha\},\indexJpc,\alpha,\indexI\backslash\{r\},\indexJp\backslash\{u^{'}\}}
        \sgn
            {\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
            {\indexjpc{l},\indexJp\backslash\{u^{'}\}}
    \end{pmatrix*}
    \notag
    \\
    =&
    (-1)^{q}
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJpc}  
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {u^{'},r,\indexIc\backslash\{\alpha\},\indexJpc,\alpha,\indexI\backslash\{r\},\indexJp\backslash\{u^{'}\}}
    \sgn
        {\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
        {\indexjpc{l},\indexJp\backslash\{u^{'}\}}
    .
\label{EQ-simplification for RHS of (alpha,I,J)-lemma 8-no2}
\end{align}


We use the following properties of the sign of permutation:
\begin{itemize}
    \item 
$
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {u^{'},r,\indexIc\backslash\{\alpha\},\indexJpc,\alpha,\indexI\backslash\{r\},\indexJp\backslash\{u^{'}\}}
    =
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\indexIc\backslash\{\alpha\},\indexJpc,\alpha,u^{'},r,\indexI\backslash\{r\},\indexJp\backslash\{u^{'}\}}
$,
    \item 
$
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\indexIc\backslash\{\alpha\},\indexJpc,\alpha,u^{'},r,\indexI\backslash\{r\},\indexJp\backslash\{u^{'}\}}
    =
    (-1)^{n-p-1+n-q}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\alpha,\indexIc\backslash\{\alpha\},\indexJpc,u^{'},r,\indexI\backslash\{r\},\indexJp\backslash\{u^{'}\}} 
$,
    \item 
$
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\alpha,\indexIc\backslash\{\alpha\},\indexJpc,u^{'},r,\indexI\backslash\{r\},\indexJp\backslash\{u^{'}\}} 
    =
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\alpha,\indexIc\backslash\{\alpha\},\indexJpc,\indexI,\indexJp}
    \sgn
        {u^{'},r,\indexI\backslash\{r\},\indexJp\backslash\{u^{'}\}}
        {\indexI,\indexJp}
$.
\end{itemize}
We simplify (\ref{EQ-simplification for RHS of (alpha,I,J)-lemma 8-no2}) to
\begin{align}
    &
        \begin{pmatrix*}[l]
            \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJpc}
        (-1)^{q}
        (-1)^{n-p-1+n-q}
        \\
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\alpha,\indexIc\backslash\{\alpha\},\indexJpc,\indexI,\indexJp}
        \sgn
            {u^{'},r,\indexI\backslash\{r\},\indexJp\backslash\{u^{'}\}}
            {\indexI,\indexJp}
        \sgn
            {\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
            {\indexjpc{l},\indexJp\backslash\{u^{'}\}}
        \end{pmatrix*}
    \notag
    \\
    =&
        \begin{pmatrix*}[l]
            \sgn
                {1,\cdots,n,1^{'},\cdots,n^{'}}
                {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJpc}
            (-1)^{p+1}
            \sgn
                {1^{'},\cdots,n^{'},1,\cdots,n}
                {\alpha,\indexIc\backslash\{\alpha\},\indexJpc,\indexI,\indexJp}
            \\
            \sgn
                {u^{'},r,\indexI\backslash\{r\},\indexJp\backslash\{u^{'}\}}
                {\indexI,\indexJp}
            \sgn
                {\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
                {\indexjpc{l},\indexJp\backslash\{u^{'}\}}
        \end{pmatrix*}
    .
\label{EQ-simplification for RHS of (alpha,I,J)-lemma 8-no3}
\end{align}


We use the following properties of the sign of permutation:
\begin{itemize}
    \item 
$
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\alpha,\indexIc\backslash\{\alpha\},\indexJpc,\indexI,\indexJp}
    =
    (-1)^{(n-p-1+n-q)(p+q)}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJpc}
    \\
    =
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJpc}
$,
    \item 
$
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJpc}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\alpha,\indexI,\indexJp,\indexIc\backslash\{\alpha\},\indexJpc}
    =
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {1^{'},\cdots,n^{'},1,\cdots,n}
    =
    (-1)^{n^2}
$.
\end{itemize}
We simplify (\ref{EQ-simplification for RHS of (alpha,I,J)-lemma 8-no3}) to
\begin{align*}
    (-1)^{p+1}
    (-1)^{n^2}
    \sgn
        {u^{'},r,\indexI\backslash\{r\},\indexJp\backslash\{u^{'}\}}
        {\indexI,\indexJp}
    \sgn
        {\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
        {\indexjpc{l},\indexJp\backslash\{u^{'}\}}
    ,
\end{align*}
which completes the proof of Lemma \ref{Lemma-simplification for RHS of (alpha,I,J)-lemma 8}.
\end{proof}
%%%%%%%%%      finish Lemma 8      %%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> 5/simplification_for_RHS_of__i,j_.tex <==
In this section, we simplify the following three formulas:
\begin{align}
    &
    \begin{pmatrix*}[l]
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {i,j^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
        \sgn
            {1,\cdots,\widehat{i},\cdots,n}
            {k,1,\cdots,\widehat{i},\cdots,\widehat{k},\cdots,n}
        \sgn
            {1,\cdots,\widehat{i},\cdots,k-1,k,i,k+1,\cdots,n}
            {1,\cdots,n}
        \\
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {j^{'},1,\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
    \end{pmatrix*}
    ,
\label{EQ-simplification for RHS of (i,j)-target 1}
    \\
    &
    \begin{pmatrix*}[l]
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {i,j^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
        \sgn
            {1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
            {l^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,\widehat{l^{'}},\cdots,n^{'}}
        \\
        \sgn
            {1,\cdots,\widehat{i}\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,(l-1)^{'},l^{'},i,(l+1)^{'},\cdots,n^{'}}
            {1,\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {j^{'},1,\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
    \end{pmatrix*}
    ,
\label{EQ-simplification for RHS of (i,j)-target 2}
    \\
    &
    \begin{pmatrix*}[l]
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {i,j^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
        \sgn
            {1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
            {l^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,\widehat{l^{'}},\cdots,n^{'}}
        \\
        \sgn
            {1,\cdots,\widehat{i}\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,(l-1)^{'},j^{'},i,(l+1)^{'},\cdots,n^{'}}
            {1,\cdots,n,1^{'},\cdots,\widehat{l^{'}},\cdots,n^{'}}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {l^{'},1,\cdots,n,1^{'},\cdots,\widehat{l^{'}},\cdots,n^{'}}
    \end{pmatrix*}
    ,
\label{EQ-simplification for RHS of (i,j)-target 3}
\end{align}
which are from (\ref{EQ-Kahler identity on Lie agbd-calculation for RHS of (i,j)-no5}) in Lemma \ref{Lemma-Kahler identity on Lie algebroid-the first lemma}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lemma}
$
    \begin{pmatrix*}
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {i,j^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
    \sgn
        {1,\cdots,\widehat{i},\cdots,n}
        {k,1,\cdots,\widehat{i},\cdots,\widehat{k},\cdots,n}
    \sgn
        {1,\cdots,\widehat{i},\cdots,k-1,k,i,k+1,\cdots,n}
        {1,\cdots,n}
    \\
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {j^{'},1,\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
    \end{pmatrix*}
    =
    (-1)^{n^2}.
$
\end{lemma}

\begin{proof}
We use the following properties of the sign of permutation:
\begin{itemize}
    \item
$
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {i,j^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
    =
    -
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {j^{'},i,1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}},
$
    \item 
$
    \sgn
        {1,\cdots,\widehat{i},\cdots,k-1,k,i,k+1,\cdots,n}
        {1,\cdots,n}
    =
    \sgn
        {k,i,1,\cdots,\widehat{i},\cdots,k-1,k+1,\cdots,n}
        {1,\cdots,n}
    =
    -\sgn
        {i,k,1,\cdots,\widehat{i},\cdots,k-1,k+1,\cdots,n}
        {1,\cdots,n},
$
    \item
$
    \sgn
        {1,\cdots,\widehat{i},\cdots,n}
        {k,1,\cdots,\widehat{i},\cdots,\widehat{k},\cdots,n}
    \sgn
        {i,k,1,\cdots,\widehat{i},\cdots,k-1,k+1,\cdots,n}
        {1,\cdots,n}
    =
    \sgn
        {i,1,\cdots,\widehat{i},\cdots,n}
        {1,\cdots,n}.
$
\end{itemize}
Expression (\ref{EQ-simplification for RHS of (i,j)-target 1}) is simplified to
\begin{align}
    (-1)
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {j^{'},i,1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
    (-1)
    \sgn
        {i,1,\cdots,\widehat{i},\cdots,n}
        {1,\cdots,n}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {j^{'},1,\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}.
    \label{EQ-simplification for RHS of (i,j)-simplify of target 1-no1}
\end{align}
We continue the computation with the following properties of the sign of permutation:
\begin{itemize}
    \item 
$
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {j^{'},i,1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
    \sgn
        {i,1,\cdots,\widehat{i},\cdots,n}
        {1,\cdots,n}
    =
     \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {j^{'},1,\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}},
$
    \item
$
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {j^{'},1,\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {j^{'},1,\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
    =
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {1^{'},\cdots,n^{'},1,\cdots,n}.
$
\end{itemize}
Expression (\ref{EQ-simplification for RHS of (i,j)-simplify of target 1-no1}) is then simplified to
\begin{align*}
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {1^{'},\cdots,n^{'},1,\cdots,n}
    =
    (-1)^{n^2}.
\end{align*}
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{lemma}
    $
    \begin{pmatrix*}[l]
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {i,j^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
        \sgn
            {1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
            {l^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,\widehat{l^{'}},\cdots,n^{'}}
        \\
        \sgn
            {1,\cdots,\widehat{i}\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,(l-1)^{'},l^{'},i,(l+1)^{'},\cdots,n^{'}}
            {1,\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {j^{'},1,\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
    \end{pmatrix*}
    =
    (-1)^{n^2}.
    $
\end{lemma}

\begin{proof}
We use the following properties of the sign of permutation:
\begin{itemize}
    \item
$
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {i,j^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
    =
    (-1)
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {j^{'},i,1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
$,
    \item 
$
    \sgn
        {1,\cdots,\widehat{i}\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,(l-1)^{'},l^{'},i,(l+1)^{'},\cdots,n^{'}}
        {1,\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
    =
    \sgn
        {l^{'},i,1,\cdots,\widehat{i}\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,(l-1)^{'},(l+1)^{'},\cdots,n^{'}}
        {1,\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
$
    \\
$
    =
    (-1)
    \sgn
        {i,l^{'},1,\cdots,\widehat{i}\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,(l-1)^{'},(l+1)^{'},\cdots,n^{'}}
        {1,\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
$,
    \item
$
    \sgn
            {1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
            {l^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,\widehat{l^{'}},\cdots,n^{'}}
    \sgn
        {i,l^{'},1,\cdots,\widehat{i}\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,\widehat{l^{'}},\cdots,n^{'}}
        {1,\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
    =
    \sgn
        {i,1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
        {1,\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
$.
\end{itemize}
We simplify expression (\ref{EQ-simplification for RHS of (i,j)-target 2}) to
\begin{align}
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {j^{'},i,1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
    \sgn
        {i,1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
        {1,\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {j^{'},1,\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}.
    \label{EQ-simplification for RHS of (i,j)-simplify of target 2-no1}
\end{align}
We continue the computation with the following properties of the sign of permutation:
\begin{itemize}
    \item 
$
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {j^{'},i,1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
    \sgn
        {i,1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
        {1,\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
    =
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {j^{'},1,\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}},
$
    \item
$
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {j^{'},1,\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {j^{'},1,\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
    =
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {1,\cdots,n,1^{'},\cdots,n^{'}}
$.
\end{itemize}
We obtain the simplification of (\ref{EQ-simplification for RHS of (i,j)-simplify of target 2-no1}):
\begin{align*}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {1,\cdots,n,1^{'},\cdots,n^{'}}
    =
    (-1)^{n^2}.
\end{align*}
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lemma}
$
    \begin{pmatrix*}
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {i,j^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
        \sgn
            {1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
            {l^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,\widehat{l^{'}},\cdots,n^{'}}
        \\
        \sgn
            {1,\cdots,\widehat{i}\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,(l-1)^{'},j^{'},i,(l+1)^{'},\cdots,n^{'}}
            {1,\cdots,n,1^{'},\cdots,\widehat{l^{'}},\cdots,n^{'}}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {l^{'},1,\cdots,n,1^{'},\cdots,\widehat{l^{'}},\cdots,n^{'}}
    \end{pmatrix*}
    =
    -(-1)^{n^2}.
$
\end{lemma}

\begin{proof}
We use the following properties of the sign of permutation:
\begin{itemize}
    \item 
$
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {i,j^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
    =
    (-1)
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {j^{'},i,1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
$,
    \item
$
    \begin{matrix*}[l]
    \sgn
        {1,\cdots,\widehat{i}\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,(l-1)^{'},j^{'},i,(l+1)^{'},\cdots,n^{'}}
        {1,\cdots,n,1^{'},\cdots,\widehat{l^{'}},\cdots,n^{'}}
    &=
    \sgn
        {j^{'},i,1,\cdots,\widehat{i}\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,\widehat{l^{'}},\cdots,n^{'}}
        {1,\cdots,n,1^{'},\cdots,\widehat{l^{'}},\cdots,n^{'}}
    \\
    &=
    \sgn
        {j^{'},i,l^{'},1,\cdots,\widehat{i}\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,\widehat{l^{'}},\cdots,n^{'}}
        {l^{'},1,\cdots,n,1^{'},\cdots,\widehat{l^{'}},\cdots,n^{'}}
    \end{matrix*}
$,
    \item 
$
    \sgn
        {1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
        {l^{'},1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,\widehat{l^{'}},\cdots,n^{'}}
    \sgn
        {j^{'},i,l^{'},1,\cdots,\widehat{i}\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,\widehat{l^{'}},\cdots,n^{'}}
        {l^{'},1,\cdots,n,1^{'},\cdots,\widehat{l^{'}},\cdots,n^{'}}
    =
    \sgn
        {j^{'},i,1,\cdots,\widehat{i}\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
        {l^{'},1,\cdots,n,1^{'},\cdots,\widehat{l^{'}},\cdots,n^{'}}
$.
\end{itemize}
Expression (\ref{EQ-simplification for RHS of (i,j)-target 3}) is then simplified to
\begin{align}
    (-1)
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {j^{'},i,1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
    \sgn
        {j^{'},i,1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
        {l^{'},1,\cdots,n,1^{'},\cdots,\widehat{l^{'}},\cdots,n^{'}}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {l^{'},1,\cdots,n,1^{'},\cdots,\widehat{l^{'}},\cdots,n^{'}}.
\label{EQ-simplification for RHS of (i,j)-simplify of target 3-no1}
\end{align}
We continue the computation with the following properties:
\begin{itemize}
    \item 
$
    \sgn
        {j^{'},i,1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
        {l^{'},1,\cdots,n,1^{'},\cdots,\widehat{l^{'}},\cdots,n^{'}}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {l^{'},1,\cdots,n,1^{'},\cdots,\widehat{l^{'}},\cdots,n^{'}}
    =
    \sgn
        {j^{'},i,1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
        {1^{'},\cdots,n^{'},1,\cdots,n}
$,
    \item 
$
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {j^{'},i,1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
    \sgn
        {j^{'},i,1,\cdots,\widehat{i},\cdots,n,1^{'},\cdots,\widehat{j^{'}},\cdots,n^{'}}
        {1^{'},\cdots,n^{'},1,\cdots,n}
    =
     \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {1^{'},\cdots,n^{'},1,\cdots,n}
$.
\end{itemize}
We then simplify (\ref{EQ-simplification for RHS of (i,j)-simplify of target 3-no1}) as follows:
\begin{align*}
    (-1)
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {1^{'},\cdots,n^{'},1,\cdots,n}
    =
    -(-1)^{n^2}
    .
\end{align*}
\end{proof}


==> 5/simplification_for_RHS_of_alpha,_I,J_.tex <==
In this section, we calculate the following signs:
\begin{itemize}
    \item 
$
    \begin{pmatrix*} 
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\indexI,\indexJp,\indexIc,\indexJpc}
        \sgn
            {\indexIc}
            {\indexic{k},\indexIc\backslash\{\indexic{k}\}}
        \sgn
            {\indexic{1},\cdots,\indexic{k-1},\order{\indexic{k},r},\indexic{k+1},\cdots,\indexic{n-p}}
            {\order{\indexIc\cup\{r\}}}
        \\
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\order{\indexIc\cup\{r\}},\indexJpc,\indexI\backslash\{r\},\indexJp}
    \end{pmatrix*} 
$,
    \item 
$
    \begin{pmatrix*}
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\indexI,\indexJp,\indexIc,\indexJpc}
        \sgn
            {\indexIc}
            {\indexic{k},\indexIc\backslash\{\indexic{k}\}}
        \sgn
            {\indexic{1},\cdots,\indexic{k-1},\order{r_1,r_2},\indexic{k+1},\cdots,\indexic{n-p}}
            {\order{(\indexIc\backslash\{\indexic{k}\})\cup\{r_1,r_2\}}}
        \\
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\order{(\indexIc\backslash\{\indexic{k}\})\cup\{r_1,r_2\}},\indexJpc,\order{(\indexI\backslash\{r_1,r_2\})\cup\{\indexic{k}\}},\indexJp}
    \end{pmatrix*}
$,
    \item 
$
    \begin{pmatrix*}
            \sgn
                {1,\cdots,n,1^{'},\cdots,n^{'}}
                {\indexI,\indexJp,\indexIc,\indexJpc}
            \sgn
                {\indexIc,\indexJpc}
                {\indexjpc{l},\indexIc,\indexJpc\backslash\{\indexjpc{l}\}}
            \\
            \sgn
                {\indexIc,\indexjpc{1},\cdots,\indexjpc{l-1},\indexjpc{l},r,\indexjpc{l+1},\cdots,\indexjpc{n-1}}
                {\order{\indexIc\cup\{r\}},\indexJpc}
            \sgn
                {1^{'},\cdots,n^{'},1,\cdots,n}
                {\order{\indexIc\cup\{r\}},\indexJpc,\indexI\backslash\{r\},\indexJp}
        \end{pmatrix*}
$,
    \item 
$
    \begin{pmatrix*}
            \sgn
                {1,\cdots,n,1^{'},\cdots,n^{'}}
                {\indexI,\indexJp,\indexIc,\indexJpc}
            \sgn
                {\indexIc,\indexJpc}
                {\indexjpc{l},\indexIc,\indexJpc\backslash\{\indexjpc{l}\}}
            \sgn
                {\indexIc,\indexjpc{1},\cdots,\indexjpc{l-1},u^{'},r,\indexjpc{l+1},\cdots,\indexjpc{n-1}}
                {\order{\indexIc\cup\{r\}},\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}}}
            \\
            \sgn
                {1^{'},\cdots,n^{'},1,\cdots,n}
                {\order{\indexIc\cup\{r\}},\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}},\indexI\backslash\{r\},\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
        \end{pmatrix*}
$,
\end{itemize}
which are from (\ref{EQ-For alpha, (I ,J), calculation for RHS-step 3,unsimplified close to the target}) in Section \ref{subsection-For (alpha, I, J), calculation for RHS}. We need these signs to simplify the expression of $
\star\,\LieagbdPartialbar\,\star
(\basexi{\indexI}\wedge\basedualxi{\indexJp})
$ and compute $
\basexi{\alpha}\wedge
\sqrt{-1}\LieagbdPartial^{*}
(\basexi{\indexI}\wedge\basedualxi{\indexJp})
$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%      start Lemma 1      %%%%%%%%%
\begin{lemma}
\label{Lemma-simplification for RHS of alpha,(I,J)-lemma 1}
    \begin{align*}
        \begin{pmatrix*} 
            \sgn
                {1,\cdots,n,1^{'},\cdots,n^{'}}
                {\indexI,\indexJp,\indexIc,\indexJpc}
            \sgn
                {\indexIc}
                {\indexic{k},\indexIc\backslash\{\indexic{k}\}}
            \\
            \sgn
                {\indexic{1},\cdots,\indexic{k-1},\order{\indexic{k},r},\indexic{k+1},\cdots,\indexic{n-p}}
                {\order{\indexIc\cup\{r\}}}
            \\
            \sgn
                {1^{'},\cdots,n^{'},1,\cdots,n}
                {\order{\indexIc\cup\{r\}},\indexJpc,\indexI\backslash\{r\},\indexJp}
        \end{pmatrix*} 
        =
        (-1)^{n^2}
        \sgn
            {\order{\indexic{k},r}}
            {r,\indexic{k}}
        \sgn
            {r,\indexI\backslash\{r\}}
            {\indexI}.
    \end{align*}
\end{lemma}
\begin{proof}
We use the following properties of the sign of permutation:
\begin{itemize}
    \item 
$
        \sgn
            {\indexic{1},\cdots,\indexic{k-1},\order{\indexic{k},r},\indexic{k+1},\cdots,\indexic{n-p}}
            {\order{\indexIc\cup\{r\}}}
        =
        \sgn
            {\order{\indexic{k},r},\indexIc\backslash\{\indexic{k}\}}
            {\order{\indexIc\cup\{r\}}}    
$,
    \item 
$
        \sgn
            {\order{\indexic{k},r},\indexIc\backslash\{\indexic{k}\}}
            {\order{\indexIc\cup\{r\}}}
        =
        \sgn
            {\order{\indexic{k},r}}
            {r,\indexic{k}}
        \sgn
            {r,\indexic{k},\indexIc\backslash\{\indexic{k}\}}
            {\order{\indexIc\cup\{r\}}}
$,
    \item 
$
        \sgn
            {r,\indexic{k},\indexIc\backslash\{\indexic{k}\}}
            {\order{\indexIc\cup\{r\}}}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\order{\indexIc\cup\{r\}},\indexJpc,\indexI\backslash\{r\},\indexJp}
        =
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {r,\indexic{k},\indexIc\backslash\{\indexic{k}\},\indexJpc,\indexI\backslash\{r\},\indexJp}
$.
\end{itemize}
We simplify the left-hand side of the equation in Lemma \ref{Lemma-simplification for RHS of alpha,(I,J)-lemma 1} to
\begin{align}
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\indexI,\indexJp,\indexIc,\indexJpc}
    \sgn
        {\indexIc}
        {\indexic{k},\indexIc\backslash\{\indexic{k}\}}
    \sgn
        {\order{\indexic{k},r}}
        {r,\indexic{k}}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {r,\indexic{k},\indexIc\backslash\{\indexic{k}\},\indexJpc,\indexI\backslash\{r\},\indexJp}
    .
    \label{EQ-simplification for RHS of alpha,(I,J)-lemma 1-no1}
\end{align}


We use the following properties of the sign of permutation:
\begin{itemize}
    \item 
$
        \sgn
            {\indexIc}
            {\indexic{k},\indexIc\backslash\{\indexic{k}\}}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {r,\indexic{k},\indexIc\backslash\{\indexic{k}\},\indexJpc,\indexI\backslash\{r\},\indexJp}
        =
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {r,\indexIc,\indexJpc,\indexI\backslash\{r\},\indexJp}
$,
    \item
$
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {r,\indexIc,\indexJpc,\indexI\backslash\{r\},\indexJp}
        =
        (-1)^{n-p+n-q}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\indexIc,\indexJpc,r,\indexI\backslash\{r\},\indexJp}
        =
        (-1)^{p+q}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\indexIc,\indexJpc,r,\indexI\backslash\{r\},\indexJp},
$
    \item 
$
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\indexIc,\indexJpc,r,\indexI\backslash\{r\},\indexJp}
        =
        \sgn
            {r,\indexI\backslash\{r\}}
            {\indexI}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\indexIc,\indexJpc,\indexI,\indexJp}
$.
\end{itemize}
We simplify (\ref{EQ-simplification for RHS of alpha,(I,J)-lemma 1-no1}) to
\begin{align}
    \sgn
        {1,\cdots,n,1^{'},\cdots,n^{'}}
        {\indexI,\indexJp,\indexIc,\indexJpc}
    \sgn
        {\order{\indexic{k},r}}
        {r,\indexic{k}}
    (-1)^{p+q}
    \sgn
        {r,\indexI\backslash\{r\}}
        {\indexI}
    \sgn
        {1^{'},\cdots,n^{'},1,\cdots,n}
        {\indexIc,\indexJpc,\indexI,\indexJp}
    .
\label{EQ-simplification for RHS of alpha,(I,J)-lemma 1-no2}
\end{align}


We use the following properties of the sign of permutation:
\begin{itemize}
    \item 
$
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\indexIc,\indexJpc,\indexI,\indexJp}
        =
        (-1)^{(n-p+n-q)(p+q)}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\indexI,\indexJp,\indexIc,\indexJpc}
        =
        (-1)^{(p+q)^2}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\indexI,\indexJp,\indexIc,\indexJpc}
$,
    \item 
$
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\indexI,\indexJp,\indexIc,\indexJpc}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\indexI,\indexJp,\indexIc,\indexJpc}
        =
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {1^{'},\cdots,n^{'},1,\cdots,n}
        =
        (-1)^{n^2}
$.
\end{itemize}
We simplify (\ref{EQ-simplification for RHS of alpha,(I,J)-lemma 1-no2}) to
\begin{align*}
    (-1)^{(p+q)}
    (-1)^{(p+q)^2}
    (-1)^{n^2}
    \sgn
        {\order{\indexic{k},r}}
        {r,\indexic{k}}
    \sgn
        {r,\indexI\backslash\{r\}}
        {\indexI}
    =
    (-1)^{n^2}
    \sgn
        {\order{\indexic{k},r}}
        {r,\indexic{k}}
    \sgn
        {r,\indexI\backslash\{r\}}
        {\indexI}
    ,
\end{align*}
which completes the proof of Lemma \ref{Lemma-simplification for RHS of alpha,(I,J)-lemma 1}.

\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%      finish Lemma 1      %%%%%%%%%





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%      start Lemma 2      %%%%%%%%%
\begin{lemma}
\label{Lemma-simplification for RHS of alpha,(I,J)-lemma 2}
    \begin{align*}
        \begin{pmatrix*}
            \sgn
                {1,\cdots,n,1^{'},\cdots,n^{'}}
                {\indexI,\indexJp,\indexIc,\indexJpc}
            \sgn
                {\indexIc}
                {\indexic{k},\indexIc\backslash\{\indexic{k}\}}
            \\
            \sgn
                {\indexic{1},\cdots,\indexic{k-1},\order{r_1,r_2},\indexic{k+1},\cdots,\indexic{n-p}}
                {\order{(\indexIc\backslash\{\indexic{k}\})\cup\{r_1,r_2\}}}
            \\
            \sgn
                {1^{'},\cdots,n^{'},1,\cdots,n}
                {\order{(\indexIc\backslash\{\indexic{k}\})\cup\{r_1,r_2\}},\indexJpc,\order{(\indexI\backslash\{r_1,r_2\})\cup\{\indexic{k}\}},\indexJp}
        \end{pmatrix*}
        =
        \begin{pmatrix*}[l]
            -(-1)^{n^2}
            \\
            \sgn
                {\order{r_1,r_2},\indexI\backslash\{r_1,r_2\}}
                {\indexI}
            \\
            \sgn
                {\order{(\indexI\backslash\{r_1,r_2\})\cup\{\indexic{k}\}}}
                {\indexic{k},\indexI\backslash\{r_1,r_2\}}
        \end{pmatrix*}
        .
    \end{align*}
\end{lemma}

\begin{proof}
We use the following properties of the sign of permutation:
\begin{itemize}
    \item 
$
        \sgn
            {\indexic{1},\cdots,\indexic{k-1},\order{r_1,r_2},\indexic{k+1},\cdots,\indexic{n-p}}
            {\order{(\indexIc\backslash\{\indexic{k}\})\cup\{r_1,r_2\}}}
        =
        \sgn
            {\order{r_1,r_2},\indexIc\backslash\{\indexic{k}\}}
            {\order{(\indexIc\backslash\{\indexic{k}\})\cup\{r_1,r_2\}}}
$,
    \item 
$
        \sgn
            {\order{r_1,r_2},\indexIc\backslash\{\indexic{k}\}}
            {\order{(\indexIc\backslash\{\indexic{k}\})\cup\{r_1,r_2\}}}
        =
        \sgn
            {\indexic{k},\order{r_1,r_2},\indexIc\backslash\{\indexic{k}\}}
            {\indexic{k},\order{(\indexIc\backslash\{\indexic{k}\})\cup\{r_1,r_2\}}}
        \\
        =
        \sgn
            {\order{r_1,r_2},\indexic{k},\indexIc\backslash\{\indexic{k}\}}
            {\indexic{k},\order{(\indexIc\backslash\{\indexic{k}\})\cup\{r_1,r_2\}}}
$,
    \item 
$
        \sgn
            {\indexIc}
            {\indexic{k},\indexIc\backslash\{\indexic{k}\}}
        \sgn
            {\order{r_1,r_2},\indexic{k},\indexIc\backslash\{\indexic{k}\}}
            {\indexic{k},\order{(\indexIc\backslash\{\indexic{k}\})\cup\{r_1,r_2\}}}
        =
        \sgn
            {\order{r_1,r_2},\indexIc}
            {\indexic{k},\order{(\indexIc\backslash\{\indexic{k}\})\cup\{r_1,r_2\}}}
$.
\end{itemize}
We simplify the left-hand side of the equation in Lemma \ref{Lemma-simplification for RHS of alpha,(I,J)-lemma 2} to
\begin{align}
    \begin{pmatrix*}[l]
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\indexI,\indexJp,\indexIc,\indexJpc}
        \sgn
            {\order{r_1,r_2},\indexIc}
            {\indexic{k},\order{(\indexIc\backslash\{\indexic{k}\})\cup\{r_1,r_2\}}}
        \\
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\order{(\indexIc\backslash\{\indexic{k}\})\cup\{r_1,r_2\}},\indexJpc,\order{(\indexI\backslash\{r_1,r_2\})\cup\{\indexic{k}\}},\indexJp}
    \end{pmatrix*}.
\label{EQ-simplification for RHS of alpha,(I,J)-lemma 2-no1}
\end{align}


We use the following properties of the sign of permutation:
\begin{itemize}
    \item 
$
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\order{(\indexIc\backslash\{\indexic{k}\})\cup\{r_1,r_2\}},\indexJpc,\order{(\indexI\backslash\{r_1,r_2\})\cup\{\indexic{k}\}},\indexJp}
        \\
        =
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\order{(\indexIc\backslash\{\indexic{k}\})\cup\{r_1,r_2\}},\indexJpc,\indexic{k},\indexI\backslash\{r_1,r_2\},\indexJp}
        \sgn
            {\order{(\indexI\backslash\{r_1,r_2\})\cup\{\indexic{k}\}}}
            {\indexic{k},\indexI\backslash\{r_1,r_2\}}
$,
    \item 
$
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\order{(\indexIc\backslash\{\indexic{k}\})\cup\{r_1,r_2\}},\indexJpc,\indexic{k},\indexI\backslash\{r_1,r_2\},\indexJp}
        \\
        =
        (-1)^{n-p+1+n-q}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\indexic{k},\order{(\indexIc\backslash\{\indexic{k}\})\cup\{r_1,r_2\}},\indexJpc,\indexI\backslash\{r_1,r_2\},\indexJp}
$,
    \item 
$
        \sgn
            {\order{r_1,r_2},\indexIc}
            {\indexic{k},\order{(\indexIc\backslash\{\indexic{k}\})\cup\{r_1,r_2\}}}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\indexic{k},\order{(\indexIc\backslash\{\indexic{k}\})\cup\{r_1,r_2\}},\indexJpc,\indexI\backslash\{r_1,r_2\},\indexJp}
        \\
        =
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\order{r_1,r_2},\indexIc,\indexJpc,\indexI\backslash\{r_1,r_2\},\indexJp}
$.
\end{itemize}
We simplify (\ref{EQ-simplification for RHS of alpha,(I,J)-lemma 2-no1}) to
\begin{align}
    &
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\indexI,\indexJp,\indexIc,\indexJpc}
        (-1)^{n-p+1+n-q}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\order{r_1,r_2},\indexIc,\indexJpc,\indexI\backslash\{r_1,r_2\},\indexJp}
        \sgn
            {\order{(\indexI\backslash\{r_1,r_2\})\cup\{\indexic{k}\}}}
            {\indexic{k},\indexI\backslash\{r_1,r_2\}}
    \notag
    \\
    =&
        (-1)^{p+q+1}
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\indexI,\indexJp,\indexIc,\indexJpc}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\order{r_1,r_2},\indexIc,\indexJpc,\indexI\backslash\{r_1,r_2\},\indexJp}
        \sgn
            {\order{(\indexI\backslash\{r_1,r_2\})\cup\{\indexic{k}\}}}
            {\indexic{k},\indexI\backslash\{r_1,r_2\}}
    .
\label{EQ-simplification for RHS of alpha,(I,J)-lemma 2-no2}
\end{align}


We use the following properties of the sign of permutation:
\begin{itemize}
    \item 
$
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\order{r_1,r_2},\indexIc,\indexJpc,\indexI\backslash\{r_1,r_2\},\indexJp}
        =
        (-1)^{(n-p+n-q)(p-2+q)}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\order{r_1,r_2},\indexI\backslash\{r_1,r_2\},\indexJp,\indexIc,\indexJpc}
$,
    \item 
$
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\order{r_1,r_2},\indexI\backslash\{r_1,r_2\},\indexJp,\indexIc,\indexJpc}
        =
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\indexI,\indexJp,\indexIc,\indexJpc}
        \sgn
            {\order{r_1,r_2},\indexI\backslash\{r_1,r_2\}}
            {\indexI}
$,
    \item 
$
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\indexI,\indexJp,\indexIc,\indexJpc}  
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\indexI,\indexJp,\indexIc,\indexJpc}
        =
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {1^{'},\cdots,n^{'},1,\cdots,n}
        =
        (-1)^{n^2}
$.
\end{itemize}
We simplify (\ref{EQ-simplification for RHS of alpha,(I,J)-lemma 2-no2}) to
\begin{align*}
    &
        (-1)^{p+q+1}
        (-1)^{(n-p+n-q)(p-2+q)}
        (-1)^{n^2}
        \sgn
                {\order{r_1,r_2},\indexI\backslash\{r_1,r_2\}}
                {\indexI}
        \sgn
            {\order{(\indexI\backslash\{r_1,r_2\})\cup\{\indexic{k}\}}}
            {\indexic{k},\indexI\backslash\{r_1,r_2\}}
    \\
    =&
        -(-1)^{p+q}
        (-1)^{(p+q)^2}
        (-1)^{n^2}
        \sgn
                {\order{r_1,r_2},\indexI\backslash\{r_1,r_2\}}
                {\indexI}
        \sgn
            {\order{(\indexI\backslash\{r_1,r_2\})\cup\{\indexic{k}\}}}
            {\indexic{k},\indexI\backslash\{r_1,r_2\}}
    \\
    =&
        -(-1)^{(p+q)(p+q+1)}
        (-1)^{n^2}
        \sgn
                {\order{r_1,r_2},\indexI\backslash\{r_1,r_2\}}
                {\indexI}
        \sgn
            {\order{(\indexI\backslash\{r_1,r_2\})\cup\{\indexic{k}\}}}
            {\indexic{k},\indexI\backslash\{r_1,r_2\}}
    \\
    =&
        -(-1)^{n^2}
        \sgn
                {\order{r_1,r_2},\indexI\backslash\{r_1,r_2\}}
                {\indexI}
        \sgn
            {\order{(\indexI\backslash\{r_1,r_2\})\cup\{\indexic{k}\}}}
            {\indexic{k},\indexI\backslash\{r_1,r_2\}}
    ,
\end{align*}
which completes the proof of Lemma \ref{Lemma-simplification for RHS of alpha,(I,J)-lemma 2}.
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%      finish Lemma 2      %%%%%%%%%





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%      start Lemma 3      %%%%%%%%%
\begin{lemma}
\label{Lemma-simplification for RHS of alpha,(I,J)-lemma 3}
    \begin{align*}
        \begin{pmatrix*}
            \sgn
                {1,\cdots,n,1^{'},\cdots,n^{'}}
                {\indexI,\indexJp,\indexIc,\indexJpc}
            \sgn
                {\indexIc,\indexJpc}
                {\indexjpc{l},\indexIc,\indexJpc\backslash\{\indexjpc{l}\}}
            \\
            \sgn
                {\indexIc,\indexjpc{1},\cdots,\indexjpc{l-1},\indexjpc{l},r,\indexjpc{l+1},\cdots,\indexjpc{n-1}}
                {\order{\indexIc\cup\{r\}},\indexJpc}
            \sgn
                {1^{'},\cdots,n^{'},1,\cdots,n}
                {\order{\indexIc\cup\{r\}},\indexJpc,\indexI\backslash\{r\},\indexJp}
        \end{pmatrix*}
        =
        -(-1)^{n^2}
        \sgn
            {r,\indexI\backslash\{r\}}
            {\indexI}.
    \end{align*}
\end{lemma}

\begin{proof}
We use the following properties of the sign of permutation:
\begin{itemize}
    \item 
$
        \sgn
            {\indexIc,\indexJpc}
            {\indexjpc{l},\indexIc,\indexJpc\backslash\{\indexjpc{l}\}}
        =
        (-1)^{n-p+l-1}
$,
    \item 
$
        \sgn
            {\indexIc,\indexjpc{1},\cdots,\indexjpc{l-1},\indexjpc{l},r,\indexjpc{l+1},\cdots,\indexjpc{n-1}}
            {\order{\indexIc\cup\{r\}},\indexJpc}
        =
        (-1)^{n-p+l}
        \sgn
            {r,\indexIc,\indexJpc}
            {\order{\indexIc\cup\{r\}},\indexJpc}
$,
    \item 
$
        \sgn
            {r,\indexIc,\indexJpc}
            {\order{\indexIc\cup\{r\}},\indexJpc}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\order{\indexIc\cup\{r\}},\indexJpc,\indexI\backslash\{r\},\indexJp}
        =
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {r,\indexIc,\indexJpc,\indexI\backslash\{r\},\indexJp}
$.
\end{itemize}
We simplify the left-hand side of the equation in Lemma \ref{Lemma-simplification for RHS of alpha,(I,J)-lemma 3} to
\begin{align}
    &
        (-1)^{n-p+l-1}
        (-1)^{n-p+l}
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\indexI,\indexJp,\indexIc,\indexJpc}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {r,\indexIc,\indexJpc,\indexI\backslash\{r\},\indexJp}
    \notag
    \\
    =&
        (-1)
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\indexI,\indexJp,\indexIc,\indexJpc}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {r,\indexIc,\indexJpc,\indexI\backslash\{r\},\indexJp}
    .
\label{EQ-simplification for RHS of alpha,(I,J)-lemma 3-no1}
\end{align}


We use the following properties of the sign of permutation:
\begin{itemize}
    \item 
$
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {r,\indexIc,\indexJpc,\indexI\backslash\{r\},\indexJp}
        =
        (-1)^{(n-p+n-q)(p-q+1)}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {r,\indexI\backslash\{r\},\indexJp,\indexIc,\indexJpc},
$
    \item 
$
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {r,\indexI\backslash\{r\},\indexJp,\indexIc,\indexJpc}
        =
        (-1)^{(n-p+n-q)(p-q+1)}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {r,\indexI\backslash\{r\},\indexJp,\indexIc,\indexJpc}
$,
    \item 
$
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\indexI,\indexJp,\indexIc,\indexJpc}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\indexI,\indexJp,\indexIc,\indexJpc}
        =
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {1^{'},\cdots,n^{'},1,\cdots,n}
        =
        (-1)^{n^2}
$.
\end{itemize}
We simplify (\ref{EQ-simplification for RHS of alpha,(I,J)-lemma 3-no1}) to
\begin{align*}
    &
        (-1)
        (-1)^{n^2}
        (-1)^{(n-p+n-q)(p-q+1)}
        \sgn
            {r,\indexI\backslash\{r\}}
            {\indexI}
    \\
    =&
        (-1)
        (-1)^{n^2}
        (-1)^{(p+q)(p+q+1)}
        \sgn
            {r,\indexI\backslash\{r\}}
            {\indexI}
    \\
        =&
        -(-1)^{n^2}
        \sgn
            {r,\indexI\backslash\{r\}}
            {\indexI}
    ,
\end{align*}
which completes the proof of Lemma \ref{Lemma-simplification for RHS of alpha,(I,J)-lemma 3}.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%      finish Lemma 3      %%%%%%%%%





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%      start Lemma 4      %%%%%%%%%
\begin{lemma}
\label{Lemma-simplification for RHS of alpha,(I,J)-lemma 4}
    \begin{align*}
        &
        \begin{pmatrix*}
            \sgn
                {1,\cdots,n,1^{'},\cdots,n^{'}}
                {\indexI,\indexJp,\indexIc,\indexJpc}
            \sgn
                {\indexIc,\indexJpc}
                {\indexjpc{l},\indexIc,\indexJpc\backslash\{\indexjpc{l}\}}
            \sgn
                {\indexIc,\indexjpc{1},\cdots,\indexjpc{l-1},u^{'},r,\indexjpc{l+1},\cdots,\indexjpc{n-1}}
                {\order{\indexIc\cup\{r\}},\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}}}
            \\
            \sgn
                {1^{'},\cdots,n^{'},1,\cdots,n}
                {\order{\indexIc\cup\{r\}},\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}},\indexI\backslash\{r\},\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
        \end{pmatrix*}
        \\
        =&
            (-1)^{p}
            (-1)^{n^2}
            \sgn
                {u^{'},r,\indexI\backslash\{r\},\indexJpc\backslash\{u^{'}\}}
                {\indexI,\indexJp}
            \sgn
                {\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
                {\indexjpc{l},\indexJpc\backslash\{u^{'}\}}.
    \end{align*}
\end{lemma}

\begin{proof}
We use the following properties of the sign of permutation:
\begin{itemize}
    \item 
$
        \sgn
            {\indexIc,\indexjpc{1},\cdots,\indexjpc{l-1},u^{'},r,\indexjpc{l+1},\cdots,\indexjpc{n-1}}
            {\order{\indexIc\cup\{r\}},\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}}}
        =
        \sgn
            {u^{'},r,\indexIc,\indexJpc\backslash\{\
            \indexjpc{l}\}}
            {\order{\indexIc\cup\{r\}},\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}}}
$,
    \item
$
        \sgn
            {u^{'},r,\indexIc,\indexJpc\backslash\{\
            \indexjpc{l}\}}
            {\order{\indexIc\cup\{r\}},\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}}}
        =
        \sgn
            {u^{'},r,\indexjpc{l},\indexIc,\indexJpc\backslash\{\
            \indexjpc{l}\}}
            {\indexjpc{l},\order{\indexIc\cup\{r\}},\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}}}
$,
    \item 
$
        \sgn
            {\indexIc,\indexJpc}
            {\indexjpc{l},\indexIc,\indexJpc\backslash\{\indexjpc{l}\}}
        \sgn
            {u^{'},r,\indexjpc{l},\indexIc,\indexJpc\backslash\{\
            \indexjpc{l}\}}
            {\indexjpc{l},\order{\indexIc\cup\{r\}},\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}}}
        \\
        =
        \sgn
            {u^{'},r,\indexIc,\indexJpc}
            {\indexjpc{l},\order{\indexIc\cup\{r\}},\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}}}
$.
\end{itemize}
We simplify the left-hand side of the equation in Lemma \ref{Lemma-simplification for RHS of alpha,(I,J)-lemma 4} to
\begin{align}
    \begin{pmatrix*}
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\indexI,\indexJp,\indexIc,\indexJpc}
        \sgn
            {u^{'},r,\indexIc,\indexJpc}
            {\indexjpc{l},\order{\indexIc\cup\{r\}},\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}}}
        \\
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\order{\indexIc\cup\{r\}},\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}},\indexI\backslash\{r\},\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
    \end{pmatrix*}
    .
\label{EQ-simplification for RHS of alpha,(I,J)-lemma 4-no1}
\end{align}


We use the following properties of the sign of permutation:
\begin{itemize}
    \item 
$
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\order{\indexIc\cup\{r\}},\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}},\indexI\backslash\{r\},\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
        \\
        =
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\order{\indexIc\cup\{r\}},\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}},\indexI\backslash\{r\},\indexjpc{l},\indexJpc\backslash\{u^{'}\}}
        \sgn
            {\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
            {\indexjpc{l},\indexJpc\backslash\{u^{'}\}}
$,
    \item 
$
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\order{\indexIc\cup\{r\}},\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}},\indexI\backslash\{r\},\indexjpc{l},\indexJpc\backslash\{u^{'}\}}
        \\
        =
        (-1)^{p-1+n-q+n-p+1}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\indexjpc{l},\order{\indexIc\cup\{r\}},\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}},\indexI\backslash\{r\},\indexJpc\backslash\{u^{'}\}}
$,
    \item 
$
        \begin{pmatrix*}[l]
            \sgn
            {u^{'},r,\indexIc,\indexJpc}
            {\indexjpc{l},\order{\indexIc\cup\{r\}},\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}}}
            \\
            \sgn
                {1^{'},\cdots,n^{'},1,\cdots,n}
                {\indexjpc{l},\order{\indexIc\cup\{r\}},\order{(\indexJpc\backslash\{\indexjpc{l}\})\cup\{u^{'}\}},\indexI\backslash\{r\},\indexJpc\backslash\{u^{'}\}}
        \end{pmatrix*}
        \\
        =
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {u^{'},r,\indexIc,\indexJpc,\indexI\backslash\{r\},\indexJpc\backslash\{u^{'}\}}
$.
\end{itemize}
We simplify (\ref{EQ-simplification for RHS of alpha,(I,J)-lemma 4-no1}) to
\begin{align}
    &
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\indexI,\indexJp,\indexIc,\indexJpc}
        (-1)^{p-1+n-q+n-p+1}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {u^{'},r,\indexIc,\indexJpc,\indexI\backslash\{r\},\indexJpc\backslash\{u^{'}\}}
        \sgn
            {\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
            {\indexjpc{l},\indexJpc\backslash\{u^{'}\}} 
    \notag
    \\
    =&
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\indexI,\indexJp,\indexIc,\indexJpc}
        (-1)^{q}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {u^{'},r,\indexIc,\indexJpc,\indexI\backslash\{r\},\indexJpc\backslash\{u^{'}\}}
        \sgn
            {\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
            {\indexjpc{l},\indexJpc\backslash\{u^{'}\}} 
    .
\label{EQ-simplification for RHS of alpha,(I,J)-lemma 4-no2}
\end{align}


We use the following properties of the sign of permutation:
\begin{itemize}
    \item 
$
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {u^{'},r,\indexIc,\indexJpc,\indexI\backslash\{r\},\indexJpc\backslash\{u^{'}\}}
        =
        (-1)^{(n-p+n-q)(p-1+q-1)}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {u^{'},r,\indexI\backslash\{r\},\indexJpc\backslash\{u^{'}\},\indexIc,\indexJpc}
$,
    \item 
$
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {u^{'},r,\indexI\backslash\{r\},\indexJpc\backslash\{u^{'}\},\indexIc,\indexJpc}
        =
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\indexI,\indexJp,\indexIc,\indexJpc}
        \sgn
            {u^{'},r,\indexI\backslash\{r\},\indexJpc\backslash\{u^{'}\}}
            {\indexI,\indexJp}
$,
    \item 
$
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {\indexI,\indexJp,\indexIc,\indexJpc}
        \sgn
            {1^{'},\cdots,n^{'},1,\cdots,n}
            {\indexI,\indexJp,\indexIc,\indexJpc}
        =
        \sgn
            {1,\cdots,n,1^{'},\cdots,n^{'}}
            {1^{'},\cdots,n^{'},1,\cdots,n}
        =
        (-1)^{n^2}
$.
\end{itemize}
We simplify (\ref{EQ-simplification for RHS of alpha,(I,J)-lemma 4-no2}) to
\begin{align*}
    &
        (-1)^{q}
        (-1)^{(n-p+n-q)(p-1+q-1)}
        (-1)^{n^2}
        \sgn
            {u^{'},r,\indexI\backslash\{r\},\indexJpc\backslash\{u^{'}\}}
            {\indexI,\indexJp}
        \sgn
            {\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
            {\indexjpc{l},\indexJpc\backslash\{u^{'}\}}
    \\
    =&
        (-1)^{q}
        (-1)^{(p+q)^2}
        (-1)^{n^2}
        \sgn
            {u^{'},r,\indexI\backslash\{r\},\indexJpc\backslash\{u^{'}\}}
            {\indexI,\indexJp}
        \sgn
            {\order{(\indexJp\backslash\{u^{'}\})\cup\{\indexjpc{l}\}}}
            {\indexjpc{l},\indexJpc\backslash\{u^{'}\}}
    .
\end{align*}
Since $(-1)^{(p+q)^2}=(-1)^{p+q}$, we can simplify $(-1)^{q}(-1)^{p+q}=(-1)^{p+2q}=(-1)^{p}$, which completes the proof of Lemma \ref{Lemma-simplification for RHS of alpha,(I,J)-lemma 4}.
\end{proof}
